Real-Time Adaptive Velocity Optimization for Autonomous Electric Cars at the Limits of Handling

With the evolution of self-driving cars, autonomous racing series like Roborace and the Indy Autonomous Challenge are rapidly attracting growing attention. Researchers participating in these competitions hope to subsequently transfer their developed functionality to passenger vehicles, in order to improve self-driving technology for reasons of safety, and due to environmental and social benefits. The race track has the advantage of being a safe environment where challenging situations for the algorithms are permanently created. To achieve minimum lap times on the race track, it is important to gather and process information about external influences including, e.g., the position of other cars and the friction potential between the road and the tires. Furthermore, the predicted behavior of the ego-car's propulsion system is crucial for leveraging the available energy as efficiently as possible. In this paper, we therefore present an optimization-based velocity planner, mathematically formulated as a multi-parametric Sequential Quadratic Problem (mpSQP). This planner can handle a spatially and temporally varying friction coefficient, and transfer a race Energy Strategy (ES) to the road. It further handles the velocity-profile-generation task for performance and emergency trajectories in real time on the vehicle's Electronic Control Unit (ECU).

==> ressources/energy_strategy/energy80_global.tex <==
0,0
3,2.75E-09
6,5.42E-09
9,8.01E-09
12,1.05E-08
15,1.30E-08
18,1.52E-08
21,1.91E-08
24,2.33E-08
27,2.76E-08
30,3.20E-08
33,3.64E-08
36,4.06E-08
39,4.45E-08
42,4.83E-08
45,5.19E-08
48,5.54E-08
51,5.87E-08
54,6.19E-08
57,6.50E-08
60,6.80E-08
63,7.08E-08
66,7.35E-08
69,7.61E-08
72,7.86E-08
75,8.10E-08
78,8.33E-08
81,8.54E-08
84,8.75E-08
87,8.94E-08
90,9.13E-08
93,9.30E-08
96,9.46E-08
99,9.62E-08
102,9.76E-08
105,9.90E-08
108,1.00E-07
111,1.01E-07
114,1.02E-07
117,1.03E-07
120,1.04E-07
123,1.05E-07
126,1.06E-07
129,1.07E-07
132,1.07E-07
135,1.08E-07
138,1.09E-07
141,1.09E-07
144,1.10E-07
147,1.11E-07
150,1.12E-07
153,1.13E-07
156,1.15E-07
159,1.16E-07
162,1.18E-07
165,1.40E-07
168,0.001891385315367
171,0.003691081426489
174,0.006488546127723
177,0.009757704708822
180,0.012729815620728
183,0.015520994067478
186,0.018323748692228
189,0.021282701019454
192,0.024483860256852
195,0.027949479088437
198,0.031658730743909
201,0.035576275974133
204,0.039665022425668
207,0.043887650261083
210,0.048206791459209
213,0.052587296070442
216,0.057000628624975
219,0.061431742030579
222,0.065884919115166
225,0.070391227678377
228,0.075028586321324
231,0.07818904441103
234,0.079009243670511
237,0.07900925423961
240,0.079009259364515
243,0.079009262975189
246,0.079009265482023
249,0.079009269498595
252,0.079009273767795
255,0.079009276977432
258,0.079009279697752
261,0.079009282048335
264,0.0790092840925
267,0.079009285878682
270,0.079009287442902
273,0.079009288814399
276,0.079009290021753
279,0.079009291097108
282,0.07900929207599
285,0.079009292994574
288,0.079009293888315
291,0.079009294792643
294,0.079009295746476
297,0.079009296798001
300,0.079009298012914
303,0.079009299495724
306,0.079009301566336
309,0.079009303243724
312,0.079009308741475
315,0.081094453776736
318,0.083577533260636
321,0.086116190221571
324,0.088679781017909
327,0.091245194763686
330,0.093779958013402
333,0.096219555836417
336,0.098421019815389
339,0.100541218648118
342,0.100541228622715
345,0.100541232114599
348,0.100541234971803
351,0.100541236737217
354,0.10054123817693
357,0.100541239445933
360,0.100541240636826
363,0.100541241832223
366,0.100541243147985
369,0.100541244847236
372,0.100541246270843
375,0.100541248375371
378,0.100541259750771
381,0.10271681908782
384,0.104823337852579
387,0.106744781860447
390,0.10842645338633
393,0.111150551071527
396,0.1143665820033
399,0.117416960955953
402,0.120425340046149
405,0.123555071934328
408,0.126910494685266
411,0.130531775022937
414,0.134414080923536
417,0.138531587404151
420,0.142851547371069
423,0.1473393949391
426,0.151960216462184
429,0.15667923792214
432,0.161462938954315
435,0.166284335231772
438,0.171129791614148
441,0.175997158803864
444,0.180893685231279
447,0.185847712269801
450,0.190045943309854
453,0.191891393268089
456,0.191891432953339
459,0.19189143962629
462,0.191891444220632
465,0.191891447709528
468,0.191891450145994
471,0.191891454316054
474,0.191891458654073
477,0.191891462215519
480,0.191891464915898
483,0.19189146720665
486,0.19189146915387
489,0.191891470815293
492,0.191891472250812
495,0.191891473520086
498,0.191891474675159
501,0.191891475756762
504,0.19189147679622
507,0.19189147781989
510,0.19189147885394
513,0.191891479929133
516,0.191891481085757
519,0.191891482379644
522,0.191891483892663
525,0.191891485762842
528,0.191891488462752
531,0.191891490592041
534,0.191891504059805
537,0.194125182092199
540,0.196435491877799
543,0.198800055453794
546,0.201199071896583
549,0.203597306902839
552,0.205915114181872
555,0.207959632756936
558,0.211780085433902
561,0.21292805891493
564,0.212928062014935
567,0.212928065781642
570,0.212928070008717
573,0.21292807420289
576,0.21292807779869
579,0.212928080386711
582,0.21292808209525
585,0.212928083987593
588,0.212928086662768
591,0.212928099070093
594,0.214702712945258
597,0.216399823768912
600,0.218730607369037
603,0.221716037410579
606,0.224513852399554
609,0.227049182790401
612,0.229473652419278
615,0.231924836881472
618,0.234499287160949
621,0.237251375876572
624,0.240194920491711
627,0.243314731083823
630,0.246576134090045
633,0.249926718242271
636,0.253297358956285
639,0.256611706059751
642,0.25980906037269
645,0.262868698810121
648,0.265815595175554
651,0.266959037702684
654,0.266959051274244
657,0.266959056429478
660,0.266959059912324
663,0.266959062151783
666,0.266959066353804
669,0.266959069324609
672,0.266959071641582
675,0.266959073554082
678,0.266959075169223
681,0.266959076532654
684,0.266959077649548
687,0.266959078495027
690,0.266959079108952
693,0.266959079608828
696,0.266959080095007
699,0.266959080638783
702,0.266959081315426
705,0.26695908227009
708,0.266959084059619
711,0.266959087690118
714,0.269449919952274
717,0.271981250934308
720,0.274522521902864
723,0.276891329879432
726,0.280604880500875
729,0.280822898439682
732,0.280822899804449
735,0.280822900347979
738,0.280822900884293
741,0.28082290163406
744,0.280822902921132
747,0.280822906181488
750,0.283002518232697
753,0.284894711763372
756,0.287900882101327
759,0.291204807101995
762,0.294213567015007
765,0.297160549778364
768,0.300240083777309
771,0.303556383628939
774,0.30713384233687
777,0.310954582779552
780,0.314993405652491
783,0.319226555929621
786,0.32362927737399
789,0.32817768932876
792,0.332851379122814
795,0.337633569561477
798,0.342510616963255
801,0.347471455998259
804,0.352507081119525
807,0.357610264959785
810,0.36277542190085
813,0.367998091965283
816,0.373274260434192
819,0.37860018496842
822,0.383972511471746
825,0.389388243218716
828,0.39484462625423
831,0.400339054748383
834,0.405868996027424
837,0.411431934604691
840,0.417025332765817
843,0.422646596833507
846,0.428293020011871
849,0.433961645922429
852,0.439648972545327
855,0.445350418401616
858,0.451059535071883
861,0.456767101587478
864,0.462460482306193
867,0.468124049596159
870,0.473741992706746
873,0.479303731518952
876,0.48481043400003
879,0.490280866101358
882,0.494739699070027
885,0.497498028845934
888,0.498541904257482
891,0.498542008841934
894,0.498542024627234
897,0.498542036470471
900,0.498542045913452
903,0.498542053746922
906,0.498542060426872
909,0.498542066238867
912,0.498542071374867
915,0.498542075967975
918,0.498542080115785
921,0.498542083891823
924,0.498542087352849
927,0.498542090543583
930,0.498542093499878
933,0.498542096250897
936,0.498542098685893
939,0.498542102486362
942,0.498542106761185
945,0.498542111127272
948,0.498542115521559
951,0.498542119409339
954,0.498542122842927
957,0.498542126032637
960,0.498542128991979
963,0.498542131733642
966,0.49854213428095
969,0.498542136633733
972,0.498542138798107
975,0.498542140782006
978,0.498542142597101
981,0.498542144256751
984,0.498542145772185
987,0.498542147149842
990,0.498542148393217
993,0.498542149510957
996,0.498542150524165
999,0.498542151464592
1002,0.498542152366504
1005,0.498542153260071
1008,0.498542154170615
1011,0.498542155122504
1014,0.498542156145015
1017,0.498542157279882
1020,0.498542158588692
1023,0.498542160152649
1026,0.4985421620604
1029,0.498542164553615
1032,0.498542166171575
1035,0.498542168624006
1038,0.498542174103263
1041,0.499474442292749
1044,0.501263329925876
1047,0.503188325139213
1050,0.50612813814096
1053,0.50931776568905
1056,0.512182878196162
1059,0.514812261503985
1062,0.517381598069778
1065,0.520027449747009
1068,0.522839794906394
1071,0.525858123190109
1074,0.52908078591435
1077,0.532487622432815
1080,0.536056112126985
1083,0.539766502003378
1086,0.543604505634838
1089,0.547566154316692
1092,0.551654198300526
1095,0.555863149190491
1098,0.560172120136195
1101,0.564548538944241
1104,0.568949554275729
1107,0.573320549367444
1110,0.577596343925004
1113,0.581709553218259
1116,0.585607924802966
1119,0.589273765881239
1122,0.592291079174064
1125,0.593540671301162
1128,0.593540705323782
1131,0.593540713439492
1134,0.593540719110236
1137,0.593540723468074
1140,0.593540727002391
1143,0.593540729864521
1146,0.593540733312268
1149,0.593540737592301
1152,0.59354074195506
1155,0.593540745505275
1158,0.593540748180879
1161,0.593540750448569
1164,0.593540752388554
1167,0.593540754085201
1170,0.593540755612727
1173,0.593540757025902
1176,0.593540758361785
1179,0.593540759646222
1182,0.593540760899918
1185,0.593540762142901
1188,0.593540763398547
1191,0.593540764698578
1194,0.593540766090603
1197,0.593540767650992
1200,0.593540769505295
1203,0.593540771811357
1206,0.593540774634608
1209,0.593540778089499
1212,0.593540780366443
1215,0.593540782339991
1218,0.593540784457072
1221,0.593540786803156
1224,0.593540789542154
1227,0.593540792947797
1230,0.593540797545693
1233,0.59354080454524
1236,0.593540821638384
1239,0.594113710437064
1242,0.595957709073113
1245,0.598247814180516
1248,0.600555078654433
1251,0.602869019006464
1254,0.605183268766765
1257,0.607493602681539
1260,0.60979700946346
1263,0.612091179145529
1266,0.61437433414845
1269,0.616645301330113
1272,0.618904100153676
1275,0.62115402879036
1278,0.623402042158463
1281,0.625651607093268
1284,0.627892923905018
1287,0.63009426797929
1290,0.632181519960165
1293,0.634045257323495
1296,0.638230698618089
1299,0.642845119208976
1302,0.645938648752472
1305,0.645938686081325
1308,0.645938691199236
1311,0.645938696537336
1314,0.645938703023505
1317,0.645938711250564
1320,0.645938721545828
1323,0.645938733456988
1326,0.645938745862755
1329,0.645938758490646
1332,0.645938771370836
1335,0.645938783560525
1338,0.645938795990421
1341,0.645938816857843
1344,0.646424937187975
1347,0.648155579625123
1350,0.650128563510602
1353,0.65272518350471
1356,0.655592522952456
1359,0.6582708945496
1362,0.660683454093091
1365,0.662920361031057
1368,0.665086028019107
1371,0.667263802771593
1374,0.669512924999412
1377,0.671862079766073
1380,0.674307693564754
1383,0.676830513733078
1386,0.679419464544741
1389,0.682083455133374
1392,0.684848078821965
1395,0.687744853524213
1398,0.690799919259421
1401,0.694026934942998
1404,0.697426571193094
1407,0.700991118881388
1410,0.704709876883444
1413,0.708572094422193
1416,0.712567521632195
1419,0.716685988094866
1422,0.720916918424929
1425,0.725249017132423
1428,0.72967039529668
1431,0.734169499922658
1434,0.738735119308844
1437,0.743354136787915
1440,0.748010947875619
1443,0.752691780366798
1446,0.757392550312076
1449,0.76212871924652
1452,0.766943479694141
1455,0.770734903801112
1458,0.772591845864198
1461,0.772781165772932
1464,0.772781178696639
1467,0.772781186970357
1470,0.772781193267844
1473,0.772781198337484
1476,0.772781202571064
1479,0.77278120619725
1482,0.772781209362099
1485,0.772781212048586
1488,0.772781215653884
1491,0.772781219938371
1494,0.772781224313296
1497,0.772781228504548
1500,0.77278123178349
1503,0.772781234724873
1506,0.772781237357167
1509,0.772781239715365
1512,0.77278124182136
1515,0.772781243692759
1518,0.772781245338907
1521,0.772781246772784
1524,0.772781248013913
1527,0.77278124908386
1530,0.772781250015233
1533,0.772781250857989
1536,0.772781251669219
1539,0.772781252502929
1542,0.772781253411849
1545,0.772781254455745
1548,0.772781255713178
1551,0.77278125733542
1554,0.772781259532613
1557,0.772781261909584
1560,0.773536256297675
1563,0.775551161316631
1566,0.777442852758251
1569,0.779240206120033
1572,0.782049369420499
1575,0.785450800316518
1578,0.788698057360046
1581,0.791934509404606
1584,0.795411497558091
1587,0.799279209684157
1590,0.803565764027679
1593,0.808240302270645
1596,0.813254238157225
1599,0.818550795422122
1602,0.824061732711185
1605,0.829703247430622
1608,0.835386525307642
1611,0.841060926991249
1614,0.846722358344561
1617,0.852373129116385
1620,0.858025580971272
1623,0.863693981595715
1626,0.869346081742213
1629,0.874964612367361
1632,0.880560248019288
1635,0.886160726170451
1638,0.891790469341954
1641,0.897463827611404
1644,0.903186003199245
1647,0.908955979270264
1650,0.914768196259369
1653,0.920613309505761
1656,0.926479759271749
1659,0.932356760048966
1662,0.938242967801295
1665,0.94413704777647
1668,0.950037567248117
1671,0.955943034270542
1674,0.961851928529445
1677,0.967762729166236
1680,0.973674098185707
1683,0.979585248244182
1686,0.985495960064155
1689,0.991406195583564
1692,0.997315902714492
1695,1.00322502618177
1698,1.00910567187084
1701,1.0149287099299
1704,1.02069653086263
1707,1.02641139981891
1710,1.03207545266361
1713,1.03769071564043
1716,1.04325911898913
1719,1.04878250335273
1722,1.05426262587071
1725,1.05970115722868
1728,1.06509968548815
1731,1.07045972239091
1734,1.07578269825768
1737,1.08106996079779
1740,1.08632278000237
1743,1.09154235678898
1746,1.09672982066316
1749,1.10188622144197
1752,1.10701253463153
1755,1.11210967510713
1758,1.11717850638307
1761,1.12221984649566
1764,1.12723447290533
1767,1.13222312646287
1770,1.13718651459213
1773,1.14212531375772
1776,1.14704017142377
1779,1.15193170768695
1782,1.15680051672705
1785,1.16164716816732
1788,1.16647220839045
1791,1.17127616182221
1794,1.17605953217542
1797,1.18082280364003
1800,1.18556644200565
1803,1.19029089570756
1806,1.19499659679317
1809,1.19968396181082
1812,1.2043533926263
1815,1.20900527717424
1818,1.21363999015207
1821,1.21825789366296
1824,1.22285933781307
1827,1.2274446612659
1830,1.23201419175417
1833,1.23656824654662
1836,1.24110713286272
1839,1.24563114822139
1842,1.25014058069411
1845,1.25463570899387
1848,1.25911680218941
1851,1.2635837249968
1854,1.26754138837859
1857,1.27062261526659
1860,1.2726632805209
1863,1.2737057001492
1866,1.27399955945962
1869,1.27399964695925
1872,1.27399968406135
1875,1.27399971410869
1878,1.27399973929768
1881,1.27399976093701
1884,1.27399977986971
1887,1.27399979667068
1890,1.27399981174944
1893,1.27399982540804
1896,1.27399983787565
1899,1.27399984933021
1902,1.27399985991269
1905,1.27399986973664
1908,1.27399987889487
1911,1.27399988746421
1914,1.27399989550898
1917,1.27399990308358
1920,1.27399991023439
1923,1.27399991700134
1926,1.27399992341897
1929,1.27399992951745
1932,1.27399993532319
1935,1.27399994085953
1938,1.27399994614714
1941,1.27399995120441
1944,1.2739999560478
1947,1.2739999606921
1950,1.27399996515061
1953,1.27399996943539
1956,1.27399997355738
1959,1.27399997752653
1962,1.27399998135198
1965,1.27399998504206
1968,1.2739999886044
1971,1.27399999204597
1974,1.27399999537317
1977,1.27399999859191
1980,1.27400000170766
1983,1.27400000472548
1986,1.27400000765005
1989,1.27400001048576


==> ressources/energy_strategy/power80_global.tex <==
0,-0.000460451334085189
3,-0.000547507709238968
6,-0.000661467192726535
9,-0.000818151355966257
12,-0.00104874919222835
15,-0.00379820177207262
18,-35.5407741151564
21,-110.881855247743
24,-206.224811043017
27,-301.195827981848
30,-375.267568421168
33,-408.370690005468
36,-404.238702428022
39,-398.024414714693
42,-389.722261678824
45,-380.562587628065
48,-371.466499328887
51,-362.419710139433
54,-353.422675942372
57,-344.471399314439
60,-335.561176717362
63,-326.687662771755
66,-317.846451225051
69,-309.032657390295
72,-300.240552588415
75,-291.463671251288
78,-282.694945161125
81,-273.926664487214
84,-265.150402440093
87,-256.35671096782
90,-247.480382321041
93,-236.686140896414
96,-223.686135703674
99,-208.79904582958
102,-192.699219163968
105,-176.023820394882
108,-159.142113767614
111,-142.167897460984
114,-125.102709458455
117,-108.012608302927
120,-91.2119291883141
123,-75.388600076447
126,-61.5048201813787
129,-50.3580192717428
132,-42.0696776848118
135,-36.0295708276489
138,-31.3079841771774
141,-27.130092620895
144,-23.2437002942246
147,-20.0293575354971
150,-17.9316427499102
153,-16.7727364192987
156,-6.34781383767679
159,-1.08741688078553e-05
162,0.000337857117010227
165,31.4547893103418
168,29.8678563133632
171,46.6211266841894
174,55.4090233388146
177,51.4426788689862
180,49.4605986049974
183,51.0740008501078
186,55.6134213853435
189,62.1111964692893
192,69.5018323980261
195,77.0456415346592
198,84.4180358164295
201,91.4728090345729
204,98.0702835120987
207,104.055362244147
210,109.311828215542
213,113.791941393735
216,117.556770518457
219,120.928921753812
222,124.751884466153
225,130.620216393722
228,90.1141745016529
231,23.4239306685471
234,0.000223692504273467
237,3.71848216229211e-05
240,-5.60474156372299e-05
243,-0.000412949260480396
246,-32.5828434112631
249,-79.495065778823
252,-77.3887948295014
255,-73.1158723331319
258,-70.9981971117396
261,-69.6168447781404
264,-67.7413372848108
267,-64.4344041863268
270,-59.4156595898904
273,-53.3143872905058
276,-47.2264755812371
279,-41.9509087040698
282,-37.6664704277136
285,-34.0852752441985
288,-30.7416932036494
291,-27.2857975108528
294,-23.7674192942565
297,-20.7060348781539
300,-18.5977740372401
303,-17.3697916198331
306,-0.000197708857881807
309,5.95930465351141e-05
312,34.3153545407272
315,40.8070377511819
318,42.0903409174485
321,43.1911271948349
324,44.1747150767857
327,44.9083801039286
330,44.8139980776783
333,42.0751586391468
336,42.0069811433968
339,0.000145738873397758
342,-9.48439874900755
345,-40.1668238945881
348,-29.0302587787953
351,-23.3575800660511
354,-20.0389016854355
357,-17.9121283031644
360,-16.543226474239
363,-15.6641132402637
366,-15.0642942799902
369,-1.33689446929758
372,-1.42907733909017e-05
375,0.000153596261956623
378,32.9743245668505
381,32.7367753374818
384,30.5938482725303
387,27.3079419524321
390,45.3116178133161
393,55.3148860031973
396,54.0585208146749
399,54.6458608070287
402,58.2436442787252
405,64.0748640463962
408,71.0942267236874
411,78.5089089728619
414,85.9173628708868
417,93.1538720295988
420,100.136134539318
423,106.800370141717
426,113.082905243098
429,118.918784563197
432,124.254653649572
435,129.084059564476
438,133.521520046457
441,137.934890137611
444,143.088739061999
447,123.926034120945
450,55.178220941387
453,0.00112222750808775
456,0.000103122014025072
459,1.17241366419866e-05
462,-7.47017318502581e-05
465,-0.000605267445638202
468,-47.9402933159951
471,-117.608400441663
474,-138.026349648125
477,-114.331010275578
480,-94.4297787249031
483,-77.8877111779392
486,-64.651684485642
489,-54.787416066667
492,-47.958884303053
495,-43.4441798246994
498,-40.4174226590204
501,-38.1434700040191
504,-36.0371123304011
507,-33.6688184276088
510,-30.7813748683075
513,-27.3723436733382
516,-23.8283487173327
519,-20.842241796889
522,-18.8595936093631
525,-17.7219646424154
528,-6.33888152599422e-05
531,0.000215270763054696
534,40.1701498710733
537,41.6688529364605
540,42.7913681485565
543,43.6436875418591
546,44.0953103602997
549,43.412441646334
552,39.2077819861898
555,75.8921547558619
558,23.5115037571388
561,-6.70102845878614e-05
564,-16.9271442891474
567,-27.168289723606
570,-19.7547377779748
573,-11.0325351222533
576,-4.51691163988781
579,-0.000559302365190273
582,-8.86330145572127e-05
585,-1.23714902352573e-06
588,0.000204816187202973
591,32.8791218806658
594,31.7435630772605
597,44.193845161685
600,57.9221545651953
603,55.5341834282574
606,51.0247611122722
609,49.1241263426239
612,49.9089820425013
615,52.778244297673
618,56.995896513429
621,61.7700325067802
624,66.4748678738296
627,70.6580139421572
630,73.8826314400804
633,75.6878147750603
636,75.7867631965249
639,74.4159139286708
642,72.4311891276461
645,70.9119378325849
648,27.7821726782734
651,0.000268849115610946
654,3.355397727982e-05
657,-6.01071740086281e-05
660,-0.00263748162863017
663,-47.2818404682542
666,-60.2417854895975
669,-66.5601529476105
672,-72.3218784490898
675,-74.0544076693578
678,-67.7792489809848
681,-54.0862537624946
684,-38.506595464225
687,-27.2891650067464
690,-21.5286038452641
693,-18.9206397904141
696,-17.5923086148311
699,-16.716226587179
702,-16.0516611895691
705,-15.5809993042447
708,1.97343265587335e-05
711,35.6632073457349
714,37.6959929746749
717,39.2338567424506
720,37.7737065701236
723,61.5497210934616
726,3.69244782535362
729,-21.6809031179147
732,-15.3983011672426
735,-14.549773687405
738,-14.1366402309706
741,-8.28187284539015
744,2.79581734251957e-05
747,29.1452919198771
750,25.7373922638472
753,42.2844819548916
756,48.9183305496597
759,46.7021778757259
762,47.6292776814247
765,51.8108429133406
768,58.2323908997391
771,65.7100487500411
774,73.4279626515976
777,81.0546294551755
780,88.4972073031972
783,95.7259423999112
786,102.725340148355
789,109.49034246547
792,116.025814907314
795,122.343519049331
798,128.458803051864
801,134.38810736169
804,140.147553226561
807,145.752312443056
810,151.216068833345
813,156.550397529719
816,161.764590497332
819,166.866034784931
822,171.86058816285
825,176.752691438171
828,181.545392008671
831,186.240421687843
834,190.838364594751
837,195.338844361816
840,199.740410707848
843,204.039403710923
846,208.226663193617
849,212.280905212873
852,216.158480210395
855,219.781575533629
858,223.030757171051
861,225.752300432885
864,227.794473409122
867,229.086463114406
870,229.760615721127
873,230.277276098156
876,231.426654655754
879,190.516426597669
882,118.613326542267
885,44.9847892485034
888,0.00440946286171061
891,0.000572045850375824
894,0.000395246783618963
897,0.000284271411665527
900,0.000206452359022249
903,0.000147057123253446
906,9.83859029817901e-05
909,5.59220004661814e-05
912,1.64210974124992e-05
915,-2.26266446951236e-05
918,-6.37589240732967e-05
921,-0.000110112653487509
924,-0.000166358639233981
927,-0.000240676626393092
930,-0.000349930185725536
933,-0.000851399030155245
936,-26.7804816778915
939,-103.933959014288
942,-197.088845892213
945,-270.741323615387
948,-290.209521666166
951,-281.418989442166
954,-272.620708677669
957,-263.806711565904
960,-254.967287359458
963,-246.073042012331
966,-234.15980360727
969,-218.617780475823
972,-199.707342088745
975,-178.491690872591
978,-156.084716066741
981,-133.185516098243
984,-110.479206426183
987,-89.3735264123345
990,-71.8182011659294
993,-58.993973735233
996,-50.629311440992
999,-45.586091509933
1002,-42.5892031652816
1005,-40.5575095495849
1008,-38.6625167768578
1011,-36.2831462921938
1014,-32.9892509129707
1017,-28.7322939165159
1020,-24.2461466747034
1023,-20.7865585660048
1026,-18.8170158295872
1029,-0.000406458017047054
1032,-1.80744886238931e-05
1035,7.18521621041785e-05
1038,17.697447604075
1041,33.5690691114775
1044,35.8559026854373
1047,54.945516726221
1050,60.5489605491809
1053,55.3613996256374
1056,51.6567506370787
1059,51.3124152714195
1062,53.8059512172575
1065,58.4208790978632
1068,64.267128355345
1071,70.5347781252145
1074,76.7998266499214
1077,82.9391315322789
1080,88.9245482013259
1083,94.7344507478813
1086,100.348271931436
1089,105.739341963887
1092,110.845586932572
1095,115.542564951331
1098,119.624544393388
1101,122.783498619314
1104,124.605629733737
1107,124.647172515975
1110,122.656540497148
1113,118.890741722686
1116,114.236570643159
1119,95.7970610320753
1122,40.1325790836241
1125,0.00102410384940579
1128,0.000166933677811454
1131,6.87028700384173e-05
1134,-2.04573507692811e-06
1137,-7.46847204464914e-05
1140,-0.00021783682613862
1143,-10.9372640309336
1146,-77.5345420083993
1149,-144.40776221039
1152,-151.553646455603
1155,-114.12863179913
1158,-86.5474978469411
1161,-68.1145673165099
1164,-56.8075319182439
1167,-50.3465988920861
1170,-46.8449689088044
1173,-44.9674603637737
1176,-43.8346759578816
1179,-42.900941483133
1182,-41.8542431473209
1185,-40.5212048817603
1188,-38.7710735844727
1191,-36.4426447294838
1194,-33.3568066638636
1197,-29.5288339794268
1200,-25.544156988393
1203,-22.1440066389041
1206,-19.7443741924056
1209,-2.59162402318982
1212,-0.000255417595497882
1215,-0.00011865417378094
1218,-6.11746032854039e-05
1221,-2.42347120729005e-05
1224,5.72100192968297e-06
1227,3.81858827191841e-05
1230,8.75248528261298e-05
1233,0.000269099657908645
1236,9.9384977148842
1239,32.0925506829247
1242,40.5132224093827
1245,41.6098364074133
1248,42.5218345948573
1251,43.3233383052528
1254,44.0553164463665
1257,44.7407224805089
1260,45.392534346604
1263,46.0176893684684
1266,46.6185775510652
1269,47.1925499744944
1272,47.7287246573036
1275,48.1992244099282
1278,48.5363901656027
1281,48.578304089213
1284,47.9386109168429
1287,45.6812247969905
1290,40.9547222658172
1293,93.3471178381933
1296,105.919192940995
1299,72.544757712338
1302,0.000825332686514343
1305,3.44849701056271e-05
1308,3.62293618488459e-05
1311,6.89364826138828e-05
1314,0.000115736916546876
1317,0.000169069033101814
1320,0.000211547074210183
1323,0.000227636056069115
1326,0.000236935272708065
1329,0.000245567657743735
1332,0.000230760856294444
1335,0.000236947357226686
1338,0.000427311147500838
1341,10.7493776450625
1344,38.3245916349019
1347,44.1072884452924
1350,58.9107103094181
1353,66.347595659048
1356,63.199806702131
1359,57.8618696367081
1362,54.3521936026284
1365,53.1670884423092
1368,53.8847708092033
1371,55.9890033021892
1374,58.8066350470805
1377,61.5844217712386
1380,63.9393187069662
1383,66.0759955241323
1386,68.5102910240019
1389,71.6939050389849
1392,75.8161972652804
1395,80.7745620040175
1398,86.2725203688547
1401,91.9925540623105
1404,97.7292965916517
1407,103.408156768545
1410,109.027085656436
1413,114.597045612944
1416,120.114614868514
1419,125.558842934343
1422,130.89464282657
1425,136.07272037837
1428,141.025314631309
1431,145.662921922352
1434,149.884356438021
1437,153.619924564259
1440,156.922272845746
1443,160.095788086495
1446,163.813140003926
1449,169.090026837424
1452,134.920330251605
1455,66.5995208259616
1458,6.80077911563425
1461,0.000371717371600031
1464,0.000191603243947192
1467,0.000106258089494736
1470,4.34131177911001e-05
1473,-1.21846226369908e-05
1476,-7.12365372209176e-05
1479,-0.000147119962539152
1482,-0.000342858102078584
1485,-16.3897415698464
1488,-93.3483643564099
1491,-183.820999228714
1494,-239.209228556264
1497,-232.002984948613
1500,-224.555019104707
1503,-215.981345387905
1506,-206.056826097769
1509,-192.888204262694
1512,-174.895615190902
1515,-151.158176834882
1518,-123.354163463691
1521,-95.6878026604276
1524,-72.162491634178
1527,-54.9647363116171
1530,-43.7882347744262
1533,-36.6769195953645
1536,-31.4864608078747
1539,-26.8122820179468
1542,-22.4884274649783
1545,-19.3169151160225
1548,-17.596922028134
1551,-11.614669945146
1554,-5.80860214549044e-06
1557,13.2784529880319
1560,35.4779864114658
1563,33.4450879314834
1566,31.7971483494765
1569,50.0931172766253
1572,61.935510455685
1575,60.6856414356469
1578,62.2955949886793
1581,69.3405815885806
1584,80.2774978019897
1587,92.6380380652098
1590,105.046336005002
1593,117.108806576439
1596,128.569673307984
1599,138.984206844543
1602,147.772111429385
1605,154.528899217243
1608,159.988365336981
1611,165.290982174527
1614,170.448037689243
1617,175.475472236453
1620,180.376521622886
1623,183.860378863987
1626,186.513701750821
1629,189.30162412014
1632,192.872005176615
1635,197.195767173456
1638,201.98243742886
1641,206.94092501835
1644,211.860680401095
1647,216.576794374454
1650,220.941745467641
1653,224.859794726496
1656,228.347515709735
1659,231.767440655876
1662,235.127131249016
1665,238.42829977339
1668,241.672550749726
1671,244.861401023904
1674,247.996244618244
1677,251.078370244112
1680,254.109071979336
1683,257.089858799833
1686,260.022468700031
1689,262.90854455202
1692,265.749296600672
1695,267.274069413962
1698,267.374580699114
1701,267.468282514246
1704,267.556741374515
1707,267.64023495605
1710,267.71890662665
1713,267.79309864235
1716,267.863192691203
1719,267.929564718655
1722,267.992084699867
1725,268.050585171812
1728,268.105272080262
1731,268.156316762791
1734,268.204052096413
1737,268.248939407967
1740,268.291470031206
1743,268.332082276128
1746,268.371116582706
1749,268.408803600703
1752,268.445279010455
1755,268.480612093155
1758,268.514834908548
1761,268.547960265299
1764,268.579996165344
1767,268.610956422464
1770,268.64086158632
1773,268.66973931931
1776,268.69762344428
1779,268.724552270263
1782,268.750566732716
1785,268.77570866854
1788,268.800019407068
1791,268.82353876024
1794,268.84630441186
1797,268.868351643326
1800,268.889713301215
1803,268.910419909553
1806,268.930499846081
1809,268.949979525436
1812,268.968883553824
1815,268.987234835039
1818,269.005054615125
1821,269.022362452435
1824,269.039176090454
1827,269.05551118849
1830,269.07138081933
1833,269.086794545276
1836,269.101756661884
1839,269.116262646139
1842,269.130291305151
1845,269.143783827482
1848,269.132805945999
1851,239.112140998666
1854,186.514530229974
1857,123.615917154785
1860,63.1129969782523
1863,17.7633982121412
1866,0.00514807338124078
1869,0.00209811508928814
1872,0.0016674061856797
1875,0.00137017318300688
1878,0.00115242726243348
1881,0.000985844147626225
1884,0.000854108834878132
1887,0.000747158900031697
1890,0.000658449322133801
1893,0.000583537385453961
1896,0.000519299666071716
1899,0.000463474499001747
1902,0.000414382270427608
1905,0.000370747766911095
1908,0.000331583584575417
1911,0.000296111392880067
1914,0.000263707397012512
1917,0.000233863683322931
1920,0.000206160226897388
1923,0.000180244190830955
1926,0.000155814286481972
1929,0.000132608687862033
1932,0.00011039546608452
1935,8.89648175703553e-05
1938,6.8122543422306e-05
1941,4.76843779097351e-05
1944,2.74707861274905e-05
1947,7.30180078814352e-06
1950,-1.30080541348936e-05
1953,-3.36551224163155e-05
1956,-5.48529689092713e-05
1959,-7.68423562959001e-05
1962,-9.99079175941385e-05
1965,-0.000124395614259551
1968,-0.000150726210414934
1971,-0.000179419086419289
1974,-0.000211137528481968
1977,-0.000246755551019338
1980,-0.000287455565170805
1983,-0.00033488039490495
1986,-0.000391381796947021
1989,-0.000460451334085189



==> ressources/eps.tex <==
\definecolor{colBlau}{RGB}{0,101,189}%
\definecolor{colBlueDark}{RGB}{0,82,147}%
\definecolor{colRed}{RGB}{227,114,34}%
\definecolor{colGreen}{RGB}{162,173,0}%
\definecolor{colGray}{RGB}{153,153,153}%
%
\tikzstyle{simpleNode} = [rectangle, rounded corners, minimum width=1cm, minimum height=1cm,text centered, draw=black, line width=0.5mm]
\tikzstyle{arrow} = [->,-triangle 45,line width=0.5mm,black]
\tikzstyle{lineE} = [-,line width=0.5mm,colGray,dashed]
\tikzstyle{lineM} = [-,line width=1.5mm,black]
%
\begin{tikzpicture}[node distance=1cm]
\coordinate (Zero) at (0,0);
\node (Battery) [simpleNode, align=center] {$B$};
\node (InverterF) [simpleNode, align=center, left of=Battery, xshift=-0.5cm] {$I_{\mathrm{l/r}}$};
\node (MotorF) [simpleNode, align=center, left of=InverterF,xshift=-0.5cm] {$M_{\mathrm{l/r}}$};
\node (GearF) [simpleNode, align=center, left of=MotorF, xshift=-0.15cm] {$G_{\mathrm{l/r}}$};
\node (WheelFR) [simpleNode, align=center, above of=GearF, minimum height=0.6cm, yshift=0.3cm] {$W_{\mathrm{rl}}$};
\node (WheelFL) [simpleNode, align=center, below of=GearF, minimum height=0.6cm, yshift=-0.3cm] {$W_{\mathrm{rr}}$};
\node (Aux) [simpleNode, align=center, above of=Battery, yshift=0.3cm] {$A_\mathrm{x}$};
%
\node (InverterR) [simpleNode, minimum width=0cm, right of=Battery, draw=white, xshift=0.25cm] {};
%%% Edges %%%
\draw [lineE] ([yshift=0.2cm]Battery.west) to ([yshift=0.2cm]InverterF.east);
\draw [lineE] ([yshift=-0.2cm]Battery.west) to ([yshift=-0.2cm]InverterF.east);
\draw [lineE] ([yshift=0.2cm]Battery.east) to ([yshift=0.2cm]InverterR.west);
\draw [lineE] ([yshift=-0.2cm]Battery.east) to ([yshift=-0.2cm]InverterR.west);
% To Aux
\draw [lineE] ([xshift=0.2cm]Battery.north) to ([xshift=0.2cm]Aux.south);
\draw [lineE] ([xshift=-0.2cm]Battery.north) to ([xshift=-0.2cm]Aux.south);
%
\draw [lineE] (InverterF)[anchor=left] to (MotorF)[anchor=right];
\draw [lineE] ([yshift=0.25cm]InverterF.west) to ([yshift=0.25cm]MotorF.east);
\draw [lineE] ([yshift=-0.25cm]InverterF.west) to ([yshift=-0.25cm]MotorF.east);
\draw [lineM] (MotorF)[anchor=left] to (GearF)[anchor=right];
\draw [lineM] (GearF)[anchor=left] to (WheelFR)[anchor=right];
\draw [lineM] (GearF)[anchor=left] to (WheelFL)[anchor=right];
%\draw [arrow] (Battery) to[bend left] (InverterF);
\draw [thick] ($(InverterR.west)+(0,1)$) to [out=300,in=120] ($(InverterR.west)+(0,-1)$);
\end{tikzpicture}

==> ressources/path_concept/follow_overtake_visual.tex <==
% This file was created by tikzplotlib v0.8.7.
\begin{tikzpicture}

\begin{axis}[
height=0.8\columnwidth,
width=0.8\columnwidth,
xmin=75,
xmax=315,
ymin=-400,
ymax=-135,
tick align=outside,
tick pos=both,
xlabel={east in \SI{}{\meter}},
ylabel={north in \SI{}{\meter}},
ytick style={color=black},
legend cell align={left},
legend style={draw=none, at={(1.0,0.1)}, anchor=south east},
]
\addplot [line width=0.5pt, black, forget plot]
table {%
138.116987020723 -138.033028535533
162.01906947079 -156.065938488086
185.868081607164 -174.16988378918
209.901499698905 -192.110685035005
233.075678834268 -209.556541120489
239.784674326861 -214.460716342581
246.183474268932 -219.47901873543
251.38806860499 -225.764625357847
253.348486073808 -233.789940679736
251.722336421186 -241.928915796705
246.66212048069 -248.369294979527
239.47407066817 -251.910957572636
231.485049063605 -253.340063856613
223.640092935412 -254.152276675046
215.678236921469 -255.05366961563
207.34840935238 -256.110313258523
177.690202096416 -260.121628536036
168.514469311292 -261.961417510006
159.396234945727 -264.054990685492
150.362633127182 -266.367381889118
141.199205048079 -268.844993432851
131.425249326207 -271.887179975399
121.537436536619 -277.620965883905
114.741919715917 -287.591060879784
114.486314648012 -299.794399516322
119.310659042575 -310.226920963108
125.198858445981 -318.444916242261
130.827947127908 -325.787588293774
135.795548313488 -332.830989416747
139.170800055928 -340.355439568678
139.284178767877 -348.612150168904
136.157276544672 -356.197329047435
130.298689005601 -361.823327140237
122.594119941146 -364.710779376475
114.084326080252 -364.106951985703
106.229718250776 -361.037070550676
98.6575165753604 -357.495479640682
90.8154030965665 -353.861865058256
64.3395871970776 -341.761881521398
41.1797625786303 -331.217591185204
33.4167709608513 -327.321642677076
26.7759745339163 -322.294560780801
21.9942770207346 -315.845196551688
18.9622478159802 -308.157198474146
18.8519803009538 -299.823373034845
22.6737298337935 -292.601420048961
29.5931585738283 -287.935872510074
37.7190728584643 -283.479780178728
45.3718005193704 -276.679230065479
51.3161693253251 -266.803419164557
54.3071117930155 -255.313128070196
53.47176085842 -243.538027139297
49.2809089546896 -233.060887665359
42.2197513247012 -224.772521388341
33.5096661723015 -218.920527621755
24.5721210205625 -214.583918330206
15.5908965975869 -211.261208973645
6.50527500494586 -208.884428419855
-2.63710491850381 -207.338555797304
-11.8457285636876 -206.814568922283
-21.0672724122605 -207.44770638204
-30.3868140838081 -208.955352515077
-40.1519241621886 -211.509402191687
-50.2701421109438 -216.738955611896
-57.74066175634 -226.768945740554
-58.188937666259 -239.699341811216
-52.5560006476991 -249.33853782213
-46.2569541212998 -255.86791206308
-45.3734994938776 -263.630006061954
-51.0443908449928 -269.409673778292
-57.347663019582 -272.131634890076
-64.448142614821 -273.925126877142
-72.3334454492319 -274.772614843783
-80.472559543878 -274.775262288901
-88.8548307107264 -273.946638772346
-117.119493313026 -268.137800386094
-144.458591677802 -258.137794944311
-172.109112312018 -247.600676877324
-200.248765155356 -236.816563599473
-228.303640645067 -226.139767541361
-255.920100818749 -215.430261211702
-266.912303436912 -211.291206828256
-274.71760283428 -208.341182429322
-282.055207094885 -205.664667175476
-289.575238461823 -202.043963857893
-295.672753508439 -196.166326831839
-298.962732150996 -188.514650984685
-299.454126777407 -180.104787440843
-296.722422135094 -172.093998284933
-291.487081821778 -165.896361966374
-284.934664354041 -161.314755044065
-278.309812723911 -156.974162938106
-271.595896256756 -152.471069748698
-264.7392964509 -147.847167967354
-257.602446059169 -143.049781907846
-230.619714777062 -131.291870508806
-200.90968240777 -131.405361375565
-191.310586408786 -132.643016374685
-180.923009557403 -132.72047212373
-170.598618987339 -129.849109699842
-161.319260664508 -123.902495243846
-153.691927823892 -115.45111022438
-148.433718489322 -105.254636190565
-146.120667425122 -94.0326494273386
-147.163619656072 -82.5617617623424
-151.295217614812 -71.7759017555067
-157.997505457457 -62.5573751996545
-166.991728328991 -55.4768117857169
-177.728057241339 -51.0793607879947
-189.000082227084 -49.7482606908868
-199.610475270908 -51.5540895101371
-208.347790383437 -55.2454414530434
-216.07183268922 -59.2228047238243
-224.072521797645 -62.446860758726
-232.572588117702 -62.4867640101324
-240.542080519938 -59.4568652829289
-247.656501787198 -54.7867907731293
-253.964426840688 -49.054834873329
-259.440454205027 -42.4867873199616
-263.169475390843 -34.8214992093295
-264.975417638251 -26.4266304316931
-265.174173102672 -17.7695104726456
-264.092444541108 -9.17735314802875
-262.325821714475 -0.77391236793324
-260.016422711953 7.51184279292988
-248.82645784614 34.2674903890581
-236.168782173397 60.7721944614818
-223.337635669756 87.6026917875725
-217.129536401687 100.807535321913
-213.782852558007 108.103769697559
-210.765063287585 114.82794095335
-206.123727422987 121.730978505852
-198.574695441873 125.236015299371
-190.367295925859 124.200441778828
-183.778692952494 119.208619442698
-178.201003595748 113.005407935787
-172.786873393374 106.77844779029
-167.236650604601 100.555365900099
-146.677695585054 78.7845878905356
-122.721205023943 59.2898943183168
-98.6065452608939 41.0155628182014
-74.6621515703362 22.8230980753256
-50.7674461109932 4.68320033558364
-26.7975437846994 -13.3306975766329
-2.95180409358416 -31.5052618542037
20.9805922462664 -49.55568425383
44.8530793671585 -67.6786729042223
68.7597709613145 -85.7452678809894
92.6702355060307 -103.795288544077
116.584305081323 -121.827979090175
nan nan
144.989131092817 -128.833419213417
168.928961256724 -146.867694979123
192.829928803241 -164.946392827476
216.770741617965 -182.96154410145
241.055407509795 -200.994065210463
248.623954975812 -206.683210379716
256.430825041137 -213.323663034942
263.001056889201 -222.540970417705
265.205092447492 -234.21292964618
262.637079369829 -246.166581502578
255.613889446558 -255.952382196113
245.884799419419 -261.824940398496
235.82306934627 -264.322652780913
226.295557874421 -265.61803980245
217.085318443029 -266.79870913387
207.932631977533 -267.934384236216
178.092572130033 -271.763429925598
169.533625503441 -273.304127219044
161.357015740327 -275.387082695592
153.584744734942 -277.522053643563
145.976118138128 -279.53323953658
138.392694209663 -281.537521987156
131.016849941599 -284.884706969166
126.076070744926 -291.487880670254
126.483050505156 -299.660270025693
130.657512713043 -306.395516185358
135.236135125511 -312.178614270549
140.429050605405 -319.052769122092
146.188257714293 -327.428689973828
150.723762897474 -338.293521508331
150.906197980943 -350.822697741898
146.105100200058 -362.864095586076
136.627489613763 -371.739775415352
125.148907180393 -376.337191797349
113.953203528081 -375.883202912874
104.1452737393 -372.614639369347
95.3279264135916 -368.712887382295
86.877960292984 -364.922984694077
59.352850221894 -352.12396417451
34.2989699293058 -340.537529945506
25.6022242411947 -336.213867399255
17.604281780447 -329.717178440286
11.1185686381006 -320.568666423082
7.3050838708085 -309.5546965629
7.1419901351141 -297.528985071538
12.2861726475045 -286.618099792315
20.7656528827825 -279.401538758427
29.3339623766934 -274.942112252604
36.0735399053662 -269.661411807544
40.5444078615853 -262.61816135393
42.6010960676145 -254.302649335075
41.89895292102 -246.041065413935
38.7947678744046 -238.360095285852
33.0770485046182 -232.154709882972
25.9526108193331 -227.75652126412
18.5922581793447 -224.514537691475
11.11220920234 -222.029373787834
3.52386620665728 -220.060406532724
-4.17046671145141 -218.947580116658
-11.7535692420996 -218.596425186449
-19.2118529834593 -219.075096842624
-26.6293878729466 -220.131379700228
-33.8315933290271 -221.432928349496
-41.0179347169547 -224.101182013512
-46.4636779103213 -229.899826750435
-46.52003879119 -237.746935874146
-40.4271019792382 -244.438689238106
-33.9690523215023 -253.440662057415
-33.7835283329164 -266.65088639321
-41.6611219007016 -276.910987536455
-51.861587523219 -282.639603430364
-61.7407992066639 -285.480385774896
-71.3362846969693 -286.757927338298
-80.8228422133798 -286.673957222154
-90.1340882971058 -285.787376944119
-119.984405688197 -279.515104394591
-148.408719544409 -269.299747957975
-176.477950030785 -258.538377543843
-204.412569803016 -247.791942154362
-232.386364249342 -237.076403061114
-260.45600160294 -226.378760767563
-271.716162728747 -222.078968496462
-280.327298490059 -218.770163449988
-289.421924887407 -214.974943257447
-298.586660205845 -209.596928167758
-306.028966395446 -201.558533987076
-310.573800521368 -191.084478361745
-311.180769590557 -179.300029786147
-307.955150837421 -168.24168499484
-301.360589585639 -159.489054360083
-293.559699273372 -152.916682784689
-285.557069384187 -147.438187710941
-277.698187876145 -142.237732686032
-269.830587325757 -137.153794415391
-261.827773927665 -132.090264998232
-232.519690570476 -119.879902953181
-201.413660969453 -119.845603406497
-192.938561318556 -121.272662891182
-184.347520483807 -121.61392645265
-175.983245372571 -119.55146505324
-168.810524234462 -115.006899740309
-163.215428366474 -108.742246649759
-159.529230024173 -101.097291801777
-158.023220897554 -92.8541720719034
-158.755971696991 -84.8793944804992
-161.453552955545 -77.5555089850691
-166.168911796944 -70.9467549919986
-172.668082920442 -65.7049953458229
-180.348429221763 -62.3680173713856
-188.759748591361 -61.3344786592153
-197.215555849268 -62.7634532282236
-205.427119884119 -66.3823736469783
-214.16807998922 -70.7482040276206
-224.161471817659 -73.933424051489
-235.050407964241 -73.5910858442907
-245.518765738261 -70.1101246106389
-254.835662668947 -64.3687465658586
-262.785362065112 -57.0063858832726
-269.386284407287 -48.4475798895637
-274.018303149826 -38.7954163700381
-276.402946751579 -28.6331929322303
-276.902472961468 -18.4454437583623
-276.001923503261 -8.539730765245
-274.115588890548 0.96352218836544
-271.568517234434 10.1052454491978
-259.743305973477 38.4660356553289
-246.898590215704 65.7305110693787
-234.048441336169 92.8444817406482
-227.504313197115 106.43246021955
-223.458858145009 114.827416663469
-218.734544051498 124.027266907188
-211.169960178724 132.790900555958
-200.054640744296 137.277632575184
-188.064624498049 136.662659238188
-178.251979621609 130.475151998191
-171.104914897821 122.96819244435
-164.65300780468 115.983313361395
-158.443071403717 109.195190845139
-138.257799894245 87.0241387675423
-115.28010290283 68.1876282749504
-91.4846913888007 50.1758927017112
-67.6514559870563 32.1187922853762
-43.7399446460804 14.0947859300256
-19.896205351212 -4.039863455542
3.96928644323584 -22.1534533939912
27.8543986763264 -40.2476851652628
51.7749352455178 -58.2996693994387
75.6762601214784 -76.3819134804445
99.5783373336458 -94.4658965917211
123.467369071346 -112.568983250506
};
\addplot [line width=1.5pt, TUMred]
table {%
nan nan
191.682001016097 -166.467239417641
215.725762604927 -184.353351287096
239.2006003 -202.98432612
245.45573870498 -209.470860406527
250.605534069048 -216.822785763258
254.090295353301 -225.014512949792
255.16584796 -233.85477576
253.37518359681 -242.570636250054
248.83437064 -250.2094187
242.241707108743 -256.191017017472
234.279330037522 -260.414359797127
225.702651846176 -263.057990909768
216.81995642 -264.5837078
207.803303001811 -265.316897472484
177.880005135764 -265.613213650747
168.882187573041 -266.053941825572
159.928979904366 -267.133924804917
151.150929739414 -269.096396592832
142.701907273037 -272.207259167688
135.009108483381 -276.851046524356
128.67354436 -283.08911432
124.437059 -290.92436838
123.017492916044 -299.699016688095
124.53961404 -308.46129996
128.408945728237 -316.44084911246
133.411811911222 -323.975102664338
138.031457748214 -331.668727312824
140.931045979012 -340.041279217845
140.92102664 -348.9234842
137.560898967162 -357.13799942151
};
\addlegendentry{follow/emergency}
\addplot [line width=1.5pt, TUMblue, dashed]
table {%
167.904150635021 -148.743291219323
169.885034908736 -150.22109622536
171.866037471711 -151.698742687274
173.847155742151 -153.176234023419
175.828387138263 -154.653573652151
177.809729078253 -156.130764991823
179.791178980327 -157.607811460791
181.772734262692 -159.084716477408
183.754392343553 -160.561483460029
185.736150641118 -162.038115827008
187.718006573593 -163.5146169967
189.699957559184 -164.99099038746
191.682001016097 -166.467239417641
193.528105211852 -167.867335801069
195.349302984894 -169.298194292682
197.146244225836 -170.758711691244
198.919578825293 -172.247784795519
200.669956673878 -173.764310404271
202.398027662208 -175.307185316263
204.104441680895 -176.875306330259
205.789848620554 -178.467570245024
207.454898371799 -180.08287385932
209.100240825244 -181.720113971911
210.726525871505 -183.378187381562
212.334403401194 -185.055990887035
213.924523304927 -186.752421287096
215.601060439822 -188.578182700147
217.265195572928 -190.416024166488
218.923949761037 -192.25813042798
220.584344060942 -194.096686226482
222.253399529437 -195.923876303853
223.938137223314 -197.731885401953
225.645578199366 -199.512898262642
227.382743514386 -201.259099627779
229.156654225167 -202.962674239224
230.974331388501 -204.615806838836
232.842796061181 -206.210682168475
234.7690693 -207.73948497
236.487733866589 -209.011675544151
238.23173634792 -210.256173269047
239.977624906537 -211.500892078551
241.70194770498 -212.773745906527
243.362160766204 -214.080554366626
244.973948086958 -215.44584370591
246.53270443274 -216.873536284685
248.033824569048 -218.367554463258
249.494403390094 -219.963349028834
250.854182214749 -221.641454775936
252.077008812617 -223.411219063332
253.126730953301 -225.281989249792
253.995736237493 -227.323179523784
254.631784942133 -229.452247595941
255.025085904031 -231.639383122575
255.16584796 -233.85477576
255.049209912639 -236.080288970085
254.694313391364 -238.286556232995
254.127518063609 -240.45589838192
253.37518359681 -242.570636250054
252.461988888033 -244.611191316946
251.396529616307 -246.570584873757
250.18519409563 -248.439699731202
248.83437064 -250.2094187
247.350725429977 -251.872860856804
245.747962301333 -253.425623844202
244.040237459209 -254.865683838868
242.241707108743 -256.191017017472
240.343862353024 -257.413922616694
238.377551218745 -258.522223335357
236.35272376166 -259.520756589992
234.279330037522 -260.414359797127
232.177726593165 -261.204494821322
230.043810304829 -261.903316824643
227.883484335002 -262.518568092366
225.702651846176 -263.057990909768
223.498429120511 -263.53044547738
221.281741168402 -263.939052947544
219.054834698637 -264.288558621378
216.81995642 -264.5837078
214.571353859126 -264.830017154787
212.318220929428 -265.031138510228
210.061792390469 -265.191841928677
207.803303001811 -265.316897472484
205.312121187768 -265.419010560202
202.820065149493 -265.489003548756
200.327264808359 -265.53228955483
197.833850085737 -265.554281695108
195.339950902998 -265.560393086274
192.845697181514 -265.556036845012
190.351218842656 -265.546626088006
187.856645807796 -265.537573931939
185.362107998305 -265.534293493496
182.867735335555 -265.542197889361
180.373657740918 -265.566700236216
177.880005135764 -265.613213650747
175.628408676139 -265.678718045766
173.377850097396 -265.771041314367
171.128914647156 -265.894632794865
168.882187573041 -266.053941825572
166.635677676107 -266.25360637142
164.393571158841 -266.49750952318
162.157470931506 -266.789624570973
159.928979904366 -267.133924804917
157.7150914381 -267.533201306807
155.512620630157 -267.991370753881
153.32381691808 -268.511435173452
151.150929739414 -269.096396592832
148.993793360076 -269.75116940939
146.861897430596 -270.482360286569
144.762262038931 -271.298284960593
142.701907273037 -272.207259167688
140.690398826304 -273.215012389439
138.732688692559 -274.324489614389
136.83638815164 -275.536298455155
135.009108483381 -276.851046524356
133.276004887603 -278.255382414409
131.632656008528 -279.762421473521
130.093642336035 -281.373290006962
128.67354436 -283.08911432
127.382693285961 -284.914908751135
126.238268187537 -286.836610338575
125.252359835344 -288.843377431728
124.437059 -290.92436838
123.80369045782 -293.064235484048
123.354551844675 -295.250890130169
123.091775288203 -297.467945978229
123.017492916044 -299.699016688095
123.132142954117 -301.928100303828
123.429394499773 -304.140830222989
123.901225534554 -306.32322419268
124.53961404 -308.46129996
125.329690245194 -310.533923124564
126.253462587001 -312.552360026522
127.287643577366 -314.520154183335
128.408945728237 -316.44084911246
129.6162293218 -318.353359147866
130.867347003275 -320.236235420226
132.139980592977 -322.104981926672
133.411811911222 -323.975102664338
134.651965520298 -325.847706546046
135.848905871543 -327.747286428289
136.982210701875 -329.684180590678
138.031457748214 -331.668727312824
138.966614951478 -333.687510629374
139.776732236801 -335.75875694108
140.43910933553 -337.878126414913
140.931045979012 -340.041279217845
141.233743100755 -342.251759770841
141.336373668243 -344.482194975239
141.233835556363 -346.712723546479
140.92102664 -348.9234842
140.39420192957 -351.094604132681
139.655901490364 -353.202867897427
138.710131707766 -355.225068618837
137.560898967162 -357.13799942151
};
\addlegendentry{overtake}
\addplot [semithick, black, mark=square*, mark size=3, mark options={solid, fill=black}, only marks]
table {%
	168.453622372312 -149.145628971799
};
\addlegendentry{EGO}
\addplot [semithick, black, mark=*, mark size=2, mark options={solid, fill=black}, only marks]
table {%
	224.161004819131 -190.6713730709
};
\addlegendentry{OP}
\end{axis}

\end{tikzpicture}


==> ressources/solver_benchmark/scenario/bounds.tex <==
\addplot [line width=0.5599999999999999pt, black]
table {%
5.29929318275232 -38.6274835696298
-19.7530013951774 -22.1576063162077
-44.7455028561287 -5.59286648947496
-69.649403774385 11.1094562148838
-94.6106954768797 27.7300571280032
-119.625882404879 44.2738723902808
-144.601462875557 60.8809270984799
-169.654363605951 77.3752158531742
-194.683198520362 93.9087899525306
-219.621077761655 110.582758538354
-244.64738595424 127.126321643443
-269.582670439703 143.80345622804
-294.647479602027 160.274269628114
-319.648155600856 176.833853872934
-344.668437854297 193.35595254896
-369.605757531968 209.997362679655
-394.545806252567 226.631422987155
-419.536011848845 243.183687552377
-444.542167008443 259.699441483368
-469.511248910739 276.251795911861
-494.478063571428 292.716814128477
-506.413146297155 300.511772528793
-513.044973621819 304.780092884065
-519.304111290012 308.619717904813
-525.546482734455 313.690882645573
-528.647993608537 321.173877358308
-526.389282899835 328.844377651254
-519.967685961555 333.772658649848
-512.194315768232 334.559913086149
-504.920598613445 334.022513921479
-497.830702651901 333.683295806161
-490.246301754339 333.586516107828
-481.989320666273 333.501485228727
-452.464776539133 331.875352864768
-426.546769879068 317.632390062491
-401.869612034778 301.255402948146
-377.002769702098 284.47758990235
-352.019475708475 267.783284768495
-341.968709073766 261.142032194487
-334.216829866479 256.057727222911
-325.854430457474 250.73756465693
-315.682341769538 245.931962288324
-303.395929401975 245.598062684091
-291.906236936424 251.621810123533
-284.501532372823 262.006216467385
-281.943443517496 273.763587677756
-281.096264625985 283.9372963532
-280.163647393197 292.511188295173
-279.387664063 299.876661628724
-278.689121549568 307.089445423123
-276.978275544541 315.278943852754
-272.239332872313 322.47288440568
-264.454392049905 326.086653892313
-255.811040507297 325.984238524864
-247.631419294177 324.759271226907
-239.521711741673 323.304901142698
-231.158133038038 321.864969052861
-202.30743313704 317.235029926376
-173.234701072251 312.760299800832
-144.370558678785 308.284534577759
-116.623566352046 298.542448327578
-94.9220645541587 278.21310801219
-73.6508673393142 258.470806726336
-51.9426522386481 238.623459826207
-29.9642323956338 218.327973380921
-7.87533022567174 198.055542289257
14.2305576139022 177.778521366063
36.2233740758306 157.285276649377
58.4323020793889 136.961823443304
80.549283484264 116.634500675945
102.626245843971 96.3402740131194
125.033845316756 75.9598254059118
131.921181657758 69.6559454777697
139.077666884294 63.2693545926095
146.576322316574 56.7302880479264
154.949071996829 51.2490338497055
164.618888740301 49.2129280893819
174.765786761825 50.2418122474335
184.497099360773 51.4340693418652
193.887434533557 52.7148684818438
203.032925567892 54.0488876799632
212.058637029904 55.3429700838063
242.468126135312 59.8645900296938
271.467313746448 63.9897295122312
279.374144645991 65.1481287662372
287.309721444826 66.33547698426
295.41866506963 67.5511842600362
303.830585612128 68.5042866518592
312.413856365128 68.2378084905216
320.847163427221 66.4073146197272
328.827897307336 63.1137486807755
336.099440974589 58.4878555501693
342.553237798644 52.7534226201233
347.775513347412 45.8008859327381
351.779856811719 38.0456960761247
354.4081520277 29.74757060321
355.416821683959 21.1869820842561
355.016311518954 12.6338715615358
354.026522128626 4.1788142122786
352.949178176063 -4.27709141336005
349.448947577128 -33.0816901801229
345.73567554098 -62.8595691485267
342.074903998562 -92.6436412918349
339.833156022357 -122.549121614873
338.319115940485 -152.629072441516
333.751781184036 -181.651586717985
332.18576963293 -189.82748555104
330.36885722345 -197.841385697104
328.285551583211 -205.752587472485
325.070058741356 -213.34605375678
319.715210136995 -219.871930841364
312.697706445517 -224.779144958612
304.576216207567 -227.59123976182
296.049637852738 -227.848685100143
287.811919242697 -225.83330075576
280.196073145061 -222.068820259636
273.151985679369 -217.25550598328
266.079529281841 -212.355754853481
242.280148285388 -196.360476488124
217.629004206991 -179.825056616793
192.535565777613 -163.269360103336
167.604391092183 -146.612649631858
142.681585849874 -129.924175754029
117.68590211679 -113.332660954669
92.6861849342056 -96.753976700374
67.6083206216054 -80.3020507830256
42.8300809765956 -63.4077459929606
17.8287475395014 -46.8569201386717
nan nan
-2.70945871734768 -50.6658633403298
-27.6754169457528 -34.0531436635881
-52.644807507833 -17.4456807107373
-77.6743620505538 -0.92882757171846
-102.647000387047 15.6727517485551
-127.611528574664 32.2855396290297
-152.620366964654 48.8305232015647
-177.585724124541 65.439310616398
-202.498451168603 82.125807378003
-227.507687050753 98.6650942988931
-252.516155020091 115.203498957638
-277.068451469088 132.434802862243
-302.307235671001 148.62663810361
-327.433436224177 164.992582975798
-352.417454934216 181.579279590617
-377.38129473575 198.202008926031
-402.394484090685 214.753749399967
-427.352722021523 231.385975825064
-452.325788418287 247.98614934654
-477.292806779782 264.579088750316
-502.223580770371 281.214521852845
-514.84450061783 289.641879344718
-522.726567836962 294.902584354082
-531.343170492596 300.857676042611
-540.135386687382 309.51874639504
-543.590844030718 322.275485505051
-539.685435493062 335.544314668624
-529.774021114723 344.248697743226
-518.00646375032 347.403488929949
-507.417694783385 347.597944998915
-497.849871723044 347.245664543779
-488.611070362704 346.835158525442
-479.368640871512 346.373174553421
-447.320642737194 344.20854252766
-420.176427862977 328.466884395892
-394.471943126412 311.466845381823
-369.27695733144 295.098131891066
-344.610511083195 278.743083279198
-335.169098132427 272.070781202163
-328.574899554671 267.376545465664
-322.476082627754 263.055244443204
-315.658267485634 259.223104222463
-307.870930877144 257.870822785234
-300.592088916587 261.103995110695
-296.315893779649 268.033028193424
-295.004113937353 275.941306632068
-293.954122285774 284.603838906239
-292.857504282245 293.817700591634
-291.710048019232 303.156010301608
-290.115181039986 313.198861971653
-286.770538950377 323.860777452923
-279.711805372633 332.947378622617
-269.648418712599 337.950706552058
-258.71191912615 338.632882703255
-248.607209310824 337.538478021917
-239.141919247103 336.20429830207
-229.946693890534 334.718594941252
-200.141465932846 329.950187628956
-170.457323005841 325.010393174338
-139.934378336891 320.164241695462
-110.466943539722 309.807498260185
-87.4002202388514 288.611159715254
-65.1439933593037 268.041097574477
-42.9437054190065 247.677098992292
-20.750014089512 227.338928172104
1.37582110088639 207.023217687628
23.3660179764262 186.577005244474
45.4716894731079 166.271445784771
67.4415525801292 146.121317303381
89.163404016381 126.044032236672
111.251231555103 105.642605889247
132.521364871062 86.1948765385793
138.640123108106 80.4723361608025
144.944254239233 74.5580489029011
151.616078943908 68.5641225826245
159.096983354415 63.5418326670171
167.881621186213 62.1337204876765
176.949542507539 63.1110315181413
185.61869328173 64.3210703320198
193.921646304004 65.6025542747856
201.95487421382 66.8103918225001
209.992698362817 67.9378106812
238.319298912912 71.8929472143155
268.683562004197 76.4843890179969
277.80264331403 77.7582726523816
286.985249573811 79.0591715391525
296.400942293517 80.2883448290817
306.178326552944 81.0684194278963
316.127305068274 80.3106174331119
325.978069061394 77.9621213901224
335.399956896437 73.9333552247662
344.138730234539 68.3353976140474
351.821535803822 61.1788829929112
358.224038538436 52.9222019765511
363.106476058463 43.7812218472437
366.42137542547 34.074710105031
367.941751662744 24.0714107793724
367.757179767609 14.203548688473
366.76006576077 4.682105452312
365.616389442356 -4.57122352413625
362.000092003154 -34.6192711135371
358.423511709058 -64.3780079374835
354.70895180102 -94.1519738771119
351.239092519409 -123.910460422499
347.621924162402 -153.671215610388
343.972963108179 -183.632997218874
342.824043728728 -192.776639553117
341.603184605192 -202.287942998239
340.034814168231 -212.591885296022
335.375677350595 -222.479230605691
327.808190696286 -230.71436852364
318.47962987303 -237.252287610953
307.760248684564 -241.11883546868
296.482125449697 -242.140151031362
285.766710007887 -239.795952581298
276.320816311576 -235.252299270654
267.843379167546 -230.259982304948
259.900972796113 -225.220616477988
234.571225745123 -208.372467250531
209.573827000582 -191.708069412024
184.640995194933 -175.073527774015
159.668833514665 -158.475730978282
134.685983754998 -141.890606426221
109.69789773379 -125.315238530988
84.6826759445607 -108.781780126363
59.7464479243596 -92.1293505717344
34.7701540841678 -75.536151436047
9.8253347368529 -58.8939681260401
};


==> ressources/solver_benchmark/scenario/chosen_path.tex <==
\draw[draw=green,fill=green] (axis cs:-426.353362317105,232.894303170476) circle (2);
\addplot [semithick, color0, mark=*, mark size=3, mark options={solid}, only marks, forget plot]
table {%
-400.484182212832 215.822625046664
};
\addplot [line width=0.5599999999999999pt, yellow, forget plot]
table {%
-351.24982109704 183.353806823386
-376.288648948732 199.859533447812
-401.326287201231 216.370288419848
-426.353362317105 232.894303170476
-451.359340468007 249.440522135324
-476.333697423046 266.01779843358
-501.260677496731 282.644457982621
-513.501989287183 291.372675395685
-520.257956182711 297.421150215265
-525.81622128 304.42111156
-529.559153517081 312.543338643113
-530.49733078 321.31021312
-528.156768780911 329.735014547851
-522.80766872 336.80659232
-515.455604553819 341.766648013633
-506.864058890701 344.588110618649
-497.847317199148 345.43830545114
-488.850950039795 344.891653721598
-479.967485673176 343.431897921253
-451.404353403183 334.417743899321
-424.756499032292 320.677231186508
-399.792309674727 304.122826961
-375.50566122 286.5356393
};
\addplot [line width=0.5599999999999999pt, yellow, forget plot]
table {%
-399.240079882736 214.993987452452
-401.326287201231 216.370288419848
-403.412318141957 217.746623326118
-405.498278856544 219.123068375412
-407.584166339321 220.49962686971
-409.669977584616 221.876302110995
-411.755709586759 223.253097401247
-413.841359340078 224.630016042446
-415.926923838902 226.007061336574
-418.012400077559 227.384236585611
-420.09778505038 228.761545091539
-422.183075751691 230.138990156339
-424.268269175824 231.516575081991
-426.353362317105 232.894303170476
-428.437990608709 234.271941792304
-430.522503022921 235.649741935725
-432.606890862285 237.027721305637
-434.691145429345 238.405897606939
-436.775258026642 239.784288544532
-438.85921995672 241.162911823314
-440.943022522123 242.541785148183
-443.026657025392 243.92092622404
-445.110114769073 245.300352755784
-447.193387055706 246.680082448313
-449.276465187837 248.060133006526
-451.359340468007 249.440522135324
-453.441368795907 250.820834950888
-455.523199587836 252.201468937826
-457.604846727404 253.582389210688
-459.686324098222 254.963560884021
-461.7676455839 256.344949072376
-463.84882506805 257.726518890301
-465.929876434282 259.108235452345
-468.010813566206 260.490063873059
-470.091650347434 261.87196926699
-472.172400661577 263.253916748687
-474.253078392244 264.635871432701
-476.333697423046 266.01779843358
-478.413418011888 267.399145433635
-480.493000423637 268.780620900528
-482.572351261454 270.162415819429
-484.651377128503 271.544721175506
-486.729984627946 272.927727953926
-488.808080362945 274.311627139858
-490.885570936664 275.696609718471
-492.962362952264 277.082866674931
-495.038363012909 278.470588994409
-497.113477721759 279.859967662071
-499.187613681979 281.251193663085
-501.260677496731 282.644457982621
-503.042748886364 283.845802735891
-504.820116952546 285.053871836276
-506.588941176863 286.273739365227
-508.3453810409 287.510479404193
-510.085596026243 288.769166034625
-511.805745614475 290.054873337972
-513.501989287183 291.372675395685
-515.262063756796 292.804857731612
-516.981329689296 294.285592624924
-518.649917144621 295.821987608511
-520.257956182711 297.421150215265
-521.775395882579 299.066380566848
-523.214268505204 300.780721121428
-524.564551240904 302.565266559111
-525.81622128 304.42111156
-526.960227860891 306.352606134196
-527.977289096115 308.352804391456
-528.849549482552 310.417713003766
-529.559153517081 312.543338643113
-530.084048073333 314.696305029348
-530.422356791521 316.886909043553
-530.563608188219 319.097446476759
-530.49733078 321.31021312
-530.218789196953 323.490435031955
-529.731724099843 325.634951752023
-529.042321843039 327.723299513042
-528.156768780911 329.735014547851
-527.06757116329 331.676336155503
-525.801119769892 333.50840710996
-524.375217866776 335.221676226399
-522.80766872 336.80659232
-521.117974330691 338.253434471628
-519.319537761437 339.56252180701
-517.427150629919 340.733658322296
-515.455604553819 341.766648013633
-513.3805761572 342.677303974826
-511.249692270743 343.448431879146
-509.073878110045 344.084033501963
-506.864058890701 344.588110618649
-504.629369812339 344.965882628028
-502.37764220681 345.226511734238
-500.114937520337 345.380488990775
-497.847317199148 345.43830545114
-495.59283431143 345.410334594778
-493.340961044066 345.305003571431
-491.093174064405 345.129660555553
-488.850950039795 344.891653721598
-486.6188748642 344.598325443945
-484.3940908255 344.254292217887
-482.176870302293 343.864000793598
-479.967485673176 343.431897921253
-477.711102783219 342.949561029742
-475.463529230701 342.428837135948
-473.225054235831 341.870601805416
-470.995967018814 341.275730603691
-468.776556799857 340.645099096316
-466.567112799167 339.979582848838
-464.367924236951 339.2800574268
-462.179280333415 338.547398395746
-460.001470308767 337.782481321223
-457.834783383213 336.986181768774
-455.679508776959 336.159375303945
-453.535935710214 335.302937492278
-451.404353403183 334.417743899321
-449.284528840314 333.504466780454
};
\addplot [line width=0.5599999999999999pt, TUMred, forget plot]
table {%
-399.240079882736 214.993987452452
-401.326287201231 216.370288419848
-403.412318141957 217.746623326118
-405.498278856544 219.123068375412
-407.584166339321 220.49962686971
-409.669977584616 221.876302110995
-411.755709586759 223.253097401247
-413.841359340078 224.630016042446
-415.926923838902 226.007061336574
-418.012400077559 227.384236585611
-420.09778505038 228.761545091539
-422.183075751691 230.138990156339
-424.268269175824 231.516575081991
-426.353362317105 232.894303170476
-428.437990608709 234.271941792304
-430.522503022921 235.649741935725
-432.606890862285 237.027721305637
-434.691145429345 238.405897606939
-436.775258026642 239.784288544532
-438.85921995672 241.162911823314
-440.943022522123 242.541785148183
-443.026657025392 243.92092622404
-445.110114769073 245.300352755784
-447.193387055706 246.680082448313
-449.276465187837 248.060133006526
-451.359340468007 249.440522135324
-453.441368795907 250.820834950888
-455.523199587836 252.201468937826
-457.604846727404 253.582389210688
-459.686324098222 254.963560884021
-461.7676455839 256.344949072376
-463.84882506805 257.726518890301
-465.929876434282 259.108235452345
-468.010813566206 260.490063873059
-470.091650347434 261.87196926699
-472.172400661577 263.253916748687
-474.253078392244 264.635871432701
-476.333697423046 266.01779843358
-478.413418011888 267.399145433635
-480.493000423637 268.780620900528
-482.572351261454 270.162415819429
-484.651377128503 271.544721175506
-486.729984627946 272.927727953926
-488.808080362945 274.311627139858
-490.885570936664 275.696609718471
-492.962362952264 277.082866674931
-495.038363012909 278.470588994409
-497.113477721759 279.859967662071
-499.187613681979 281.251193663085
-501.260677496731 282.644457982621
-503.042748886364 283.845802735891
-504.820116952546 285.053871836276
-506.588941176863 286.273739365227
-508.3453810409 287.510479404193
-510.085596026243 288.769166034625
-511.805745614475 290.054873337972
-513.501989287183 291.372675395685
-515.262063756796 292.804857731612
-516.981329689296 294.285592624924
-518.649917144621 295.821987608511
-520.257956182711 297.421150215265
-521.775395882579 299.066380566848
-523.214268505204 300.780721121428
-524.564551240904 302.565266559111
-525.81622128 304.42111156
-526.960227860891 306.352606134196
-527.977289096115 308.352804391456
-528.849549482552 310.417713003766
-529.559153517081 312.543338643113
-530.084048073333 314.696305029348
-530.422356791521 316.886909043553
-530.563608188219 319.097446476759
-530.49733078 321.31021312
-530.218789196953 323.490435031955
-529.731724099843 325.634951752023
-529.042321843039 327.723299513042
-528.156768780911 329.735014547851
-527.06757116329 331.676336155503
-525.801119769892 333.50840710996
-524.375217866776 335.221676226399
-522.80766872 336.80659232
-521.117974330691 338.253434471628
-519.319537761437 339.56252180701
-517.427150629919 340.733658322296
-515.455604553819 341.766648013633
-513.3805761572 342.677303974826
-511.249692270743 343.448431879146
-509.073878110045 344.084033501963
-506.864058890701 344.588110618649
-504.629369812339 344.965882628028
-502.37764220681 345.226511734238
-500.114937520337 345.380488990775
-497.847317199148 345.43830545114
-495.59283431143 345.410334594778
-493.340961044066 345.305003571431
-491.093174064405 345.129660555553
-488.850950039795 344.891653721598
-486.6188748642 344.598325443945
-484.3940908255 344.254292217887
-482.176870302293 343.864000793598
-479.967485673176 343.431897921253
-477.711102783219 342.949561029742
-475.463529230701 342.428837135948
-473.225054235831 341.870601805416
-470.995967018814 341.275730603691
-468.776556799857 340.645099096316
-466.567112799167 339.979582848838
-464.367924236951 339.2800574268
-462.179280333415 338.547398395746
-460.001470308767 337.782481321223
-457.834783383213 336.986181768774
-455.679508776959 336.159375303945
-453.535935710214 335.302937492278
-451.404353403183 334.417743899321
-449.284528840314 333.504466780454
};

==> ressources/solver_benchmark/scenario/nodes.tex <==
\addplot [semithick, TUMblue, mark=x, mark size=1, mark options={solid}, only marks]
table {%
-1.75329377814429 -49.228601104573
-1.47634682814429 -48.812307454573
-1.19939987814429 -48.396013804573
-0.92245292814429 -47.979720154573
-0.64550597814429 -47.563426504573
-0.36855902814429 -47.147132854573
-0.09161207814429 -46.730839204573
0.18533487185571 -46.314545554573
0.46228182185571 -45.898251904573
0.73922877185571 -45.481958254573
1.01617572185571 -45.065664604573
1.29312267185571 -44.649370954573
1.57006962185571 -44.233077304573
1.84701657185571 -43.816783654573
2.12396352185571 -43.400490004573
2.40091047185571 -42.984196354573
2.67785742185571 -42.567902704573
2.95480437185571 -42.151609054573
3.23175132185571 -41.735315404573
3.50869827185571 -41.319021754573
3.78564522185571 -40.902728104573
4.06259217185571 -40.486434454573
4.33953912185571 -40.070140804573
-26.7258494442021 -32.6273644165333
-26.4486917442021 -32.2112110665333
-26.1715340442021 -31.7950577165333
-25.8943763442021 -31.3789043665333
-25.6172186442021 -30.9627510165333
-25.3400609442021 -30.5465976665333
-25.0629032442021 -30.1304443165333
-24.7857455442021 -29.7142909665333
-24.5085878442021 -29.2981376165333
-24.2314301442021 -28.8819842665333
-23.9542724442021 -28.4658309165333
-23.6771147442021 -28.0496775665333
-23.3999570442021 -27.6335242165333
-23.1227993442021 -27.2173708665333
-22.8456416442021 -26.8012175165333
-22.5684839442021 -26.3850641665333
-22.2913262442021 -25.9689108165333
-22.0141685442021 -25.5527574665333
-21.7370108442021 -25.1366041165333
-21.4598531442021 -24.7204507665333
-21.1826954442021 -24.3042974165333
-20.9055377442021 -23.8881440665333
-20.6283800442021 -23.4719907165333
-51.701341994585 -16.0300217450733
-51.424054394585 -15.6139549450733
-51.146766794585 -15.1978881450733
-50.869479194585 -14.7818213450733
-50.592191594585 -14.3657545450733
-50.314903994585 -13.9496877450733
-50.037616394585 -13.5336209450733
-49.760328794585 -13.1175541450733
-49.483041194585 -12.7014873450733
-49.205753594585 -12.2854205450733
-48.928465994585 -11.8693537450733
-48.651178394585 -11.4532869450733
-48.373890794585 -11.0372201450733
-48.096603194585 -10.6211533450733
-47.819315594585 -10.2050865450733
-47.542027994585 -9.78901974507328
-47.264740394585 -9.37295294507328
-46.987452794585 -8.95688614507328
-46.710165194585 -8.54081934507328
-46.432877594585 -8.12475254507328
-46.155589994585 -7.70868574507328
-45.878302394585 -7.29261894507328
-45.601014794585 -6.87655214507328
-76.680309189896 0.56235655954599
-76.402972589896 0.97839070954599
-76.125635989896 1.39442485954599
-75.848299389896 1.81045900954599
-75.570962789896 2.22649315954599
-75.293626189896 2.64252730954599
-75.016289589896 3.05856145954599
-74.738952989896 3.47459560954599
-74.461616389896 3.89062975954599
-74.184279789896 4.30666390954599
-73.906943189896 4.72269805954599
-73.629606589896 5.13873220954599
-73.352269989896 5.55476635954599
-73.074933389896 5.97080050954599
-72.797596789896 6.38683465954599
-72.520260189896 6.80286880954599
-72.242923589896 7.21890295954599
-71.965586989896 7.63493710954599
-71.688250389896 8.05097125954599
-71.410913789896 8.46700540954599
-71.133577189896 8.88303955954599
-70.856240589896 9.29907370954599
-70.578903989896 9.71510785954599
-101.663273987831 17.1486899736175
-101.385969237831 17.5647453736175
-101.108664487831 17.9808007736175
-100.831359737831 18.3968561736175
-100.554054987831 18.8129115736175
-100.276750237831 19.2289669736175
-99.9994454878307 19.6450223736175
-99.7221407378307 20.0610777736175
-99.4448359878307 20.4771331736175
-99.1675312378307 20.8931885736175
-98.8902264878307 21.3092439736175
-98.6129217378307 21.7252993736175
-98.3356169878307 22.1413547736175
-98.0583122378307 22.5574101736175
-97.7810074878307 22.9734655736175
-97.5037027378307 23.3895209736175
-97.2263979878307 23.8055763736175
-96.9490932378307 24.2216317736175
-96.6717884878307 24.6376871736175
-96.3944837378307 25.0537425736175
-96.1171789878307 25.4697979736175
-95.8398742378307 25.8858533736175
-95.5625694878307 26.3019087736175
-126.650751380691 33.7278921282357
-126.373559330691 34.1440225782357
-126.096367280691 34.5601530282357
-125.819175230691 34.9762834782357
-125.541983180691 35.3924139282357
-125.264791130691 35.8085443782357
-124.987599080691 36.2246748282357
-124.710407030691 36.6408052782357
-124.433214980691 37.0569357282357
-124.156022930691 37.4730661782357
-123.878830880691 37.8891966282357
-123.601638830691 38.3053270782357
-123.324446780691 38.7214575282357
-123.047254730691 39.1375879782357
-122.770062680691 39.5537184282357
-122.492870630691 39.9698488782357
-122.215678580691 40.3859793282357
-121.938486530691 40.8021097782357
-121.661294480691 41.2182402282357
-121.384102430691 41.6343706782357
-121.106910380691 42.0505011282357
-120.829718330691 42.4666315782357
-120.552526280691 42.8827620282357
-151.643255697699 50.2988766434079
-151.366257197699 50.7151359934079
-151.089258697699 51.1313953434079
-150.812260197699 51.5476546934079
-150.535261697699 51.9639140434079
-150.258263197699 52.3801733934079
-149.981264697699 52.7964327434079
-149.704266197699 53.2126920934079
-149.427267697699 53.6289514434079
-149.150269197699 54.0452107934079
-148.873270697699 54.4614701434079
-148.596272197699 54.8777294934079
-148.319273697699 55.2939888434079
-148.042275197699 55.7102481934079
-147.765276697699 56.1265075434079
-147.488278197699 56.5427668934079
-147.211279697699 56.9590262434079
-146.934281197699 57.3752855934079
-146.657282697699 57.7915449434079
-146.380284197699 58.2078042934079
-146.103285697699 58.6240636434079
-145.826287197699 59.0403229934079
-145.549288697699 59.4565823434079
-176.641307621955 66.8605631054873
-176.364583671955 67.2770050054873
-176.087859721955 67.6934469054873
-175.811135771955 68.1098888054873
-175.534411821955 68.5263307054873
-175.257687871955 68.9427726054873
-174.980963921955 69.3592145054873
-174.704239971955 69.7756564054873
-174.427516021955 70.1920983054873
-174.150792071955 70.6085402054873
-173.874068121955 71.0249821054873
-173.597344171955 71.4414240054873
-173.320620221955 71.8578659054873
-173.043896271955 72.2743078054873
-172.767172321955 72.6907497054873
-172.490448371955 73.1071916054873
-172.213724421955 73.5236335054873
-171.937000471955 73.9400754054873
-171.660276521955 74.3565173054873
-171.383552571955 74.7729592054873
-171.106828621955 75.1894011054873
-170.830104671955 75.6058430054873
-170.553380721955 76.0222849054873
-201.645441748717 83.4118816206171
-201.369073398717 83.8285595706171
-201.092705048717 84.2452375206171
-200.816336698717 84.6619154706171
-200.539968348717 85.0785934206171
-200.263599998717 85.4952713706171
-199.987231648717 85.9119493206171
-199.710863298717 86.3286272706171
-199.434494948717 86.7453052206171
-199.158126598717 87.1619831706171
-198.881758248717 87.5786611206171
-198.605389898717 87.9953390706171
-198.329021548717 88.4120170206171
-198.052653198717 88.8286949706171
-197.776284848717 89.2453729206171
-197.499916498717 89.6620508706171
-197.223548148717 90.0787288206171
-196.947179798717 90.4954067706171
-196.670811448717 90.9120847206171
-196.394443098717 91.3287626706171
-196.118074748717 91.7454406206171
-195.841706398717 92.1621185706171
-195.565338048717 92.5787965206171
-226.656213599453 99.9517783895372
-226.380282099453 100.368745789537
-226.104350599453 100.785713189537
-225.828419099453 101.202680589537
-225.552487599453 101.619647989537
-225.276556099453 102.036615389537
-225.000624599453 102.453582789537
-224.724693099453 102.870550189537
-224.448761599453 103.287517589537
-224.172830099453 103.704484989537
-223.896898599453 104.121452389537
-223.620967099453 104.538419789537
-223.345035599453 104.955387189537
-223.069104099453 105.372354589537
-222.793172599453 105.789321989537
-222.517241099453 106.206289389537
-222.241309599453 106.623256789537
-221.965378099453 107.040224189537
-221.689446599453 107.457191589537
-221.413515099453 107.874158989537
-221.137583599453 108.291126389537
-220.861652099453 108.708093789537
-220.585720599453 109.125061189537
-251.674172161192 116.479278211943
-251.398758211192 116.896587661943
-251.123344261192 117.313897111943
-250.847930311192 117.731206561943
-250.572516361192 118.148516011943
-250.297102411192 118.565825461943
-250.021688461192 118.983134911943
-249.746274511192 119.400444361943
-249.470860561192 119.817753811943
-249.195446611192 120.235063261943
-248.920032661192 120.652372711943
-248.644618711192 121.069682161943
-248.369204761192 121.486991611943
-248.093790811192 121.904301061943
-247.818376861192 122.321610511943
-247.542962911192 122.738919961943
-247.267548961192 123.156229411943
-246.992135011192 123.573538861943
-246.716721061192 123.990848311943
-246.441307111192 124.408157761943
-246.165893161192 124.825467211943
-245.890479211192 125.242776661943
-245.615065261192 125.660086111943
-276.148649158058 133.831706351418
-275.873676758058 134.249306851418
-275.598704358058 134.666907351418
-275.323731958058 135.084507851418
-275.048759558058 135.502108351418
-274.773787158058 135.919708851418
-274.498814758058 136.337309351418
-274.223842358058 136.754909851418
-273.948869958058 137.172510351418
-273.673897558058 137.590110851418
-273.398925158058 138.007711351418
-273.123952758058 138.425311851418
-272.848980358058 138.842912351418
-272.574007958058 139.260512851418
-272.299035558058 139.678113351418
-272.024063158058 140.095713851418
-271.749090758058 140.513314351418
-271.474118358058 140.930914851418
-271.199145958058 141.348515351418
-270.924173558058 141.766115851418
-270.649201158058 142.183716351418
-270.374228758058 142.601316851418
-301.453551376352 149.924773450582
-301.178822226352 150.342534000582
-300.904093076352 150.760294550582
-300.629363926352 151.178055100582
-300.354634776352 151.595815650582
-300.079905626352 152.013576200582
-299.805176476352 152.431336750582
-299.530447326352 152.849097300582
-299.255718176352 153.266857850582
-298.980989026352 153.684618400582
-298.706259876352 154.102378950582
-298.431530726352 154.520139500582
-298.156801576352 154.937900050582
-297.882072426352 155.355660600582
-297.607343276352 155.773421150582
-297.332614126352 156.191181700582
-297.057884976352 156.608942250582
-296.783155826352 157.026702800582
-296.508426676352 157.444463350582
-296.233697526352 157.862223900582
-295.958968376352 158.279984450582
-295.684239226352 158.697745000582
-326.487566151275 166.431234234324
-326.212881751275 166.849024234324
-325.938197351275 167.266814234324
-325.663512951275 167.684604234324
-325.388828551275 168.102394234324
-325.114144151275 168.520184234324
-324.839459751275 168.937974234324
-324.564775351275 169.355764234324
-324.290090951275 169.773554234324
-324.015406551275 170.191344234324
-323.740722151275 170.609134234324
-323.466037751275 171.026924234324
-323.191353351275 171.444714234324
-322.916668951275 171.862504234324
-322.641984551275 172.280294234324
-322.367300151275 172.698084234324
-322.092615751275 173.115874234324
-321.817931351275 173.533664234324
-321.543246951275 173.951454234324
-321.268562551275 174.369244234324
-320.993878151275 174.787034234324
-320.719193751275 175.204824234324
-320.444509351275 175.622614234324
-351.52465919704 182.936117923386
-351.24982109704 183.353806823386
-350.97498299704 183.771495723386
-350.70014489704 184.189184623386
-350.42530679704 184.606873523386
-350.15046869704 185.024562423386
-349.87563059704 185.442251323386
-349.60079249704 185.859940223386
-349.32595439704 186.277629123386
-349.05111629704 186.695318023386
-348.77627819704 187.113006923386
-348.50144009704 187.530695823386
-348.22660199704 187.948384723386
-347.95176389704 188.366073623386
-347.67692579704 188.783762523386
-347.40208769704 189.201451423386
-347.12724959704 189.619140323386
-346.85241149704 190.036829223386
-346.57757339704 190.454518123386
-346.30273529704 190.872207023386
-346.02789719704 191.289895923386
-345.75305909704 191.707584823386
-345.47822099704 192.125273723386
-376.563838348732 199.442075947812
-376.288648948732 199.859533447812
-376.013459548732 200.276990947811
-375.738270148732 200.694448447812
-375.463080748732 201.111905947812
-375.187891348732 201.529363447812
-374.912701948732 201.946820947812
-374.637512548732 202.364278447812
-374.362323148732 202.781735947812
-374.087133748732 203.199193447811
-373.811944348732 203.616650947812
-373.536754948732 204.034108447812
-373.261565548732 204.451565947812
-372.986376148732 204.869023447812
-372.711186748732 205.286480947811
-372.435997348732 205.703938447812
-372.160807948732 206.121395947812
-371.885618548732 206.538853447812
-371.610429148732 206.956310947812
-371.335239748732 207.373768447811
-371.060050348732 207.791225947812
-370.784860948732 208.208683447811
-370.509671548732 208.626140947812
-401.601938551231 215.953135769848
-401.326287201231 216.370288419848
-401.050635851231 216.787441069848
-400.774984501231 217.204593719848
-400.499333151231 217.621746369848
-400.223681801231 218.038899019848
-399.948030451231 218.456051669848
-399.672379101231 218.873204319848
-399.396727751231 219.290356969848
-399.121076401231 219.707509619848
-398.845425051231 220.124662269848
-398.569773701231 220.541814919848
-398.294122351231 220.958967569848
-398.018471001231 221.376120219848
-397.742819651231 221.793272869848
-397.467168301231 222.210425519848
-397.191516951231 222.627578169848
-396.915865601231 223.044730819848
-396.640214251231 223.461883469848
-396.364562901231 223.879036119848
-396.088911551231 224.296188769848
-395.813260201231 224.713341419848
-395.537608851231 225.130494069848
-426.353362317105 232.894303170476
-426.077197917105 233.311116370476
-425.801033517105 233.727929570476
-425.524869117105 234.144742770476
-425.248704717105 234.561555970476
-424.972540317105 234.978369170476
-424.696375917105 235.395182370476
-424.420211517105 235.811995570476
-424.144047117105 236.228808770476
-423.867882717105 236.645621970476
-423.591718317105 237.062435170476
-423.315553917105 237.479248370476
-423.039389517105 237.896061570476
-422.763225117105 238.312874770476
-422.487060717105 238.729687970476
-422.210896317105 239.146501170476
-421.934731917105 239.563314370476
-421.658567517105 239.980127570476
-421.382403117105 240.396940770476
-421.106238717105 240.813753970476
-420.830074317105 241.230567170476
-420.553909917105 241.647380370476
-451.359340468007 249.440522135324
-451.082611918007 249.856960985324
-450.805883368007 250.273399835324
-450.529154818007 250.689838685324
-450.252426268007 251.106277535324
-449.975697718007 251.522716385324
-449.698969168007 251.939155235324
-449.422240618007 252.355594085324
-449.145512068007 252.772032935324
-448.868783518007 253.188471785324
-448.592054968007 253.604910635324
-448.315326418007 254.021349485324
-448.038597868007 254.437788335324
-447.761869318007 254.854227185324
-447.485140768007 255.270666035324
-447.208412218007 255.687104885324
-446.931683668007 256.103543735324
-446.654955118007 256.519982585324
-446.378226568007 256.936421435324
-446.101498018007 257.352860285324
-445.824769468007 257.769299135324
-445.548040918007 258.185737985324
-476.333697423046 266.01779843358
-476.056353423046 266.433827633581
-475.779009423046 266.849856833581
-475.501665423046 267.265886033581
-475.224321423046 267.681915233581
-474.946977423046 268.09794443358
-474.669633423046 268.513973633581
-474.392289423046 268.93000283358
-474.114945423046 269.346032033581
-473.837601423046 269.76206123358
-473.560257423046 270.178090433581
-473.282913423046 270.594119633581
-473.005569423046 271.010148833581
-472.728225423046 271.426178033581
-472.450881423046 271.84220723358
-472.173537423046 272.258236433581
-471.896193423046 272.67426563358
-471.618849423046 273.090294833581
-471.341505423046 273.50632403358
-471.064161423046 273.922353233581
-470.786817423046 274.33838243358
-470.509473423046 274.754411633581
-501.260677496731 282.644457982621
-500.981400246731 283.059191882621
-500.702122996731 283.473925782621
-500.422845746731 283.888659682621
-500.143568496731 284.303393582621
-499.864291246731 284.718127482621
-499.585013996731 285.132861382621
-499.305736746731 285.547595282621
-499.026459496731 285.962329182621
-498.747182246731 286.377063082621
-498.467904996731 286.791796982621
-498.188627746731 287.206530882621
-497.909350496731 287.621264782621
-497.630073246731 288.035998682621
-497.350795996731 288.450732582621
-497.071518746731 288.865466482621
-496.792241496731 289.280200382621
-496.512964246731 289.694934282621
-496.233686996731 290.109668182621
-495.954409746731 290.524402082621
-495.675132496731 290.939135982621
-495.395855246731 291.353869882621
-513.808438287183 290.977594395685
-513.501989287183 291.372675395685
-513.195540287183 291.767756395685
-512.889091287183 292.162837395685
-512.582642287183 292.557918395685
-512.276193287183 292.952999395685
-511.969744287183 293.348080395685
-511.663295287183 293.743161395685
-511.356846287183 294.138242395685
-511.050397287183 294.533323395685
-510.743948287183 294.928404395685
-510.437499287183 295.323485395685
-510.131050287183 295.718566395685
-509.824601287183 296.113647395685
-509.518152287183 296.508728395685
-509.211703287183 296.903809395685
-508.905254287183 297.298890395685
-508.598805287183 297.693971395685
-508.292356287183 298.089052395685
-507.985907287183 298.484133395685
-507.679458287183 298.879214395685
-507.373009287183 299.274295395685
-521.657933982711 295.992842815265
-521.307939532711 296.349919665265
-520.957945082711 296.706996515265
-520.607950632711 297.064073365265
-520.257956182711 297.421150215265
-519.907961732711 297.778227065265
-519.557967282711 298.135303915265
-519.207972832711 298.492380765265
-518.857978382711 298.849457615265
-518.507983932711 299.206534465265
-518.157989482711 299.563611315265
-517.807995032711 299.920688165265
-517.458000582711 300.277765015265
-517.108006132711 300.634841865265
-516.758011682711 300.991918715265
-516.408017232711 301.348995565265
-516.058022782711 301.706072415265
-515.708028332711 302.063149265265
-515.358033882711 302.420226115265
-515.008039432711 302.777302965265
-514.658044982711 303.134379815265
-514.308050532711 303.491456665265
-530.01851428 301.71173256
-529.59828498 301.98267046
-529.17805568 302.25360836
-528.75782638 302.52454626
-528.33759708 302.79548416
-527.91736778 303.06642206
-527.49713848 303.33735996
-527.07690918 303.60829786
-526.65667988 303.87923576
-526.23645058 304.15017366
-525.81622128 304.42111156
-525.39599198 304.69204946
-524.97576268 304.96298736
-524.55553338 305.23392526
-524.13530408 305.50486316
-523.71507478 305.77580106
-523.29484548 306.04673896
-522.87461618 306.31767686
-522.45438688 306.58861476
-522.03415758 306.85955266
-521.61392828 307.13049056
-521.19369898 307.40142846
-520.77346968 307.67236636
-538.692989317081 309.931243343113
-538.212261117081 310.068722043113
-537.731532917081 310.206200743113
-537.250804717081 310.343679443113
-536.770076517081 310.481158143113
-536.289348317081 310.618636843113
-535.808620117081 310.756115543113
-535.327891917081 310.893594243113
-534.847163717081 311.031072943113
-534.366435517081 311.168551643113
-533.885707317081 311.306030343113
-533.404979117081 311.443509043113
-532.924250917081 311.580987743113
-532.443522717081 311.718466443113
-531.962794517081 311.855945143113
-531.482066317081 311.993423843113
-531.001338117081 312.130902543113
-530.520609917081 312.268381243113
-530.039881717081 312.405859943113
-529.559153517081 312.543338643113
-529.078425317081 312.680817343113
-528.597697117081 312.818296043113
-528.116968917081 312.955774743113
-527.636240717081 313.093253443113
-527.155512517081 313.230732143113
-541.96620718 322.15571497
-541.46756038 322.11895402
-540.96891358 322.08219307
-540.47026678 322.04543212
-539.97161998 322.00867117
-539.47297318 321.97191022
-538.97432638 321.93514927
-538.47567958 321.89838832
-537.97703278 321.86162737
-537.47838598 321.82486642
-536.97973918 321.78810547
-536.48109238 321.75134452
-535.98244558 321.71458357
-535.48379878 321.67782262
-534.98515198 321.64106167
-534.48650518 321.60430072
-533.98785838 321.56753977
-533.48921158 321.53077882
-532.99056478 321.49401787
-532.49191798 321.45725692
-531.99327118 321.42049597
-531.49462438 321.38373502
-530.99597758 321.34697407
-530.49733078 321.31021312
-538.426609180911 334.909991547851
-537.980094380911 334.684992547851
-537.533579580911 334.459993547851
-537.087064780911 334.234994547851
-536.640549980911 334.009995547851
-536.194035180911 333.784996547851
-535.747520380911 333.559997547851
-535.301005580911 333.334998547851
-534.854490780911 333.109999547851
-534.407975980911 332.885000547851
-533.961461180911 332.660001547851
-533.514946380911 332.435002547851
-533.068431580911 332.210003547851
-532.621916780911 331.985004547851
-532.175401980911 331.760005547851
-531.728887180911 331.535006547851
-531.282372380911 331.310007547851
-530.835857580911 331.085008547851
-530.389342780911 330.860009547851
-529.942827980911 330.635010547851
-529.496313180911 330.410011547851
-529.049798380911 330.185012547851
-528.603283580911 329.960013547851
-528.156768780911 329.735014547851
-527.710253980911 329.510015547851
-528.61645312 343.01207597
-528.27475992 342.64704752
-527.93306672 342.28201907
-527.59137352 341.91699062
-527.24968032 341.55196217
-526.90798712 341.18693372
-526.56629392 340.82190527
-526.22460072 340.45687682
-525.88290752 340.09184837
-525.54121432 339.72681992
-525.19952112 339.36179147
-524.85782792 338.99676302
-524.51613472 338.63173457
-524.17444152 338.26670612
-523.83274832 337.90167767
-523.49105512 337.53664922
-523.14936192 337.17162077
-522.80766872 336.80659232
-522.46597552 336.44156387
-522.12428232 336.07653542
-521.78258912 335.71150697
-521.44089592 335.34647852
-521.09920272 334.98145007
-517.310878953819 345.866398663633
-517.104737353819 345.410870813633
-516.898595753819 344.955342963633
-516.692454153819 344.499815113633
-516.486312553819 344.044287263633
-516.280170953819 343.588759413633
-516.074029353819 343.133231563633
-515.867887753819 342.677703713633
-515.661746153819 342.222175863633
-515.455604553819 341.766648013633
-515.249462953819 341.311120163633
-515.043321353819 340.855592313633
-514.837179753819 340.400064463633
-514.631038153819 339.944536613633
-514.424896553819 339.489008763633
-514.218754953819 339.033480913633
-514.012613353819 338.577953063633
-513.806471753819 338.122425213633
-513.600330153819 337.666897363633
-513.394188553819 337.211369513633
-513.188046953819 336.755841663633
-512.981905353819 336.300313813633
-512.775763753819 335.844785963633
-507.135419840701 346.063360918649
-507.044966190701 345.571610818649
-506.954512540701 345.079860718649
-506.864058890701 344.588110618649
-506.773605240701 344.096360518649
-506.683151590701 343.604610418649
-506.592697940701 343.112860318649
-506.502244290701 342.621110218649
-506.411790640701 342.129360118649
-506.321336990701 341.637610018649
-506.230883340701 341.145859918649
-506.140429690701 340.654109818649
-506.049976040701 340.162359718649
-505.959522390701 339.670609618649
-505.869068740701 339.178859518649
-505.778615090701 338.687109418649
-505.688161440701 338.195359318649
-505.597707790701 337.703609218649
-505.507254140701 337.211859118649
-505.416800490701 336.720109018649
-505.326346840701 336.228358918649
-505.235893190701 335.736608818649
-497.847317199148 345.43830545114
-497.846610499148 344.93830595114
-497.845903799148 344.43830645114
-497.845197099148 343.93830695114
-497.844490399148 343.43830745114
-497.843783699148 342.93830795114
-497.843076999148 342.43830845114
-497.842370299148 341.93830895114
-497.841663599148 341.43830945114
-497.840956899148 340.93830995114
-497.840250199148 340.43831045114
-497.839543499148 339.93831095114
-497.838836799148 339.43831145114
-497.838130099148 338.93831195114
-497.837423399148 338.43831245114
-497.836716699148 337.93831295114
-497.836009999148 337.43831345114
-497.835303299148 336.93831395114
-497.834596599148 336.43831445114
-497.833889899148 335.93831495114
-497.833183199148 335.43831545114
-488.789701639795 345.387888171598
-488.850950039795 344.891653721598
-488.912198439795 344.395419271598
-488.973446839795 343.899184821598
-489.034695239795 343.402950371598
-489.095943639795 342.906715921598
-489.157192039795 342.410481471598
-489.218440439795 341.914247021598
-489.279688839795 341.418012571598
-489.340937239795 340.921778121598
-489.402185639795 340.425543671598
-489.463434039795 339.929309221598
-489.524682439795 339.433074771598
-489.585930839795 338.936840321598
-489.647179239795 338.440605871598
-489.708427639795 337.944371421598
-489.769676039795 337.448136971598
-489.830924439795 336.951902521598
-489.892172839795 336.455668071598
-489.953421239795 335.959433621598
-490.014669639795 335.463199171598
-479.668224873176 344.901742521253
-479.767978473176 344.411794321253
-479.867732073176 343.921846121253
-479.967485673176 343.431897921253
-480.067239273176 342.941949721253
-480.166992873176 342.452001521253
-480.266746473176 341.962053321253
-480.366500073176 341.472105121253
-480.466253673176 340.982156921253
-480.566007273176 340.492208721253
-480.665760873176 340.002260521253
-480.765514473176 339.512312321253
-480.865268073176 339.022364121253
-480.965021673176 338.532415921253
-481.064775273176 338.042467721253
-481.164528873176 337.552519521253
-481.264282473176 337.062571321253
-481.364036073176 336.572623121253
-481.463789673176 336.082674921253
-481.563543273176 335.592726721253
-481.663296873176 335.102778521253
-447.939771003183 342.724166999321
-448.132247803183 342.262699049321
-448.324724603183 341.801231099321
-448.517201403183 341.339763149321
-448.709678203183 340.878295199321
-448.902155003183 340.416827249321
-449.094631803183 339.955359299321
-449.287108603183 339.493891349321
-449.479585403183 339.032423399321
-449.672062203183 338.570955449321
-449.864539003183 338.109487499321
-450.057015803183 337.648019549321
-450.249492603183 337.186551599321
-450.441969403183 336.725083649321
-450.634446203183 336.263615699321
-450.826923003183 335.802147749321
-451.019399803183 335.340679799321
-451.211876603183 334.879211849321
-451.404353403183 334.417743899321
-451.596830203183 333.956275949321
-451.789307003183 333.494807999321
-420.955129282292 327.142491436508
-421.208553932292 326.711474086508
-421.461978582292 326.280456736508
-421.715403232292 325.849439386508
-421.968827882292 325.418422036508
-422.222252532292 324.987404686508
-422.475677182292 324.556387336508
-422.729101832292 324.125369986508
-422.982526482292 323.694352636508
-423.235951132292 323.263335286508
-423.489375782292 322.832317936508
-423.742800432292 322.401300586508
-423.996225082292 321.970283236508
-424.249649732292 321.539265886508
-424.503074382292 321.108248536508
-424.756499032292 320.677231186508
-425.009923682292 320.246213836508
-425.263348332292 319.815196486508
-425.516772982292 319.384179136508
-425.770197632292 318.953161786508
-395.392247174727 310.196494961
-395.685584674727 309.791583761
-395.978922174727 309.386672561
-396.272259674727 308.981761361
-396.565597174727 308.576850161
-396.858934674727 308.171938961
-397.152272174727 307.767027761
-397.445609674727 307.362116561
-397.738947174727 306.957205361
-398.032284674727 306.552294161
-398.325622174727 306.147382961
-398.618959674727 305.742471761
-398.912297174727 305.337560561
-399.205634674727 304.932649361
-399.498972174727 304.527738161
-399.792309674727 304.122826961
-400.085647174727 303.717915761
-400.378984674727 303.313004561
-400.672322174727 302.908093361
-400.965659674727 302.503182161
-370.21131762 293.8136828
-370.50544782 293.40934705
-370.79957802 293.0050113
-371.09370822 292.60067555
-371.38783842 292.1963398
-371.68196862 291.79200405
-371.97609882 291.3876683
-372.27022902 290.98333255
-372.56435922 290.5789968
-372.85848942 290.17466105
-373.15261962 289.7703253
-373.44674982 289.36598955
-373.74088002 288.9616538
-374.03501022 288.55731805
-374.32914042 288.1529823
-374.62327062 287.74864655
-374.91740082 287.3443108
-375.21153102 286.93997505
-375.50566122 286.5356393
-375.79979142 286.13130355
-376.09392162 285.7269678
-345.45268854 277.49728232
-345.73271314 277.08305262
-346.01273774 276.66882292
-346.29276234 276.25459322
-346.57278694 275.84036352
-346.85281154 275.42613382
-347.13283614 275.01190412
-347.41286074 274.59767442
-347.69288534 274.18344472
-347.97290994 273.76921502
-348.25293454 273.35498532
-348.53295914 272.94075562
-348.81298374 272.52652592
-349.09300834 272.11229622
-349.37303294 271.69806652
-349.65305754 271.28383682
-349.93308214 270.86960712
-350.21310674 270.45537742
-350.49313134 270.04114772
-350.77315594 269.62691802
-351.05318054 269.21268832
-336.001018270444 270.733668467147
-336.265155220444 270.309131467147
-336.529292170444 269.884594467147
-336.793429120444 269.460057467147
-337.057566070444 269.035520467147
-337.321703020444 268.610983467147
-337.585839970444 268.186446467147
-337.849976920444 267.761909467147
-338.114113870444 267.337372467147
-338.378250820444 266.912835467147
-338.642387770444 266.488298467147
-338.906524720444 266.063761467147
-339.170661670444 265.639224467147
-339.434798620444 265.214687467147
-339.698935570444 264.790150467147
-339.963072520444 264.365613467147
-340.227209470444 263.941076467147
-340.491346420444 263.516539467147
-340.755483370444 263.092002467147
-341.019620320444 262.667465467147
-329.273864734266 265.974284291099
-329.496918534266 265.526794641099
-329.719972334266 265.079304991099
-329.943026134266 264.631815341099
-330.166079934266 264.1843256911
-330.389133734266 263.736836041099
-330.612187534266 263.289346391099
-330.835241334266 262.841856741099
-331.058295134266 262.394367091099
-331.281348934266 261.9468774411
-331.504402734266 261.499387791099
-331.727456534266 261.051898141099
-331.950510334266 260.604408491099
-332.173564134266 260.156918841099
-332.396617934266 259.7094291911
-332.619671734266 259.261939541099
-332.842725534266 258.814449891099
-333.065779334266 258.366960241099
-333.288833134266 257.919470591099
-333.511886934266 257.4719809411
-322.909829395966 261.473775018368
-323.042079545966 260.991582218368
-323.174329695966 260.509389418368
-323.306579845966 260.027196618368
-323.438829995966 259.545003818368
-323.571080145966 259.062811018368
-323.703330295966 258.580618218368
-323.835580445966 258.098425418368
-323.967830595966 257.616232618368
-324.100080745966 257.134039818368
-324.232330895966 256.651847018368
-324.364581045966 256.169654218368
-324.496831195966 255.687461418368
-324.629081345966 255.205268618368
-324.761331495966 254.723075818368
-324.893581645966 254.240883018368
-325.025831795966 253.758690218368
-325.158081945966 253.276497418368
-325.290332095966 252.794304618368
-325.422582245966 252.312111818368
-315.661558214901 257.406329529307
-315.662463864901 256.906330329307
-315.663369514901 256.406331129307
-315.664275164901 255.906331929307
-315.665180814901 255.406332729307
-315.666086464901 254.906333529307
-315.666992114901 254.406334329307
-315.667897764901 253.906335129307
-315.668803414901 253.406335929307
-315.669709064901 252.906336729307
-315.670614714901 252.406337529307
-315.671520364901 251.906338329307
-315.672426014901 251.406339129307
-315.673331664901 250.906339929307
-315.674237314901 250.406340729307
-315.675142964901 249.906341529307
-315.676048614901 249.406342329307
-315.676954264901 248.906343129307
-315.677859914901 248.406343929307
-315.678765564901 247.906344729307
-315.679671214901 247.406345529307
-307.32450448 256.37224002
-307.15322128 255.90249322
-306.98193808 255.43274642
-306.81065488 254.96299962
-306.63937168 254.49325282
-306.46808848 254.02350602
-306.29680528 253.55375922
-306.12552208 253.08401242
-305.95423888 252.61426562
-305.78295568 252.14451882
-305.61167248 251.67477202
-305.44038928 251.20502522
-305.26910608 250.73527842
-305.09782288 250.26553162
-304.92653968 249.79578482
-304.75525648 249.32603802
-304.58397328 248.85629122
-304.41269008 248.38654442
-304.24140688 247.91679762
-304.07012368 247.44705082
-303.89884048 246.97730402
-299.541650593178 259.957250896896
-299.203918243178 259.588554696896
-298.866185893178 259.219858496896
-298.528453543178 258.851162296896
-298.190721193178 258.482466096896
-297.852988843178 258.113769896896
-297.515256493178 257.745073696896
-297.177524143178 257.376377496896
-296.839791793178 257.007681296896
-296.502059443178 256.638985096896
-296.164327093178 256.270288896896
-295.826594743178 255.901592696896
-295.488862393178 255.532896496896
-295.151130043178 255.164200296896
-294.813397693178 254.795504096896
-294.475665343178 254.426807896896
-294.137932993178 254.058111696896
-293.800200643178 253.689415496896
-293.462468293178 253.320719296896
-293.124735943178 252.952023096896
-294.69388277 267.20559837
-294.24848772 266.97839082
-293.80309267 266.75118327
-293.35769762 266.52397572
-292.91230257 266.29676817
-292.46690752 266.06956062
-292.02151247 265.84235307
-291.57611742 265.61514552
-291.13072237 265.38793797
-290.68532732 265.16073042
-290.23993227 264.93352287
-289.79453722 264.70631532
-289.34914217 264.47910777
-288.90374712 264.25190022
-288.45835207 264.02469267
-288.01295702 263.79748512
-287.56756197 263.57027757
-287.12216692 263.34307002
-286.67677187 263.11586247
-286.23137682 262.88865492
-285.78598177 262.66144737
-293.435881624009 275.679821645176
-292.942690424009 275.597587595176
-292.449499224009 275.515353545176
-291.956308024009 275.433119495176
-291.463116824009 275.350885445176
-290.969925624009 275.268651395176
-290.476734424009 275.186417345176
-289.983543224009 275.104183295176
-289.490352024009 275.021949245176
-288.997160824009 274.939715195176
-288.503969624009 274.857481145176
-288.010778424009 274.775247095176
-287.517587224009 274.693013045176
-287.024396024009 274.610778995176
-286.531204824009 274.528544945176
-286.038013624009 274.446310895176
-285.544822424009 274.364076845176
-285.051631224009 274.281842795176
-284.558440024009 274.199608745176
-284.065248824009 274.117374695176
-283.572057624009 274.035140645176
-292.395191519092 284.523025000787
-291.895862019092 284.497140100787
-291.396532519092 284.471255200787
-290.897203019092 284.445370300787
-290.397873519092 284.419485400787
-289.898544019092 284.393600500787
-289.399214519092 284.367715600787
-288.899885019092 284.341830700787
-288.400555519092 284.315945800787
-287.901226019092 284.290060900787
-287.401896519092 284.264176000787
-286.902567019092 284.238291100787
-286.403237519092 284.212406200787
-285.903908019092 284.186521300787
-285.404578519092 284.160636400787
-284.905249019092 284.134751500787
-284.405919519092 284.108866600787
-283.906590019092 284.082981700787
-283.407260519092 284.057096800787
-282.907931019092 284.031211900787
-291.262700648538 293.653555794974
-290.765328148538 293.602363844974
-290.267955648538 293.551171894974
-289.770583148538 293.499979944974
-289.273210648538 293.448787994974
-288.775838148538 293.397596044974
-288.278465648538 293.346404094974
-287.781093148538 293.295212144974
-287.283720648538 293.244020194974
-286.786348148538 293.192828244974
-286.288975648538 293.141636294974
-285.791603148538 293.090444344974
-285.294230648538 293.039252394974
-284.796858148538 292.988060444974
-284.299485648538 292.936868494974
-283.802113148538 292.885676544974
-283.304740648538 292.834484594974
-282.807368148538 292.783292644974
-282.309995648538 292.732100694974
-281.812623148538 292.680908744974
-290.17816098 302.74833012
-289.69497893 302.61974117
-289.21179688 302.49115222
-288.72861483 302.36256327
-288.24543278 302.23397432
-287.76225073 302.10538537
-287.27906868 301.97679642
-286.79588663 301.84820747
-286.31270458 301.71961852
-285.82952253 301.59102957
-285.34634048 301.46244062
-284.86315843 301.33385167
-284.37997638 301.20526272
-283.89679433 301.07667377
-283.41361228 300.94808482
-282.93043023 300.81949587
-282.44724818 300.69090692
-281.96406613 300.56231797
-281.48088408 300.43372902
-280.99770203 300.30514007
-288.55195865689 312.363020297248
-288.11103110689 312.127260097248
-287.67010355689 311.891499897248
-287.22917600689 311.655739697248
-286.78824845689 311.419979497248
-286.34732090689 311.184219297248
-285.90639335689 310.948459097248
-285.46546580689 310.712698897248
-285.02453825689 310.476938697248
-284.58361070689 310.241178497248
-284.14268315689 310.005418297248
-283.70175560689 309.769658097248
-283.26082805689 309.533897897248
-282.81990050689 309.298137697248
-282.37897295689 309.062377497248
-281.93804540689 308.826617297248
-281.49711785689 308.590857097248
-281.05619030689 308.355096897248
-280.61526275689 308.119336697248
-280.17433520689 307.883576497248
-285.550018223383 322.791126305838
-285.173988873383 322.461578255838
-284.797959523383 322.132030205838
-284.421930173383 321.802482155838
-284.045900823383 321.472934105838
-283.669871473383 321.143386055838
-283.293842123383 320.813838005838
-282.917812773383 320.484289955838
-282.541783423383 320.154741905838
-282.165754073383 319.825193855838
-281.789724723383 319.495645805838
-281.413695373383 319.166097755838
-281.037666023383 318.836549705838
-280.661636673383 318.507001655838
-280.285607323383 318.177453605838
-279.909577973383 317.847905555838
-279.533548623383 317.518357505838
-279.157519273383 317.188809455838
-278.781489923383 316.859261405838
-278.405460573383 316.529713355838
-278.752234293172 331.60230552638
-278.461854793172 331.19526777638
-278.171475293172 330.78823002638
-277.881095793172 330.38119227638
-277.590716293172 329.97415452638
-277.300336793172 329.56711677638
-277.009957293172 329.16007902638
-276.719577793172 328.75304127638
-276.429198293172 328.34600352638
-276.138818793172 327.93896577638
-275.848439293172 327.53192802638
-275.558059793172 327.12489027638
-275.267680293172 326.71785252638
-274.977300793172 326.31081477638
-274.686921293172 325.90377702638
-274.396541793172 325.49673927638
-274.106162293172 325.08970152638
-273.815782793172 324.68266377638
-273.525403293172 324.27562602638
-273.235023793172 323.86858827638
-269.026745191005 336.530697014884
-268.826222241005 336.072668014884
-268.625699291005 335.614639014884
-268.425176341005 335.156610014884
-268.224653391005 334.698581014884
-268.024130441005 334.240552014884
-267.823607491005 333.782523014884
-267.623084541005 333.324494014884
-267.422561591005 332.866465014884
-267.222038641005 332.408436014884
-267.021515691005 331.950407014884
-266.820992741005 331.492378014884
-266.620469791005 331.034349014884
-266.419946841005 330.576320014884
-266.219423891005 330.118291014884
-266.018900941005 329.660262014884
-265.818377991005 329.202233014884
-265.617855041005 328.744204014884
-265.417332091005 328.286175014884
-265.216809141005 327.828146014884
-265.016286191005 327.370117014884
-258.31700722631 336.910956087495
-258.20523747631 336.423608637495
-258.09346772631 335.936261187495
-257.98169797631 335.448913737495
-257.86992822631 334.961566287495
-257.75815847631 334.474218837495
-257.64638872631 333.986871387495
-257.53461897631 333.499523937495
-257.42284922631 333.012176487495
-257.31107947631 332.524829037495
-257.19930972631 332.037481587495
-257.08753997631 331.550134137495
-256.97577022631 331.062786687495
-256.86400047631 330.575439237495
-256.75223072631 330.088091787495
-256.64046097631 329.600744337495
-256.52869122631 329.113396887495
-256.41692147631 328.626049437495
-256.30515172631 328.138701987495
-256.19338197631 327.651354537495
-248.487509471732 335.970856944646
-248.449441471732 335.472308244646
-248.411373471732 334.973759544646
-248.373305471732 334.475210844646
-248.335237471732 333.976662144646
-248.297169471732 333.478113444646
-248.259101471732 332.979564744646
-248.221033471732 332.481016044646
-248.182965471732 331.982467344646
-248.144897471732 331.483918644646
-248.106829471732 330.985369944646
-248.068761471732 330.486821244646
-248.030693471732 329.988272544646
-247.992625471732 329.489723844646
-247.954557471732 328.991175144646
-247.916489471732 328.492626444646
-247.878421471732 327.994077744646
-247.840353471732 327.495529044646
-247.802285471732 326.996980344646
-247.764217471732 326.498431644646
-239.197356146667 334.321421217921
-239.212071096667 333.821637817921
-239.226786046667 333.321854417921
-239.241500996667 332.822071017921
-239.256215946667 332.322287617921
-239.270930896667 331.822504217921
-239.285645846667 331.322720817921
-239.300360796667 330.822937417921
-239.315075746667 330.323154017921
-239.329790696667 329.823370617921
-239.344505646667 329.323587217921
-239.359220596667 328.823803817921
-239.373935546667 328.324020417921
-239.388650496667 327.824237017921
-239.403365446667 327.324453617921
-239.418080396667 326.824670217921
-239.432795346667 326.324886817921
-239.447510296667 325.825103417921
-239.462225246667 325.325320017921
-239.476940196667 324.825536617921
-230.07839239072 333.321245965909
-230.12530889072 332.823451965909
-230.17222539072 332.325657965909
-230.21914189072 331.827863965909
-230.26605839072 331.330069965909
-230.31297489072 330.832275965909
-230.35989139072 330.334481965909
-230.40680789072 329.836687965909
-230.45372439072 329.338893965909
-230.50064089072 328.841099965909
-230.54755739072 328.343305965909
-230.59447389072 327.845511965909
-230.64139039072 327.347717965909
-230.68830689072 326.849923965909
-230.73522339072 326.352129965909
-230.78213989072 325.854335965909
-230.82905639072 325.356541965909
-230.87597289072 324.858747965909
-230.92288939072 324.360953965909
-230.96980589072 323.863159965909
-231.01672239072 323.365365965909
-200.431984645119 328.244718019374
-200.515947795119 327.751818269374
-200.599910945119 327.258918519375
-200.683874095119 326.766018769375
-200.767837245119 326.273119019375
-200.851800395119 325.780219269375
-200.935763545119 325.287319519374
-201.019726695119 324.794419769374
-201.103689845119 324.301520019374
-201.187652995119 323.808620269375
-201.271616145119 323.315720519375
-201.355579295119 322.822820769375
-201.439542445119 322.329921019375
-201.523505595119 321.837021269374
-201.607468745119 321.344121519374
-201.691431895119 320.851221769374
-201.775395045119 320.358322019374
-201.859358195119 319.865422269375
-201.943321345119 319.372522519375
-202.027284495119 318.879622769375
-170.836779028555 323.336738526597
-170.947334678555 322.849114226597
-171.057890328555 322.361489926597
-171.168445978555 321.873865626597
-171.279001628555 321.386241326597
-171.389557278555 320.898617026597
-171.500112928555 320.410992726597
-171.610668578555 319.923368426597
-171.721224228555 319.435744126597
-171.831779878555 318.948119826597
-171.942335528555 318.460495526597
-172.052891178555 317.972871226597
-172.163446828555 317.485246926597
-172.274002478555 316.997622626597
-172.384558128555 316.509998326597
-172.495113778555 316.022374026597
-172.605669428555 315.534749726597
-172.716225078555 315.047125426597
-172.826780728555 314.559501126597
-140.58761773771 318.414923101222
-140.76253253771 317.946516401222
-140.93744733771 317.478109701222
-141.11236213771 317.009703001222
-141.28727693771 316.541296301223
-141.46219173771 316.072889601223
-141.63710653771 315.604482901223
-141.81202133771 315.136076201223
-141.98693613771 314.667669501223
-142.16185093771 314.199262801223
-142.33676573771 313.730856101223
-142.51168053771 313.262449401223
-142.68659533771 312.794042701223
-142.86151013771 312.325636001223
-143.03642493771 311.857229301223
-143.21133973771 311.388822601223
-143.38625453771 310.920415901222
-143.56116933771 310.452009201222
-143.73608413771 309.983602501222
-111.305616031182 308.272941445288
-111.545403731182 307.834191095288
-111.785191431182 307.395440745288
-112.024979131182 306.956690395288
-112.264766831182 306.517940045288
-112.504554531182 306.079189695288
-112.744342231182 305.640439345288
-112.984129931182 305.201688995288
-113.223917631182 304.762938645288
-113.463705331182 304.324188295288
-113.703493031182 303.885437945288
-113.943280731182 303.446687595288
-114.183068431182 303.007937245288
-114.422856131182 302.569186895288
-114.662643831182 302.130436545288
-114.902431531182 301.691686195288
-115.142219231182 301.252935845288
-115.382006931182 300.814185495288
-115.621794631182 300.375435145288
-115.861582331182 299.936684795288
-88.38049847 287.2560421
-88.67355452 286.8509271
-88.96661057 286.4458121
-89.25966662 286.0406971
-89.55272267 285.6355821
-89.84577872 285.2304671
-90.13883477 284.8253521
-90.43189082 284.4202371
-90.72494687 284.0151221
-91.01800292 283.6100071
-91.31105897 283.2048921
-91.60411502 282.7997771
-91.89717107 282.3946621
-92.19022712 281.9895471
-92.48328317 281.5844321
-92.77633922 281.1793171
-93.06939527 280.7742021
-93.36245132 280.3690871
-93.65550737 279.9639721
-93.94856342 279.5588571
-66.171091941681 266.885604712332
-66.503272741681 266.511899062332
-66.835453541681 266.138193412332
-67.167634341681 265.764487762332
-67.499815141681 265.390782112332
-67.831995941681 265.017076462332
-68.164176741681 264.643370812332
-68.496357541681 264.269665162332
-68.828538341681 263.895959512332
-69.160719141681 263.522253862332
-69.492899941681 263.148548212332
-69.825080741681 262.774842562332
-70.157261541681 262.401136912332
-70.489442341681 262.027431262332
-70.821623141681 261.653725612332
-71.153803941681 261.280019962332
-71.485984741681 260.906314312332
-71.818165541681 260.532608662332
-72.150346341681 260.158903012332
-72.482527141681 259.785197362332
-44.2190941209642 246.393958938745
-44.5715747709642 246.039336038745
-44.9240554209642 245.684713138745
-45.2765360709642 245.330090238745
-45.6290167209642 244.975467338745
-45.9814973709642 244.620844438745
-46.3339780209642 244.266221538745
-46.6864586709642 243.911598638745
-47.0389393209642 243.556975738745
-47.3914199709642 243.202352838745
-47.7439006209642 242.847729938745
-48.0963812709642 242.493107038745
-48.4488619209642 242.138484138745
-48.8013425709642 241.783861238745
-49.1538232209642 241.429238338745
-49.5063038709642 241.074615438745
-49.8587845209642 240.719992538745
-50.2112651709642 240.365369638745
-50.5637458209642 240.010746738745
-50.9162264709642 239.656123838745
-22.0276812163313 226.08944608524
-22.3851555163313 225.73985758524
-22.7426298163313 225.39026908524
-23.1001041163313 225.04068058524
-23.4575784163313 224.69109208524
-23.8150527163313 224.34150358524
-24.1725270163313 223.99191508524
-24.5300013163313 223.64232658524
-24.8874756163313 223.29273808524
-25.2449499163313 222.94314958524
-25.6024242163313 222.59356108524
-25.9598985163313 222.24397258524
-26.3173728163313 221.89438408524
-26.6748471163313 221.54479558524
-27.0323214163313 221.19520708524
-27.3897957163313 220.84561858524
-27.7472700163313 220.49603008524
-28.1047443163313 220.14644158524
-28.4622186163313 219.79685308524
-28.8196929163313 219.44726458524
0.17003962354202 205.854384046441
-0.18897142645798 205.506373896441
-0.54798247645798 205.158363746441
-0.90699352645798 204.810353596441
-1.26600457645798 204.462343446441
-1.62501562645798 204.114333296441
-1.98402667645798 203.766323146441
-2.34303772645798 203.418312996441
-2.70204877645798 203.070302846441
-3.06105982645798 202.722292696441
-3.42007087645798 202.374282546441
-3.77908192645798 202.026272396441
-4.13809297645798 201.678262246441
-4.49710402645798 201.330252096441
-4.85611507645798 200.982241946441
-5.21512612645798 200.634231796441
-5.57413717645798 200.286221646441
-5.93314822645798 199.938211496441
-6.29215927645798 199.590201346441
-6.65117032645798 199.242191196441
22.3185236069918 185.568149428077
21.9583905569918 185.221300478077
21.5982575069918 184.874451528077
21.2381244569918 184.527602578077
20.8779914069918 184.180753628077
20.5178583569918 183.833904678077
20.1577253069918 183.487055728077
19.7975922569918 183.140206778077
19.4374592069918 182.793357828077
19.0773261569918 182.446508878077
18.7171931069918 182.099659928077
18.3570600569918 181.752810978077
17.9969270069918 181.405962028077
17.6367939569918 181.059113078077
17.2766609069918 180.712264128077
16.9165278569918 180.365415178077
16.5563948069918 180.018566228077
16.1962617569918 179.671717278077
15.8361287069918 179.324868328077
15.4759956569918 178.978019378077
44.2947553724756 165.127872232704
43.9361562224756 164.779437682704
43.5775570724756 164.431003132704
43.2189579224756 164.082568582704
42.8603587724756 163.734134032704
42.5017596224756 163.385699482704
42.1431604724756 163.037264932704
41.7845613224756 162.688830382704
41.4259621724756 162.340395832704
41.0673630224756 161.991961282704
40.7087638724756 161.643526732704
40.3501647224756 161.295092182704
39.9915655724756 160.946657632704
39.6329664224756 160.598223082704
39.2743672724756 160.249788532704
38.9157681224756 159.901353982704
38.5571689724756 159.552919432704
38.1985698224756 159.204484882704
37.8399706724756 158.856050332704
37.4813715224756 158.507615782704
66.1555732055899 144.813892209106
65.8049554555899 144.457427359106
65.4543377055899 144.100962509106
65.10371995559 143.744497659106
64.75310220559 143.388032809106
64.4024844555899 143.031567959106
64.0518667055899 142.675103109106
63.7012489555899 142.318638259106
63.3506312055899 141.962173409106
63.00001345559 141.605708559106
62.6493957055899 141.249243709106
62.2987779555899 140.892778859106
61.94816020559 140.536314009106
61.5975424555899 140.179849159106
61.2469247055899 139.823384309106
60.8963069555899 139.466919459106
60.5456892055899 139.110454609106
60.1950714555899 138.753989759106
59.8444537055899 138.397524909106
59.4938359555899 138.041060059106
87.9539327344448 124.722880743987
87.6163107844448 124.354083443987
87.2786888344448 123.985286143987
86.9410668844448 123.616488843987
86.6034449344448 123.247691543987
86.2658229844448 122.878894243987
85.9282010344448 122.510096943987
85.5905790844448 122.141299643987
85.2529571344448 121.772502343987
84.9153351844448 121.403705043987
84.5777132344448 121.034907743987
84.2400912844448 120.666110443987
83.9024693344448 120.297313143987
83.5648473844448 119.928515843987
83.2272254344448 119.559718543987
82.8896034844448 119.190921243987
82.5519815344448 118.822123943987
82.2143595844448 118.453326643987
81.8767376344448 118.084529343987
81.5391156844448 117.715732043987
110.298710618359 104.615280607871
109.958758068359 104.248630557871
109.618805518359 103.881980507871
109.278852968359 103.515330457871
108.938900418359 103.148680407871
108.598947868359 102.782030357871
108.258995318359 102.415380307871
107.919042768359 102.048730257871
107.579090218359 101.682080207871
107.239137668359 101.315430157871
106.899185118359 100.948780107871
106.559232568359 100.582130057871
106.219280018359 100.215480007871
105.879327468359 99.8488299578706
105.539374918359 99.4821799078706
105.199422368359 99.1155298578706
104.859469818359 98.7488798078706
104.519517268359 98.3822297578706
104.179564718359 98.0155797078706
103.839612168359 97.6489296578706
131.552258974802 84.8701590097299
131.257043574802 84.4666148597299
130.961828174802 84.0630707097299
130.666612774802 83.6595265597299
130.371397374802 83.2559824097299
130.076181974802 82.8524382597299
129.780966574802 82.4488941097299
129.485751174802 82.0453499597299
129.190535774802 81.6418058097299
128.895320374802 81.2382616597299
128.600104974802 80.8347175097299
128.304889574802 80.4311733597299
128.009674174802 80.0276292097299
127.714458774802 79.6240850597299
127.419243374802 79.2205409097299
127.124027974802 78.8169967597299
126.828812574802 78.4134526097299
126.533597174802 78.0099084597299
126.238381774802 77.6063643097299
125.943166374802 77.2028201597299
137.6822505985 78.9303189598792
137.4184183985 78.5055925098792
137.1545861985 78.0808660598792
136.8907539985 77.6561396098792
136.6269217985 77.2314131598792
136.3630895985 76.8066867098792
136.0992573985 76.3819602598792
135.8354251985 75.9572338098792
135.5715929985 75.5325073598792
135.3077607985 75.1077809098792
135.0439285985 74.6830544598792
134.7800963985 74.2583280098792
134.5162641985 73.8336015598792
134.2524319985 73.4088751098792
133.9885997985 72.9841486598792
133.7247675985 72.5594222098792
133.4609353985 72.1346957598792
133.1971031985 71.7099693098792
132.9332709985 71.2852428598792
132.6694387985 70.8605164098792
144.109905682285 72.952565981099
143.879338632285 72.5089007310989
143.648771582285 72.065235481099
143.418204532285 71.621570231099
143.187637482285 71.1779049810989
142.957070432285 70.734239731099
142.726503382285 70.290574481099
142.495936332285 69.8469092310989
142.265369282285 69.403243981099
142.034802232285 68.9595787310989
141.804235182285 68.5159134810989
141.573668132285 68.072248231099
141.343101082285 67.6285829810989
141.112534032285 67.1849177310989
140.881966982285 66.741252481099
140.651399932285 66.2975872310989
140.420832882285 65.8539219810989
140.190265832285 65.410256731099
139.959698782285 64.9665914810989
139.729131732285 64.5229262310989
150.929101035321 66.9510322093478
150.733189085321 66.4910120593478
150.537277135321 66.0309919093478
150.341365185321 65.5709717593478
150.145453235321 65.1109516093478
149.949541285321 64.6509314593478
149.753629335321 64.1909113093478
149.557717385321 63.7308911593478
149.361805435321 63.2708710093478
149.165893485321 62.8108508593478
148.969981535321 62.3508307093478
148.774069585321 61.8908105593478
148.578157635321 61.4307904093478
148.382245685321 60.9707702593478
148.186333735321 60.5107501093478
147.990421785321 60.0507299593478
147.794509835321 59.5907098093478
147.598597885321 59.1306896593478
147.402685935321 58.6706695093478
147.206773985321 58.2106493593478
158.540835322447 61.8936258274158
158.380977422447 61.4198690774158
158.221119522447 60.9461123274158
158.061261622447 60.4723555774158
157.901403722447 59.9985988274158
157.741545822447 59.5248420774158
157.581687922447 59.0510853274158
157.421830022447 58.5773285774158
157.261972122447 58.1035718274158
157.102114222447 57.6298150774158
156.942256322447 57.1560583274158
156.782398422447 56.6823015774158
156.622540522447 56.2085448274158
156.462682622447 55.7347880774158
156.302824722447 55.2610313274158
156.142966822447 54.7872745774158
155.983108922447 54.3135178274158
155.823251022447 53.8397610774158
155.663393122447 53.3660043274158
155.503535222447 52.8922475774158
167.420941088867 60.3093747901648
167.298524738867 59.8245920901648
167.176108388867 59.3398093901648
167.053692038867 58.8550266901648
166.931275688867 58.3702439901648
166.808859338867 57.8854612901648
166.686442988867 57.4006785901648
166.564026638867 56.9158958901648
166.441610288867 56.4311131901648
166.319193938867 55.9463304901648
166.196777588867 55.4615477901648
166.074361238867 54.9767650901648
165.951944888867 54.4919823901648
165.829528538867 54.0071996901648
165.707112188867 53.5224169901648
165.584695838867 53.0376342901648
165.462279488867 52.5528515901648
165.339863138867 52.0680688901648
165.217446788867 51.5832861901648
165.095030438867 51.0985034901648
164.972614088867 50.6137207901648
176.664187601337 61.4293897571094
176.580539201337 60.9364364571094
176.496890801337 60.4434831571094
176.413242401337 59.9505298571094
176.329594001337 59.4575765571094
176.245945601337 58.9646232571094
176.162297201337 58.4716699571094
176.078648801337 57.9787166571094
175.995000401337 57.4857633571094
175.911352001337 56.9928100571094
175.827703601337 56.4998567571094
175.744055201337 56.0069034571094
175.660406801337 55.5139501571094
175.576758401337 55.0209968571094
175.493110001337 54.5280435571094
175.409461601337 54.0350902571094
175.325813201337 53.5421369571094
175.242164801337 53.0491836571094
175.158516401337 52.5562303571094
175.074868001337 52.0632770571094
185.48957805396 62.8375493918338
185.44622545396 62.3394323918338
185.40287285396 61.8413153918338
185.35952025396 61.3431983918338
185.31616765396 60.8450813918338
185.27281505396 60.3469643918338
185.22946245396 59.8488473918338
185.18610985396 59.3507303918338
185.14275725396 58.8526133918338
185.09940465396 58.3544963918338
185.05605205396 57.8563793918338
185.01269945396 57.3582623918338
184.96934685396 56.8601453918338
184.92599425396 56.3620283918338
184.88264165396 55.8639113918338
184.83928905396 55.3657943918338
184.79593645396 54.8676773918338
184.75258385396 54.3695603918338
184.70923125396 53.8714433918338
184.66587865396 53.3733263918338
184.62252605396 52.8752093918338
193.917352701934 63.9851403357542
193.916025401934 63.4851420857542
193.914698101934 62.9851438357542
193.913370801934 62.4851455857542
193.912043501934 61.9851473357542
193.910716201934 61.4851490857542
193.909388901934 60.9851508357542
193.908061601934 60.4851525857542
193.906734301934 59.9851543357542
193.905407001934 59.4851560857542
193.904079701934 58.9851578357543
193.902752401934 58.4851595857542
193.901425101934 57.9851613357542
193.900097801934 57.4851630857542
193.898770501934 56.9851648357542
193.897443201934 56.4851665857542
193.896115901934 55.9851683357542
193.894788601934 55.4851700857542
193.893461301934 54.9851718357542
193.892134001934 54.4851735857542
202.0800591 65.32850746
202.1221476 64.83028206
202.1642361 64.33205666
202.2063246 63.83383126
202.2484131 63.33560586
202.2905016 62.83738046
202.3325901 62.33915506
202.3746786 61.84092966
202.4167671 61.34270426
202.4588556 60.84447886
202.5009441 60.34625346
202.5430326 59.84802806
202.5851211 59.34980266
202.6272096 58.85157726
202.6692981 58.35335186
202.7113866 57.85512646
202.7534751 57.35690106
202.7955636 56.85867566
202.8376521 56.36045026
202.8797406 55.86222486
210.253295715122 66.3490984097875
210.334229415122 65.8556921597875
210.415163115122 65.3622859097875
210.496096815122 64.8688796597875
210.577030515122 64.3754734097875
210.657964215122 63.8820671597875
210.738897915122 63.3886609097875
210.819831615122 62.8952546597875
210.900765315122 62.4018484097875
210.981699015122 61.9084421597875
211.062632715122 61.4150359097875
211.143566415122 60.9216296597875
211.224500115122 60.4282234097875
211.305433815122 59.9348171597875
211.386367515122 59.4414109097875
211.467301215122 58.9480046597875
211.548234915122 58.4545984097875
211.629168615122 57.9611921597875
211.710102315122 57.4677859097875
211.791036015122 56.9743796597875
238.85492942924 70.3400372414483
239.01796402924 69.8673642914483
239.18099862924 69.3946913414483
239.34403322924 68.9220183914483
239.50706782924 68.4493454414483
239.67010242924 67.9766724914483
239.83313702924 67.5039995414483
239.99617162924 67.0313265914483
240.15920622924 66.5586536414483
240.32224082924 66.0859806914483
240.48527542924 65.6133077414483
240.64831002924 65.1406347914483
240.81134462924 64.6679618414483
240.97437922924 64.1952888914483
241.13741382924 63.7226159414483
241.30044842924 63.2499429914483
241.46348302924 62.7772700414483
241.62651762924 62.3045970914483
241.78955222924 61.8319241414483
241.95258682924 61.3592511914483
269.062130859088 74.7852112969529
269.170862609088 74.2971770469529
269.279594359088 73.8091427969529
269.388326109088 73.3211085469529
269.497057859088 72.8330742969528
269.605789609088 72.3450400469528
269.714521359088 71.8570057969528
269.823253109088 71.3689715469528
269.931984859088 70.8809372969529
270.040716609088 70.3929030469529
270.149448359088 69.9048687969529
270.258180109088 69.4168345469529
270.366911859088 68.9288002969529
270.475643609088 68.4407660469528
270.584375359088 67.9527317969528
270.693107109088 67.4646975469528
270.801838859088 66.9766632969529
270.910570609088 66.4886290469529
271.019302359088 66.0005947969529
271.128034109088 65.5125605469529
277.980771401385 76.3289255904152
278.042604101385 75.8327635904152
278.104436801385 75.3366015904152
278.166269501385 74.8404395904152
278.228102201385 74.3442775904152
278.289934901385 73.8481155904152
278.351767601385 73.3519535904152
278.413600301385 72.8557915904152
278.475433001385 72.3596295904152
278.537265701385 71.8634675904152
278.599098401385 71.3673055904152
278.660931101385 70.8711435904152
278.722763801385 70.3749815904152
278.784596501385 69.8788195904152
278.846429201385 69.3826575904152
278.908261901385 68.8864955904152
278.970094601385 68.3903335904152
279.031927301385 67.8941715904152
279.093760001385 67.3980095904152
279.155592701385 66.9018475904152
287.024526117414 77.51899875804
287.037272667414 77.01916125804
287.050019217414 76.51932375804
287.062765767414 76.01948625804
287.075512317414 75.51964875804
287.088258867414 75.01981125804
287.101005417414 74.51997375804
287.113751967414 74.02013625804
287.126498517414 73.52029875804
287.139245067414 73.02046125804
287.151991617414 72.52062375804
287.164738167414 72.02078625804
287.177484717414 71.52094875804
287.190231267414 71.02111125804
287.202977817414 70.52127375804
287.215724367414 70.02143625804
287.228470917414 69.52159875804
287.241217467414 69.02176125804
287.253964017414 68.52192375804
287.266710567414 68.02208625804
296.285397062368 78.790073133122
296.246951712368 78.291553383122
296.208506362368 77.793033633122
296.170061012368 77.294513883122
296.131615662368 76.795994133122
296.093170312368 76.297474383122
296.054724962368 75.798954633122
296.016279612368 75.300434883122
295.977834262368 74.801915133122
295.939388912368 74.303395383122
295.900943562368 73.804875633122
295.862498212368 73.306355883122
295.824052862368 72.807836133122
295.785607512368 72.309316383122
295.747162162368 71.810796633122
295.708716812368 71.312276883122
295.670271462368 70.813757133122
295.631826112368 70.315237383122
295.593380762368 69.816717633122
295.554935412368 69.318197883122
305.895364518415 79.5541243408225
305.803523868415 79.0626313908225
305.711683218415 78.5711384408225
305.619842568415 78.0796454908225
305.528001918415 77.5881525408225
305.436161268415 77.0966595908225
305.344320618415 76.6051666408225
305.252479968415 76.1136736908225
305.160639318415 75.6221807408225
305.068798668415 75.1306877908225
304.976958018415 74.6391948408225
304.885117368415 74.1477018908225
304.793276718415 73.6562089408225
304.701436068415 73.1647159908225
304.609595418415 72.6732230408225
304.517754768415 72.1817300908225
304.425914118415 71.6902371408225
304.334073468415 71.1987441908225
304.242232818415 70.7072512408225
304.150392168415 70.2157582908225
315.637030530082 78.7166837875511
315.490033230082 78.2387802375511
315.343035930082 77.7608766875511
315.196038630082 77.2829731375511
315.049041330082 76.8050695875511
314.902044030082 76.3271660375511
314.755046730082 75.8492624875511
314.608049430082 75.3713589375511
314.461052130082 74.8934553875511
314.314054830082 74.4155518375511
314.167057530082 73.9376482875511
314.020060230082 73.4597447375511
313.873062930082 72.9818411875511
313.726065630082 72.5039376375511
313.579068330082 72.0260340875511
313.432071030082 71.5481305375511
313.285073730082 71.0702269875511
313.138076430082 70.5923234375511
312.991079130082 70.1144198875511
312.844081830082 69.6365163375511
325.402682291208 76.6663495670234
325.199763791208 76.2093768170234
324.996845291208 75.7524040670234
324.793926791208 75.2954313170234
324.591008291208 74.8384585670234
324.388089791208 74.3814858170234
324.185171291208 73.9245130670234
323.982252791208 73.4675403170234
323.779334291208 73.0105675670234
323.576415791208 72.5535948170234
323.373497291208 72.0966220670234
323.170578791208 71.6396493170234
322.967660291208 71.1826765670234
322.764741791208 70.7257038170234
322.561823291208 70.2687310670234
322.358904791208 69.8117583170234
322.155986291208 69.3547855670234
321.953067791208 68.8978128170234
321.750149291208 68.4408400670234
321.547230791208 67.9838673170234
334.501957202755 72.45497493461
334.242381202755 72.0276339846099
333.982805202755 71.6002930346099
333.723229202755 71.1729520846099
333.463653202755 70.7456111346099
333.204077202755 70.3182701846099
332.944501202755 69.8909292346099
332.684925202755 69.4635882846099
332.425349202755 69.03624733461
332.165773202755 68.60890638461
331.906197202755 68.18156543461
331.646621202755 67.7542244846099
331.387045202755 67.3268835346099
331.127469202755 66.8995425846099
330.867893202755 66.4722016346099
330.608317202755 66.0448606846099
330.348741202755 65.6175197346099
330.089165202755 65.1901787846099
329.829589202755 64.76283783461
329.570013202755 64.33549688461
343.054336778755 67.0070948469335
342.738137228756 66.6197734969335
342.421937678756 66.2324521469335
342.105738128756 65.8451307969335
341.789538578756 65.4578094469335
341.473339028756 65.0704880969335
341.157139478756 64.6831667469335
340.840939928756 64.2958453969335
340.524740378756 63.9085240469335
340.208540828756 63.5212026969335
339.892341278756 63.1338813469335
339.576141728756 62.7465599969335
339.259942178756 62.3592386469335
338.943742628756 61.9719172969335
338.627543078756 61.5845959469335
338.311343528756 61.1972745969335
337.995143978756 60.8099532469335
337.678944428756 60.4226318969335
337.362744878756 60.0353105469335
337.046545328756 59.6479891969335
350.485687594669 59.9645137371982
350.115712294669 59.6281831371982
349.745736994669 59.2918525371982
349.375761694669 58.9555219371982
349.005786394669 58.6191913371982
348.635811094669 58.2828607371982
348.265835794669 57.9465301371982
347.895860494669 57.6101995371982
347.525885194669 57.2738689371982
347.155909894669 56.9375383371982
346.785934594669 56.6012077371982
346.415959294669 56.2648771371982
346.045983994669 55.9285465371982
345.676008694669 55.5922159371982
345.306033394669 55.2558853371982
344.936058094669 54.9195547371982
344.566082794669 54.5832241371982
344.196107494669 54.2468935371982
343.826132194669 53.9105629371982
356.820329149639 51.9654872241304
356.407166199639 51.6838911241304
355.994003249639 51.4022950241304
355.580840299639 51.1206989241304
355.167677349639 50.8391028241304
354.754514399639 50.5575067241304
354.341351449639 50.2759106241304
353.928188499639 49.9943145241304
353.515025549639 49.7127184241304
353.101862599639 49.4311223241304
352.688699649639 49.1495262241304
352.275536699639 48.8679301241304
351.862373749639 48.5863340241304
351.449210799639 48.3047379241304
351.036047849639 48.0231418241304
350.622884899639 47.7415457241304
350.209721949639 47.4599496241304
349.796558999639 47.1783535241304
349.383396049639 46.8967574241304
348.970233099639 46.6151613241304
361.543750565182 42.9898954907515
361.097680365182 42.7640163407515
360.651610165182 42.5381371907515
360.205539965182 42.3122580407515
359.759469765182 42.0863788907515
359.313399565182 41.8604997407515
358.867329365182 41.6346205907515
358.421259165182 41.4087414407515
357.975188965182 41.1828622907515
357.529118765182 40.9569831407515
357.083048565182 40.7311039907515
356.636978365182 40.5052248407515
356.190908165182 40.2793456907515
355.744837965182 40.0534665407515
355.298767765182 39.8275873907515
354.852697565182 39.6017082407515
354.406627365182 39.3758290907515
353.960557165182 39.1499499407515
353.514486965182 38.9240707907515
353.068416765182 38.6981916407515
365.030019330575 33.57354636904
364.559605330575 33.40410416904
364.089191330575 33.23466196904
363.618777330575 33.06521976904
363.148363330575 32.89577756904
362.677949330575 32.72633536904
362.207535330575 32.55689316904
361.737121330575 32.38745096904
361.266707330575 32.21800876904
360.796293330575 32.04856656904
360.325879330575 31.87912436904
359.855465330575 31.70968216904
359.385051330575 31.54023996904
358.914637330575 31.37079776904
358.444223330575 31.20135556904
357.973809330575 31.03191336904
357.503395330575 30.86247116904
357.032981330575 30.69302896904
356.562567330575 30.52358676904
356.092153330575 30.35414456904
366.356577683826 23.7063531447758
365.869331533826 23.5941427947758
365.382085383826 23.4819324447759
364.894839233826 23.3697220947758
364.407593083826 23.2575117447759
363.920346933826 23.1453013947758
363.433100783826 23.0330910447759
362.945854633826 22.9208806947758
362.458608483826 22.8086703447759
361.971362333826 22.6964599947759
361.484116183826 22.5842496447758
360.996870033826 22.4720392947759
360.509623883826 22.3598289447758
360.022377733826 22.2476185947759
359.535131583826 22.1354082447758
359.047885433826 22.0231978947759
358.560639283826 21.9109875447758
358.073393133826 21.7987771947759
357.586146983826 21.6865668447759
357.098900833826 21.5743564947758
366.100330927486 13.9994246306477
365.604082827486 13.9382867806477
365.107834727486 13.8771489306477
364.611586627486 13.8160110806477
364.115338527486 13.7548732306477
363.619090427486 13.6937353806477
363.122842327486 13.6325975306477
362.626594227486 13.5714596806477
362.130346127486 13.5103218306477
361.634098027486 13.4491839806477
361.137849927486 13.3880461306477
360.641601827486 13.3269082806477
360.145353727486 13.2657704306477
359.649105627486 13.2046325806477
359.152857527486 13.1434947306477
358.656609427486 13.0823568806477
358.160361327486 13.0212190306477
357.664113227486 12.9600811806477
357.167865127486 12.8989433306477
356.671617027486 12.8378054806477
364.976005671279 4.6115907675806
364.476395771279 4.5918437675806
363.976785871279 4.5720967675806
363.477175971279 4.5523497675806
362.977566071279 4.5326027675806
362.477956171279 4.5128557675806
361.978346271279 4.4931087675806
361.478736371279 4.4733617675806
360.979126471279 4.4536147675806
360.479516571279 4.4338677675806
359.979906671279 4.4141207675806
359.480296771279 4.3943737675806
358.980686871279 4.3746267675806
358.481076971279 4.3548797675806
357.981467071279 4.3351327675806
357.481857171279 4.3153857675806
356.982247271279 4.2956387675806
356.482637371279 4.2758917675806
355.983027471279 4.2561447675806
355.483417571279 4.2363977675806
364.160143606405 -4.53740955731017
363.660278356405 -4.52580270731017
363.160413106405 -4.51419585731017
362.660547856405 -4.50258900731017
362.160682606405 -4.49098215731017
361.660817356405 -4.47937530731017
361.160952106405 -4.46776845731017
360.661086856405 -4.45616160731017
360.161221606405 -4.44455475731017
359.661356356405 -4.43294790731017
359.161491106405 -4.42134105731017
358.661625856405 -4.40973420731017
358.161760606405 -4.39812735731017
357.661895356405 -4.38652050731017
357.162030106405 -4.37491365731017
356.662164856405 -4.36330680731017
356.162299606405 -4.35169995731017
355.662434356405 -4.34009310731017
355.162569106405 -4.32848625731017
354.662703856405 -4.31687940731017
360.228269226936 -34.4022135428782
359.731979426936 -34.3414154428782
359.235689626936 -34.2806173428782
358.739399826936 -34.2198192428782
358.243110026936 -34.1590211428782
357.746820226936 -34.0982230428782
357.250530426936 -34.0374249428782
356.754240626936 -33.9766268428782
356.257950826936 -33.9158287428782
355.761661026936 -33.8550306428782
355.265371226936 -33.7942325428782
354.769081426936 -33.7334344428782
354.272791626936 -33.6726363428782
353.776501826936 -33.6118382428782
353.280212026936 -33.5510401428782
352.783922226936 -33.4902420428782
352.287632426936 -33.4294439428782
351.791342626936 -33.3686458428782
351.295052826936 -33.3078477428782
356.887395661852 -64.1941705865344
356.390938261852 -64.1347561865344
355.894480861852 -64.0753417865344
355.398023461852 -64.0159273865344
354.901566061852 -63.9565129865344
354.405108661852 -63.8970985865344
353.908651261852 -63.8376841865344
353.412193861852 -63.7782697865344
352.915736461852 -63.7188553865344
352.419279061852 -63.6594409865344
351.922821661852 -63.6000265865344
351.426364261852 -63.5406121865344
350.929906861852 -63.4811977865344
350.433449461852 -63.4217833865344
349.936992061852 -63.3623689865344
349.440534661852 -63.3029545865344
348.944077261852 -63.2435401865344
348.447619861852 -63.1841257865344
347.951162461852 -63.1247113865344
347.454705061852 -63.0652969865344
353.099793436261 -93.9598623674527
352.603319086261 -93.9005901174527
352.106844736261 -93.8413178674527
351.610370386261 -93.7820456174527
351.113896036261 -93.7227733674527
350.617421686261 -93.6635011174527
350.120947336261 -93.6042288674527
349.624472986261 -93.5449566174527
349.127998636261 -93.4856843674527
348.631524286261 -93.4264121174527
348.135049936261 -93.3671398674527
347.638575586261 -93.3078676174527
347.142101236261 -93.2485953674527
346.645626886261 -93.1893231174527
346.149152536261 -93.1300508674527
345.652678186261 -93.0707786174527
345.156203836261 -93.0115063674527
344.659729486261 -92.9522341174527
344.163255136261 -92.8929618674527
343.666780786261 -92.8336896174527
349.677185328163 -123.724041282439
349.180709028163 -123.664785082439
348.684232728163 -123.605528882439
348.187756428163 -123.546272682439
347.691280128163 -123.487016482439
347.194803828163 -123.427760282439
346.698327528163 -123.368504082439
346.201851228163 -123.309247882439
345.705374928163 -123.249991682439
345.208898628163 -123.190735482439
344.712422328163 -123.131479282439
344.215946028163 -123.072223082439
343.719469728163 -123.012966882439
343.222993428163 -122.953710682439
342.726517128163 -122.894454482439
342.230040828163 -122.835198282439
341.733564528163 -122.775942082439
341.237088228163 -122.716685882439
345.937579448675 -153.482527603975
345.440687598675 -153.426863503975
344.943795748675 -153.371199403975
344.446903898675 -153.315535303975
343.950012048675 -153.259871203975
343.453120198675 -153.204207103975
342.956228348675 -153.148543003975
342.459336498675 -153.092878903975
341.962444648675 -153.037214803975
341.465552798675 -152.981550703975
340.968660948675 -152.925886603975
340.471769098675 -152.870222503975
339.974877248675 -152.814558403975
342.5490179 -183.35696065
342.0581559 -183.2618054
341.5672939 -183.16665015
341.0764319 -183.0714949
340.5855699 -182.97633965
340.0947079 -182.8811844
339.6038459 -182.78602915
339.1129839 -182.6908739
338.6221219 -182.59571865
338.1312599 -182.5005634
337.6403979 -182.40540815
337.1495359 -182.3102529
336.6586739 -182.21509765
336.1678119 -182.1199424
335.6769499 -182.02478715
335.1860879 -181.9296319
341.459312899886 -192.398307377297
340.977484849886 -192.264734477297
340.495656799886 -192.131161577297
340.013828749886 -191.997588677297
339.532000699886 -191.864015777297
339.050172649886 -191.730442877297
338.568344599886 -191.596869977297
338.086516549886 -191.463297077297
337.604688499886 -191.329724177297
337.122860449886 -191.196151277297
336.641032399886 -191.062578377297
336.159204349886 -190.929005477297
335.677376299886 -190.795432577297
335.195548249886 -190.661859677297
334.713720199886 -190.528286777297
334.231892149886 -190.394713877297
333.750064099886 -190.261140977297
339.864444389768 -201.599747992258
339.399535939768 -201.415736792258
338.934627489768 -201.231725592258
338.469719039768 -201.047714392258
338.004810589768 -200.863703192258
337.539902139768 -200.679691992258
337.074993689768 -200.495680792258
336.610085239768 -200.311669592258
336.145176789768 -200.127658392258
335.680268339768 -199.943647192258
335.215359889768 -199.759635992258
334.750451439768 -199.575624792258
334.285542989768 -199.391613592258
333.820634539768 -199.207602392258
333.355726089768 -199.023591192258
332.890817639768 -198.839579992258
332.425909189768 -198.655568792258
331.961000739768 -198.471557592258
338.620464912885 -211.768586326081
338.188344512885 -211.517047126081
337.756224112885 -211.265507926081
337.324103712885 -211.013968726081
336.891983312885 -210.762429526081
336.459862912885 -210.510890326081
336.027742512885 -210.259351126081
335.595622112885 -210.007811926081
335.163501712885 -209.756272726081
334.731381312885 -209.504733526081
334.299260912885 -209.253194326081
333.867140512885 -209.001655126081
333.435020112885 -208.750115926081
333.002899712885 -208.498576726081
332.570779312885 -208.247037526081
332.138658912885 -207.995498326081
331.706538512885 -207.743959126081
331.274418112885 -207.492419926081
330.842297712885 -207.240880726081
330.410177312885 -206.989341526081
329.978056912885 -206.737802326081
329.545936512885 -206.486263126081
334.09162688 -221.34126301
333.71742908 -221.00963666
333.34323128 -220.67801031
332.96903348 -220.34638396
332.59483568 -220.01475761
332.22063788 -219.68313126
331.84644008 -219.35150491
331.47224228 -219.01987856
331.09804448 -218.68825221
330.72384668 -218.35662586
330.34964888 -218.02499951
329.97545108 -217.69337316
329.60125328 -217.36174681
329.22705548 -217.03012046
328.85285768 -216.69849411
328.47865988 -216.36686776
328.10446208 -216.03524141
327.73026428 -215.70361506
327.35606648 -215.37198871
326.98186868 -215.04036236
326.60767088 -214.70873601
326.23347308 -214.37710966
326.81812678371 -229.387946670167
326.51904638371 -228.987258620167
326.21996598371 -228.586570570167
325.92088558371 -228.185882520167
325.62180518371 -227.785194470167
325.32272478371 -227.384506420167
325.02364438371 -226.983818370167
324.72456398371 -226.583130320167
324.42548358371 -226.182442270167
324.12640318371 -225.781754220167
323.82732278371 -225.381066170167
323.52824238371 -224.980378120167
323.22916198371 -224.579690070167
322.93008158371 -224.179002020167
322.63100118371 -223.778313970167
322.33192078371 -223.377625920167
322.03284038371 -222.976937870167
321.73375998371 -222.576249820167
321.43467958371 -222.175561770167
321.13559918371 -221.774873720167
320.83651878371 -221.374185670167
317.847487 -235.88858774
317.637206 -235.43495584
317.426925 -234.98132394
317.216644 -234.52769204
317.006363 -234.07406014
316.796082 -233.62042824
316.585801 -233.16679634
316.37552 -232.71316444
316.165239 -232.25953254
315.954958 -231.80590064
315.744677 -231.35226874
315.534396 -230.89863684
315.324115 -230.44500494
315.113834 -229.99137304
314.903553 -229.53774114
314.693272 -229.08410924
314.482991 -228.63047734
314.27271 -228.17684544
314.062429 -227.72321354
313.852148 -227.26958164
313.641867 -226.81594974
313.431586 -226.36231784
307.380601154546 -239.50587506884
307.266045054546 -239.01917506884
307.151488954546 -238.53247506884
307.036932854546 -238.04577506884
306.922376754546 -237.55907506884
306.807820654546 -237.07237506884
306.693264554546 -236.58567506884
306.578708454546 -236.09897506884
306.464152354546 -235.61227506884
306.349596254546 -235.12557506884
306.235040154546 -234.63887506884
306.120484054546 -234.15217506884
306.005927954546 -233.66547506884
305.891371854546 -233.17877506884
305.776815754546 -232.69207506884
305.662259654546 -232.20537506884
305.547703554546 -231.71867506884
305.433147454546 -231.23197506884
305.318591354546 -230.74527506884
305.204035254546 -230.25857506884
305.089479154546 -229.77187506884
304.974923054546 -229.28517506884
296.43059338 -240.43728412
296.41546933 -239.93751292
296.40034528 -239.43774172
296.38522123 -238.93797052
296.37009718 -238.43819932
296.35497313 -237.93842812
296.33984908 -237.43865692
296.32472503 -236.93888572
296.30960098 -236.43911452
296.29447693 -235.93934332
296.27935288 -235.43957212
296.26422883 -234.93980092
296.24910478 -234.44002972
296.23398073 -233.94025852
296.21885668 -233.44048732
296.20373263 -232.94071612
296.18860858 -232.44094492
296.17348453 -231.94117372
296.15836048 -231.44140252
296.14323643 -230.94163132
296.12811238 -230.44186012
296.11298833 -229.94208892
296.09786428 -229.44231772
285.978674662639 -238.348869014865
286.051139962639 -237.854148114865
286.123605262638 -237.359427214865
286.196070562639 -236.864706314865
286.268535862638 -236.369985414865
286.341001162639 -235.875264514865
286.413466462638 -235.380543614865
286.485931762639 -234.885822714865
286.558397062639 -234.391101814865
286.630862362638 -233.896380914865
286.703327662639 -233.401660014865
286.775792962638 -232.906939114865
286.848258262639 -232.412218214865
286.920723562638 -231.917497314865
286.993188862638 -231.422776414865
287.065654162639 -230.928055514865
287.138119462638 -230.433334614865
287.210584762639 -229.938613714865
287.283050062638 -229.443892814865
287.355515362639 -228.949171914865
287.427980662639 -228.454451014865
287.500445962638 -227.959730114865
287.572911262639 -227.465009214865
276.732983116108 -233.850123195605
276.873991366108 -233.370418395605
277.014999616108 -232.890713595605
277.156007866108 -232.411008795605
277.297016116108 -231.931303995605
277.438024366108 -231.451599195605
277.579032616108 -230.971894395605
277.720040866108 -230.492189595605
277.861049116108 -230.012484795605
278.002057366108 -229.532779995605
278.143065616108 -229.053075195605
278.284073866108 -228.573370395605
278.425082116108 -228.093665595605
278.566090366108 -227.613960795605
278.707098616108 -227.134255995605
278.848106866108 -226.654551195605
278.989115116108 -226.174846395605
279.130123366108 -225.695141595605
279.271131616108 -225.215436795605
279.412139866108 -224.735731995605
279.553148116108 -224.256027195605
279.694156366108 -223.776322395605
268.378743623341 -228.948501717087
268.567712173341 -228.485586067087
268.756680723341 -228.022670417087
268.945649273341 -227.559754767087
269.134617823341 -227.096839117087
269.323586373341 -226.633923467087
269.512554923341 -226.171007817087
269.701523473341 -225.708092167087
269.890492023341 -225.245176517087
270.079460573341 -224.782260867087
270.268429123341 -224.319345217087
270.457397673341 -223.856429567087
270.646366223341 -223.393513917087
270.835334773341 -222.930598267087
271.024303323341 -222.467682617087
271.213271873341 -222.004766967087
271.402240423341 -221.541851317087
271.591208973341 -221.078935667087
271.780177523341 -220.616020017087
271.969146073341 -220.153104367087
272.158114623341 -219.690188717087
272.347083173341 -219.227273067087
272.536051723341 -218.764357417087
260.5362362 -223.89788425
260.7526992 -223.4471695
260.9691622 -222.99645475
261.1856252 -222.54574
261.4020882 -222.09502525
261.6185512 -221.6443105
261.8350142 -221.19359575
262.0514772 -220.742881
262.2679402 -220.29216625
262.4844032 -219.8414515
262.7008662 -219.39073675
262.9173292 -218.940022
263.1337922 -218.48930725
263.3502552 -218.0385925
263.5667182 -217.58787775
263.7831812 -217.137163
263.9996442 -216.68644825
264.2161072 -216.2357335
264.4325702 -215.78501875
264.6490332 -215.334304
264.8654962 -214.88358925
265.0819592 -214.4328745
265.2984222 -213.98215975
235.57422251168 -206.809604498743
235.84427721168 -206.388807098743
236.11433191168 -205.968009698743
236.38438661168 -205.547212298743
236.65444131168 -205.126414898743
236.92449601168 -204.705617498743
237.19455071168 -204.284820098743
237.46460541168 -203.864022698743
237.73466011168 -203.443225298743
238.00471481168 -203.022427898743
238.27476951168 -202.601630498743
238.54482421168 -202.180833098743
238.81487891168 -201.760035698743
239.08493361168 -201.339238298743
239.35498831168 -200.918440898743
239.62504301168 -200.497643498743
239.89509771168 -200.076846098743
240.16515241168 -199.656048698743
240.43520711168 -199.235251298743
240.70526181168 -198.814453898743
240.97531651168 -198.393656498743
241.24537121168 -197.972859098743
241.51542591168 -197.552061698743
210.624480422329 -190.158143478173
210.90503327233 -189.744271378173
211.18558612233 -189.330399278173
211.46613897233 -188.916527178173
211.74669182233 -188.502655078173
212.02724467233 -188.088782978173
212.30779752233 -187.674910878173
212.58835037233 -187.261038778173
212.86890322233 -186.847166678173
213.14945607233 -186.433294578173
213.43000892233 -186.019422478173
213.710561772329 -185.605550378173
213.99111462233 -185.191678278173
214.27166747233 -184.777806178173
214.55222032233 -184.363934078173
214.832773172329 -183.950061978173
215.11332602233 -183.536189878173
215.39387887233 -183.122317778173
215.67443172233 -182.708445678173
215.95498457233 -182.294573578173
216.23553742233 -181.880701478173
216.51609027233 -181.466829378173
216.796643122329 -181.052957278173
185.578785901757 -173.671318669997
185.856748151757 -173.255702269997
186.134710401757 -172.840085869997
186.412672651757 -172.424469469997
186.690634901757 -172.008853069997
186.968597151757 -171.593236669997
187.246559401757 -171.177620269997
187.524521651757 -170.762003869997
187.802483901757 -170.346387469997
188.080446151757 -169.930771069997
188.358408401757 -169.515154669997
188.636370651757 -169.099538269997
188.914332901757 -168.683921869997
189.192295151757 -168.268305469997
189.470257401757 -167.852689069997
189.748219651757 -167.437072669997
190.026181901757 -167.021456269997
190.304144151757 -166.605839869997
190.582106401757 -166.190223469997
190.860068651757 -165.774607069997
191.138030901757 -165.358990669997
191.415993151757 -164.943374269997
191.693955401757 -164.527757869997
160.461066867805 -157.291399742343
160.739067517805 -156.875808992343
161.017068167805 -156.460218242343
161.295068817805 -156.044627492343
161.573069467805 -155.629036742343
161.851070117805 -155.213445992343
162.129070767805 -154.797855242343
162.407071417805 -154.382264492343
162.685072067805 -153.966673742343
162.963072717805 -153.551082992343
163.241073367805 -153.135492242343
163.519074017805 -152.719901492343
163.797074667805 -152.304310742343
164.075075317805 -151.888719992343
164.353075967805 -151.473129242343
164.631076617805 -151.057538492343
164.909077267805 -150.641947742343
165.187077917805 -150.226356992343
165.465078567805 -149.810766242343
165.743079217805 -149.395175492343
166.021079867805 -148.979584742343
166.299080517805 -148.563993992343
166.577081167805 -148.148403242343
135.54823248 -140.60014206
135.82601493 -140.18440546
136.10379738 -139.76866886
136.38157983 -139.35293226
136.65936228 -138.93719566
136.93714473 -138.52145906
137.21492718 -138.10572246
137.49270963 -137.68998586
137.77049208 -137.27424926
138.04827453 -136.85851266
138.32605698 -136.44277606
138.60383943 -136.02703946
138.88162188 -135.61130286
139.15940433 -135.19556626
139.43718678 -134.77982966
139.71496923 -134.36409306
139.99275168 -133.94835646
140.27053413 -133.53261986
140.54831658 -133.11688326
140.82609903 -132.70114666
141.10388148 -132.28541006
141.38166393 -131.86967346
141.65944638 -131.45393686
110.603542236609 -123.956707039106
110.880883186609 -123.540675789106
111.158224136609 -123.124644539106
111.435565086609 -122.708613289106
111.712906036609 -122.292582039106
111.990246986609 -121.876550789106
112.267587936609 -121.460519539106
112.544928886609 -121.044488289106
112.822269836609 -120.628457039106
113.099610786609 -120.212425789106
113.376951736609 -119.796394539106
113.654292686609 -119.380363289106
113.931633636609 -118.964332039106
114.208974586609 -118.548300789106
114.486315536609 -118.132269539106
114.763656486609 -117.716238289106
115.040997436609 -117.300207039106
115.318338386609 -116.884175789106
115.595679336609 -116.468144539106
115.873020286609 -116.052113289106
116.150361236609 -115.636082039106
116.427702186609 -115.220050789106
116.705043136609 -114.804019539106
85.6448477903712 -107.335812634054
85.9218377403712 -106.919547634054
86.1988276903712 -106.503282634054
86.4758176403712 -106.087017634054
86.7528075903712 -105.670752634054
87.0297975403712 -105.254487634054
87.3067874903712 -104.838222634054
87.5837774403712 -104.421957634054
87.8607673903712 -104.005692634054
88.1377573403712 -103.589427634054
88.4147472903712 -103.173162634054
88.6917372403712 -102.756897634054
88.9687271903712 -102.340632634054
89.2457171403712 -101.924367634054
89.5227070903712 -101.508102634054
89.7996970403712 -101.091837634054
90.0766869903712 -100.675572634054
90.3536769403712 -100.259307634054
90.6306668903712 -99.843042634054
90.9076568403712 -99.426777634054
91.1846467903712 -99.010512634054
91.4616367403712 -98.594247634054
91.7386266903712 -98.177982634054
60.6770553502117 -90.7293567744541
60.9538447502117 -90.3129583744541
61.2306341502117 -89.8965599744541
61.5074235502117 -89.4801615744541
61.7842129502117 -89.0637631744541
62.0610023502117 -88.6473647744541
62.3377917502117 -88.2309663744541
62.6145811502117 -87.8145679744541
62.8913705502117 -87.3981695744541
63.1681599502117 -86.9817711744541
63.4449493502117 -86.5653727744541
63.7217387502117 -86.1489743744541
63.9985281502117 -85.7325759744541
64.2753175502117 -85.3161775744541
64.5521069502117 -84.8997791744541
64.8288963502117 -84.4833807744541
65.1056857502117 -84.0669823744541
65.3824751502117 -83.6505839744541
65.6592645502117 -83.2341855744541
65.9360539502117 -82.8177871744541
66.2128433502117 -82.4013887744541
66.4896327502117 -81.9849903744541
66.7664221502117 -81.5685919744541
35.7046765844827 -74.1299019835669
35.9814160344827 -73.7134703835669
36.2581554844827 -73.2970387835669
36.5348949344827 -72.8806071835669
36.8116343844827 -72.4641755835669
37.0883738344827 -72.0477439835669
37.3651132844827 -71.6313123835669
37.6418527344827 -71.2148807835669
37.9185921844827 -70.7984491835669
38.1953316344827 -70.3820175835669
38.4720710844827 -69.9655859835669
38.7488105344827 -69.5491543835669
39.0255499844827 -69.1327227835669
39.3022894344827 -68.7162911835669
39.5790288844827 -68.2998595835669
39.8557683344827 -67.8834279835669
40.1325077844827 -67.4669963835669
40.4092472344827 -67.0505647835669
40.6859866844827 -66.6341331835669
40.9627261344827 -66.2177015835669
41.2394655844827 -65.8012699835669
41.5162050344827 -65.3848383835669
41.7929444844827 -64.9684067835669
10.7322114652489 -57.5300351430109
11.0090516152489 -57.1136704930109
11.2858917652489 -56.6973058430109
11.5627319152489 -56.2809411930109
11.8395720652489 -55.8645765430109
12.1164122152489 -55.4482118930109
12.3932523652489 -55.0318472430109
12.6700925152489 -54.6154825930109
12.9469326652489 -54.1991179430109
13.2237728152489 -53.7827532930109
13.5006129652489 -53.3663886430109
13.7774531152489 -52.9500239930109
14.0542932652489 -52.5336593430109
14.3311334152489 -52.1172946930109
14.6079735652489 -51.7009300430109
14.8848137152489 -51.2845653930109
15.1616538652489 -50.8682007430109
15.4384940152489 -50.4518360930109
15.7153341652489 -50.0354714430109
15.9921743152489 -49.6191067930109
16.2690144652489 -49.2027421430109
16.5458546152489 -48.7863774930109
16.8226947652489 -48.3700128430109
};


==> ressources/solver_benchmark/scenario/raceline.tex <==
\addplot [line width=1pt, TUMred]
table {%
-1.75329377814429 -49.228601104573
-1.47634682814429 -48.812307454573
-1.19939987814429 -48.396013804573
-0.92245292814429 -47.979720154573
-0.64550597814429 -47.563426504573
-0.36855902814429 -47.147132854573
-0.09161207814429 -46.730839204573
0.18533487185571 -46.314545554573
0.46228182185571 -45.898251904573
0.73922877185571 -45.481958254573
1.01617572185571 -45.065664604573
1.29312267185571 -44.649370954573
1.57006962185571 -44.233077304573
1.84701657185571 -43.816783654573
2.12396352185571 -43.400490004573
2.40091047185571 -42.984196354573
2.67785742185571 -42.567902704573
2.95480437185571 -42.151609054573
3.23175132185571 -41.735315404573
3.50869827185571 -41.319021754573
3.78564522185571 -40.902728104573
4.06259217185571 -40.486434454573
4.33953912185571 -40.070140804573
-26.7258494442021 -32.6273644165333
-26.4486917442021 -32.2112110665333
-26.1715340442021 -31.7950577165333
-25.8943763442021 -31.3789043665333
-25.6172186442021 -30.9627510165333
-25.3400609442021 -30.5465976665333
-25.0629032442021 -30.1304443165333
-24.7857455442021 -29.7142909665333
-24.5085878442021 -29.2981376165333
-24.2314301442021 -28.8819842665333
-23.9542724442021 -28.4658309165333
-23.6771147442021 -28.0496775665333
-23.3999570442021 -27.6335242165333
-23.1227993442021 -27.2173708665333
-22.8456416442021 -26.8012175165333
-22.5684839442021 -26.3850641665333
-22.2913262442021 -25.9689108165333
-22.0141685442021 -25.5527574665333
-21.7370108442021 -25.1366041165333
-21.4598531442021 -24.7204507665333
-21.1826954442021 -24.3042974165333
-20.9055377442021 -23.8881440665333
-20.6283800442021 -23.4719907165333
-51.701341994585 -16.0300217450733
-51.424054394585 -15.6139549450733
-51.146766794585 -15.1978881450733
-50.869479194585 -14.7818213450733
-50.592191594585 -14.3657545450733
-50.314903994585 -13.9496877450733
-50.037616394585 -13.5336209450733
-49.760328794585 -13.1175541450733
-49.483041194585 -12.7014873450733
-49.205753594585 -12.2854205450733
-48.928465994585 -11.8693537450733
-48.651178394585 -11.4532869450733
-48.373890794585 -11.0372201450733
-48.096603194585 -10.6211533450733
-47.819315594585 -10.2050865450733
-47.542027994585 -9.78901974507328
-47.264740394585 -9.37295294507328
-46.987452794585 -8.95688614507328
-46.710165194585 -8.54081934507328
-46.432877594585 -8.12475254507328
-46.155589994585 -7.70868574507328
-45.878302394585 -7.29261894507328
-45.601014794585 -6.87655214507328
-76.680309189896 0.56235655954599
-76.402972589896 0.97839070954599
-76.125635989896 1.39442485954599
-75.848299389896 1.81045900954599
-75.570962789896 2.22649315954599
-75.293626189896 2.64252730954599
-75.016289589896 3.05856145954599
-74.738952989896 3.47459560954599
-74.461616389896 3.89062975954599
-74.184279789896 4.30666390954599
-73.906943189896 4.72269805954599
-73.629606589896 5.13873220954599
-73.352269989896 5.55476635954599
-73.074933389896 5.97080050954599
-72.797596789896 6.38683465954599
-72.520260189896 6.80286880954599
-72.242923589896 7.21890295954599
-71.965586989896 7.63493710954599
-71.688250389896 8.05097125954599
-71.410913789896 8.46700540954599
-71.133577189896 8.88303955954599
-70.856240589896 9.29907370954599
-70.578903989896 9.71510785954599
-101.663273987831 17.1486899736175
-101.385969237831 17.5647453736175
-101.108664487831 17.9808007736175
-100.831359737831 18.3968561736175
-100.554054987831 18.8129115736175
-100.276750237831 19.2289669736175
-99.9994454878307 19.6450223736175
-99.7221407378307 20.0610777736175
-99.4448359878307 20.4771331736175
-99.1675312378307 20.8931885736175
-98.8902264878307 21.3092439736175
-98.6129217378307 21.7252993736175
-98.3356169878307 22.1413547736175
-98.0583122378307 22.5574101736175
-97.7810074878307 22.9734655736175
-97.5037027378307 23.3895209736175
-97.2263979878307 23.8055763736175
-96.9490932378307 24.2216317736175
-96.6717884878307 24.6376871736175
-96.3944837378307 25.0537425736175
-96.1171789878307 25.4697979736175
-95.8398742378307 25.8858533736175
-95.5625694878307 26.3019087736175
-126.650751380691 33.7278921282357
-126.373559330691 34.1440225782357
-126.096367280691 34.5601530282357
-125.819175230691 34.9762834782357
-125.541983180691 35.3924139282357
-125.264791130691 35.8085443782357
-124.987599080691 36.2246748282357
-124.710407030691 36.6408052782357
-124.433214980691 37.0569357282357
-124.156022930691 37.4730661782357
-123.878830880691 37.8891966282357
-123.601638830691 38.3053270782357
-123.324446780691 38.7214575282357
-123.047254730691 39.1375879782357
-122.770062680691 39.5537184282357
-122.492870630691 39.9698488782357
-122.215678580691 40.3859793282357
-121.938486530691 40.8021097782357
-121.661294480691 41.2182402282357
-121.384102430691 41.6343706782357
-121.106910380691 42.0505011282357
-120.829718330691 42.4666315782357
-120.552526280691 42.8827620282357
-151.643255697699 50.2988766434079
-151.366257197699 50.7151359934079
-151.089258697699 51.1313953434079
-150.812260197699 51.5476546934079
-150.535261697699 51.9639140434079
-150.258263197699 52.3801733934079
-149.981264697699 52.7964327434079
-149.704266197699 53.2126920934079
-149.427267697699 53.6289514434079
-149.150269197699 54.0452107934079
-148.873270697699 54.4614701434079
-148.596272197699 54.8777294934079
-148.319273697699 55.2939888434079
-148.042275197699 55.7102481934079
-147.765276697699 56.1265075434079
-147.488278197699 56.5427668934079
-147.211279697699 56.9590262434079
-146.934281197699 57.3752855934079
-146.657282697699 57.7915449434079
-146.380284197699 58.2078042934079
-146.103285697699 58.6240636434079
-145.826287197699 59.0403229934079
-145.549288697699 59.4565823434079
-176.641307621955 66.8605631054873
-176.364583671955 67.2770050054873
-176.087859721955 67.6934469054873
-175.811135771955 68.1098888054873
-175.534411821955 68.5263307054873
-175.257687871955 68.9427726054873
-174.980963921955 69.3592145054873
-174.704239971955 69.7756564054873
-174.427516021955 70.1920983054873
-174.150792071955 70.6085402054873
-173.874068121955 71.0249821054873
-173.597344171955 71.4414240054873
-173.320620221955 71.8578659054873
-173.043896271955 72.2743078054873
-172.767172321955 72.6907497054873
-172.490448371955 73.1071916054873
-172.213724421955 73.5236335054873
-171.937000471955 73.9400754054873
-171.660276521955 74.3565173054873
-171.383552571955 74.7729592054873
-171.106828621955 75.1894011054873
-170.830104671955 75.6058430054873
-170.553380721955 76.0222849054873
-201.645441748717 83.4118816206171
-201.369073398717 83.8285595706171
-201.092705048717 84.2452375206171
-200.816336698717 84.6619154706171
-200.539968348717 85.0785934206171
-200.263599998717 85.4952713706171
-199.987231648717 85.9119493206171
-199.710863298717 86.3286272706171
-199.434494948717 86.7453052206171
-199.158126598717 87.1619831706171
-198.881758248717 87.5786611206171
-198.605389898717 87.9953390706171
-198.329021548717 88.4120170206171
-198.052653198717 88.8286949706171
-197.776284848717 89.2453729206171
-197.499916498717 89.6620508706171
-197.223548148717 90.0787288206171
-196.947179798717 90.4954067706171
-196.670811448717 90.9120847206171
-196.394443098717 91.3287626706171
-196.118074748717 91.7454406206171
-195.841706398717 92.1621185706171
-195.565338048717 92.5787965206171
-226.656213599453 99.9517783895372
-226.380282099453 100.368745789537
-226.104350599453 100.785713189537
-225.828419099453 101.202680589537
-225.552487599453 101.619647989537
-225.276556099453 102.036615389537
-225.000624599453 102.453582789537
-224.724693099453 102.870550189537
-224.448761599453 103.287517589537
-224.172830099453 103.704484989537
-223.896898599453 104.121452389537
-223.620967099453 104.538419789537
-223.345035599453 104.955387189537
-223.069104099453 105.372354589537
-222.793172599453 105.789321989537
-222.517241099453 106.206289389537
-222.241309599453 106.623256789537
-221.965378099453 107.040224189537
-221.689446599453 107.457191589537
-221.413515099453 107.874158989537
-221.137583599453 108.291126389537
-220.861652099453 108.708093789537
-220.585720599453 109.125061189537
-251.674172161192 116.479278211943
-251.398758211192 116.896587661943
-251.123344261192 117.313897111943
-250.847930311192 117.731206561943
-250.572516361192 118.148516011943
-250.297102411192 118.565825461943
-250.021688461192 118.983134911943
-249.746274511192 119.400444361943
-249.470860561192 119.817753811943
-249.195446611192 120.235063261943
-248.920032661192 120.652372711943
-248.644618711192 121.069682161943
-248.369204761192 121.486991611943
-248.093790811192 121.904301061943
-247.818376861192 122.321610511943
-247.542962911192 122.738919961943
-247.267548961192 123.156229411943
-246.992135011192 123.573538861943
-246.716721061192 123.990848311943
-246.441307111192 124.408157761943
-246.165893161192 124.825467211943
-245.890479211192 125.242776661943
-245.615065261192 125.660086111943
-276.148649158058 133.831706351418
-275.873676758058 134.249306851418
-275.598704358058 134.666907351418
-275.323731958058 135.084507851418
-275.048759558058 135.502108351418
-274.773787158058 135.919708851418
-274.498814758058 136.337309351418
-274.223842358058 136.754909851418
-273.948869958058 137.172510351418
-273.673897558058 137.590110851418
-273.398925158058 138.007711351418
-273.123952758058 138.425311851418
-272.848980358058 138.842912351418
-272.574007958058 139.260512851418
-272.299035558058 139.678113351418
-272.024063158058 140.095713851418
-271.749090758058 140.513314351418
-271.474118358058 140.930914851418
-271.199145958058 141.348515351418
-270.924173558058 141.766115851418
-270.649201158058 142.183716351418
-270.374228758058 142.601316851418
-301.453551376352 149.924773450582
-301.178822226352 150.342534000582
-300.904093076352 150.760294550582
-300.629363926352 151.178055100582
-300.354634776352 151.595815650582
-300.079905626352 152.013576200582
-299.805176476352 152.431336750582
-299.530447326352 152.849097300582
-299.255718176352 153.266857850582
-298.980989026352 153.684618400582
-298.706259876352 154.102378950582
-298.431530726352 154.520139500582
-298.156801576352 154.937900050582
-297.882072426352 155.355660600582
-297.607343276352 155.773421150582
-297.332614126352 156.191181700582
-297.057884976352 156.608942250582
-296.783155826352 157.026702800582
-296.508426676352 157.444463350582
-296.233697526352 157.862223900582
-295.958968376352 158.279984450582
-295.684239226352 158.697745000582
-326.487566151275 166.431234234324
-326.212881751275 166.849024234324
-325.938197351275 167.266814234324
-325.663512951275 167.684604234324
-325.388828551275 168.102394234324
-325.114144151275 168.520184234324
-324.839459751275 168.937974234324
-324.564775351275 169.355764234324
-324.290090951275 169.773554234324
-324.015406551275 170.191344234324
-323.740722151275 170.609134234324
-323.466037751275 171.026924234324
-323.191353351275 171.444714234324
-322.916668951275 171.862504234324
-322.641984551275 172.280294234324
-322.367300151275 172.698084234324
-322.092615751275 173.115874234324
-321.817931351275 173.533664234324
-321.543246951275 173.951454234324
-321.268562551275 174.369244234324
-320.993878151275 174.787034234324
-320.719193751275 175.204824234324
-320.444509351275 175.622614234324
-351.52465919704 182.936117923386
-351.24982109704 183.353806823386
-350.97498299704 183.771495723386
-350.70014489704 184.189184623386
-350.42530679704 184.606873523386
-350.15046869704 185.024562423386
-349.87563059704 185.442251323386
-349.60079249704 185.859940223386
-349.32595439704 186.277629123386
-349.05111629704 186.695318023386
-348.77627819704 187.113006923386
-348.50144009704 187.530695823386
-348.22660199704 187.948384723386
-347.95176389704 188.366073623386
-347.67692579704 188.783762523386
-347.40208769704 189.201451423386
-347.12724959704 189.619140323386
-346.85241149704 190.036829223386
-346.57757339704 190.454518123386
-346.30273529704 190.872207023386
-346.02789719704 191.289895923386
-345.75305909704 191.707584823386
-345.47822099704 192.125273723386
-376.563838348732 199.442075947812
-376.288648948732 199.859533447812
-376.013459548732 200.276990947811
-375.738270148732 200.694448447812
-375.463080748732 201.111905947812
-375.187891348732 201.529363447812
-374.912701948732 201.946820947812
-374.637512548732 202.364278447812
-374.362323148732 202.781735947812
-374.087133748732 203.199193447811
-373.811944348732 203.616650947812
-373.536754948732 204.034108447812
-373.261565548732 204.451565947812
-372.986376148732 204.869023447812
-372.711186748732 205.286480947811
-372.435997348732 205.703938447812
-372.160807948732 206.121395947812
-371.885618548732 206.538853447812
-371.610429148732 206.956310947812
-371.335239748732 207.373768447811
-371.060050348732 207.791225947812
-370.784860948732 208.208683447811
-370.509671548732 208.626140947812
-401.601938551231 215.953135769848
-401.326287201231 216.370288419848
-401.050635851231 216.787441069848
-400.774984501231 217.204593719848
-400.499333151231 217.621746369848
-400.223681801231 218.038899019848
-399.948030451231 218.456051669848
-399.672379101231 218.873204319848
-399.396727751231 219.290356969848
-399.121076401231 219.707509619848
-398.845425051231 220.124662269848
-398.569773701231 220.541814919848
-398.294122351231 220.958967569848
-398.018471001231 221.376120219848
-397.742819651231 221.793272869848
-397.467168301231 222.210425519848
-397.191516951231 222.627578169848
-396.915865601231 223.044730819848
-396.640214251231 223.461883469848
-396.364562901231 223.879036119848
-396.088911551231 224.296188769848
-395.813260201231 224.713341419848
-395.537608851231 225.130494069848
-426.353362317105 232.894303170476
-426.077197917105 233.311116370476
-425.801033517105 233.727929570476
-425.524869117105 234.144742770476
-425.248704717105 234.561555970476
-424.972540317105 234.978369170476
-424.696375917105 235.395182370476
-424.420211517105 235.811995570476
-424.144047117105 236.228808770476
-423.867882717105 236.645621970476
-423.591718317105 237.062435170476
-423.315553917105 237.479248370476
-423.039389517105 237.896061570476
-422.763225117105 238.312874770476
-422.487060717105 238.729687970476
-422.210896317105 239.146501170476
-421.934731917105 239.563314370476
-421.658567517105 239.980127570476
-421.382403117105 240.396940770476
-421.106238717105 240.813753970476
-420.830074317105 241.230567170476
-420.553909917105 241.647380370476
-451.359340468007 249.440522135324
-451.082611918007 249.856960985324
-450.805883368007 250.273399835324
-450.529154818007 250.689838685324
-450.252426268007 251.106277535324
-449.975697718007 251.522716385324
-449.698969168007 251.939155235324
-449.422240618007 252.355594085324
-449.145512068007 252.772032935324
-448.868783518007 253.188471785324
-448.592054968007 253.604910635324
-448.315326418007 254.021349485324
-448.038597868007 254.437788335324
-447.761869318007 254.854227185324
-447.485140768007 255.270666035324
-447.208412218007 255.687104885324
-446.931683668007 256.103543735324
-446.654955118007 256.519982585324
-446.378226568007 256.936421435324
-446.101498018007 257.352860285324
-445.824769468007 257.769299135324
-445.548040918007 258.185737985324
-476.333697423046 266.01779843358
-476.056353423046 266.433827633581
-475.779009423046 266.849856833581
-475.501665423046 267.265886033581
-475.224321423046 267.681915233581
-474.946977423046 268.09794443358
-474.669633423046 268.513973633581
-474.392289423046 268.93000283358
-474.114945423046 269.346032033581
-473.837601423046 269.76206123358
-473.560257423046 270.178090433581
-473.282913423046 270.594119633581
-473.005569423046 271.010148833581
-472.728225423046 271.426178033581
-472.450881423046 271.84220723358
-472.173537423046 272.258236433581
-471.896193423046 272.67426563358
-471.618849423046 273.090294833581
-471.341505423046 273.50632403358
-471.064161423046 273.922353233581
-470.786817423046 274.33838243358
-470.509473423046 274.754411633581
-501.260677496731 282.644457982621
-500.981400246731 283.059191882621
-500.702122996731 283.473925782621
-500.422845746731 283.888659682621
-500.143568496731 284.303393582621
-499.864291246731 284.718127482621
-499.585013996731 285.132861382621
-499.305736746731 285.547595282621
-499.026459496731 285.962329182621
-498.747182246731 286.377063082621
-498.467904996731 286.791796982621
-498.188627746731 287.206530882621
-497.909350496731 287.621264782621
-497.630073246731 288.035998682621
-497.350795996731 288.450732582621
-497.071518746731 288.865466482621
-496.792241496731 289.280200382621
-496.512964246731 289.694934282621
-496.233686996731 290.109668182621
-495.954409746731 290.524402082621
-495.675132496731 290.939135982621
-495.395855246731 291.353869882621
-513.808438287183 290.977594395685
-513.501989287183 291.372675395685
-513.195540287183 291.767756395685
-512.889091287183 292.162837395685
-512.582642287183 292.557918395685
-512.276193287183 292.952999395685
-511.969744287183 293.348080395685
-511.663295287183 293.743161395685
-511.356846287183 294.138242395685
-511.050397287183 294.533323395685
-510.743948287183 294.928404395685
-510.437499287183 295.323485395685
-510.131050287183 295.718566395685
-509.824601287183 296.113647395685
-509.518152287183 296.508728395685
-509.211703287183 296.903809395685
-508.905254287183 297.298890395685
-508.598805287183 297.693971395685
-508.292356287183 298.089052395685
-507.985907287183 298.484133395685
-507.679458287183 298.879214395685
-507.373009287183 299.274295395685
-521.657933982711 295.992842815265
-521.307939532711 296.349919665265
-520.957945082711 296.706996515265
-520.607950632711 297.064073365265
-520.257956182711 297.421150215265
-519.907961732711 297.778227065265
-519.557967282711 298.135303915265
-519.207972832711 298.492380765265
-518.857978382711 298.849457615265
-518.507983932711 299.206534465265
-518.157989482711 299.563611315265
-517.807995032711 299.920688165265
-517.458000582711 300.277765015265
-517.108006132711 300.634841865265
-516.758011682711 300.991918715265
-516.408017232711 301.348995565265
-516.058022782711 301.706072415265
-515.708028332711 302.063149265265
-515.358033882711 302.420226115265
-515.008039432711 302.777302965265
-514.658044982711 303.134379815265
-514.308050532711 303.491456665265
-530.01851428 301.71173256
-529.59828498 301.98267046
-529.17805568 302.25360836
-528.75782638 302.52454626
-528.33759708 302.79548416
-527.91736778 303.06642206
-527.49713848 303.33735996
-527.07690918 303.60829786
-526.65667988 303.87923576
-526.23645058 304.15017366
-525.81622128 304.42111156
-525.39599198 304.69204946
-524.97576268 304.96298736
-524.55553338 305.23392526
-524.13530408 305.50486316
-523.71507478 305.77580106
-523.29484548 306.04673896
-522.87461618 306.31767686
-522.45438688 306.58861476
-522.03415758 306.85955266
-521.61392828 307.13049056
-521.19369898 307.40142846
-520.77346968 307.67236636
-538.692989317081 309.931243343113
-538.212261117081 310.068722043113
-537.731532917081 310.206200743113
-537.250804717081 310.343679443113
-536.770076517081 310.481158143113
-536.289348317081 310.618636843113
-535.808620117081 310.756115543113
-535.327891917081 310.893594243113
-534.847163717081 311.031072943113
-534.366435517081 311.168551643113
-533.885707317081 311.306030343113
-533.404979117081 311.443509043113
-532.924250917081 311.580987743113
-532.443522717081 311.718466443113
-531.962794517081 311.855945143113
-531.482066317081 311.993423843113
-531.001338117081 312.130902543113
-530.520609917081 312.268381243113
-530.039881717081 312.405859943113
-529.559153517081 312.543338643113
-529.078425317081 312.680817343113
-528.597697117081 312.818296043113
-528.116968917081 312.955774743113
-527.636240717081 313.093253443113
-527.155512517081 313.230732143113
-541.96620718 322.15571497
-541.46756038 322.11895402
-540.96891358 322.08219307
-540.47026678 322.04543212
-539.97161998 322.00867117
-539.47297318 321.97191022
-538.97432638 321.93514927
-538.47567958 321.89838832
-537.97703278 321.86162737
-537.47838598 321.82486642
-536.97973918 321.78810547
-536.48109238 321.75134452
-535.98244558 321.71458357
-535.48379878 321.67782262
-534.98515198 321.64106167
-534.48650518 321.60430072
-533.98785838 321.56753977
-533.48921158 321.53077882
-532.99056478 321.49401787
-532.49191798 321.45725692
-531.99327118 321.42049597
-531.49462438 321.38373502
-530.99597758 321.34697407
-530.49733078 321.31021312
-538.426609180911 334.909991547851
-537.980094380911 334.684992547851
-537.533579580911 334.459993547851
-537.087064780911 334.234994547851
-536.640549980911 334.009995547851
-536.194035180911 333.784996547851
-535.747520380911 333.559997547851
-535.301005580911 333.334998547851
-534.854490780911 333.109999547851
-534.407975980911 332.885000547851
-533.961461180911 332.660001547851
-533.514946380911 332.435002547851
-533.068431580911 332.210003547851
-532.621916780911 331.985004547851
-532.175401980911 331.760005547851
-531.728887180911 331.535006547851
-531.282372380911 331.310007547851
-530.835857580911 331.085008547851
-530.389342780911 330.860009547851
-529.942827980911 330.635010547851
-529.496313180911 330.410011547851
-529.049798380911 330.185012547851
-528.603283580911 329.960013547851
-528.156768780911 329.735014547851
-527.710253980911 329.510015547851
-528.61645312 343.01207597
-528.27475992 342.64704752
-527.93306672 342.28201907
-527.59137352 341.91699062
-527.24968032 341.55196217
-526.90798712 341.18693372
-526.56629392 340.82190527
-526.22460072 340.45687682
-525.88290752 340.09184837
-525.54121432 339.72681992
-525.19952112 339.36179147
-524.85782792 338.99676302
-524.51613472 338.63173457
-524.17444152 338.26670612
-523.83274832 337.90167767
-523.49105512 337.53664922
-523.14936192 337.17162077
-522.80766872 336.80659232
-522.46597552 336.44156387
-522.12428232 336.07653542
-521.78258912 335.71150697
-521.44089592 335.34647852
-521.09920272 334.98145007
-517.310878953819 345.866398663633
-517.104737353819 345.410870813633
-516.898595753819 344.955342963633
-516.692454153819 344.499815113633
-516.486312553819 344.044287263633
-516.280170953819 343.588759413633
-516.074029353819 343.133231563633
-515.867887753819 342.677703713633
-515.661746153819 342.222175863633
-515.455604553819 341.766648013633
-515.249462953819 341.311120163633
-515.043321353819 340.855592313633
-514.837179753819 340.400064463633
-514.631038153819 339.944536613633
-514.424896553819 339.489008763633
-514.218754953819 339.033480913633
-514.012613353819 338.577953063633
-513.806471753819 338.122425213633
-513.600330153819 337.666897363633
-513.394188553819 337.211369513633
-513.188046953819 336.755841663633
-512.981905353819 336.300313813633
-512.775763753819 335.844785963633
-507.135419840701 346.063360918649
-507.044966190701 345.571610818649
-506.954512540701 345.079860718649
-506.864058890701 344.588110618649
-506.773605240701 344.096360518649
-506.683151590701 343.604610418649
-506.592697940701 343.112860318649
-506.502244290701 342.621110218649
-506.411790640701 342.129360118649
-506.321336990701 341.637610018649
-506.230883340701 341.145859918649
-506.140429690701 340.654109818649
-506.049976040701 340.162359718649
-505.959522390701 339.670609618649
-505.869068740701 339.178859518649
-505.778615090701 338.687109418649
-505.688161440701 338.195359318649
-505.597707790701 337.703609218649
-505.507254140701 337.211859118649
-505.416800490701 336.720109018649
-505.326346840701 336.228358918649
-505.235893190701 335.736608818649
-497.847317199148 345.43830545114
-497.846610499148 344.93830595114
-497.845903799148 344.43830645114
-497.845197099148 343.93830695114
-497.844490399148 343.43830745114
-497.843783699148 342.93830795114
-497.843076999148 342.43830845114
-497.842370299148 341.93830895114
-497.841663599148 341.43830945114
-497.840956899148 340.93830995114
-497.840250199148 340.43831045114
-497.839543499148 339.93831095114
-497.838836799148 339.43831145114
-497.838130099148 338.93831195114
-497.837423399148 338.43831245114
-497.836716699148 337.93831295114
-497.836009999148 337.43831345114
-497.835303299148 336.93831395114
-497.834596599148 336.43831445114
-497.833889899148 335.93831495114
-497.833183199148 335.43831545114
-488.789701639795 345.387888171598
-488.850950039795 344.891653721598
-488.912198439795 344.395419271598
-488.973446839795 343.899184821598
-489.034695239795 343.402950371598
-489.095943639795 342.906715921598
-489.157192039795 342.410481471598
-489.218440439795 341.914247021598
-489.279688839795 341.418012571598
-489.340937239795 340.921778121598
-489.402185639795 340.425543671598
-489.463434039795 339.929309221598
-489.524682439795 339.433074771598
-489.585930839795 338.936840321598
-489.647179239795 338.440605871598
-489.708427639795 337.944371421598
-489.769676039795 337.448136971598
-489.830924439795 336.951902521598
-489.892172839795 336.455668071598
-489.953421239795 335.959433621598
-490.014669639795 335.463199171598
-479.668224873176 344.901742521253
-479.767978473176 344.411794321253
-479.867732073176 343.921846121253
-479.967485673176 343.431897921253
-480.067239273176 342.941949721253
-480.166992873176 342.452001521253
-480.266746473176 341.962053321253
-480.366500073176 341.472105121253
-480.466253673176 340.982156921253
-480.566007273176 340.492208721253
-480.665760873176 340.002260521253
-480.765514473176 339.512312321253
-480.865268073176 339.022364121253
-480.965021673176 338.532415921253
-481.064775273176 338.042467721253
-481.164528873176 337.552519521253
-481.264282473176 337.062571321253
-481.364036073176 336.572623121253
-481.463789673176 336.082674921253
-481.563543273176 335.592726721253
-481.663296873176 335.102778521253
-447.939771003183 342.724166999321
-448.132247803183 342.262699049321
-448.324724603183 341.801231099321
-448.517201403183 341.339763149321
-448.709678203183 340.878295199321
-448.902155003183 340.416827249321
-449.094631803183 339.955359299321
-449.287108603183 339.493891349321
-449.479585403183 339.032423399321
-449.672062203183 338.570955449321
-449.864539003183 338.109487499321
-450.057015803183 337.648019549321
-450.249492603183 337.186551599321
-450.441969403183 336.725083649321
-450.634446203183 336.263615699321
-450.826923003183 335.802147749321
-451.019399803183 335.340679799321
-451.211876603183 334.879211849321
-451.404353403183 334.417743899321
-451.596830203183 333.956275949321
-451.789307003183 333.494807999321
-420.955129282292 327.142491436508
-421.208553932292 326.711474086508
-421.461978582292 326.280456736508
-421.715403232292 325.849439386508
-421.968827882292 325.418422036508
-422.222252532292 324.987404686508
-422.475677182292 324.556387336508
-422.729101832292 324.125369986508
-422.982526482292 323.694352636508
-423.235951132292 323.263335286508
-423.489375782292 322.832317936508
-423.742800432292 322.401300586508
-423.996225082292 321.970283236508
-424.249649732292 321.539265886508
-424.503074382292 321.108248536508
-424.756499032292 320.677231186508
-425.009923682292 320.246213836508
-425.263348332292 319.815196486508
-425.516772982292 319.384179136508
-425.770197632292 318.953161786508
-395.392247174727 310.196494961
-395.685584674727 309.791583761
-395.978922174727 309.386672561
-396.272259674727 308.981761361
-396.565597174727 308.576850161
-396.858934674727 308.171938961
-397.152272174727 307.767027761
-397.445609674727 307.362116561
-397.738947174727 306.957205361
-398.032284674727 306.552294161
-398.325622174727 306.147382961
-398.618959674727 305.742471761
-398.912297174727 305.337560561
-399.205634674727 304.932649361
-399.498972174727 304.527738161
-399.792309674727 304.122826961
-400.085647174727 303.717915761
-400.378984674727 303.313004561
-400.672322174727 302.908093361
-400.965659674727 302.503182161
-370.21131762 293.8136828
-370.50544782 293.40934705
-370.79957802 293.0050113
-371.09370822 292.60067555
-371.38783842 292.1963398
-371.68196862 291.79200405
-371.97609882 291.3876683
-372.27022902 290.98333255
-372.56435922 290.5789968
-372.85848942 290.17466105
-373.15261962 289.7703253
-373.44674982 289.36598955
-373.74088002 288.9616538
-374.03501022 288.55731805
-374.32914042 288.1529823
-374.62327062 287.74864655
-374.91740082 287.3443108
-375.21153102 286.93997505
-375.50566122 286.5356393
-375.79979142 286.13130355
-376.09392162 285.7269678
-345.45268854 277.49728232
-345.73271314 277.08305262
-346.01273774 276.66882292
-346.29276234 276.25459322
-346.57278694 275.84036352
-346.85281154 275.42613382
-347.13283614 275.01190412
-347.41286074 274.59767442
-347.69288534 274.18344472
-347.97290994 273.76921502
-348.25293454 273.35498532
-348.53295914 272.94075562
-348.81298374 272.52652592
-349.09300834 272.11229622
-349.37303294 271.69806652
-349.65305754 271.28383682
-349.93308214 270.86960712
-350.21310674 270.45537742
-350.49313134 270.04114772
-350.77315594 269.62691802
-351.05318054 269.21268832
-336.001018270444 270.733668467147
-336.265155220444 270.309131467147
-336.529292170444 269.884594467147
-336.793429120444 269.460057467147
-337.057566070444 269.035520467147
-337.321703020444 268.610983467147
-337.585839970444 268.186446467147
-337.849976920444 267.761909467147
-338.114113870444 267.337372467147
-338.378250820444 266.912835467147
-338.642387770444 266.488298467147
-338.906524720444 266.063761467147
-339.170661670444 265.639224467147
-339.434798620444 265.214687467147
-339.698935570444 264.790150467147
-339.963072520444 264.365613467147
-340.227209470444 263.941076467147
-340.491346420444 263.516539467147
-340.755483370444 263.092002467147
-341.019620320444 262.667465467147
-329.273864734266 265.974284291099
-329.496918534266 265.526794641099
-329.719972334266 265.079304991099
-329.943026134266 264.631815341099
-330.166079934266 264.1843256911
-330.389133734266 263.736836041099
-330.612187534266 263.289346391099
-330.835241334266 262.841856741099
-331.058295134266 262.394367091099
-331.281348934266 261.9468774411
-331.504402734266 261.499387791099
-331.727456534266 261.051898141099
-331.950510334266 260.604408491099
-332.173564134266 260.156918841099
-332.396617934266 259.7094291911
-332.619671734266 259.261939541099
-332.842725534266 258.814449891099
-333.065779334266 258.366960241099
-333.288833134266 257.919470591099
-333.511886934266 257.4719809411
-322.909829395966 261.473775018368
-323.042079545966 260.991582218368
-323.174329695966 260.509389418368
-323.306579845966 260.027196618368
-323.438829995966 259.545003818368
-323.571080145966 259.062811018368
-323.703330295966 258.580618218368
-323.835580445966 258.098425418368
-323.967830595966 257.616232618368
-324.100080745966 257.134039818368
-324.232330895966 256.651847018368
-324.364581045966 256.169654218368
-324.496831195966 255.687461418368
-324.629081345966 255.205268618368
-324.761331495966 254.723075818368
-324.893581645966 254.240883018368
-325.025831795966 253.758690218368
-325.158081945966 253.276497418368
-325.290332095966 252.794304618368
-325.422582245966 252.312111818368
-315.661558214901 257.406329529307
-315.662463864901 256.906330329307
-315.663369514901 256.406331129307
-315.664275164901 255.906331929307
-315.665180814901 255.406332729307
-315.666086464901 254.906333529307
-315.666992114901 254.406334329307
-315.667897764901 253.906335129307
-315.668803414901 253.406335929307
-315.669709064901 252.906336729307
-315.670614714901 252.406337529307
-315.671520364901 251.906338329307
-315.672426014901 251.406339129307
-315.673331664901 250.906339929307
-315.674237314901 250.406340729307
-315.675142964901 249.906341529307
-315.676048614901 249.406342329307
-315.676954264901 248.906343129307
-315.677859914901 248.406343929307
-315.678765564901 247.906344729307
-315.679671214901 247.406345529307
-307.32450448 256.37224002
-307.15322128 255.90249322
-306.98193808 255.43274642
-306.81065488 254.96299962
-306.63937168 254.49325282
-306.46808848 254.02350602
-306.29680528 253.55375922
-306.12552208 253.08401242
-305.95423888 252.61426562
-305.78295568 252.14451882
-305.61167248 251.67477202
-305.44038928 251.20502522
-305.26910608 250.73527842
-305.09782288 250.26553162
-304.92653968 249.79578482
-304.75525648 249.32603802
-304.58397328 248.85629122
-304.41269008 248.38654442
-304.24140688 247.91679762
-304.07012368 247.44705082
-303.89884048 246.97730402
-299.541650593178 259.957250896896
-299.203918243178 259.588554696896
-298.866185893178 259.219858496896
-298.528453543178 258.851162296896
-298.190721193178 258.482466096896
-297.852988843178 258.113769896896
-297.515256493178 257.745073696896
-297.177524143178 257.376377496896
-296.839791793178 257.007681296896
-296.502059443178 256.638985096896
-296.164327093178 256.270288896896
-295.826594743178 255.901592696896
-295.488862393178 255.532896496896
-295.151130043178 255.164200296896
-294.813397693178 254.795504096896
-294.475665343178 254.426807896896
-294.137932993178 254.058111696896
-293.800200643178 253.689415496896
-293.462468293178 253.320719296896
-293.124735943178 252.952023096896
-294.69388277 267.20559837
-294.24848772 266.97839082
-293.80309267 266.75118327
-293.35769762 266.52397572
-292.91230257 266.29676817
-292.46690752 266.06956062
-292.02151247 265.84235307
-291.57611742 265.61514552
-291.13072237 265.38793797
-290.68532732 265.16073042
-290.23993227 264.93352287
-289.79453722 264.70631532
-289.34914217 264.47910777
-288.90374712 264.25190022
-288.45835207 264.02469267
-288.01295702 263.79748512
-287.56756197 263.57027757
-287.12216692 263.34307002
-286.67677187 263.11586247
-286.23137682 262.88865492
-285.78598177 262.66144737
-293.435881624009 275.679821645176
-292.942690424009 275.597587595176
-292.449499224009 275.515353545176
-291.956308024009 275.433119495176
-291.463116824009 275.350885445176
-290.969925624009 275.268651395176
-290.476734424009 275.186417345176
-289.983543224009 275.104183295176
-289.490352024009 275.021949245176
-288.997160824009 274.939715195176
-288.503969624009 274.857481145176
-288.010778424009 274.775247095176
-287.517587224009 274.693013045176
-287.024396024009 274.610778995176
-286.531204824009 274.528544945176
-286.038013624009 274.446310895176
-285.544822424009 274.364076845176
-285.051631224009 274.281842795176
-284.558440024009 274.199608745176
-284.065248824009 274.117374695176
-283.572057624009 274.035140645176
-292.395191519092 284.523025000787
-291.895862019092 284.497140100787
-291.396532519092 284.471255200787
-290.897203019092 284.445370300787
-290.397873519092 284.419485400787
-289.898544019092 284.393600500787
-289.399214519092 284.367715600787
-288.899885019092 284.341830700787
-288.400555519092 284.315945800787
-287.901226019092 284.290060900787
-287.401896519092 284.264176000787
-286.902567019092 284.238291100787
-286.403237519092 284.212406200787
-285.903908019092 284.186521300787
-285.404578519092 284.160636400787
-284.905249019092 284.134751500787
-284.405919519092 284.108866600787
-283.906590019092 284.082981700787
-283.407260519092 284.057096800787
-282.907931019092 284.031211900787
-291.262700648538 293.653555794974
-290.765328148538 293.602363844974
-290.267955648538 293.551171894974
-289.770583148538 293.499979944974
-289.273210648538 293.448787994974
-288.775838148538 293.397596044974
-288.278465648538 293.346404094974
-287.781093148538 293.295212144974
-287.283720648538 293.244020194974
-286.786348148538 293.192828244974
-286.288975648538 293.141636294974
-285.791603148538 293.090444344974
-285.294230648538 293.039252394974
-284.796858148538 292.988060444974
-284.299485648538 292.936868494974
-283.802113148538 292.885676544974
-283.304740648538 292.834484594974
-282.807368148538 292.783292644974
-282.309995648538 292.732100694974
-281.812623148538 292.680908744974
-290.17816098 302.74833012
-289.69497893 302.61974117
-289.21179688 302.49115222
-288.72861483 302.36256327
-288.24543278 302.23397432
-287.76225073 302.10538537
-287.27906868 301.97679642
-286.79588663 301.84820747
-286.31270458 301.71961852
-285.82952253 301.59102957
-285.34634048 301.46244062
-284.86315843 301.33385167
-284.37997638 301.20526272
-283.89679433 301.07667377
-283.41361228 300.94808482
-282.93043023 300.81949587
-282.44724818 300.69090692
-281.96406613 300.56231797
-281.48088408 300.43372902
-280.99770203 300.30514007
-288.55195865689 312.363020297248
-288.11103110689 312.127260097248
-287.67010355689 311.891499897248
-287.22917600689 311.655739697248
-286.78824845689 311.419979497248
-286.34732090689 311.184219297248
-285.90639335689 310.948459097248
-285.46546580689 310.712698897248
-285.02453825689 310.476938697248
-284.58361070689 310.241178497248
-284.14268315689 310.005418297248
-283.70175560689 309.769658097248
-283.26082805689 309.533897897248
-282.81990050689 309.298137697248
-282.37897295689 309.062377497248
-281.93804540689 308.826617297248
-281.49711785689 308.590857097248
-281.05619030689 308.355096897248
-280.61526275689 308.119336697248
-280.17433520689 307.883576497248
-285.550018223383 322.791126305838
-285.173988873383 322.461578255838
-284.797959523383 322.132030205838
-284.421930173383 321.802482155838
-284.045900823383 321.472934105838
-283.669871473383 321.143386055838
-283.293842123383 320.813838005838
-282.917812773383 320.484289955838
-282.541783423383 320.154741905838
-282.165754073383 319.825193855838
-281.789724723383 319.495645805838
-281.413695373383 319.166097755838
-281.037666023383 318.836549705838
-280.661636673383 318.507001655838
-280.285607323383 318.177453605838
-279.909577973383 317.847905555838
-279.533548623383 317.518357505838
-279.157519273383 317.188809455838
-278.781489923383 316.859261405838
-278.405460573383 316.529713355838
-278.752234293172 331.60230552638
-278.461854793172 331.19526777638
-278.171475293172 330.78823002638
-277.881095793172 330.38119227638
-277.590716293172 329.97415452638
-277.300336793172 329.56711677638
-277.009957293172 329.16007902638
-276.719577793172 328.75304127638
-276.429198293172 328.34600352638
-276.138818793172 327.93896577638
-275.848439293172 327.53192802638
-275.558059793172 327.12489027638
-275.267680293172 326.71785252638
-274.977300793172 326.31081477638
-274.686921293172 325.90377702638
-274.396541793172 325.49673927638
-274.106162293172 325.08970152638
-273.815782793172 324.68266377638
-273.525403293172 324.27562602638
-273.235023793172 323.86858827638
-269.026745191005 336.530697014884
-268.826222241005 336.072668014884
-268.625699291005 335.614639014884
-268.425176341005 335.156610014884
-268.224653391005 334.698581014884
-268.024130441005 334.240552014884
-267.823607491005 333.782523014884
-267.623084541005 333.324494014884
-267.422561591005 332.866465014884
-267.222038641005 332.408436014884
-267.021515691005 331.950407014884
-266.820992741005 331.492378014884
-266.620469791005 331.034349014884
-266.419946841005 330.576320014884
-266.219423891005 330.118291014884
-266.018900941005 329.660262014884
-265.818377991005 329.202233014884
-265.617855041005 328.744204014884
-265.417332091005 328.286175014884
-265.216809141005 327.828146014884
-265.016286191005 327.370117014884
-258.31700722631 336.910956087495
-258.20523747631 336.423608637495
-258.09346772631 335.936261187495
-257.98169797631 335.448913737495
-257.86992822631 334.961566287495
-257.75815847631 334.474218837495
-257.64638872631 333.986871387495
-257.53461897631 333.499523937495
-257.42284922631 333.012176487495
-257.31107947631 332.524829037495
-257.19930972631 332.037481587495
-257.08753997631 331.550134137495
-256.97577022631 331.062786687495
-256.86400047631 330.575439237495
-256.75223072631 330.088091787495
-256.64046097631 329.600744337495
-256.52869122631 329.113396887495
-256.41692147631 328.626049437495
-256.30515172631 328.138701987495
-256.19338197631 327.651354537495
-248.487509471732 335.970856944646
-248.449441471732 335.472308244646
-248.411373471732 334.973759544646
-248.373305471732 334.475210844646
-248.335237471732 333.976662144646
-248.297169471732 333.478113444646
-248.259101471732 332.979564744646
-248.221033471732 332.481016044646
-248.182965471732 331.982467344646
-248.144897471732 331.483918644646
-248.106829471732 330.985369944646
-248.068761471732 330.486821244646
-248.030693471732 329.988272544646
-247.992625471732 329.489723844646
-247.954557471732 328.991175144646
-247.916489471732 328.492626444646
-247.878421471732 327.994077744646
-247.840353471732 327.495529044646
-247.802285471732 326.996980344646
-247.764217471732 326.498431644646
-239.197356146667 334.321421217921
-239.212071096667 333.821637817921
-239.226786046667 333.321854417921
-239.241500996667 332.822071017921
-239.256215946667 332.322287617921
-239.270930896667 331.822504217921
-239.285645846667 331.322720817921
-239.300360796667 330.822937417921
-239.315075746667 330.323154017921
-239.329790696667 329.823370617921
-239.344505646667 329.323587217921
-239.359220596667 328.823803817921
-239.373935546667 328.324020417921
-239.388650496667 327.824237017921
-239.403365446667 327.324453617921
-239.418080396667 326.824670217921
-239.432795346667 326.324886817921
-239.447510296667 325.825103417921
-239.462225246667 325.325320017921
-239.476940196667 324.825536617921
-230.07839239072 333.321245965909
-230.12530889072 332.823451965909
-230.17222539072 332.325657965909
-230.21914189072 331.827863965909
-230.26605839072 331.330069965909
-230.31297489072 330.832275965909
-230.35989139072 330.334481965909
-230.40680789072 329.836687965909
-230.45372439072 329.338893965909
-230.50064089072 328.841099965909
-230.54755739072 328.343305965909
-230.59447389072 327.845511965909
-230.64139039072 327.347717965909
-230.68830689072 326.849923965909
-230.73522339072 326.352129965909
-230.78213989072 325.854335965909
-230.82905639072 325.356541965909
-230.87597289072 324.858747965909
-230.92288939072 324.360953965909
-230.96980589072 323.863159965909
-231.01672239072 323.365365965909
-200.431984645119 328.244718019374
-200.515947795119 327.751818269374
-200.599910945119 327.258918519375
-200.683874095119 326.766018769375
-200.767837245119 326.273119019375
-200.851800395119 325.780219269375
-200.935763545119 325.287319519374
-201.019726695119 324.794419769374
-201.103689845119 324.301520019374
-201.187652995119 323.808620269375
-201.271616145119 323.315720519375
-201.355579295119 322.822820769375
-201.439542445119 322.329921019375
-201.523505595119 321.837021269374
-201.607468745119 321.344121519374
-201.691431895119 320.851221769374
-201.775395045119 320.358322019374
-201.859358195119 319.865422269375
-201.943321345119 319.372522519375
-202.027284495119 318.879622769375
-170.836779028555 323.336738526597
-170.947334678555 322.849114226597
-171.057890328555 322.361489926597
-171.168445978555 321.873865626597
-171.279001628555 321.386241326597
-171.389557278555 320.898617026597
-171.500112928555 320.410992726597
-171.610668578555 319.923368426597
-171.721224228555 319.435744126597
-171.831779878555 318.948119826597
-171.942335528555 318.460495526597
-172.052891178555 317.972871226597
-172.163446828555 317.485246926597
-172.274002478555 316.997622626597
-172.384558128555 316.509998326597
-172.495113778555 316.022374026597
-172.605669428555 315.534749726597
-172.716225078555 315.047125426597
-172.826780728555 314.559501126597
-140.58761773771 318.414923101222
-140.76253253771 317.946516401222
-140.93744733771 317.478109701222
-141.11236213771 317.009703001222
-141.28727693771 316.541296301223
-141.46219173771 316.072889601223
-141.63710653771 315.604482901223
-141.81202133771 315.136076201223
-141.98693613771 314.667669501223
-142.16185093771 314.199262801223
-142.33676573771 313.730856101223
-142.51168053771 313.262449401223
-142.68659533771 312.794042701223
-142.86151013771 312.325636001223
-143.03642493771 311.857229301223
-143.21133973771 311.388822601223
-143.38625453771 310.920415901222
-143.56116933771 310.452009201222
-143.73608413771 309.983602501222
-111.305616031182 308.272941445288
-111.545403731182 307.834191095288
-111.785191431182 307.395440745288
-112.024979131182 306.956690395288
-112.264766831182 306.517940045288
-112.504554531182 306.079189695288
-112.744342231182 305.640439345288
-112.984129931182 305.201688995288
-113.223917631182 304.762938645288
-113.463705331182 304.324188295288
-113.703493031182 303.885437945288
-113.943280731182 303.446687595288
-114.183068431182 303.007937245288
-114.422856131182 302.569186895288
-114.662643831182 302.130436545288
-114.902431531182 301.691686195288
-115.142219231182 301.252935845288
-115.382006931182 300.814185495288
-115.621794631182 300.375435145288
-115.861582331182 299.936684795288
-88.38049847 287.2560421
-88.67355452 286.8509271
-88.96661057 286.4458121
-89.25966662 286.0406971
-89.55272267 285.6355821
-89.84577872 285.2304671
-90.13883477 284.8253521
-90.43189082 284.4202371
-90.72494687 284.0151221
-91.01800292 283.6100071
-91.31105897 283.2048921
-91.60411502 282.7997771
-91.89717107 282.3946621
-92.19022712 281.9895471
-92.48328317 281.5844321
-92.77633922 281.1793171
-93.06939527 280.7742021
-93.36245132 280.3690871
-93.65550737 279.9639721
-93.94856342 279.5588571
-66.171091941681 266.885604712332
-66.503272741681 266.511899062332
-66.835453541681 266.138193412332
-67.167634341681 265.764487762332
-67.499815141681 265.390782112332
-67.831995941681 265.017076462332
-68.164176741681 264.643370812332
-68.496357541681 264.269665162332
-68.828538341681 263.895959512332
-69.160719141681 263.522253862332
-69.492899941681 263.148548212332
-69.825080741681 262.774842562332
-70.157261541681 262.401136912332
-70.489442341681 262.027431262332
-70.821623141681 261.653725612332
-71.153803941681 261.280019962332
-71.485984741681 260.906314312332
-71.818165541681 260.532608662332
-72.150346341681 260.158903012332
-72.482527141681 259.785197362332
-44.2190941209642 246.393958938745
-44.5715747709642 246.039336038745
-44.9240554209642 245.684713138745
-45.2765360709642 245.330090238745
-45.6290167209642 244.975467338745
-45.9814973709642 244.620844438745
-46.3339780209642 244.266221538745
-46.6864586709642 243.911598638745
-47.0389393209642 243.556975738745
-47.3914199709642 243.202352838745
-47.7439006209642 242.847729938745
-48.0963812709642 242.493107038745
-48.4488619209642 242.138484138745
-48.8013425709642 241.783861238745
-49.1538232209642 241.429238338745
-49.5063038709642 241.074615438745
-49.8587845209642 240.719992538745
-50.2112651709642 240.365369638745
-50.5637458209642 240.010746738745
-50.9162264709642 239.656123838745
-22.0276812163313 226.08944608524
-22.3851555163313 225.73985758524
-22.7426298163313 225.39026908524
-23.1001041163313 225.04068058524
-23.4575784163313 224.69109208524
-23.8150527163313 224.34150358524
-24.1725270163313 223.99191508524
-24.5300013163313 223.64232658524
-24.8874756163313 223.29273808524
-25.2449499163313 222.94314958524
-25.6024242163313 222.59356108524
-25.9598985163313 222.24397258524
-26.3173728163313 221.89438408524
-26.6748471163313 221.54479558524
-27.0323214163313 221.19520708524
-27.3897957163313 220.84561858524
-27.7472700163313 220.49603008524
-28.1047443163313 220.14644158524
-28.4622186163313 219.79685308524
-28.8196929163313 219.44726458524
0.17003962354202 205.854384046441
-0.18897142645798 205.506373896441
-0.54798247645798 205.158363746441
-0.90699352645798 204.810353596441
-1.26600457645798 204.462343446441
-1.62501562645798 204.114333296441
-1.98402667645798 203.766323146441
-2.34303772645798 203.418312996441
-2.70204877645798 203.070302846441
-3.06105982645798 202.722292696441
-3.42007087645798 202.374282546441
-3.77908192645798 202.026272396441
-4.13809297645798 201.678262246441
-4.49710402645798 201.330252096441
-4.85611507645798 200.982241946441
-5.21512612645798 200.634231796441
-5.57413717645798 200.286221646441
-5.93314822645798 199.938211496441
-6.29215927645798 199.590201346441
-6.65117032645798 199.242191196441
22.3185236069918 185.568149428077
21.9583905569918 185.221300478077
21.5982575069918 184.874451528077
21.2381244569918 184.527602578077
20.8779914069918 184.180753628077
20.5178583569918 183.833904678077
20.1577253069918 183.487055728077
19.7975922569918 183.140206778077
19.4374592069918 182.793357828077
19.0773261569918 182.446508878077
18.7171931069918 182.099659928077
18.3570600569918 181.752810978077
17.9969270069918 181.405962028077
17.6367939569918 181.059113078077
17.2766609069918 180.712264128077
16.9165278569918 180.365415178077
16.5563948069918 180.018566228077
16.1962617569918 179.671717278077
15.8361287069918 179.324868328077
15.4759956569918 178.978019378077
44.2947553724756 165.127872232704
43.9361562224756 164.779437682704
43.5775570724756 164.431003132704
43.2189579224756 164.082568582704
42.8603587724756 163.734134032704
42.5017596224756 163.385699482704
42.1431604724756 163.037264932704
41.7845613224756 162.688830382704
41.4259621724756 162.340395832704
41.0673630224756 161.991961282704
40.7087638724756 161.643526732704
40.3501647224756 161.295092182704
39.9915655724756 160.946657632704
39.6329664224756 160.598223082704
39.2743672724756 160.249788532704
38.9157681224756 159.901353982704
38.5571689724756 159.552919432704
38.1985698224756 159.204484882704
37.8399706724756 158.856050332704
37.4813715224756 158.507615782704
66.1555732055899 144.813892209106
65.8049554555899 144.457427359106
65.4543377055899 144.100962509106
65.10371995559 143.744497659106
64.75310220559 143.388032809106
64.4024844555899 143.031567959106
64.0518667055899 142.675103109106
63.7012489555899 142.318638259106
63.3506312055899 141.962173409106
63.00001345559 141.605708559106
62.6493957055899 141.249243709106
62.2987779555899 140.892778859106
61.94816020559 140.536314009106
61.5975424555899 140.179849159106
61.2469247055899 139.823384309106
60.8963069555899 139.466919459106
60.5456892055899 139.110454609106
60.1950714555899 138.753989759106
59.8444537055899 138.397524909106
59.4938359555899 138.041060059106
87.9539327344448 124.722880743987
87.6163107844448 124.354083443987
87.2786888344448 123.985286143987
86.9410668844448 123.616488843987
86.6034449344448 123.247691543987
86.2658229844448 122.878894243987
85.9282010344448 122.510096943987
85.5905790844448 122.141299643987
85.2529571344448 121.772502343987
84.9153351844448 121.403705043987
84.5777132344448 121.034907743987
84.2400912844448 120.666110443987
83.9024693344448 120.297313143987
83.5648473844448 119.928515843987
83.2272254344448 119.559718543987
82.8896034844448 119.190921243987
82.5519815344448 118.822123943987
82.2143595844448 118.453326643987
81.8767376344448 118.084529343987
81.5391156844448 117.715732043987
110.298710618359 104.615280607871
109.958758068359 104.248630557871
109.618805518359 103.881980507871
109.278852968359 103.515330457871
108.938900418359 103.148680407871
108.598947868359 102.782030357871
108.258995318359 102.415380307871
107.919042768359 102.048730257871
107.579090218359 101.682080207871
107.239137668359 101.315430157871
106.899185118359 100.948780107871
106.559232568359 100.582130057871
106.219280018359 100.215480007871
105.879327468359 99.8488299578706
105.539374918359 99.4821799078706
105.199422368359 99.1155298578706
104.859469818359 98.7488798078706
104.519517268359 98.3822297578706
104.179564718359 98.0155797078706
103.839612168359 97.6489296578706
131.552258974802 84.8701590097299
131.257043574802 84.4666148597299
130.961828174802 84.0630707097299
130.666612774802 83.6595265597299
130.371397374802 83.2559824097299
130.076181974802 82.8524382597299
129.780966574802 82.4488941097299
129.485751174802 82.0453499597299
129.190535774802 81.6418058097299
128.895320374802 81.2382616597299
128.600104974802 80.8347175097299
128.304889574802 80.4311733597299
128.009674174802 80.0276292097299
127.714458774802 79.6240850597299
127.419243374802 79.2205409097299
127.124027974802 78.8169967597299
126.828812574802 78.4134526097299
126.533597174802 78.0099084597299
126.238381774802 77.6063643097299
125.943166374802 77.2028201597299
137.6822505985 78.9303189598792
137.4184183985 78.5055925098792
137.1545861985 78.0808660598792
136.8907539985 77.6561396098792
136.6269217985 77.2314131598792
136.3630895985 76.8066867098792
136.0992573985 76.3819602598792
135.8354251985 75.9572338098792
135.5715929985 75.5325073598792
135.3077607985 75.1077809098792
135.0439285985 74.6830544598792
134.7800963985 74.2583280098792
134.5162641985 73.8336015598792
134.2524319985 73.4088751098792
133.9885997985 72.9841486598792
133.7247675985 72.5594222098792
133.4609353985 72.1346957598792
133.1971031985 71.7099693098792
132.9332709985 71.2852428598792
132.6694387985 70.8605164098792
144.109905682285 72.952565981099
143.879338632285 72.5089007310989
143.648771582285 72.065235481099
143.418204532285 71.621570231099
143.187637482285 71.1779049810989
142.957070432285 70.734239731099
142.726503382285 70.290574481099
142.495936332285 69.8469092310989
142.265369282285 69.403243981099
142.034802232285 68.9595787310989
141.804235182285 68.5159134810989
141.573668132285 68.072248231099
141.343101082285 67.6285829810989
141.112534032285 67.1849177310989
140.881966982285 66.741252481099
140.651399932285 66.2975872310989
140.420832882285 65.8539219810989
140.190265832285 65.410256731099
139.959698782285 64.9665914810989
139.729131732285 64.5229262310989
150.929101035321 66.9510322093478
150.733189085321 66.4910120593478
150.537277135321 66.0309919093478
150.341365185321 65.5709717593478
150.145453235321 65.1109516093478
149.949541285321 64.6509314593478
149.753629335321 64.1909113093478
149.557717385321 63.7308911593478
149.361805435321 63.2708710093478
149.165893485321 62.8108508593478
148.969981535321 62.3508307093478
148.774069585321 61.8908105593478
148.578157635321 61.4307904093478
148.382245685321 60.9707702593478
148.186333735321 60.5107501093478
147.990421785321 60.0507299593478
147.794509835321 59.5907098093478
147.598597885321 59.1306896593478
147.402685935321 58.6706695093478
147.206773985321 58.2106493593478
158.540835322447 61.8936258274158
158.380977422447 61.4198690774158
158.221119522447 60.9461123274158
158.061261622447 60.4723555774158
157.901403722447 59.9985988274158
157.741545822447 59.5248420774158
157.581687922447 59.0510853274158
157.421830022447 58.5773285774158
157.261972122447 58.1035718274158
157.102114222447 57.6298150774158
156.942256322447 57.1560583274158
156.782398422447 56.6823015774158
156.622540522447 56.2085448274158
156.462682622447 55.7347880774158
156.302824722447 55.2610313274158
156.142966822447 54.7872745774158
155.983108922447 54.3135178274158
155.823251022447 53.8397610774158
155.663393122447 53.3660043274158
155.503535222447 52.8922475774158
167.420941088867 60.3093747901648
167.298524738867 59.8245920901648
167.176108388867 59.3398093901648
167.053692038867 58.8550266901648
166.931275688867 58.3702439901648
166.808859338867 57.8854612901648
166.686442988867 57.4006785901648
166.564026638867 56.9158958901648
166.441610288867 56.4311131901648
166.319193938867 55.9463304901648
166.196777588867 55.4615477901648
166.074361238867 54.9767650901648
165.951944888867 54.4919823901648
165.829528538867 54.0071996901648
165.707112188867 53.5224169901648
165.584695838867 53.0376342901648
165.462279488867 52.5528515901648
165.339863138867 52.0680688901648
165.217446788867 51.5832861901648
165.095030438867 51.0985034901648
164.972614088867 50.6137207901648
176.664187601337 61.4293897571094
176.580539201337 60.9364364571094
176.496890801337 60.4434831571094
176.413242401337 59.9505298571094
176.329594001337 59.4575765571094
176.245945601337 58.9646232571094
176.162297201337 58.4716699571094
176.078648801337 57.9787166571094
175.995000401337 57.4857633571094
175.911352001337 56.9928100571094
175.827703601337 56.4998567571094
175.744055201337 56.0069034571094
175.660406801337 55.5139501571094
175.576758401337 55.0209968571094
175.493110001337 54.5280435571094
175.409461601337 54.0350902571094
175.325813201337 53.5421369571094
175.242164801337 53.0491836571094
175.158516401337 52.5562303571094
175.074868001337 52.0632770571094
185.48957805396 62.8375493918338
185.44622545396 62.3394323918338
185.40287285396 61.8413153918338
185.35952025396 61.3431983918338
185.31616765396 60.8450813918338
185.27281505396 60.3469643918338
185.22946245396 59.8488473918338
185.18610985396 59.3507303918338
185.14275725396 58.8526133918338
185.09940465396 58.3544963918338
185.05605205396 57.8563793918338
185.01269945396 57.3582623918338
184.96934685396 56.8601453918338
184.92599425396 56.3620283918338
184.88264165396 55.8639113918338
184.83928905396 55.3657943918338
184.79593645396 54.8676773918338
184.75258385396 54.3695603918338
184.70923125396 53.8714433918338
184.66587865396 53.3733263918338
184.62252605396 52.8752093918338
193.917352701934 63.9851403357542
193.916025401934 63.4851420857542
193.914698101934 62.9851438357542
193.913370801934 62.4851455857542
193.912043501934 61.9851473357542
193.910716201934 61.4851490857542
193.909388901934 60.9851508357542
193.908061601934 60.4851525857542
193.906734301934 59.9851543357542
193.905407001934 59.4851560857542
193.904079701934 58.9851578357543
193.902752401934 58.4851595857542
193.901425101934 57.9851613357542
193.900097801934 57.4851630857542
193.898770501934 56.9851648357542
193.897443201934 56.4851665857542
193.896115901934 55.9851683357542
193.894788601934 55.4851700857542
193.893461301934 54.9851718357542
193.892134001934 54.4851735857542
202.0800591 65.32850746
202.1221476 64.83028206
202.1642361 64.33205666
202.2063246 63.83383126
202.2484131 63.33560586
202.2905016 62.83738046
202.3325901 62.33915506
202.3746786 61.84092966
202.4167671 61.34270426
202.4588556 60.84447886
202.5009441 60.34625346
202.5430326 59.84802806
202.5851211 59.34980266
202.6272096 58.85157726
202.6692981 58.35335186
202.7113866 57.85512646
202.7534751 57.35690106
202.7955636 56.85867566
202.8376521 56.36045026
202.8797406 55.86222486
210.253295715122 66.3490984097875
210.334229415122 65.8556921597875
210.415163115122 65.3622859097875
210.496096815122 64.8688796597875
210.577030515122 64.3754734097875
210.657964215122 63.8820671597875
210.738897915122 63.3886609097875
210.819831615122 62.8952546597875
210.900765315122 62.4018484097875
210.981699015122 61.9084421597875
211.062632715122 61.4150359097875
211.143566415122 60.9216296597875
211.224500115122 60.4282234097875
211.305433815122 59.9348171597875
211.386367515122 59.4414109097875
211.467301215122 58.9480046597875
211.548234915122 58.4545984097875
211.629168615122 57.9611921597875
211.710102315122 57.4677859097875
211.791036015122 56.9743796597875
238.85492942924 70.3400372414483
239.01796402924 69.8673642914483
239.18099862924 69.3946913414483
239.34403322924 68.9220183914483
239.50706782924 68.4493454414483
239.67010242924 67.9766724914483
239.83313702924 67.5039995414483
239.99617162924 67.0313265914483
240.15920622924 66.5586536414483
240.32224082924 66.0859806914483
240.48527542924 65.6133077414483
240.64831002924 65.1406347914483
240.81134462924 64.6679618414483
240.97437922924 64.1952888914483
241.13741382924 63.7226159414483
241.30044842924 63.2499429914483
241.46348302924 62.7772700414483
241.62651762924 62.3045970914483
241.78955222924 61.8319241414483
241.95258682924 61.3592511914483
269.062130859088 74.7852112969529
269.170862609088 74.2971770469529
269.279594359088 73.8091427969529
269.388326109088 73.3211085469529
269.497057859088 72.8330742969528
269.605789609088 72.3450400469528
269.714521359088 71.8570057969528
269.823253109088 71.3689715469528
269.931984859088 70.8809372969529
270.040716609088 70.3929030469529
270.149448359088 69.9048687969529
270.258180109088 69.4168345469529
270.366911859088 68.9288002969529
270.475643609088 68.4407660469528
270.584375359088 67.9527317969528
270.693107109088 67.4646975469528
270.801838859088 66.9766632969529
270.910570609088 66.4886290469529
271.019302359088 66.0005947969529
271.128034109088 65.5125605469529
277.980771401385 76.3289255904152
278.042604101385 75.8327635904152
278.104436801385 75.3366015904152
278.166269501385 74.8404395904152
278.228102201385 74.3442775904152
278.289934901385 73.8481155904152
278.351767601385 73.3519535904152
278.413600301385 72.8557915904152
278.475433001385 72.3596295904152
278.537265701385 71.8634675904152
278.599098401385 71.3673055904152
278.660931101385 70.8711435904152
278.722763801385 70.3749815904152
278.784596501385 69.8788195904152
278.846429201385 69.3826575904152
278.908261901385 68.8864955904152
278.970094601385 68.3903335904152
279.031927301385 67.8941715904152
279.093760001385 67.3980095904152
279.155592701385 66.9018475904152
287.024526117414 77.51899875804
287.037272667414 77.01916125804
287.050019217414 76.51932375804
287.062765767414 76.01948625804
287.075512317414 75.51964875804
287.088258867414 75.01981125804
287.101005417414 74.51997375804
287.113751967414 74.02013625804
287.126498517414 73.52029875804
287.139245067414 73.02046125804
287.151991617414 72.52062375804
287.164738167414 72.02078625804
287.177484717414 71.52094875804
287.190231267414 71.02111125804
287.202977817414 70.52127375804
287.215724367414 70.02143625804
287.228470917414 69.52159875804
287.241217467414 69.02176125804
287.253964017414 68.52192375804
287.266710567414 68.02208625804
296.285397062368 78.790073133122
296.246951712368 78.291553383122
296.208506362368 77.793033633122
296.170061012368 77.294513883122
296.131615662368 76.795994133122
296.093170312368 76.297474383122
296.054724962368 75.798954633122
296.016279612368 75.300434883122
295.977834262368 74.801915133122
295.939388912368 74.303395383122
295.900943562368 73.804875633122
295.862498212368 73.306355883122
295.824052862368 72.807836133122
295.785607512368 72.309316383122
295.747162162368 71.810796633122
295.708716812368 71.312276883122
295.670271462368 70.813757133122
295.631826112368 70.315237383122
295.593380762368 69.816717633122
295.554935412368 69.318197883122
305.895364518415 79.5541243408225
305.803523868415 79.0626313908225
305.711683218415 78.5711384408225
305.619842568415 78.0796454908225
305.528001918415 77.5881525408225
305.436161268415 77.0966595908225
305.344320618415 76.6051666408225
305.252479968415 76.1136736908225
305.160639318415 75.6221807408225
305.068798668415 75.1306877908225
304.976958018415 74.6391948408225
304.885117368415 74.1477018908225
304.793276718415 73.6562089408225
304.701436068415 73.1647159908225
304.609595418415 72.6732230408225
304.517754768415 72.1817300908225
304.425914118415 71.6902371408225
304.334073468415 71.1987441908225
304.242232818415 70.7072512408225
304.150392168415 70.2157582908225
315.637030530082 78.7166837875511
315.490033230082 78.2387802375511
315.343035930082 77.7608766875511
315.196038630082 77.2829731375511
315.049041330082 76.8050695875511
314.902044030082 76.3271660375511
314.755046730082 75.8492624875511
314.608049430082 75.3713589375511
314.461052130082 74.8934553875511
314.314054830082 74.4155518375511
314.167057530082 73.9376482875511
314.020060230082 73.4597447375511
313.873062930082 72.9818411875511
313.726065630082 72.5039376375511
313.579068330082 72.0260340875511
313.432071030082 71.5481305375511
313.285073730082 71.0702269875511
313.138076430082 70.5923234375511
312.991079130082 70.1144198875511
312.844081830082 69.6365163375511
325.402682291208 76.6663495670234
325.199763791208 76.2093768170234
324.996845291208 75.7524040670234
324.793926791208 75.2954313170234
324.591008291208 74.8384585670234
324.388089791208 74.3814858170234
324.185171291208 73.9245130670234
323.982252791208 73.4675403170234
323.779334291208 73.0105675670234
323.576415791208 72.5535948170234
323.373497291208 72.0966220670234
323.170578791208 71.6396493170234
322.967660291208 71.1826765670234
322.764741791208 70.7257038170234
322.561823291208 70.2687310670234
322.358904791208 69.8117583170234
322.155986291208 69.3547855670234
321.953067791208 68.8978128170234
321.750149291208 68.4408400670234
321.547230791208 67.9838673170234
334.501957202755 72.45497493461
334.242381202755 72.0276339846099
333.982805202755 71.6002930346099
333.723229202755 71.1729520846099
333.463653202755 70.7456111346099
333.204077202755 70.3182701846099
332.944501202755 69.8909292346099
332.684925202755 69.4635882846099
332.425349202755 69.03624733461
332.165773202755 68.60890638461
331.906197202755 68.18156543461
331.646621202755 67.7542244846099
331.387045202755 67.3268835346099
331.127469202755 66.8995425846099
330.867893202755 66.4722016346099
330.608317202755 66.0448606846099
330.348741202755 65.6175197346099
330.089165202755 65.1901787846099
329.829589202755 64.76283783461
329.570013202755 64.33549688461
343.054336778755 67.0070948469335
342.738137228756 66.6197734969335
342.421937678756 66.2324521469335
342.105738128756 65.8451307969335
341.789538578756 65.4578094469335
341.473339028756 65.0704880969335
341.157139478756 64.6831667469335
340.840939928756 64.2958453969335
340.524740378756 63.9085240469335
340.208540828756 63.5212026969335
339.892341278756 63.1338813469335
339.576141728756 62.7465599969335
339.259942178756 62.3592386469335
338.943742628756 61.9719172969335
338.627543078756 61.5845959469335
338.311343528756 61.1972745969335
337.995143978756 60.8099532469335
337.678944428756 60.4226318969335
337.362744878756 60.0353105469335
337.046545328756 59.6479891969335
350.485687594669 59.9645137371982
350.115712294669 59.6281831371982
349.745736994669 59.2918525371982
349.375761694669 58.9555219371982
349.005786394669 58.6191913371982
348.635811094669 58.2828607371982
348.265835794669 57.9465301371982
347.895860494669 57.6101995371982
347.525885194669 57.2738689371982
347.155909894669 56.9375383371982
346.785934594669 56.6012077371982
346.415959294669 56.2648771371982
346.045983994669 55.9285465371982
345.676008694669 55.5922159371982
345.306033394669 55.2558853371982
344.936058094669 54.9195547371982
344.566082794669 54.5832241371982
344.196107494669 54.2468935371982
343.826132194669 53.9105629371982
356.820329149639 51.9654872241304
356.407166199639 51.6838911241304
355.994003249639 51.4022950241304
355.580840299639 51.1206989241304
355.167677349639 50.8391028241304
354.754514399639 50.5575067241304
354.341351449639 50.2759106241304
353.928188499639 49.9943145241304
353.515025549639 49.7127184241304
353.101862599639 49.4311223241304
352.688699649639 49.1495262241304
352.275536699639 48.8679301241304
351.862373749639 48.5863340241304
351.449210799639 48.3047379241304
351.036047849639 48.0231418241304
350.622884899639 47.7415457241304
350.209721949639 47.4599496241304
349.796558999639 47.1783535241304
349.383396049639 46.8967574241304
348.970233099639 46.6151613241304
361.543750565182 42.9898954907515
361.097680365182 42.7640163407515
360.651610165182 42.5381371907515
360.205539965182 42.3122580407515
359.759469765182 42.0863788907515
359.313399565182 41.8604997407515
358.867329365182 41.6346205907515
358.421259165182 41.4087414407515
357.975188965182 41.1828622907515
357.529118765182 40.9569831407515
357.083048565182 40.7311039907515
356.636978365182 40.5052248407515
356.190908165182 40.2793456907515
355.744837965182 40.0534665407515
355.298767765182 39.8275873907515
354.852697565182 39.6017082407515
354.406627365182 39.3758290907515
353.960557165182 39.1499499407515
353.514486965182 38.9240707907515
353.068416765182 38.6981916407515
365.030019330575 33.57354636904
364.559605330575 33.40410416904
364.089191330575 33.23466196904
363.618777330575 33.06521976904
363.148363330575 32.89577756904
362.677949330575 32.72633536904
362.207535330575 32.55689316904
361.737121330575 32.38745096904
361.266707330575 32.21800876904
360.796293330575 32.04856656904
360.325879330575 31.87912436904
359.855465330575 31.70968216904
359.385051330575 31.54023996904
358.914637330575 31.37079776904
358.444223330575 31.20135556904
357.973809330575 31.03191336904
357.503395330575 30.86247116904
357.032981330575 30.69302896904
356.562567330575 30.52358676904
356.092153330575 30.35414456904
366.356577683826 23.7063531447758
365.869331533826 23.5941427947758
365.382085383826 23.4819324447759
364.894839233826 23.3697220947758
364.407593083826 23.2575117447759
363.920346933826 23.1453013947758
363.433100783826 23.0330910447759
362.945854633826 22.9208806947758
362.458608483826 22.8086703447759
361.971362333826 22.6964599947759
361.484116183826 22.5842496447758
360.996870033826 22.4720392947759
360.509623883826 22.3598289447758
360.022377733826 22.2476185947759
359.535131583826 22.1354082447758
359.047885433826 22.0231978947759
358.560639283826 21.9109875447758
358.073393133826 21.7987771947759
357.586146983826 21.6865668447759
357.098900833826 21.5743564947758
366.100330927486 13.9994246306477
365.604082827486 13.9382867806477
365.107834727486 13.8771489306477
364.611586627486 13.8160110806477
364.115338527486 13.7548732306477
363.619090427486 13.6937353806477
363.122842327486 13.6325975306477
362.626594227486 13.5714596806477
362.130346127486 13.5103218306477
361.634098027486 13.4491839806477
361.137849927486 13.3880461306477
360.641601827486 13.3269082806477
360.145353727486 13.2657704306477
359.649105627486 13.2046325806477
359.152857527486 13.1434947306477
358.656609427486 13.0823568806477
358.160361327486 13.0212190306477
357.664113227486 12.9600811806477
357.167865127486 12.8989433306477
356.671617027486 12.8378054806477
364.976005671279 4.6115907675806
364.476395771279 4.5918437675806
363.976785871279 4.5720967675806
363.477175971279 4.5523497675806
362.977566071279 4.5326027675806
362.477956171279 4.5128557675806
361.978346271279 4.4931087675806
361.478736371279 4.4733617675806
360.979126471279 4.4536147675806
360.479516571279 4.4338677675806
359.979906671279 4.4141207675806
359.480296771279 4.3943737675806
358.980686871279 4.3746267675806
358.481076971279 4.3548797675806
357.981467071279 4.3351327675806
357.481857171279 4.3153857675806
356.982247271279 4.2956387675806
356.482637371279 4.2758917675806
355.983027471279 4.2561447675806
355.483417571279 4.2363977675806
364.160143606405 -4.53740955731017
363.660278356405 -4.52580270731017
363.160413106405 -4.51419585731017
362.660547856405 -4.50258900731017
362.160682606405 -4.49098215731017
361.660817356405 -4.47937530731017
361.160952106405 -4.46776845731017
360.661086856405 -4.45616160731017
360.161221606405 -4.44455475731017
359.661356356405 -4.43294790731017
359.161491106405 -4.42134105731017
358.661625856405 -4.40973420731017
358.161760606405 -4.39812735731017
357.661895356405 -4.38652050731017
357.162030106405 -4.37491365731017
356.662164856405 -4.36330680731017
356.162299606405 -4.35169995731017
355.662434356405 -4.34009310731017
355.162569106405 -4.32848625731017
354.662703856405 -4.31687940731017
360.228269226936 -34.4022135428782
359.731979426936 -34.3414154428782
359.235689626936 -34.2806173428782
358.739399826936 -34.2198192428782
358.243110026936 -34.1590211428782
357.746820226936 -34.0982230428782
357.250530426936 -34.0374249428782
356.754240626936 -33.9766268428782
356.257950826936 -33.9158287428782
355.761661026936 -33.8550306428782
355.265371226936 -33.7942325428782
354.769081426936 -33.7334344428782
354.272791626936 -33.6726363428782
353.776501826936 -33.6118382428782
353.280212026936 -33.5510401428782
352.783922226936 -33.4902420428782
352.287632426936 -33.4294439428782
351.791342626936 -33.3686458428782
351.295052826936 -33.3078477428782
356.887395661852 -64.1941705865344
356.390938261852 -64.1347561865344
355.894480861852 -64.0753417865344
355.398023461852 -64.0159273865344
354.901566061852 -63.9565129865344
354.405108661852 -63.8970985865344
353.908651261852 -63.8376841865344
353.412193861852 -63.7782697865344
352.915736461852 -63.7188553865344
352.419279061852 -63.6594409865344
351.922821661852 -63.6000265865344
351.426364261852 -63.5406121865344
350.929906861852 -63.4811977865344
350.433449461852 -63.4217833865344
349.936992061852 -63.3623689865344
349.440534661852 -63.3029545865344
348.944077261852 -63.2435401865344
348.447619861852 -63.1841257865344
347.951162461852 -63.1247113865344
347.454705061852 -63.0652969865344
353.099793436261 -93.9598623674527
352.603319086261 -93.9005901174527
352.106844736261 -93.8413178674527
351.610370386261 -93.7820456174527
351.113896036261 -93.7227733674527
350.617421686261 -93.6635011174527
350.120947336261 -93.6042288674527
349.624472986261 -93.5449566174527
349.127998636261 -93.4856843674527
348.631524286261 -93.4264121174527
348.135049936261 -93.3671398674527
347.638575586261 -93.3078676174527
347.142101236261 -93.2485953674527
346.645626886261 -93.1893231174527
346.149152536261 -93.1300508674527
345.652678186261 -93.0707786174527
345.156203836261 -93.0115063674527
344.659729486261 -92.9522341174527
344.163255136261 -92.8929618674527
343.666780786261 -92.8336896174527
349.677185328163 -123.724041282439
349.180709028163 -123.664785082439
348.684232728163 -123.605528882439
348.187756428163 -123.546272682439
347.691280128163 -123.487016482439
347.194803828163 -123.427760282439
346.698327528163 -123.368504082439
346.201851228163 -123.309247882439
345.705374928163 -123.249991682439
345.208898628163 -123.190735482439
344.712422328163 -123.131479282439
344.215946028163 -123.072223082439
343.719469728163 -123.012966882439
343.222993428163 -122.953710682439
342.726517128163 -122.894454482439
342.230040828163 -122.835198282439
341.733564528163 -122.775942082439
341.237088228163 -122.716685882439
345.937579448675 -153.482527603975
345.440687598675 -153.426863503975
344.943795748675 -153.371199403975
344.446903898675 -153.315535303975
343.950012048675 -153.259871203975
343.453120198675 -153.204207103975
342.956228348675 -153.148543003975
342.459336498675 -153.092878903975
341.962444648675 -153.037214803975
341.465552798675 -152.981550703975
340.968660948675 -152.925886603975
340.471769098675 -152.870222503975
339.974877248675 -152.814558403975
342.5490179 -183.35696065
342.0581559 -183.2618054
341.5672939 -183.16665015
341.0764319 -183.0714949
340.5855699 -182.97633965
340.0947079 -182.8811844
339.6038459 -182.78602915
339.1129839 -182.6908739
338.6221219 -182.59571865
338.1312599 -182.5005634
337.6403979 -182.40540815
337.1495359 -182.3102529
336.6586739 -182.21509765
336.1678119 -182.1199424
335.6769499 -182.02478715
335.1860879 -181.9296319
341.459312899886 -192.398307377297
340.977484849886 -192.264734477297
340.495656799886 -192.131161577297
340.013828749886 -191.997588677297
339.532000699886 -191.864015777297
339.050172649886 -191.730442877297
338.568344599886 -191.596869977297
338.086516549886 -191.463297077297
337.604688499886 -191.329724177297
337.122860449886 -191.196151277297
336.641032399886 -191.062578377297
336.159204349886 -190.929005477297
335.677376299886 -190.795432577297
335.195548249886 -190.661859677297
334.713720199886 -190.528286777297
334.231892149886 -190.394713877297
333.750064099886 -190.261140977297
339.864444389768 -201.599747992258
339.399535939768 -201.415736792258
338.934627489768 -201.231725592258
338.469719039768 -201.047714392258
338.004810589768 -200.863703192258
337.539902139768 -200.679691992258
337.074993689768 -200.495680792258
336.610085239768 -200.311669592258
336.145176789768 -200.127658392258
335.680268339768 -199.943647192258
335.215359889768 -199.759635992258
334.750451439768 -199.575624792258
334.285542989768 -199.391613592258
333.820634539768 -199.207602392258
333.355726089768 -199.023591192258
332.890817639768 -198.839579992258
332.425909189768 -198.655568792258
331.961000739768 -198.471557592258
338.620464912885 -211.768586326081
338.188344512885 -211.517047126081
337.756224112885 -211.265507926081
337.324103712885 -211.013968726081
336.891983312885 -210.762429526081
336.459862912885 -210.510890326081
336.027742512885 -210.259351126081
335.595622112885 -210.007811926081
335.163501712885 -209.756272726081
334.731381312885 -209.504733526081
334.299260912885 -209.253194326081
333.867140512885 -209.001655126081
333.435020112885 -208.750115926081
333.002899712885 -208.498576726081
332.570779312885 -208.247037526081
332.138658912885 -207.995498326081
331.706538512885 -207.743959126081
331.274418112885 -207.492419926081
330.842297712885 -207.240880726081
330.410177312885 -206.989341526081
329.978056912885 -206.737802326081
329.545936512885 -206.486263126081
334.09162688 -221.34126301
333.71742908 -221.00963666
333.34323128 -220.67801031
332.96903348 -220.34638396
332.59483568 -220.01475761
332.22063788 -219.68313126
331.84644008 -219.35150491
331.47224228 -219.01987856
331.09804448 -218.68825221
330.72384668 -218.35662586
330.34964888 -218.02499951
329.97545108 -217.69337316
329.60125328 -217.36174681
329.22705548 -217.03012046
328.85285768 -216.69849411
328.47865988 -216.36686776
328.10446208 -216.03524141
327.73026428 -215.70361506
327.35606648 -215.37198871
326.98186868 -215.04036236
326.60767088 -214.70873601
326.23347308 -214.37710966
326.81812678371 -229.387946670167
326.51904638371 -228.987258620167
326.21996598371 -228.586570570167
325.92088558371 -228.185882520167
325.62180518371 -227.785194470167
325.32272478371 -227.384506420167
325.02364438371 -226.983818370167
324.72456398371 -226.583130320167
324.42548358371 -226.182442270167
324.12640318371 -225.781754220167
323.82732278371 -225.381066170167
323.52824238371 -224.980378120167
323.22916198371 -224.579690070167
322.93008158371 -224.179002020167
322.63100118371 -223.778313970167
322.33192078371 -223.377625920167
322.03284038371 -222.976937870167
321.73375998371 -222.576249820167
321.43467958371 -222.175561770167
321.13559918371 -221.774873720167
320.83651878371 -221.374185670167
317.847487 -235.88858774
317.637206 -235.43495584
317.426925 -234.98132394
317.216644 -234.52769204
317.006363 -234.07406014
316.796082 -233.62042824
316.585801 -233.16679634
316.37552 -232.71316444
316.165239 -232.25953254
315.954958 -231.80590064
315.744677 -231.35226874
315.534396 -230.89863684
315.324115 -230.44500494
315.113834 -229.99137304
314.903553 -229.53774114
314.693272 -229.08410924
314.482991 -228.63047734
314.27271 -228.17684544
314.062429 -227.72321354
313.852148 -227.26958164
313.641867 -226.81594974
313.431586 -226.36231784
307.380601154546 -239.50587506884
307.266045054546 -239.01917506884
307.151488954546 -238.53247506884
307.036932854546 -238.04577506884
306.922376754546 -237.55907506884
306.807820654546 -237.07237506884
306.693264554546 -236.58567506884
306.578708454546 -236.09897506884
306.464152354546 -235.61227506884
306.349596254546 -235.12557506884
306.235040154546 -234.63887506884
306.120484054546 -234.15217506884
306.005927954546 -233.66547506884
305.891371854546 -233.17877506884
305.776815754546 -232.69207506884
305.662259654546 -232.20537506884
305.547703554546 -231.71867506884
305.433147454546 -231.23197506884
305.318591354546 -230.74527506884
305.204035254546 -230.25857506884
305.089479154546 -229.77187506884
304.974923054546 -229.28517506884
296.43059338 -240.43728412
296.41546933 -239.93751292
296.40034528 -239.43774172
296.38522123 -238.93797052
296.37009718 -238.43819932
296.35497313 -237.93842812
296.33984908 -237.43865692
296.32472503 -236.93888572
296.30960098 -236.43911452
296.29447693 -235.93934332
296.27935288 -235.43957212
296.26422883 -234.93980092
296.24910478 -234.44002972
296.23398073 -233.94025852
296.21885668 -233.44048732
296.20373263 -232.94071612
296.18860858 -232.44094492
296.17348453 -231.94117372
296.15836048 -231.44140252
296.14323643 -230.94163132
296.12811238 -230.44186012
296.11298833 -229.94208892
296.09786428 -229.44231772
285.978674662639 -238.348869014865
286.051139962639 -237.854148114865
286.123605262638 -237.359427214865
286.196070562639 -236.864706314865
286.268535862638 -236.369985414865
286.341001162639 -235.875264514865
286.413466462638 -235.380543614865
286.485931762639 -234.885822714865
286.558397062639 -234.391101814865
286.630862362638 -233.896380914865
286.703327662639 -233.401660014865
286.775792962638 -232.906939114865
286.848258262639 -232.412218214865
286.920723562638 -231.917497314865
286.993188862638 -231.422776414865
287.065654162639 -230.928055514865
287.138119462638 -230.433334614865
287.210584762639 -229.938613714865
287.283050062638 -229.443892814865
287.355515362639 -228.949171914865
287.427980662639 -228.454451014865
287.500445962638 -227.959730114865
287.572911262639 -227.465009214865
276.732983116108 -233.850123195605
276.873991366108 -233.370418395605
277.014999616108 -232.890713595605
277.156007866108 -232.411008795605
277.297016116108 -231.931303995605
277.438024366108 -231.451599195605
277.579032616108 -230.971894395605
277.720040866108 -230.492189595605
277.861049116108 -230.012484795605
278.002057366108 -229.532779995605
278.143065616108 -229.053075195605
278.284073866108 -228.573370395605
278.425082116108 -228.093665595605
278.566090366108 -227.613960795605
278.707098616108 -227.134255995605
278.848106866108 -226.654551195605
278.989115116108 -226.174846395605
279.130123366108 -225.695141595605
279.271131616108 -225.215436795605
279.412139866108 -224.735731995605
279.553148116108 -224.256027195605
279.694156366108 -223.776322395605
268.378743623341 -228.948501717087
268.567712173341 -228.485586067087
268.756680723341 -228.022670417087
268.945649273341 -227.559754767087
269.134617823341 -227.096839117087
269.323586373341 -226.633923467087
269.512554923341 -226.171007817087
269.701523473341 -225.708092167087
269.890492023341 -225.245176517087
270.079460573341 -224.782260867087
270.268429123341 -224.319345217087
270.457397673341 -223.856429567087
270.646366223341 -223.393513917087
270.835334773341 -222.930598267087
271.024303323341 -222.467682617087
271.213271873341 -222.004766967087
271.402240423341 -221.541851317087
271.591208973341 -221.078935667087
271.780177523341 -220.616020017087
271.969146073341 -220.153104367087
272.158114623341 -219.690188717087
272.347083173341 -219.227273067087
272.536051723341 -218.764357417087
260.5362362 -223.89788425
260.7526992 -223.4471695
260.9691622 -222.99645475
261.1856252 -222.54574
261.4020882 -222.09502525
261.6185512 -221.6443105
261.8350142 -221.19359575
262.0514772 -220.742881
262.2679402 -220.29216625
262.4844032 -219.8414515
262.7008662 -219.39073675
262.9173292 -218.940022
263.1337922 -218.48930725
263.3502552 -218.0385925
263.5667182 -217.58787775
263.7831812 -217.137163
263.9996442 -216.68644825
264.2161072 -216.2357335
264.4325702 -215.78501875
264.6490332 -215.334304
264.8654962 -214.88358925
265.0819592 -214.4328745
265.2984222 -213.98215975
235.57422251168 -206.809604498743
235.84427721168 -206.388807098743
236.11433191168 -205.968009698743
236.38438661168 -205.547212298743
236.65444131168 -205.126414898743
236.92449601168 -204.705617498743
237.19455071168 -204.284820098743
237.46460541168 -203.864022698743
237.73466011168 -203.443225298743
238.00471481168 -203.022427898743
238.27476951168 -202.601630498743
238.54482421168 -202.180833098743
238.81487891168 -201.760035698743
239.08493361168 -201.339238298743
239.35498831168 -200.918440898743
239.62504301168 -200.497643498743
239.89509771168 -200.076846098743
240.16515241168 -199.656048698743
240.43520711168 -199.235251298743
240.70526181168 -198.814453898743
240.97531651168 -198.393656498743
241.24537121168 -197.972859098743
241.51542591168 -197.552061698743
210.624480422329 -190.158143478173
210.90503327233 -189.744271378173
211.18558612233 -189.330399278173
211.46613897233 -188.916527178173
211.74669182233 -188.502655078173
212.02724467233 -188.088782978173
212.30779752233 -187.674910878173
212.58835037233 -187.261038778173
212.86890322233 -186.847166678173
213.14945607233 -186.433294578173
213.43000892233 -186.019422478173
213.710561772329 -185.605550378173
213.99111462233 -185.191678278173
214.27166747233 -184.777806178173
214.55222032233 -184.363934078173
214.832773172329 -183.950061978173
215.11332602233 -183.536189878173
215.39387887233 -183.122317778173
215.67443172233 -182.708445678173
215.95498457233 -182.294573578173
216.23553742233 -181.880701478173
216.51609027233 -181.466829378173
216.796643122329 -181.052957278173
185.578785901757 -173.671318669997
185.856748151757 -173.255702269997
186.134710401757 -172.840085869997
186.412672651757 -172.424469469997
186.690634901757 -172.008853069997
186.968597151757 -171.593236669997
187.246559401757 -171.177620269997
187.524521651757 -170.762003869997
187.802483901757 -170.346387469997
188.080446151757 -169.930771069997
188.358408401757 -169.515154669997
188.636370651757 -169.099538269997
188.914332901757 -168.683921869997
189.192295151757 -168.268305469997
189.470257401757 -167.852689069997
189.748219651757 -167.437072669997
190.026181901757 -167.021456269997
190.304144151757 -166.605839869997
190.582106401757 -166.190223469997
190.860068651757 -165.774607069997
191.138030901757 -165.358990669997
191.415993151757 -164.943374269997
191.693955401757 -164.527757869997
160.461066867805 -157.291399742343
160.739067517805 -156.875808992343
161.017068167805 -156.460218242343
161.295068817805 -156.044627492343
161.573069467805 -155.629036742343
161.851070117805 -155.213445992343
162.129070767805 -154.797855242343
162.407071417805 -154.382264492343
162.685072067805 -153.966673742343
162.963072717805 -153.551082992343
163.241073367805 -153.135492242343
163.519074017805 -152.719901492343
163.797074667805 -152.304310742343
164.075075317805 -151.888719992343
164.353075967805 -151.473129242343
164.631076617805 -151.057538492343
164.909077267805 -150.641947742343
165.187077917805 -150.226356992343
165.465078567805 -149.810766242343
165.743079217805 -149.395175492343
166.021079867805 -148.979584742343
166.299080517805 -148.563993992343
166.577081167805 -148.148403242343
135.54823248 -140.60014206
135.82601493 -140.18440546
136.10379738 -139.76866886
136.38157983 -139.35293226
136.65936228 -138.93719566
136.93714473 -138.52145906
137.21492718 -138.10572246
137.49270963 -137.68998586
137.77049208 -137.27424926
138.04827453 -136.85851266
138.32605698 -136.44277606
138.60383943 -136.02703946
138.88162188 -135.61130286
139.15940433 -135.19556626
139.43718678 -134.77982966
139.71496923 -134.36409306
139.99275168 -133.94835646
140.27053413 -133.53261986
140.54831658 -133.11688326
140.82609903 -132.70114666
141.10388148 -132.28541006
141.38166393 -131.86967346
141.65944638 -131.45393686
110.603542236609 -123.956707039106
110.880883186609 -123.540675789106
111.158224136609 -123.124644539106
111.435565086609 -122.708613289106
111.712906036609 -122.292582039106
111.990246986609 -121.876550789106
112.267587936609 -121.460519539106
112.544928886609 -121.044488289106
112.822269836609 -120.628457039106
113.099610786609 -120.212425789106
113.376951736609 -119.796394539106
113.654292686609 -119.380363289106
113.931633636609 -118.964332039106
114.208974586609 -118.548300789106
114.486315536609 -118.132269539106
114.763656486609 -117.716238289106
115.040997436609 -117.300207039106
115.318338386609 -116.884175789106
115.595679336609 -116.468144539106
115.873020286609 -116.052113289106
116.150361236609 -115.636082039106
116.427702186609 -115.220050789106
116.705043136609 -114.804019539106
85.6448477903712 -107.335812634054
85.9218377403712 -106.919547634054
86.1988276903712 -106.503282634054
86.4758176403712 -106.087017634054
86.7528075903712 -105.670752634054
87.0297975403712 -105.254487634054
87.3067874903712 -104.838222634054
87.5837774403712 -104.421957634054
87.8607673903712 -104.005692634054
88.1377573403712 -103.589427634054
88.4147472903712 -103.173162634054
88.6917372403712 -102.756897634054
88.9687271903712 -102.340632634054
89.2457171403712 -101.924367634054
89.5227070903712 -101.508102634054
89.7996970403712 -101.091837634054
90.0766869903712 -100.675572634054
90.3536769403712 -100.259307634054
90.6306668903712 -99.843042634054
90.9076568403712 -99.426777634054
91.1846467903712 -99.010512634054
91.4616367403712 -98.594247634054
91.7386266903712 -98.177982634054
60.6770553502117 -90.7293567744541
60.9538447502117 -90.3129583744541
61.2306341502117 -89.8965599744541
61.5074235502117 -89.4801615744541
61.7842129502117 -89.0637631744541
62.0610023502117 -88.6473647744541
62.3377917502117 -88.2309663744541
62.6145811502117 -87.8145679744541
62.8913705502117 -87.3981695744541
63.1681599502117 -86.9817711744541
63.4449493502117 -86.5653727744541
63.7217387502117 -86.1489743744541
63.9985281502117 -85.7325759744541
64.2753175502117 -85.3161775744541
64.5521069502117 -84.8997791744541
64.8288963502117 -84.4833807744541
65.1056857502117 -84.0669823744541
65.3824751502117 -83.6505839744541
65.6592645502117 -83.2341855744541
65.9360539502117 -82.8177871744541
66.2128433502117 -82.4013887744541
66.4896327502117 -81.9849903744541
66.7664221502117 -81.5685919744541
35.7046765844827 -74.1299019835669
35.9814160344827 -73.7134703835669
36.2581554844827 -73.2970387835669
36.5348949344827 -72.8806071835669
36.8116343844827 -72.4641755835669
37.0883738344827 -72.0477439835669
37.3651132844827 -71.6313123835669
37.6418527344827 -71.2148807835669
37.9185921844827 -70.7984491835669
38.1953316344827 -70.3820175835669
38.4720710844827 -69.9655859835669
38.7488105344827 -69.5491543835669
39.0255499844827 -69.1327227835669
39.3022894344827 -68.7162911835669
39.5790288844827 -68.2998595835669
39.8557683344827 -67.8834279835669
40.1325077844827 -67.4669963835669
40.4092472344827 -67.0505647835669
40.6859866844827 -66.6341331835669
40.9627261344827 -66.2177015835669
41.2394655844827 -65.8012699835669
41.5162050344827 -65.3848383835669
41.7929444844827 -64.9684067835669
10.7322114652489 -57.5300351430109
11.0090516152489 -57.1136704930109
11.2858917652489 -56.6973058430109
11.5627319152489 -56.2809411930109
11.8395720652489 -55.8645765430109
12.1164122152489 -55.4482118930109
12.3932523652489 -55.0318472430109
12.6700925152489 -54.6154825930109
12.9469326652489 -54.1991179430109
13.2237728152489 -53.7827532930109
13.5006129652489 -53.3663886430109
13.7774531152489 -52.9500239930109
14.0542932652489 -52.5336593430109
14.3311334152489 -52.1172946930109
14.6079735652489 -51.7009300430109
14.8848137152489 -51.2845653930109
15.1616538652489 -50.8682007430109
15.4384940152489 -50.4518360930109
15.7153341652489 -50.0354714430109
15.9921743152489 -49.6191067930109
16.2690144652489 -49.2027421430109
16.5458546152489 -48.7863774930109
16.8226947652489 -48.3700128430109
};


==> ressources/solver_benchmark/scenario/scenario_SQPvsNLP.tex <==
% This file was created by tikzplotlib v0.9.1.
%
\definecolor{TUMred}{RGB}{227,114,34}%
\definecolor{TUMgray}{rgb}{0.5977,0.5977,0.5977}
\definecolor{TUMgrayLight}{rgb}{0.8516,0.8398,0.7929}
\definecolor{TUMblue}{RGB}{0,101,189}%
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\def\xmin_varFric{-550.0}
\def\xmax_varFric{-325.0}
\def\ymin_varFric{150.0}
\def\ymax_varFric{375.0}
%
%
%
\begin{tikzpicture}
\begin{axis}[
width=0.7\columnwidth,
%height=2cm,
%xmajorgrids,
xmin=\xmin_varFric,
xmax=\xmax_varFric,
ymin=\ymin_varFric,
ymax=\ymax_varFric,
tick align=outside,
xtick style={color=black},
x grid style={white!69.0!black},
y grid style={white!69.0!black},
axis equal,
xtick pos=left,
ytick pos=left
]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Scenario high mu
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Bounds
\input{ressources/solver_benchmark/scenario/bounds.tex}
\addlegendentry{Bounds}
% Nodes
\input{ressources/solver_benchmark/scenario/nodes.tex}
\addlegendentry{Nodes}
%\draw[draw=color7,fill=color7] (axis cs:161.017068167805,-156.460218242343) circle (2);
% Ego-Vehicle
\addplot [semithick, black, mark=*, mark size=3, mark options={solid}, only marks, forget plot]
table {%
	188.367574290479 -174.868489956856
};
%
% Raceline
%\input{ressources/solver_benchmark/scenario/raceline.tex}
%\addlegendentry{To be chosen Path!}
%
% Chosen Path
\input{ressources/solver_benchmark/scenario/chosen_path.tex}
\end{axis}
\end{tikzpicture}


==> ressources/variable_friction/bounds.tex <==
\addplot [line width=0.56pt, black]
table {%
	5.29929318275232 -38.6274835696298
	-19.7530013951774 -22.1576063162077
	-44.7455028561287 -5.59286648947496
	-69.649403774385 11.1094562148838
	-94.6106954768797 27.7300571280032
	-119.625882404879 44.2738723902808
	-144.601462875557 60.8809270984799
	-169.654363605951 77.3752158531742
	-194.683198520362 93.9087899525306
	-219.621077761655 110.582758538354
	-244.64738595424 127.126321643443
	-269.582670439703 143.80345622804
	-294.647479602027 160.274269628114
	-319.648155600856 176.833853872934
	-344.668437854297 193.35595254896
	-369.605757531968 209.997362679655
	-394.545806252567 226.631422987155
	-419.536011848845 243.183687552377
	-444.542167008443 259.699441483368
	-469.511248910739 276.251795911861
	-494.478063571428 292.716814128477
	-506.413146297155 300.511772528793
	-513.044973621819 304.780092884065
	-519.304111290012 308.619717904813
	-525.546482734455 313.690882645573
	-528.647993608537 321.173877358308
	-526.389282899835 328.844377651254
	-519.967685961555 333.772658649848
	-512.194315768232 334.559913086149
	-504.920598613445 334.022513921479
	-497.830702651901 333.683295806161
	-490.246301754339 333.586516107828
	-481.989320666273 333.501485228727
	-452.464776539133 331.875352864768
	-426.546769879068 317.632390062491
	-401.869612034778 301.255402948146
	-377.002769702098 284.47758990235
	-352.019475708475 267.783284768495
	-341.968709073766 261.142032194487
	-334.216829866479 256.057727222911
	-325.854430457474 250.73756465693
	-315.682341769538 245.931962288324
	-303.395929401975 245.598062684091
	-291.906236936424 251.621810123533
	-284.501532372823 262.006216467385
	-281.943443517496 273.763587677756
	-281.096264625985 283.9372963532
	-280.163647393197 292.511188295173
	-279.387664063 299.876661628724
	-278.689121549568 307.089445423123
	-276.978275544541 315.278943852754
	-272.239332872313 322.47288440568
	-264.454392049905 326.086653892313
	-255.811040507297 325.984238524864
	-247.631419294177 324.759271226907
	-239.521711741673 323.304901142698
	-231.158133038038 321.864969052861
	-202.30743313704 317.235029926376
	-173.234701072251 312.760299800832
	-144.370558678785 308.284534577759
	-116.623566352046 298.542448327578
	-94.9220645541587 278.21310801219
	-73.6508673393142 258.470806726336
	-51.9426522386481 238.623459826207
	-29.9642323956338 218.327973380921
	-7.87533022567174 198.055542289257
	14.2305576139022 177.778521366063
	36.2233740758306 157.285276649377
	58.4323020793889 136.961823443304
	80.549283484264 116.634500675945
	102.626245843971 96.3402740131194
	125.033845316756 75.9598254059118
	131.921181657758 69.6559454777697
	139.077666884294 63.2693545926095
	146.576322316574 56.7302880479264
	154.949071996829 51.2490338497055
	164.618888740301 49.2129280893819
	174.765786761825 50.2418122474335
	184.497099360773 51.4340693418652
	193.887434533557 52.7148684818438
	203.032925567892 54.0488876799632
	212.058637029904 55.3429700838063
	242.468126135312 59.8645900296938
	271.467313746448 63.9897295122312
	279.374144645991 65.1481287662372
	287.309721444826 66.33547698426
	295.41866506963 67.5511842600362
	303.830585612128 68.5042866518592
	312.413856365128 68.2378084905216
	320.847163427221 66.4073146197272
	328.827897307336 63.1137486807755
	336.099440974589 58.4878555501693
	342.553237798644 52.7534226201233
	347.775513347412 45.8008859327381
	351.779856811719 38.0456960761247
	354.4081520277 29.74757060321
	355.416821683959 21.1869820842561
	355.016311518954 12.6338715615358
	354.026522128626 4.1788142122786
	352.949178176063 -4.27709141336005
	349.448947577128 -33.0816901801229
	345.73567554098 -62.8595691485267
	342.074903998562 -92.6436412918349
	339.833156022357 -122.549121614873
	338.319115940485 -152.629072441516
	333.751781184036 -181.651586717985
	332.18576963293 -189.82748555104
	330.36885722345 -197.841385697104
	328.285551583211 -205.752587472485
	325.070058741356 -213.34605375678
	319.715210136995 -219.871930841364
	312.697706445517 -224.779144958612
	304.576216207567 -227.59123976182
	296.049637852738 -227.848685100143
	287.811919242697 -225.83330075576
	280.196073145061 -222.068820259636
	273.151985679369 -217.25550598328
	266.079529281841 -212.355754853481
	242.280148285388 -196.360476488124
	217.629004206991 -179.825056616793
	192.535565777613 -163.269360103336
	167.604391092183 -146.612649631858
	142.681585849874 -129.924175754029
	117.68590211679 -113.332660954669
	92.6861849342056 -96.753976700374
	67.6083206216054 -80.3020507830256
	42.8300809765956 -63.4077459929606
	17.8287475395014 -46.8569201386717
	nan nan
	-2.70945871734768 -50.6658633403298
	-27.6754169457528 -34.0531436635881
	-52.644807507833 -17.4456807107373
	-77.6743620505538 -0.92882757171846
	-102.647000387047 15.6727517485551
	-127.611528574664 32.2855396290297
	-152.620366964654 48.8305232015647
	-177.585724124541 65.439310616398
	-202.498451168603 82.125807378003
	-227.507687050753 98.6650942988931
	-252.516155020091 115.203498957638
	-277.068451469088 132.434802862243
	-302.307235671001 148.62663810361
	-327.433436224177 164.992582975798
	-352.417454934216 181.579279590617
	-377.38129473575 198.202008926031
	-402.394484090685 214.753749399967
	-427.352722021523 231.385975825064
	-452.325788418287 247.98614934654
	-477.292806779782 264.579088750316
	-502.223580770371 281.214521852845
	-514.84450061783 289.641879344718
	-522.726567836962 294.902584354082
	-531.343170492596 300.857676042611
	-540.135386687382 309.51874639504
	-543.590844030718 322.275485505051
	-539.685435493062 335.544314668624
	-529.774021114723 344.248697743226
	-518.00646375032 347.403488929949
	-507.417694783385 347.597944998915
	-497.849871723044 347.245664543779
	-488.611070362704 346.835158525442
	-479.368640871512 346.373174553421
	-447.320642737194 344.20854252766
	-420.176427862977 328.466884395892
	-394.471943126412 311.466845381823
	-369.27695733144 295.098131891066
	-344.610511083195 278.743083279198
	-335.169098132427 272.070781202163
	-328.574899554671 267.376545465664
	-322.476082627754 263.055244443204
	-315.658267485634 259.223104222463
	-307.870930877144 257.870822785234
	-300.592088916587 261.103995110695
	-296.315893779649 268.033028193424
	-295.004113937353 275.941306632068
	-293.954122285774 284.603838906239
	-292.857504282245 293.817700591634
	-291.710048019232 303.156010301608
	-290.115181039986 313.198861971653
	-286.770538950377 323.860777452923
	-279.711805372633 332.947378622617
	-269.648418712599 337.950706552058
	-258.71191912615 338.632882703255
	-248.607209310824 337.538478021917
	-239.141919247103 336.20429830207
	-229.946693890534 334.718594941252
	-200.141465932846 329.950187628956
	-170.457323005841 325.010393174338
	-139.934378336891 320.164241695462
	-110.466943539722 309.807498260185
	-87.4002202388514 288.611159715254
	-65.1439933593037 268.041097574477
	-42.9437054190065 247.677098992292
	-20.750014089512 227.338928172104
	1.37582110088639 207.023217687628
	23.3660179764262 186.577005244474
	45.4716894731079 166.271445784771
	67.4415525801292 146.121317303381
	89.163404016381 126.044032236672
	111.251231555103 105.642605889247
	132.521364871062 86.1948765385793
	138.640123108106 80.4723361608025
	144.944254239233 74.5580489029011
	151.616078943908 68.5641225826245
	159.096983354415 63.5418326670171
	167.881621186213 62.1337204876765
	176.949542507539 63.1110315181413
	185.61869328173 64.3210703320198
	193.921646304004 65.6025542747856
	201.95487421382 66.8103918225001
	209.992698362817 67.9378106812
	238.319298912912 71.8929472143155
	268.683562004197 76.4843890179969
	277.80264331403 77.7582726523816
	286.985249573811 79.0591715391525
	296.400942293517 80.2883448290817
	306.178326552944 81.0684194278963
	316.127305068274 80.3106174331119
	325.978069061394 77.9621213901224
	335.399956896437 73.9333552247662
	344.138730234539 68.3353976140474
	351.821535803822 61.1788829929112
	358.224038538436 52.9222019765511
	363.106476058463 43.7812218472437
	366.42137542547 34.074710105031
	367.941751662744 24.0714107793724
	367.757179767609 14.203548688473
	366.76006576077 4.682105452312
	365.616389442356 -4.57122352413625
	362.000092003154 -34.6192711135371
	358.423511709058 -64.3780079374835
	354.70895180102 -94.1519738771119
	351.239092519409 -123.910460422499
	347.621924162402 -153.671215610388
	343.972963108179 -183.632997218874
	342.824043728728 -192.776639553117
	341.603184605192 -202.287942998239
	340.034814168231 -212.591885296022
	335.375677350595 -222.479230605691
	327.808190696286 -230.71436852364
	318.47962987303 -237.252287610953
	307.760248684564 -241.11883546868
	296.482125449697 -242.140151031362
	285.766710007887 -239.795952581298
	276.320816311576 -235.252299270654
	267.843379167546 -230.259982304948
	259.900972796113 -225.220616477988
	234.571225745123 -208.372467250531
	209.573827000582 -191.708069412024
	184.640995194933 -175.073527774015
	159.668833514665 -158.475730978282
	134.685983754998 -141.890606426221
	109.69789773379 -125.315238530988
	84.6826759445607 -108.781780126363
	59.7464479243596 -92.1293505717344
	34.7701540841678 -75.536151436047
	9.8253347368529 -58.8939681260401
};


==> ressources/variable_friction/chosen_path.tex <==
\addplot [line width=0.56pt, TUMred, forget plot]
table {%
	235.57422251168 -206.809604498743
	210.624480422329 -190.158143478173
	185.856748151757 -173.255702269997
	161.017068167805 -156.460218242343
	136.10379738 -139.76866886
	111.158224136609 -123.124644539106
	86.1988276903712 -106.503282634054
	61.2306341502117 -89.8965599744541
	36.2581554844827 -73.2970387835669
	11.2858917652489 -56.6973058430109
	-1.19939987814429 -48.396013804573
	-26.1715340442021 -31.7950577165333
	-51.146766794585 -15.1978881450733
	-76.125635989896 1.39442485954599
	-101.108664487831 17.9808007736175
	-126.096367280691 34.5601530282357
};
\addplot [line width=0.56pt, TUMred, forget plot]
table {%
	189.987833811882 -176.068176393537
	187.922597957575 -174.661488262091
	185.856748151757 -173.255702269997
	183.790255120118 -171.850940437303
	181.723081112466 -170.447181178621
	179.655240587042 -169.044403985224
	177.586748002083 -167.642588348383
	175.517617815828 -166.24171375937
	173.447864486515 -164.841759709459
	171.377502472385 -163.44270568992
	169.306546231674 -162.044531192026
	167.235010222622 -160.647215707049
	165.162908903467 -159.250738726262
	163.090256732449 -157.855079740936
	161.017068167805 -156.460218242343
	158.943152686774 -155.065990757029
	156.868743792729 -153.672498102431
	154.79387003223 -152.279697922251
	152.718559951841 -150.887547860188
	150.642842098121 -149.496005559944
	148.566745017632 -148.105028665218
	146.490297256937 -146.714574819712
	144.413527362595 -145.324601667127
	142.336463881169 -143.935066851162
	140.259135359221 -142.545928015519
	138.18157034331 -141.157142803898
	136.10379738 -139.76866886
	134.025811786186 -138.380449224992
	131.947654110449 -136.992487539295
	129.869331676831 -135.604772833112
	127.790851809375 -134.217294136647
	125.712221832122 -132.830040480102
	123.633449069116 -131.44300089368
	121.554540844397 -130.056164407584
	119.475504482009 -128.669520052018
	117.396347305994 -127.283056857184
	115.317076640394 -125.896763853285
	113.237699809252 -124.510630070525
	111.158224136609 -123.124644539106
	109.078730168666 -121.738847005607
	106.999146685909 -120.353183766808
	104.91947568446 -118.967651845649
	102.839719160441 -117.582248265069
	100.759879109974 -116.196970048008
	98.6799575291797 -114.811814217406
	96.5999564141806 -113.426777796202
	94.5198777610983 -112.041857807337
	92.4397235660545 -110.65705127375
	90.3594958251708 -109.27235521838
	88.2791965345692 -107.887766664169
	86.1988276903712 -106.503282634054
	84.1184460929554 -105.118936268624
	82.0379998933199 -103.734687011236
	79.9574920431707 -102.350530428231
	77.8769254942139 -100.966462085948
	75.7963031981557 -99.5824775507262
	73.7156281067018 -98.1985723889066
	71.6349031715585 -96.8147421668285
	69.5541313444318 -95.4309824508317
	67.4733155770278 -94.0472888072561
	65.3924588210523 -92.6636568024414
	63.3115640282116 -91.2800820027275
	61.2306341502117 -89.8965599744541
	59.1497012303076 -88.5131056320528
	57.0687391048479 -87.1296952229811
	54.9877507008316 -85.7463243441397
	52.9067389452578 -84.3629885924294
	50.8257067651256 -82.9796835647511
	48.7446570874339 -81.5964048580056
	46.6635928391819 -80.2131480690937
	44.5825169473685 -78.8299087949162
	42.5014323389929 -77.4466826323739
	40.420341941054 -76.0634651783677
	38.339248680551 -74.6802520297985
	36.2581554844827 -73.2970387835669
	34.1770694133012 -71.9138241194551
	32.0959883324962 -70.5306019478795
	30.0149142410228 -69.1473692621191
	27.9338491378358 -67.7641230554531
	25.8527950218902 -66.3808603211605
	23.771753892141 -64.9975780525204
	21.6907277475433 -63.6142732428118
	19.6097185870518 -62.2309428853139
	17.5287284096217 -60.8475839733058
	15.4477592142079 -59.4641935000666
	13.3668129997653 -58.0807684588752
	11.2858917652489 -56.6973058430109
	9.20498357481415 -55.3137966566309
	7.12409530104457 -53.9302575114586
	5.04321988140208 -52.5466990305805
	2.96235025334854 -51.1631318370826
	0.881479354345792 -49.7795665540514
	-1.19939987814429 -48.396013804573
	-3.28032044927286 -47.0124645002884
	-5.36125666559819 -45.6289387280198
	-7.44220877589086 -44.2454368625414
	-9.52317702892145 -42.8619592786274
	-11.6041616734606 -41.4785063510519
	-13.6851629582788 -40.0950784545891
	-15.7661811321467 -38.7116759640132
	-17.8472164438349 -37.3282992540984
	-19.9282691421139 -35.9449486996188
	-22.0093394757544 -34.5616246753487
	-24.090427693527 -33.1783275560621
	-26.1715340442021 -31.7950577165333
	-28.2526924347301 -30.4117932209706
	-30.3338696230302 -29.0285570071176
	-32.4150660246075 -27.6453497012581
	-34.4962820549668 -26.2621719296759
	-36.5775181296131 -24.8790243186551
	-38.6587746640513 -23.4959074944795
	-40.7400520737863 -22.112822083433
	-42.8213507743229 -20.7297687117995
	-44.9026711811662 -19.3467480058629
	-46.984013709821 -17.963760591907
};
\addplot [line width=0.56pt, red, forget plot]
table {%
	189.987833811882 -176.068176393537
	187.922597957575 -174.661488262091
	185.856748151757 -173.255702269997
	183.790255120118 -171.850940437303
	181.723081112466 -170.447181178621
	179.655240587042 -169.044403985224
	177.586748002083 -167.642588348383
	175.517617815828 -166.24171375937
	173.447864486515 -164.841759709459
	171.377502472385 -163.44270568992
	169.306546231674 -162.044531192026
	167.235010222622 -160.647215707049
	165.162908903467 -159.250738726262
	163.090256732449 -157.855079740936
	161.017068167805 -156.460218242343
	158.943152686774 -155.065990757029
	156.868743792729 -153.672498102431
	154.79387003223 -152.279697922251
	152.718559951841 -150.887547860188
	150.642842098121 -149.496005559944
	148.566745017632 -148.105028665218
	146.490297256937 -146.714574819712
	144.413527362595 -145.324601667127
	142.336463881169 -143.935066851162
	140.259135359221 -142.545928015519
	138.18157034331 -141.157142803898
	136.10379738 -139.76866886
	134.025811786186 -138.380449224992
	131.947654110449 -136.992487539295
	129.869331676831 -135.604772833112
	127.790851809375 -134.217294136647
	125.712221832122 -132.830040480102
	123.633449069116 -131.44300089368
	121.554540844397 -130.056164407584
	119.475504482009 -128.669520052018
	117.396347305994 -127.283056857184
	115.317076640394 -125.896763853285
	113.237699809252 -124.510630070525
	111.158224136609 -123.124644539106
	109.078730168666 -121.738847005607
	106.999146685909 -120.353183766808
	104.91947568446 -118.967651845649
	102.839719160441 -117.582248265069
	100.759879109974 -116.196970048008
	98.6799575291797 -114.811814217406
	96.5999564141806 -113.426777796202
	94.5198777610983 -112.041857807337
	92.4397235660545 -110.65705127375
	90.3594958251708 -109.27235521838
	88.2791965345692 -107.887766664169
	86.1988276903712 -106.503282634054
	84.1184460929554 -105.118936268624
	82.0379998933199 -103.734687011236
	79.9574920431707 -102.350530428231
	77.8769254942139 -100.966462085948
	75.7963031981557 -99.5824775507262
	73.7156281067018 -98.1985723889066
	71.6349031715585 -96.8147421668285
	69.5541313444318 -95.4309824508317
	67.4733155770278 -94.0472888072561
	65.3924588210523 -92.6636568024414
	63.3115640282116 -91.2800820027275
	61.2306341502117 -89.8965599744541
	59.1497012303076 -88.5131056320528
	57.0687391048479 -87.1296952229811
	54.9877507008316 -85.7463243441397
	52.9067389452578 -84.3629885924294
	50.8257067651256 -82.9796835647511
	48.7446570874339 -81.5964048580056
	46.6635928391819 -80.2131480690937
	44.5825169473685 -78.8299087949162
	42.5014323389929 -77.4466826323739
	40.420341941054 -76.0634651783677
	38.339248680551 -74.6802520297985
	36.2581554844827 -73.2970387835669
	34.1770694133012 -71.9138241194551
	32.0959883324962 -70.5306019478795
	30.0149142410228 -69.1473692621191
	27.9338491378358 -67.7641230554531
	25.8527950218902 -66.3808603211605
	23.771753892141 -64.9975780525204
	21.6907277475433 -63.6142732428118
	19.6097185870518 -62.2309428853139
	17.5287284096217 -60.8475839733058
	15.4477592142079 -59.4641935000666
	13.3668129997653 -58.0807684588752
	11.2858917652489 -56.6973058430109
	9.20498357481415 -55.3137966566309
	7.12409530104457 -53.9302575114586
	5.04321988140208 -52.5466990305805
	2.96235025334854 -51.1631318370826
	0.881479354345792 -49.7795665540514
	-1.19939987814429 -48.396013804573
	-3.28032044927286 -47.0124645002884
	-5.36125666559819 -45.6289387280198
	-7.44220877589086 -44.2454368625414
	-9.52317702892145 -42.8619592786274
	-11.6041616734606 -41.4785063510519
	-13.6851629582788 -40.0950784545891
	-15.7661811321467 -38.7116759640132
	-17.8472164438349 -37.3282992540984
	-19.9282691421139 -35.9449486996188
	-22.0093394757544 -34.5616246753487
	-24.090427693527 -33.1783275560621
	-26.1715340442021 -31.7950577165333
	-28.2526924347301 -30.4117932209706
	-30.3338696230302 -29.0285570071176
	-32.4150660246075 -27.6453497012581
	-34.4962820549668 -26.2621719296759
	-36.5775181296131 -24.8790243186551
	-38.6587746640513 -23.4959074944795
	-40.7400520737863 -22.112822083433
	-42.8213507743229 -20.7297687117995
	-44.9026711811662 -19.3467480058629
	-46.984013709821 -17.963760591907
};

==> ressources/variable_friction/friction_high.tex <==
\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:-1.1994,-48.396)
--(axis cs:-9.5349,-42.8542);

\path [draw=lightgray!34.50980392156862!black, line width=4.0pt]
(axis cs:-9.5349,-42.8542)
--(axis cs:-17.8707,-37.3127);

\path [draw=lightgray!44.96732026143791!black, line width=4.0pt]
(axis cs:-17.8707,-37.3127)
--(axis cs:-26.2068,-31.7716);

\path [draw=lightgray!60.130718954248366!black, line width=4.0pt]
(axis cs:-26.2068,-31.7716)
--(axis cs:-34.5431,-26.231);

\path [draw=lightgray!64.31372549019608!black, line width=4.0pt]
(axis cs:-34.5431,-26.231)
--(axis cs:-42.8798,-20.6909);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:-42.8798,-20.6909)
--(axis cs:-51.2169,-15.1513);

\path [draw=lightgray!40.26143790849674!black, line width=4.0pt]
(axis cs:-51.2169,-15.1513)
--(axis cs:-59.5543,-9.6123);

\path [draw=lightgray!55.94771241830067!black, line width=4.0pt]
(axis cs:-59.5543,-9.6123)
--(axis cs:-67.8921,-4.0739);

\path [draw=lightgray!37.12418300653595!black, line width=4.0pt]
(axis cs:-67.8921,-4.0739)
--(axis cs:-76.2303,1.4639);

\path [draw=lightgray!44.44444444444445!black, line width=4.0pt]
(axis cs:-76.2303,1.4639)
--(axis cs:-84.569,7.001);

\path [draw=lightgray!54.37908496732026!black, line width=4.0pt]
(axis cs:-84.569,7.001)
--(axis cs:-92.9081,12.5375);

\path [draw=lightgray!53.8562091503268!black, line width=4.0pt]
(axis cs:-92.9081,12.5375)
--(axis cs:-101.2478,18.0731);

\path [draw=lightgray!17.77777777777777!black, line width=4.0pt]
(axis cs:-101.2478,18.0731)
--(axis cs:-109.5879,23.608);

\path [draw=lightgray!66.92810457516339!black, line width=4.0pt]
(axis cs:-109.5879,23.608)
--(axis cs:-117.9286,29.1421);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:-117.9286,29.1421)
--(axis cs:-126.2699,34.6753);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:-126.2699,34.6753)
--(axis cs:-134.6118,40.2076);

\path [draw=lightgray!72.15686274509805!black, line width=4.0pt]
(axis cs:-134.6118,40.2076)
--(axis cs:-142.9543,45.7389);

\path [draw=lightgray!61.69934640522876!black, line width=4.0pt]
(axis cs:-142.9543,45.7389)
--(axis cs:-151.2974,51.2693);

\path [draw=lightgray!42.87581699346405!black, line width=4.0pt]
(axis cs:-151.2974,51.2693)
--(axis cs:-159.6412,56.7987);

\path [draw=lightgray!46.5359477124183!black, line width=4.0pt]
(axis cs:-159.6412,56.7987)
--(axis cs:-167.9857,62.3271);

\path [draw=white!84.70588235294117!black, line width=4.0pt]
(axis cs:-167.9857,62.3271)
--(axis cs:-176.3309,67.8544);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-176.3309,67.8544)
--(axis cs:-184.6768,73.3805);

\path [draw=lightgray!79.47712418300654!black, line width=4.0pt]
(axis cs:-184.6768,73.3805)
--(axis cs:-193.0235,78.9055);

\path [draw=lightgray!44.44444444444445!black, line width=4.0pt]
(axis cs:-193.0235,78.9055)
--(axis cs:-201.371,84.4294);

\path [draw=lightgray!43.39869281045751!black, line width=4.0pt]
(axis cs:-201.371,84.4294)
--(axis cs:-209.7193,89.952);

\path [draw=lightgray!48.1045751633987!black, line width=4.0pt]
(axis cs:-209.7193,89.952)
--(axis cs:-218.0685,95.4733);

\path [draw=lightgray!24.05228758169935!black, line width=4.0pt]
(axis cs:-218.0685,95.4733)
--(axis cs:-226.4185,100.9933);

\path [draw=lightgray!42.87581699346405!black, line width=4.0pt]
(axis cs:-226.4185,100.9933)
--(axis cs:-234.7693,106.512);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-234.7693,106.512)
--(axis cs:-243.1211,112.0293);

\path [draw=lightgray!57.516339869281055!black, line width=4.0pt]
(axis cs:-243.1211,112.0293)
--(axis cs:-251.4738,117.5453);

\path [draw=lightgray!47.05882352941176!black, line width=4.0pt]
(axis cs:-251.4738,117.5453)
--(axis cs:-259.8272,123.0602);

\path [draw=lightgray!30.849673202614387!black, line width=4.0pt]
(axis cs:-259.8272,123.0602)
--(axis cs:-268.1812,128.5741);

\path [draw=lightgray!63.79084967320261!black, line width=4.0pt]
(axis cs:-268.1812,128.5741)
--(axis cs:-276.5358,134.0872);

\path [draw=lightgray!49.150326797385624!black, line width=4.0pt]
(axis cs:-276.5358,134.0872)
--(axis cs:-284.891,139.5994);

\path [draw=lightgray!67.97385620915031!black, line width=4.0pt]
(axis cs:-284.891,139.5994)
--(axis cs:-293.2466,145.111);

\path [draw=lightgray!62.22222222222222!black, line width=4.0pt]
(axis cs:-293.2466,145.111)
--(axis cs:-301.6025,150.622);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-301.6025,150.622)
--(axis cs:-309.9589,156.1324);

\path [draw=lightgray!68.49673202614377!black, line width=4.0pt]
(axis cs:-309.9589,156.1324)
--(axis cs:-318.3155,161.6424);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-318.3155,161.6424)
--(axis cs:-326.6724,167.152);

\path [draw=lightgray!42.87581699346405!black, line width=4.0pt]
(axis cs:-326.6724,167.152)
--(axis cs:-335.0295,172.6613);

\path [draw=lightgray!70.58823529411765!black, line width=4.0pt]
(axis cs:-335.0295,172.6613)
--(axis cs:-343.3866,178.1705);

\path [draw=lightgray!76.86274509803921!black, line width=4.0pt]
(axis cs:-343.3866,178.1705)
--(axis cs:-351.7439,183.6795);

\path [draw=lightgray!61.69934640522876!black, line width=4.0pt]
(axis cs:-351.7439,183.6795)
--(axis cs:-360.1012,189.1885);

\path [draw=lightgray!28.235294117647065!black, line width=4.0pt]
(axis cs:-360.1012,189.1885)
--(axis cs:-368.4584,194.6976);

\path [draw=lightgray!63.79084967320261!black, line width=4.0pt]
(axis cs:-368.4584,194.6976)
--(axis cs:-376.8155,200.2069);

\path [draw=lightgray!67.45098039215685!black, line width=4.0pt]
(axis cs:-376.8155,200.2069)
--(axis cs:-385.1724,205.7165);

\path [draw=lightgray!51.764705882352935!black, line width=4.0pt]
(axis cs:-385.1724,205.7165)
--(axis cs:-393.5287,211.2269);

\path [draw=lightgray!84.18300653594771!black, line width=4.0pt]
(axis cs:-393.5287,211.2269)
--(axis cs:-401.8843,216.7385);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:-401.8843,216.7385)
--(axis cs:-410.2388,222.2516);

\path [draw=white!78.43137254901961!black, line width=4.0pt]
(axis cs:-410.2388,222.2516)
--(axis cs:-418.592,227.7668);

\path [draw=lightgray!70.58823529411765!black, line width=4.0pt]
(axis cs:-418.592,227.7668)
--(axis cs:-426.9436,233.2844);

\path [draw=lightgray!35.555555555555564!black, line width=4.0pt]
(axis cs:-426.9436,233.2844)
--(axis cs:-435.2933,238.8049);

\path [draw=lightgray!75.29411764705883!black, line width=4.0pt]
(axis cs:-435.2933,238.8049)
--(axis cs:-443.6409,244.3285);

\path [draw=lightgray!58.56209150326798!black, line width=4.0pt]
(axis cs:-443.6409,244.3285)
--(axis cs:-451.9861,249.8559);

\path [draw=white!76.07843137254902!black, line width=4.0pt]
(axis cs:-451.9861,249.8559)
--(axis cs:-460.3286,255.3873);

\path [draw=lightgray!50.19607843137255!black, line width=4.0pt]
(axis cs:-460.3286,255.3873)
--(axis cs:-468.6681,260.9231);

\path [draw=lightgray!78.43137254901961!black, line width=4.0pt]
(axis cs:-468.6681,260.9231)
--(axis cs:-477.0043,266.4639);

\path [draw=lightgray!40.7843137254902!black, line width=4.0pt]
(axis cs:-477.0043,266.4639)
--(axis cs:-485.3371,272.0099);

\path [draw=lightgray!63.79084967320261!black, line width=4.0pt]
(axis cs:-485.3371,272.0099)
--(axis cs:-493.6661,277.5616);

\path [draw=lightgray!81.5686274509804!black, line width=4.0pt]
(axis cs:-493.6661,277.5616)
--(axis cs:-501.9815,283.1336);

\path [draw=lightgray!57.516339869281055!black, line width=4.0pt]
(axis cs:-501.9815,283.1336)
--(axis cs:-510.1823,288.8716);

\path [draw=lightgray!39.215686274509814!black, line width=4.0pt]
(axis cs:-510.1823,288.8716)
--(axis cs:-517.9559,295.1673);

\path [draw=lightgray!81.04575163398694!black, line width=4.0pt]
(axis cs:-517.9559,295.1673)
--(axis cs:-524.5873,302.6383);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:-524.5873,302.6383)
--(axis cs:-529.1885,311.4764);

\path [draw=lightgray!67.97385620915031!black, line width=4.0pt]
(axis cs:-529.1885,311.4764)
--(axis cs:-530.4952,321.3255);

\path [draw=lightgray!59.6078431372549!black, line width=4.0pt]
(axis cs:-530.4952,321.3255)
--(axis cs:-527.541,330.7944);

\path [draw=lightgray!51.764705882352935!black, line width=4.0pt]
(axis cs:-527.541,330.7944)
--(axis cs:-521.0243,338.2902);

\path [draw=lightgray!20.3921568627451!black, line width=4.0pt]
(axis cs:-521.0243,338.2902)
--(axis cs:-512.2902,343.0779);

\path [draw=lightgray!17.25490196078431!black, line width=4.0pt]
(axis cs:-512.2902,343.0779)
--(axis cs:-502.5372,345.1861);

\path [draw=lightgray!34.50980392156862!black, line width=4.0pt]
(axis cs:-502.5372,345.1861)
--(axis cs:-492.5422,345.2403);

\path [draw=lightgray!85.7516339869281!black, line width=4.0pt]
(axis cs:-492.5422,345.2403)
--(axis cs:-482.6228,343.9411);

\path [draw=white, line width=4.0pt]
(axis cs:-482.6228,343.9411)
--(axis cs:-472.8557,341.7641);

\path [draw=lightgray!46.01307189542484!black, line width=4.0pt]
(axis cs:-472.8557,341.7641)
--(axis cs:-463.2668,338.9004);

\path [draw=lightgray!76.86274509803921!black, line width=4.0pt]
(axis cs:-463.2668,338.9004)
--(axis cs:-453.8778,335.4356);

\path [draw=lightgray!70.06535947712419!black, line width=4.0pt]
(axis cs:-453.8778,335.4356)
--(axis cs:-444.7102,331.4211);

\path [draw=lightgray!86.27450980392157!black, line width=4.0pt]
(axis cs:-444.7102,331.4211)
--(axis cs:-435.7665,326.929);

\path [draw=lightgray!72.15686274509805!black, line width=4.0pt]
(axis cs:-435.7665,326.929)
--(axis cs:-427.0374,322.0323);

\path [draw=lightgray!50.71895424836601!black, line width=4.0pt]
(axis cs:-427.0374,322.0323)
--(axis cs:-418.5028,316.8032);

\path [draw=lightgray!94.11764705882352!black, line width=4.0pt]
(axis cs:-418.5028,316.8032)
--(axis cs:-410.1326,311.3146);

\path [draw=white!81.96078431372548!black, line width=4.0pt]
(axis cs:-410.1326,311.3146)
--(axis cs:-401.9019,305.6186);

\path [draw=lightgray!30.326797385620914!black, line width=4.0pt]
(axis cs:-401.9019,305.6186)
--(axis cs:-393.7647,299.7896);

\path [draw=lightgray!30.849673202614387!black, line width=4.0pt]
(axis cs:-393.7647,299.7896)
--(axis cs:-385.6672,293.9054);

\path [draw=lightgray!40.26143790849674!black, line width=4.0pt]
(axis cs:-385.6672,293.9054)
--(axis cs:-377.5663,288.0259);

\path [draw=lightgray!61.69934640522876!black, line width=4.0pt]
(axis cs:-377.5663,288.0259)
--(axis cs:-369.4533,282.163);

\path [draw=lightgray!17.77777777777777!black, line width=4.0pt]
(axis cs:-369.4533,282.163)
--(axis cs:-361.3271,276.3187);

\path [draw=lightgray!73.72549019607844!black, line width=4.0pt]
(axis cs:-361.3271,276.3187)
--(axis cs:-353.1078,270.6062);

\path [draw=lightgray!18.823529411764714!black, line width=4.0pt]
(axis cs:-353.1078,270.6062)
--(axis cs:-344.7821,265.0501);

\path [draw=lightgray!67.45098039215685!black, line width=4.0pt]
(axis cs:-344.7821,265.0501)
--(axis cs:-336.1884,259.9258);

\path [draw=lightgray!77.38562091503267!black, line width=4.0pt]
(axis cs:-336.1884,259.9258)
--(axis cs:-327.0159,255.9504);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:-327.0159,255.9504)
--(axis cs:-317.2399,253.9848);

\path [draw=lightgray!28.235294117647065!black, line width=4.0pt]
(axis cs:-317.2399,253.9848)
--(axis cs:-307.3934,255.3083);

\path [draw=lightgray!27.18954248366014!black, line width=4.0pt]
(axis cs:-307.3934,255.3083)
--(axis cs:-298.9726,260.5441);

\path [draw=white!76.47058823529412!black, line width=4.0pt]
(axis cs:-298.9726,260.5441)
--(axis cs:-293.4551,268.7963);

\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:-293.4551,268.7963)
--(axis cs:-290.9505,278.4527);

\path [draw=lightgray!17.77777777777777!black, line width=4.0pt]
(axis cs:-290.9505,278.4527)
--(axis cs:-290.1581,288.4283);

\path [draw=lightgray!64.83660130718954!black, line width=4.0pt]
(axis cs:-290.1581,288.4283)
--(axis cs:-289.0812,298.3724);

\path [draw=lightgray!38.69281045751634!black, line width=4.0pt]
(axis cs:-289.0812,298.3724)
--(axis cs:-286.2447,307.9439);

\path [draw=lightgray!49.150326797385624!black, line width=4.0pt]
(axis cs:-286.2447,307.9439)
--(axis cs:-281.045,316.4579);

\path [draw=lightgray!31.37254901960785!black, line width=4.0pt]
(axis cs:-281.045,316.4579)
--(axis cs:-273.8621,323.3829);

\path [draw=lightgray!52.81045751633987!black, line width=4.0pt]
(axis cs:-273.8621,323.3829)
--(axis cs:-265.2129,328.3673);

\path [draw=lightgray!37.12418300653595!black, line width=4.0pt]
(axis cs:-265.2129,328.3673)
--(axis cs:-255.6729,331.3363);

\path [draw=lightgray!79.47712418300654!black, line width=4.0pt]
(axis cs:-255.6729,331.3363)
--(axis cs:-245.7629,332.6653);

\path [draw=lightgray!34.50980392156862!black, line width=4.0pt]
(axis cs:-245.7629,332.6653)
--(axis cs:-235.7592,332.7092);

\path [draw=lightgray!64.83660130718954!black, line width=4.0pt]
(axis cs:-235.7592,332.7092)
--(axis cs:-225.7862,331.8767);

\path [draw=lightgray!58.56209150326798!black, line width=4.0pt]
(axis cs:-225.7862,331.8767)
--(axis cs:-215.8554,330.6253);

\path [draw=lightgray!21.960784313725487!black, line width=4.0pt]
(axis cs:-215.8554,330.6253)
--(axis cs:-205.9552,329.151);

\path [draw=lightgray!47.05882352941176!black, line width=4.0pt]
(axis cs:-205.9552,329.151)
--(axis cs:-196.0844,327.4902);

\path [draw=lightgray!68.49673202614377!black, line width=4.0pt]
(axis cs:-196.0844,327.4902)
--(axis cs:-186.2429,325.6638);

\path [draw=lightgray!48.1045751633987!black, line width=4.0pt]
(axis cs:-186.2429,325.6638)
--(axis cs:-176.4462,323.612);

\path [draw=lightgray!58.03921568627452!black, line width=4.0pt]
(axis cs:-176.4462,323.612)
--(axis cs:-166.7136,321.2753);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:-166.7136,321.2753)
--(axis cs:-157.0649,318.6138);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-157.0649,318.6138)
--(axis cs:-147.5264,315.5818);

\path [draw=lightgray!28.758169934640527!black, line width=4.0pt]
(axis cs:-147.5264,315.5818)
--(axis cs:-138.1414,312.1048);

\path [draw=lightgray!71.63398692810458!black, line width=4.0pt]
(axis cs:-138.1414,312.1048)
--(axis cs:-128.9394,308.1688);

\path [draw=lightgray!60.130718954248366!black, line width=4.0pt]
(axis cs:-128.9394,308.1688)
--(axis cs:-119.9374,303.7943);

\path [draw=lightgray!71.63398692810458!black, line width=4.0pt]
(axis cs:-119.9374,303.7943)
--(axis cs:-111.1463,299.0101);

\path [draw=lightgray!3.137254901960788!black, line width=4.0pt]
(axis cs:-111.1463,299.0101)
--(axis cs:-102.5719,293.8472);

\path [draw=lightgray!31.89542483660131!black, line width=4.0pt]
(axis cs:-102.5719,293.8472)
--(axis cs:-94.2249,288.3242);

\path [draw=lightgray!96.73202614379085!black, line width=4.0pt]
(axis cs:-94.2249,288.3242)
--(axis cs:-86.1059,282.471);

\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:-86.1059,282.471)
--(axis cs:-78.1987,276.3343);

\path [draw=lightgray!72.67973856209152!black, line width=4.0pt]
(axis cs:-78.1987,276.3343)
--(axis cs:-70.4884,269.9518);

\path [draw=lightgray!53.333333333333336!black, line width=4.0pt]
(axis cs:-70.4884,269.9518)
--(axis cs:-62.9535,263.363);

\path [draw=lightgray!48.1045751633987!black, line width=4.0pt]
(axis cs:-62.9535,263.363)
--(axis cs:-55.572,256.6027);

\path [draw=lightgray!48.1045751633987!black, line width=4.0pt]
(axis cs:-55.572,256.6027)
--(axis cs:-48.3241,249.6993);

\path [draw=lightgray!52.28758169934641!black, line width=4.0pt]
(axis cs:-48.3241,249.6993)
--(axis cs:-41.1822,242.686);

\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:-41.1822,242.686)
--(axis cs:-34.1192,235.5933);

\path [draw=lightgray!58.03921568627452!black, line width=4.0pt]
(axis cs:-34.1192,235.5933)
--(axis cs:-27.1104,228.447);

\path [draw=lightgray!56.99346405228759!black, line width=4.0pt]
(axis cs:-27.1104,228.447)
--(axis cs:-20.1405,221.2628);

\path [draw=lightgray!92.02614379084967!black, line width=4.0pt]
(axis cs:-20.1405,221.2628)
--(axis cs:-13.1998,214.0503);

\path [draw=lightgray!65.88235294117646!black, line width=4.0pt]
(axis cs:-13.1998,214.0503)
--(axis cs:-6.2795,206.8183);

\path [draw=lightgray!94.640522875817!black, line width=4.0pt]
(axis cs:-6.2795,206.8183)
--(axis cs:0.6303,199.5761);

\path [draw=lightgray!67.45098039215685!black, line width=4.0pt]
(axis cs:0.6303,199.5761)
--(axis cs:7.5388,192.3329);

\path [draw=lightgray!51.24183006535947!black, line width=4.0pt]
(axis cs:7.5388,192.3329)
--(axis cs:14.4559,185.0977);

\path [draw=lightgray!70.58823529411765!black, line width=4.0pt]
(axis cs:14.4559,185.0977)
--(axis cs:21.3908,177.8796);

\path [draw=lightgray!53.8562091503268!black, line width=4.0pt]
(axis cs:21.3908,177.8796)
--(axis cs:28.3522,170.6872);

\path [draw=lightgray!47.58169934640524!black, line width=4.0pt]
(axis cs:28.3522,170.6872)
--(axis cs:35.347,163.5272);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:35.347,163.5272)
--(axis cs:42.3792,156.4039);

\path [draw=lightgray!96.20915032679738!black, line width=4.0pt]
(axis cs:42.3792,156.4039)
--(axis cs:49.4537,149.3226);

\path [draw=lightgray!16.732026143790847!black, line width=4.0pt]
(axis cs:49.4537,149.3226)
--(axis cs:56.5762,142.2897);

\path [draw=lightgray!41.830065359477125!black, line width=4.0pt]
(axis cs:56.5762,142.2897)
--(axis cs:63.7503,135.3093);

\path [draw=lightgray!40.7843137254902!black, line width=4.0pt]
(axis cs:63.7503,135.3093)
--(axis cs:70.9792,128.3858);

\path [draw=lightgray!58.56209150326798!black, line width=4.0pt]
(axis cs:70.9792,128.3858)
--(axis cs:78.2484,121.5045);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:78.2484,121.5045)
--(axis cs:85.5382,114.6451);

\path [draw=lightgray!59.08496732026144!black, line width=4.0pt]
(axis cs:85.5382,114.6451)
--(axis cs:92.851,107.8101);

\path [draw=lightgray!65.359477124183!black, line width=4.0pt]
(axis cs:92.851,107.8101)
--(axis cs:100.1909,101.0044);

\path [draw=lightgray!66.40522875816993!black, line width=4.0pt]
(axis cs:100.1909,101.0044)
--(axis cs:107.5806,94.2528);

\path [draw=lightgray!40.26143790849674!black, line width=4.0pt]
(axis cs:107.5806,94.2528)
--(axis cs:115.1067,87.6541);

\path [draw=lightgray!43.92156862745099!black, line width=4.0pt]
(axis cs:115.1067,87.6541)
--(axis cs:122.8881,81.3596);

\path [draw=lightgray!54.37908496732026!black, line width=4.0pt]
(axis cs:122.8881,81.3596)
--(axis cs:131.0096,75.5123);

\path [draw=lightgray!28.235294117647065!black, line width=4.0pt]
(axis cs:131.0096,75.5123)
--(axis cs:139.5498,70.2979);

\path [draw=lightgray!49.150326797385624!black, line width=4.0pt]
(axis cs:139.5498,70.2979)
--(axis cs:148.5069,65.8378);

\path [draw=lightgray!80.52287581699348!black, line width=4.0pt]
(axis cs:148.5069,65.8378)
--(axis cs:157.8094,62.1524);

\path [draw=lightgray!92.02614379084967!black, line width=4.0pt]
(axis cs:157.8094,62.1524)
--(axis cs:167.3963,59.2872);

\path [draw=lightgray!33.464052287581694!black, line width=4.0pt]
(axis cs:167.3963,59.2872)
--(axis cs:177.2027,57.2999);

\path [draw=lightgray!80.52287581699348!black, line width=4.0pt]
(axis cs:177.2027,57.2999)
--(axis cs:187.1481,56.2066);

\path [draw=lightgray!13.0718954248366!black, line width=4.0pt]
(axis cs:187.1481,56.2066)
--(axis cs:197.1521,56.0381);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:197.1521,56.0381)
--(axis cs:207.1271,56.8173);

\path [draw=lightgray!52.28758169934641!black, line width=4.0pt]
(axis cs:207.1271,56.8173)
--(axis cs:216.999,58.453);

\path [draw=lightgray!50.19607843137255!black, line width=4.0pt]
(axis cs:216.999,58.453)
--(axis cs:226.7268,60.8026);

\path [draw=lightgray!33.464052287581694!black, line width=4.0pt]
(axis cs:226.7268,60.8026)
--(axis cs:236.3057,63.7036);

\path [draw=white!81.17647058823529!black, line width=4.0pt]
(axis cs:236.3057,63.7036)
--(axis cs:245.7969,66.883);

\path [draw=lightgray!27.712418300653603!black, line width=4.0pt]
(axis cs:245.7969,66.883)
--(axis cs:255.3044,70.013);

\path [draw=lightgray!57.516339869281055!black, line width=4.0pt]
(axis cs:255.3044,70.013)
--(axis cs:264.9253,72.7698);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:264.9253,72.7698)
--(axis cs:274.7143,74.8418);

\path [draw=lightgray!89.41176470588236!black, line width=4.0pt]
(axis cs:274.7143,74.8418)
--(axis cs:284.6604,75.9157);

\path [draw=lightgray!83.66013071895425!black, line width=4.0pt]
(axis cs:284.6604,75.9157)
--(axis cs:294.6635,75.8808);

\path [draw=lightgray!44.96732026143791!black, line width=4.0pt]
(axis cs:294.6635,75.8808)
--(axis cs:304.5966,74.7025);

\path [draw=lightgray!83.66013071895425!black, line width=4.0pt]
(axis cs:304.5966,74.7025)
--(axis cs:314.3088,72.3128);

\path [draw=lightgray!25.620915032679736!black, line width=4.0pt]
(axis cs:314.3088,72.3128)
--(axis cs:323.6198,68.6648);

\path [draw=lightgray!1.0457516339869244!black, line width=4.0pt]
(axis cs:323.6198,68.6648)
--(axis cs:332.3287,63.7516);

\path [draw=lightgray!67.97385620915031!black, line width=4.0pt]
(axis cs:332.3287,63.7516)
--(axis cs:340.1802,57.5628);

\path [draw=lightgray!25.620915032679736!black, line width=4.0pt]
(axis cs:340.1802,57.5628)
--(axis cs:346.9426,50.2003);

\path [draw=lightgray!9.93464052287581!black, line width=4.0pt]
(axis cs:346.9426,50.2003)
--(axis cs:352.498,41.8871);

\path [draw=lightgray!55.94771241830067!black, line width=4.0pt]
(axis cs:352.498,41.8871)
--(axis cs:356.7546,32.8381);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:356.7546,32.8381)
--(axis cs:359.7572,23.2982);	

\path [draw=lightgray!54.90196078431372!black, line width=4.0pt]
(axis cs:359.7572,23.2982)
--(axis cs:361.6308,13.471);

\path [draw=lightgray!58.03921568627452!black, line width=4.0pt]
(axis cs:361.6308,13.471)
--(axis cs:362.5213,3.5047);

\path [draw=lightgray!39.215686274509814!black, line width=4.0pt]
(axis cs:362.5213,3.5047)
--(axis cs:362.6164,-6.5018);

\path [draw=lightgray!62.745098039215684!black, line width=4.0pt]
(axis cs:362.6164,-6.5018)
--(axis cs:362.0877,-16.4961);

\path [draw=lightgray!69.54248366013073!black, line width=4.0pt]
(axis cs:362.0877,-16.4961)
--(axis cs:361.1467,-26.4611);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:361.1467,-26.4611)
--(axis cs:359.98,-36.4023);

\path [draw=lightgray!76.33986928104575!black, line width=4.0pt]
(axis cs:359.98,-36.4023)
--(axis cs:358.7131,-46.3315);

\path [draw=lightgray!69.01960784313724!black, line width=4.0pt]
(axis cs:358.7131,-46.3315)
--(axis cs:357.424,-56.2578);

\path [draw=lightgray!65.88235294117646!black, line width=4.0pt]
(axis cs:357.424,-56.2578)
--(axis cs:356.1224,-66.1825);

\path [draw=white!78.03921568627452!black, line width=4.0pt]
(axis cs:356.1224,-66.1825)
--(axis cs:354.8297,-76.1083);

\path [draw=lightgray!88.8888888888889!black, line width=4.0pt]
(axis cs:354.8297,-76.1083)
--(axis cs:353.5684,-86.0382);

\path [draw=white!78.82352941176471!black, line width=4.0pt]
(axis cs:353.5684,-86.0382)
--(axis cs:352.3545,-95.9739);

\path [draw=lightgray!54.90196078431372!black, line width=4.0pt]
(axis cs:352.3545,-95.9739)
--(axis cs:351.1846,-105.915);

\path [draw=lightgray!29.80392156862745!black, line width=4.0pt]
(axis cs:351.1846,-105.915)
--(axis cs:350.051,-115.8602);

\path [draw=lightgray!43.39869281045751!black, line width=4.0pt]
(axis cs:350.051,-115.8602)
--(axis cs:348.9443,-125.8085);

\path [draw=lightgray!7.3202614379085!black, line width=4.0pt]
(axis cs:348.9443,-125.8085)
--(axis cs:347.8561,-135.7588);

\path [draw=lightgray!21.437908496732025!black, line width=4.0pt]
(axis cs:347.8561,-135.7588)
--(axis cs:346.778,-145.7103);

\path [draw=lightgray!50.71895424836601!black, line width=4.0pt]
(axis cs:346.778,-145.7103)
--(axis cs:345.7015,-155.6619);

\path [draw=lightgray!65.359477124183!black, line width=4.0pt]
(axis cs:345.7015,-155.6619)
--(axis cs:344.6084,-165.6116);

\path [draw=lightgray!20.915032679738562!black, line width=4.0pt]
(axis cs:344.6084,-165.6116)
--(axis cs:343.3479,-175.5411);

\path [draw=lightgray!15.163398692810462!black, line width=4.0pt]
(axis cs:343.3479,-175.5411)
--(axis cs:341.6186,-185.3981);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:341.6186,-185.3981)
--(axis cs:339.0784,-195.0746);

\path [draw=lightgray!69.54248366013073!black, line width=4.0pt]
(axis cs:339.0784,-195.0746)
--(axis cs:335.2924,-204.3284);

\path [draw=lightgray!19.869281045751638!black, line width=4.0pt]
(axis cs:335.2924,-204.3284)
--(axis cs:330.0462,-212.834);

\path [draw=lightgray!47.58169934640524!black, line width=4.0pt]
(axis cs:330.0462,-212.834)
--(axis cs:323.2118,-220.1137);

\path [draw=lightgray!95.68627450980392!black, line width=4.0pt]
(axis cs:323.2118,-220.1137)
--(axis cs:314.8874,-225.6253);

\path [draw=lightgray!36.60130718954249!black, line width=4.0pt]
(axis cs:314.8874,-225.6253)
--(axis cs:305.5398,-229.1319);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:305.5398,-229.1319)
--(axis cs:295.641,-230.4422);

\path [draw=lightgray!29.80392156862745!black, line width=4.0pt]
(axis cs:295.641,-230.4422)
--(axis cs:285.6767,-229.6874);

\path [draw=lightgray!46.01307189542484!black, line width=4.0pt]
(axis cs:285.6767,-229.6874)
--(axis cs:275.9511,-227.3606);

\path [draw=white!77.64705882352942!black, line width=4.0pt]
(axis cs:275.9511,-227.3606)
--(axis cs:266.57,-223.8839);

\path [draw=lightgray!63.79084967320261!black, line width=4.0pt]
(axis cs:266.57,-223.8839)
--(axis cs:257.5246,-219.6033);

\path [draw=lightgray!7.843137254901962!black, line width=4.0pt]
(axis cs:257.5246,-219.6033)
--(axis cs:248.7385,-214.8102);

\path [draw=lightgray!80.52287581699348!black, line width=4.0pt]
(axis cs:248.7385,-214.8102)
--(axis cs:240.1459,-209.6768);

\path [draw=lightgray!35.03267973856208!black, line width=4.0pt]
(axis cs:240.1459,-209.6768)
--(axis cs:231.6964,-204.3108);

\path [draw=lightgray!51.764705882352935!black, line width=4.0pt]
(axis cs:231.6964,-204.3108)
--(axis cs:223.3482,-198.7883);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:223.3482,-198.7883)
--(axis cs:215.0582,-193.1787);

\path [draw=lightgray!70.06535947712419!black, line width=4.0pt]
(axis cs:215.0582,-193.1787)
--(axis cs:206.7879,-187.54);

\path [draw=lightgray!66.40522875816993!black, line width=4.0pt]
(axis cs:206.7879,-187.54)
--(axis cs:198.5222,-181.8944);

\path [draw=lightgray!64.83660130718954!black, line width=4.0pt]
(axis cs:198.5222,-181.8944)
--(axis cs:190.2547,-176.2516);

\path [draw=lightgray!46.01307189542484!black, line width=4.0pt]
(axis cs:190.2547,-176.2516)
--(axis cs:181.9793,-170.6204);

\path [draw=lightgray!10.98039215686275!black, line width=4.0pt]
(axis cs:181.9793,-170.6204)
--(axis cs:173.6925,-165.0059);

\path [draw=lightgray!46.5359477124183!black, line width=4.0pt]
(axis cs:173.6925,-165.0059)
--(axis cs:165.3952,-159.4069);

\path [draw=lightgray!89.41176470588236!black, line width=4.0pt]
(axis cs:165.3952,-159.4069)
--(axis cs:157.0892,-153.8209);

\path [draw=lightgray!65.359477124183!black, line width=4.0pt]
(axis cs:157.0892,-153.8209)
--(axis cs:148.7761,-148.2455);

\path [draw=lightgray!40.7843137254902!black, line width=4.0pt]
(axis cs:148.7761,-148.2455)
--(axis cs:140.4573,-142.6785);

\path [draw=lightgray!75.81699346405229!black, line width=4.0pt]
(axis cs:140.4573,-142.6785)
--(axis cs:132.1346,-137.1175);

\path [draw=lightgray!52.28758169934641!black, line width=4.0pt]
(axis cs:132.1346,-137.1175)
--(axis cs:123.8091,-131.5605);

\path [draw=lightgray!91.50326797385621!black, line width=4.0pt]
(axis cs:123.8091,-131.5605)
--(axis cs:115.4816,-126.0066);

\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:115.4816,-126.0066)
--(axis cs:107.1524,-120.4553);

\path [draw=black, line width=4.0pt]
(axis cs:107.1524,-120.4553)
--(axis cs:98.8217,-114.9061);

\path [draw=lightgray!49.150326797385624!black, line width=4.0pt]
(axis cs:98.8217,-114.9061)
--(axis cs:90.4897,-109.359);

\path [draw=lightgray!21.960784313725487!black, line width=4.0pt]
(axis cs:90.4897,-109.359)
--(axis cs:82.1565,-103.8136);

\path [draw=lightgray!77.90849673202615!black, line width=4.0pt]
(axis cs:82.1565,-103.8136)
--(axis cs:73.8224,-98.2696);

\path [draw=lightgray!64.83660130718954!black, line width=4.0pt]
(axis cs:73.8224,-98.2696)
--(axis cs:65.4875,-92.7269);

\path [draw=lightgray!37.12418300653595!black, line width=4.0pt]
(axis cs:65.4875,-92.7269)
--(axis cs:57.152,-87.185);

\path [draw=lightgray!73.72549019607844!black, line width=4.0pt]
(axis cs:57.152,-87.185)
--(axis cs:48.816,-81.6438);

\path [draw=lightgray!70.58823529411765!black, line width=4.0pt]
(axis cs:48.816,-81.6438)
--(axis cs:40.4798,-76.103);

\path [draw=lightgray!20.3921568627451!black, line width=4.0pt]
(axis cs:40.4798,-76.103)
--(axis cs:32.1435,-70.5622);

\path [draw=lightgray!41.830065359477125!black, line width=4.0pt]
(axis cs:32.1435,-70.5622)
--(axis cs:23.8073,-65.0213);

\path [draw=lightgray!39.215686274509814!black, line width=4.0pt]
(axis cs:23.8073,-65.0213)
--(axis cs:15.4715,-59.48);

\path [draw=lightgray!66.92810457516339!black, line width=4.0pt]
(axis cs:15.4715,-59.48)
--(axis cs:7.136,-53.9381);

\path [draw=lightgray!58.56209150326798!black, line width=4.0pt]
(axis cs:7.136,-53.9381)
--(axis cs:-1.1994,-48.396);

==> ressources/variable_friction/friction_low.tex <==
\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:-1.1994,-48.396)
--(axis cs:-9.5349,-42.8542);

\path [draw=lightgray!34.50980392156862!black, line width=4.0pt]
(axis cs:-9.5349,-42.8542)
--(axis cs:-17.8707,-37.3127);

\path [draw=lightgray!44.96732026143791!black, line width=4.0pt]
(axis cs:-17.8707,-37.3127)
--(axis cs:-26.2068,-31.7716);

\path [draw=lightgray!60.130718954248366!black, line width=4.0pt]
(axis cs:-26.2068,-31.7716)
--(axis cs:-34.5431,-26.231);

\path [draw=lightgray!64.31372549019608!black, line width=4.0pt]
(axis cs:-34.5431,-26.231)
--(axis cs:-42.8798,-20.6909);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:-42.8798,-20.6909)
--(axis cs:-51.2169,-15.1513);

\path [draw=lightgray!40.26143790849674!black, line width=4.0pt]
(axis cs:-51.2169,-15.1513)
--(axis cs:-59.5543,-9.6123);

\path [draw=lightgray!55.94771241830067!black, line width=4.0pt]
(axis cs:-59.5543,-9.6123)
--(axis cs:-67.8921,-4.0739);

\path [draw=lightgray!37.12418300653595!black, line width=4.0pt]
(axis cs:-67.8921,-4.0739)
--(axis cs:-76.2303,1.4639);

\path [draw=lightgray!44.44444444444445!black, line width=4.0pt]
(axis cs:-76.2303,1.4639)
--(axis cs:-84.569,7.001);

\path [draw=lightgray!54.37908496732026!black, line width=4.0pt]
(axis cs:-84.569,7.001)
--(axis cs:-92.9081,12.5375);

\path [draw=lightgray!53.8562091503268!black, line width=4.0pt]
(axis cs:-92.9081,12.5375)
--(axis cs:-101.2478,18.0731);

\path [draw=lightgray!17.77777777777777!black, line width=4.0pt]
(axis cs:-101.2478,18.0731)
--(axis cs:-109.5879,23.608);

\path [draw=lightgray!66.92810457516339!black, line width=4.0pt]
(axis cs:-109.5879,23.608)
--(axis cs:-117.9286,29.1421);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:-117.9286,29.1421)
--(axis cs:-126.2699,34.6753);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:-126.2699,34.6753)
--(axis cs:-134.6118,40.2076);

\path [draw=lightgray!72.15686274509805!black, line width=4.0pt]
(axis cs:-134.6118,40.2076)
--(axis cs:-142.9543,45.7389);

\path [draw=lightgray!61.69934640522876!black, line width=4.0pt]
(axis cs:-142.9543,45.7389)
--(axis cs:-151.2974,51.2693);

\path [draw=lightgray!42.87581699346405!black, line width=4.0pt]
(axis cs:-151.2974,51.2693)
--(axis cs:-159.6412,56.7987);

\path [draw=lightgray!46.5359477124183!black, line width=4.0pt]
(axis cs:-159.6412,56.7987)
--(axis cs:-167.9857,62.3271);

\path [draw=white!84.70588235294117!black, line width=4.0pt]
(axis cs:-167.9857,62.3271)
--(axis cs:-176.3309,67.8544);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-176.3309,67.8544)
--(axis cs:-184.6768,73.3805);

\path [draw=lightgray!79.47712418300654!black, line width=4.0pt]
(axis cs:-184.6768,73.3805)
--(axis cs:-193.0235,78.9055);

\path [draw=lightgray!44.44444444444445!black, line width=4.0pt]
(axis cs:-193.0235,78.9055)
--(axis cs:-201.371,84.4294);

\path [draw=lightgray!43.39869281045751!black, line width=4.0pt]
(axis cs:-201.371,84.4294)
--(axis cs:-209.7193,89.952);

\path [draw=lightgray!48.1045751633987!black, line width=4.0pt]
(axis cs:-209.7193,89.952)
--(axis cs:-218.0685,95.4733);

\path [draw=lightgray!24.05228758169935!black, line width=4.0pt]
(axis cs:-218.0685,95.4733)
--(axis cs:-226.4185,100.9933);

\path [draw=lightgray!42.87581699346405!black, line width=4.0pt]
(axis cs:-226.4185,100.9933)
--(axis cs:-234.7693,106.512);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-234.7693,106.512)
--(axis cs:-243.1211,112.0293);

\path [draw=lightgray!57.516339869281055!black, line width=4.0pt]
(axis cs:-243.1211,112.0293)
--(axis cs:-251.4738,117.5453);

\path [draw=lightgray!47.05882352941176!black, line width=4.0pt]
(axis cs:-251.4738,117.5453)
--(axis cs:-259.8272,123.0602);

\path [draw=lightgray!30.849673202614387!black, line width=4.0pt]
(axis cs:-259.8272,123.0602)
--(axis cs:-268.1812,128.5741);

\path [draw=lightgray!63.79084967320261!black, line width=4.0pt]
(axis cs:-268.1812,128.5741)
--(axis cs:-276.5358,134.0872);

\path [draw=lightgray!49.150326797385624!black, line width=4.0pt]
(axis cs:-276.5358,134.0872)
--(axis cs:-284.891,139.5994);

\path [draw=lightgray!67.97385620915031!black, line width=4.0pt]
(axis cs:-284.891,139.5994)
--(axis cs:-293.2466,145.111);

\path [draw=lightgray!62.22222222222222!black, line width=4.0pt]
(axis cs:-293.2466,145.111)
--(axis cs:-301.6025,150.622);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-301.6025,150.622)
--(axis cs:-309.9589,156.1324);

\path [draw=lightgray!68.49673202614377!black, line width=4.0pt]
(axis cs:-309.9589,156.1324)
--(axis cs:-318.3155,161.6424);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-318.3155,161.6424)
--(axis cs:-326.6724,167.152);

\path [draw=lightgray!42.87581699346405!black, line width=4.0pt]
(axis cs:-326.6724,167.152)
--(axis cs:-335.0295,172.6613);

\path [draw=lightgray!70.58823529411765!black, line width=4.0pt]
(axis cs:-335.0295,172.6613)
--(axis cs:-343.3866,178.1705);

\path [draw=lightgray!76.86274509803921!black, line width=4.0pt]
(axis cs:-343.3866,178.1705)
--(axis cs:-351.7439,183.6795);

\path [draw=lightgray!61.69934640522876!black, line width=4.0pt]
(axis cs:-351.7439,183.6795)
--(axis cs:-360.1012,189.1885);

\path [draw=lightgray!28.235294117647065!black, line width=4.0pt]
(axis cs:-360.1012,189.1885)
--(axis cs:-368.4584,194.6976);

\path [draw=lightgray!63.79084967320261!black, line width=4.0pt]
(axis cs:-368.4584,194.6976)
--(axis cs:-376.8155,200.2069);

\path [draw=lightgray!67.45098039215685!black, line width=4.0pt]
(axis cs:-376.8155,200.2069)
--(axis cs:-385.1724,205.7165);

\path [draw=lightgray!51.764705882352935!black, line width=4.0pt]
(axis cs:-385.1724,205.7165)
--(axis cs:-393.5287,211.2269);

\path [draw=lightgray!84.18300653594771!black, line width=4.0pt]
(axis cs:-393.5287,211.2269)
--(axis cs:-401.8843,216.7385);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:-401.8843,216.7385)
--(axis cs:-410.2388,222.2516);

\path [draw=white!78.43137254901961!black, line width=4.0pt]
(axis cs:-410.2388,222.2516)
--(axis cs:-418.592,227.7668);

\path [draw=lightgray!70.58823529411765!black, line width=4.0pt]
(axis cs:-418.592,227.7668)
--(axis cs:-426.9436,233.2844);

\path [draw=lightgray!35.555555555555564!black, line width=4.0pt]
(axis cs:-426.9436,233.2844)
--(axis cs:-435.2933,238.8049);

\path [draw=lightgray!75.29411764705883!black, line width=4.0pt]
(axis cs:-435.2933,238.8049)
--(axis cs:-443.6409,244.3285);

\path [draw=lightgray!58.56209150326798!black, line width=4.0pt]
(axis cs:-443.6409,244.3285)
--(axis cs:-451.9861,249.8559);

\path [draw=white!76.07843137254902!black, line width=4.0pt]
(axis cs:-451.9861,249.8559)
--(axis cs:-460.3286,255.3873);

\path [draw=lightgray!50.19607843137255!black, line width=4.0pt]
(axis cs:-460.3286,255.3873)
--(axis cs:-468.6681,260.9231);

\path [draw=lightgray!78.43137254901961!black, line width=4.0pt]
(axis cs:-468.6681,260.9231)
--(axis cs:-477.0043,266.4639);

\path [draw=lightgray!40.7843137254902!black, line width=4.0pt]
(axis cs:-477.0043,266.4639)
--(axis cs:-485.3371,272.0099);

\path [draw=lightgray!63.79084967320261!black, line width=4.0pt]
(axis cs:-485.3371,272.0099)
--(axis cs:-493.6661,277.5616);

\path [draw=lightgray!81.5686274509804!black, line width=4.0pt]
(axis cs:-493.6661,277.5616)
--(axis cs:-501.9815,283.1336);

\path [draw=lightgray!57.516339869281055!black, line width=4.0pt]
(axis cs:-501.9815,283.1336)
--(axis cs:-510.1823,288.8716);

\path [draw=lightgray!39.215686274509814!black, line width=4.0pt]
(axis cs:-510.1823,288.8716)
--(axis cs:-517.9559,295.1673);

\path [draw=lightgray!81.04575163398694!black, line width=4.0pt]
(axis cs:-517.9559,295.1673)
--(axis cs:-524.5873,302.6383);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:-524.5873,302.6383)
--(axis cs:-529.1885,311.4764);

\path [draw=lightgray!67.97385620915031!black, line width=4.0pt]
(axis cs:-529.1885,311.4764)
--(axis cs:-530.4952,321.3255);

\path [draw=lightgray!59.6078431372549!black, line width=4.0pt]
(axis cs:-530.4952,321.3255)
--(axis cs:-527.541,330.7944);

\path [draw=lightgray!51.764705882352935!black, line width=4.0pt]
(axis cs:-527.541,330.7944)
--(axis cs:-521.0243,338.2902);

\path [draw=lightgray!20.3921568627451!black, line width=4.0pt]
(axis cs:-521.0243,338.2902)
--(axis cs:-512.2902,343.0779);

\path [draw=lightgray!17.25490196078431!black, line width=4.0pt]
(axis cs:-512.2902,343.0779)
--(axis cs:-502.5372,345.1861);

\path [draw=lightgray!34.50980392156862!black, line width=4.0pt]
(axis cs:-502.5372,345.1861)
--(axis cs:-492.5422,345.2403);

\path [draw=lightgray!85.7516339869281!black, line width=4.0pt]
(axis cs:-492.5422,345.2403)
--(axis cs:-482.6228,343.9411);

\path [draw=white, line width=4.0pt]
(axis cs:-482.6228,343.9411)
--(axis cs:-472.8557,341.7641);

\path [draw=lightgray!46.01307189542484!black, line width=4.0pt]
(axis cs:-472.8557,341.7641)
--(axis cs:-463.2668,338.9004);

\path [draw=lightgray!76.86274509803921!black, line width=4.0pt]
(axis cs:-463.2668,338.9004)
--(axis cs:-453.8778,335.4356);

\path [draw=lightgray!70.06535947712419!black, line width=4.0pt]
(axis cs:-453.8778,335.4356)
--(axis cs:-444.7102,331.4211);

\path [draw=lightgray!86.27450980392157!black, line width=4.0pt]
(axis cs:-444.7102,331.4211)
--(axis cs:-435.7665,326.929);

\path [draw=lightgray!72.15686274509805!black, line width=4.0pt]
(axis cs:-435.7665,326.929)
--(axis cs:-427.0374,322.0323);

\path [draw=lightgray!50.71895424836601!black, line width=4.0pt]
(axis cs:-427.0374,322.0323)
--(axis cs:-418.5028,316.8032);

\path [draw=lightgray!94.11764705882352!black, line width=4.0pt]
(axis cs:-418.5028,316.8032)
--(axis cs:-410.1326,311.3146);

\path [draw=white!81.96078431372548!black, line width=4.0pt]
(axis cs:-410.1326,311.3146)
--(axis cs:-401.9019,305.6186);

\path [draw=lightgray!30.326797385620914!black, line width=4.0pt]
(axis cs:-401.9019,305.6186)
--(axis cs:-393.7647,299.7896);

\path [draw=lightgray!30.849673202614387!black, line width=4.0pt]
(axis cs:-393.7647,299.7896)
--(axis cs:-385.6672,293.9054);

\path [draw=lightgray!40.26143790849674!black, line width=4.0pt]
(axis cs:-385.6672,293.9054)
--(axis cs:-377.5663,288.0259);

\path [draw=lightgray!61.69934640522876!black, line width=4.0pt]
(axis cs:-377.5663,288.0259)
--(axis cs:-369.4533,282.163);

\path [draw=lightgray!17.77777777777777!black, line width=4.0pt]
(axis cs:-369.4533,282.163)
--(axis cs:-361.3271,276.3187);

\path [draw=lightgray!73.72549019607844!black, line width=4.0pt]
(axis cs:-361.3271,276.3187)
--(axis cs:-353.1078,270.6062);

\path [draw=lightgray!18.823529411764714!black, line width=4.0pt]
(axis cs:-353.1078,270.6062)
--(axis cs:-344.7821,265.0501);

\path [draw=lightgray!67.45098039215685!black, line width=4.0pt]
(axis cs:-344.7821,265.0501)
--(axis cs:-336.1884,259.9258);

\path [draw=lightgray!77.38562091503267!black, line width=4.0pt]
(axis cs:-336.1884,259.9258)
--(axis cs:-327.0159,255.9504);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:-327.0159,255.9504)
--(axis cs:-317.2399,253.9848);

\path [draw=lightgray!28.235294117647065!black, line width=4.0pt]
(axis cs:-317.2399,253.9848)
--(axis cs:-307.3934,255.3083);

\path [draw=lightgray!27.18954248366014!black, line width=4.0pt]
(axis cs:-307.3934,255.3083)
--(axis cs:-298.9726,260.5441);

\path [draw=white!76.47058823529412!black, line width=4.0pt]
(axis cs:-298.9726,260.5441)
--(axis cs:-293.4551,268.7963);

\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:-293.4551,268.7963)
--(axis cs:-290.9505,278.4527);

\path [draw=lightgray!17.77777777777777!black, line width=4.0pt]
(axis cs:-290.9505,278.4527)
--(axis cs:-290.1581,288.4283);

\path [draw=lightgray!64.83660130718954!black, line width=4.0pt]
(axis cs:-290.1581,288.4283)
--(axis cs:-289.0812,298.3724);

\path [draw=lightgray!38.69281045751634!black, line width=4.0pt]
(axis cs:-289.0812,298.3724)
--(axis cs:-286.2447,307.9439);

\path [draw=lightgray!49.150326797385624!black, line width=4.0pt]
(axis cs:-286.2447,307.9439)
--(axis cs:-281.045,316.4579);

\path [draw=lightgray!31.37254901960785!black, line width=4.0pt]
(axis cs:-281.045,316.4579)
--(axis cs:-273.8621,323.3829);

\path [draw=lightgray!52.81045751633987!black, line width=4.0pt]
(axis cs:-273.8621,323.3829)
--(axis cs:-265.2129,328.3673);

\path [draw=lightgray!37.12418300653595!black, line width=4.0pt]
(axis cs:-265.2129,328.3673)
--(axis cs:-255.6729,331.3363);

\path [draw=lightgray!79.47712418300654!black, line width=4.0pt]
(axis cs:-255.6729,331.3363)
--(axis cs:-245.7629,332.6653);

\path [draw=lightgray!34.50980392156862!black, line width=4.0pt]
(axis cs:-245.7629,332.6653)
--(axis cs:-235.7592,332.7092);

\path [draw=lightgray!64.83660130718954!black, line width=4.0pt]
(axis cs:-235.7592,332.7092)
--(axis cs:-225.7862,331.8767);

\path [draw=lightgray!58.56209150326798!black, line width=4.0pt]
(axis cs:-225.7862,331.8767)
--(axis cs:-215.8554,330.6253);

\path [draw=lightgray!21.960784313725487!black, line width=4.0pt]
(axis cs:-215.8554,330.6253)
--(axis cs:-205.9552,329.151);

\path [draw=lightgray!47.05882352941176!black, line width=4.0pt]
(axis cs:-205.9552,329.151)
--(axis cs:-196.0844,327.4902);

\path [draw=lightgray!68.49673202614377!black, line width=4.0pt]
(axis cs:-196.0844,327.4902)
--(axis cs:-186.2429,325.6638);

\path [draw=lightgray!48.1045751633987!black, line width=4.0pt]
(axis cs:-186.2429,325.6638)
--(axis cs:-176.4462,323.612);

\path [draw=lightgray!58.03921568627452!black, line width=4.0pt]
(axis cs:-176.4462,323.612)
--(axis cs:-166.7136,321.2753);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:-166.7136,321.2753)
--(axis cs:-157.0649,318.6138);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-157.0649,318.6138)
--(axis cs:-147.5264,315.5818);

\path [draw=lightgray!28.758169934640527!black, line width=4.0pt]
(axis cs:-147.5264,315.5818)
--(axis cs:-138.1414,312.1048);

\path [draw=lightgray!71.63398692810458!black, line width=4.0pt]
(axis cs:-138.1414,312.1048)
--(axis cs:-128.9394,308.1688);

\path [draw=lightgray!60.130718954248366!black, line width=4.0pt]
(axis cs:-128.9394,308.1688)
--(axis cs:-119.9374,303.7943);

\path [draw=lightgray!71.63398692810458!black, line width=4.0pt]
(axis cs:-119.9374,303.7943)
--(axis cs:-111.1463,299.0101);

\path [draw=lightgray!3.137254901960788!black, line width=4.0pt]
(axis cs:-111.1463,299.0101)
--(axis cs:-102.5719,293.8472);

\path [draw=lightgray!31.89542483660131!black, line width=4.0pt]
(axis cs:-102.5719,293.8472)
--(axis cs:-94.2249,288.3242);

\path [draw=lightgray!96.73202614379085!black, line width=4.0pt]
(axis cs:-94.2249,288.3242)
--(axis cs:-86.1059,282.471);

\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:-86.1059,282.471)
--(axis cs:-78.1987,276.3343);

\path [draw=lightgray!72.67973856209152!black, line width=4.0pt]
(axis cs:-78.1987,276.3343)
--(axis cs:-70.4884,269.9518);

\path [draw=lightgray!53.333333333333336!black, line width=4.0pt]
(axis cs:-70.4884,269.9518)
--(axis cs:-62.9535,263.363);

\path [draw=lightgray!48.1045751633987!black, line width=4.0pt]
(axis cs:-62.9535,263.363)
--(axis cs:-55.572,256.6027);

\path [draw=lightgray!48.1045751633987!black, line width=4.0pt]
(axis cs:-55.572,256.6027)
--(axis cs:-48.3241,249.6993);

\path [draw=lightgray!52.28758169934641!black, line width=4.0pt]
(axis cs:-48.3241,249.6993)
--(axis cs:-41.1822,242.686);

\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:-41.1822,242.686)
--(axis cs:-34.1192,235.5933);

\path [draw=lightgray!58.03921568627452!black, line width=4.0pt]
(axis cs:-34.1192,235.5933)
--(axis cs:-27.1104,228.447);

\path [draw=lightgray!56.99346405228759!black, line width=4.0pt]
(axis cs:-27.1104,228.447)
--(axis cs:-20.1405,221.2628);

\path [draw=lightgray!92.02614379084967!black, line width=4.0pt]
(axis cs:-20.1405,221.2628)
--(axis cs:-13.1998,214.0503);

\path [draw=lightgray!65.88235294117646!black, line width=4.0pt]
(axis cs:-13.1998,214.0503)
--(axis cs:-6.2795,206.8183);

\path [draw=lightgray!94.640522875817!black, line width=4.0pt]
(axis cs:-6.2795,206.8183)
--(axis cs:0.6303,199.5761);

\path [draw=lightgray!67.45098039215685!black, line width=4.0pt]
(axis cs:0.6303,199.5761)
--(axis cs:7.5388,192.3329);

\path [draw=lightgray!51.24183006535947!black, line width=4.0pt]
(axis cs:7.5388,192.3329)
--(axis cs:14.4559,185.0977);

\path [draw=lightgray!70.58823529411765!black, line width=4.0pt]
(axis cs:14.4559,185.0977)
--(axis cs:21.3908,177.8796);

\path [draw=lightgray!53.8562091503268!black, line width=4.0pt]
(axis cs:21.3908,177.8796)
--(axis cs:28.3522,170.6872);

\path [draw=lightgray!47.58169934640524!black, line width=4.0pt]
(axis cs:28.3522,170.6872)
--(axis cs:35.347,163.5272);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:35.347,163.5272)
--(axis cs:42.3792,156.4039);

\path [draw=lightgray!96.20915032679738!black, line width=4.0pt]
(axis cs:42.3792,156.4039)
--(axis cs:49.4537,149.3226);

\path [draw=lightgray!16.732026143790847!black, line width=4.0pt]
(axis cs:49.4537,149.3226)
--(axis cs:56.5762,142.2897);

\path [draw=lightgray!41.830065359477125!black, line width=4.0pt]
(axis cs:56.5762,142.2897)
--(axis cs:63.7503,135.3093);

\path [draw=lightgray!40.7843137254902!black, line width=4.0pt]
(axis cs:63.7503,135.3093)
--(axis cs:70.9792,128.3858);

\path [draw=lightgray!58.56209150326798!black, line width=4.0pt]
(axis cs:70.9792,128.3858)
--(axis cs:78.2484,121.5045);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:78.2484,121.5045)
--(axis cs:85.5382,114.6451);

\path [draw=lightgray!59.08496732026144!black, line width=4.0pt]
(axis cs:85.5382,114.6451)
--(axis cs:92.851,107.8101);

\path [draw=lightgray!65.359477124183!black, line width=4.0pt]
(axis cs:92.851,107.8101)
--(axis cs:100.1909,101.0044);

\path [draw=lightgray!66.40522875816993!black, line width=4.0pt]
(axis cs:100.1909,101.0044)
--(axis cs:107.5806,94.2528);

\path [draw=lightgray!40.26143790849674!black, line width=4.0pt]
(axis cs:107.5806,94.2528)
--(axis cs:115.1067,87.6541);

\path [draw=lightgray!43.92156862745099!black, line width=4.0pt]
(axis cs:115.1067,87.6541)
--(axis cs:122.8881,81.3596);

\path [draw=lightgray!54.37908496732026!black, line width=4.0pt]
(axis cs:122.8881,81.3596)
--(axis cs:131.0096,75.5123);

\path [draw=lightgray!28.235294117647065!black, line width=4.0pt]
(axis cs:131.0096,75.5123)
--(axis cs:139.5498,70.2979);

\path [draw=lightgray!49.150326797385624!black, line width=4.0pt]
(axis cs:139.5498,70.2979)
--(axis cs:148.5069,65.8378);

\path [draw=lightgray!80.52287581699348!black, line width=4.0pt]
(axis cs:148.5069,65.8378)
--(axis cs:157.8094,62.1524);

\path [draw=lightgray!92.02614379084967!black, line width=4.0pt]
(axis cs:157.8094,62.1524)
--(axis cs:167.3963,59.2872);

\path [draw=lightgray!33.464052287581694!black, line width=4.0pt]
(axis cs:167.3963,59.2872)
--(axis cs:177.2027,57.2999);

\path [draw=lightgray!80.52287581699348!black, line width=4.0pt]
(axis cs:177.2027,57.2999)
--(axis cs:187.1481,56.2066);

\path [draw=lightgray!13.0718954248366!black, line width=4.0pt]
(axis cs:187.1481,56.2066)
--(axis cs:197.1521,56.0381);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:197.1521,56.0381)
--(axis cs:207.1271,56.8173);

\path [draw=lightgray!52.28758169934641!black, line width=4.0pt]
(axis cs:207.1271,56.8173)
--(axis cs:216.999,58.453);

\path [draw=lightgray!50.19607843137255!black, line width=4.0pt]
(axis cs:216.999,58.453)
--(axis cs:226.7268,60.8026);

\path [draw=lightgray!33.464052287581694!black, line width=4.0pt]
(axis cs:226.7268,60.8026)
--(axis cs:236.3057,63.7036);

\path [draw=white!81.17647058823529!black, line width=4.0pt]
(axis cs:236.3057,63.7036)
--(axis cs:245.7969,66.883);

\path [draw=lightgray!27.712418300653603!black, line width=4.0pt]
(axis cs:245.7969,66.883)
--(axis cs:255.3044,70.013);

\path [draw=lightgray!57.516339869281055!black, line width=4.0pt]
(axis cs:255.3044,70.013)
--(axis cs:264.9253,72.7698);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:264.9253,72.7698)
--(axis cs:274.7143,74.8418);

\path [draw=lightgray!89.41176470588236!black, line width=4.0pt]
(axis cs:274.7143,74.8418)
--(axis cs:284.6604,75.9157);

\path [draw=lightgray!83.66013071895425!black, line width=4.0pt]
(axis cs:284.6604,75.9157)
--(axis cs:294.6635,75.8808);

\path [draw=lightgray!44.96732026143791!black, line width=4.0pt]
(axis cs:294.6635,75.8808)
--(axis cs:304.5966,74.7025);

\path [draw=lightgray!83.66013071895425!black, line width=4.0pt]
(axis cs:304.5966,74.7025)
--(axis cs:314.3088,72.3128);

\path [draw=lightgray!25.620915032679736!black, line width=4.0pt]
(axis cs:314.3088,72.3128)
--(axis cs:323.6198,68.6648);

\path [draw=lightgray!1.0457516339869244!black, line width=4.0pt]
(axis cs:323.6198,68.6648)
--(axis cs:332.3287,63.7516);

\path [draw=lightgray!67.97385620915031!black, line width=4.0pt]
(axis cs:332.3287,63.7516)
--(axis cs:340.1802,57.5628);

\path [draw=lightgray!25.620915032679736!black, line width=4.0pt]
(axis cs:340.1802,57.5628)
--(axis cs:346.9426,50.2003);

\path [draw=lightgray!9.93464052287581!black, line width=4.0pt]
(axis cs:346.9426,50.2003)
--(axis cs:352.498,41.8871);

\path [draw=lightgray!55.94771241830067!black, line width=4.0pt]
(axis cs:352.498,41.8871)
--(axis cs:356.7546,32.8381);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:356.7546,32.8381)
--(axis cs:359.7572,23.2982);	

\path [draw=lightgray!54.90196078431372!black, line width=4.0pt]
(axis cs:359.7572,23.2982)
--(axis cs:361.6308,13.471);

\path [draw=lightgray!58.03921568627452!black, line width=4.0pt]
(axis cs:361.6308,13.471)
--(axis cs:362.5213,3.5047);

\path [draw=lightgray!39.215686274509814!black, line width=4.0pt]
(axis cs:362.5213,3.5047)
--(axis cs:362.6164,-6.5018);

\path [draw=lightgray!62.745098039215684!black, line width=4.0pt]
(axis cs:362.6164,-6.5018)
--(axis cs:362.0877,-16.4961);

\path [draw=lightgray!69.54248366013073!black, line width=4.0pt]
(axis cs:362.0877,-16.4961)
--(axis cs:361.1467,-26.4611);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:361.1467,-26.4611)
--(axis cs:359.98,-36.4023);

\path [draw=lightgray!76.33986928104575!black, line width=4.0pt]
(axis cs:359.98,-36.4023)
--(axis cs:358.7131,-46.3315);

\path [draw=lightgray!69.01960784313724!black, line width=4.0pt]
(axis cs:358.7131,-46.3315)
--(axis cs:357.424,-56.2578);

\path [draw=lightgray!65.88235294117646!black, line width=4.0pt]
(axis cs:357.424,-56.2578)
--(axis cs:356.1224,-66.1825);

\path [draw=white!78.03921568627452!black, line width=4.0pt]
(axis cs:356.1224,-66.1825)
--(axis cs:354.8297,-76.1083);

\path [draw=lightgray!88.8888888888889!black, line width=4.0pt]
(axis cs:354.8297,-76.1083)
--(axis cs:353.5684,-86.0382);

\path [draw=white!78.82352941176471!black, line width=4.0pt]
(axis cs:353.5684,-86.0382)
--(axis cs:352.3545,-95.9739);

\path [draw=lightgray!54.90196078431372!black, line width=4.0pt]
(axis cs:352.3545,-95.9739)
--(axis cs:351.1846,-105.915);

\path [draw=lightgray!29.80392156862745!black, line width=4.0pt]
(axis cs:351.1846,-105.915)
--(axis cs:350.051,-115.8602);

\path [draw=lightgray!43.39869281045751!black, line width=4.0pt]
(axis cs:350.051,-115.8602)
--(axis cs:348.9443,-125.8085);

\path [draw=lightgray!7.3202614379085!black, line width=4.0pt]
(axis cs:348.9443,-125.8085)
--(axis cs:347.8561,-135.7588);

\path [draw=lightgray!21.437908496732025!black, line width=4.0pt]
(axis cs:347.8561,-135.7588)
--(axis cs:346.778,-145.7103);

\path [draw=lightgray!50.71895424836601!black, line width=4.0pt]
(axis cs:346.778,-145.7103)
--(axis cs:345.7015,-155.6619);

\path [draw=lightgray!65.359477124183!black, line width=4.0pt]
(axis cs:345.7015,-155.6619)
--(axis cs:344.6084,-165.6116);

\path [draw=lightgray!20.915032679738562!black, line width=4.0pt]
(axis cs:344.6084,-165.6116)
--(axis cs:343.3479,-175.5411);

\path [draw=lightgray!15.163398692810462!black, line width=4.0pt]
(axis cs:343.3479,-175.5411)
--(axis cs:341.6186,-185.3981);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:341.6186,-185.3981)
--(axis cs:339.0784,-195.0746);

\path [draw=lightgray!69.54248366013073!black, line width=4.0pt]
(axis cs:339.0784,-195.0746)
--(axis cs:335.2924,-204.3284);

\path [draw=lightgray!19.869281045751638!black, line width=4.0pt]
(axis cs:335.2924,-204.3284)
--(axis cs:330.0462,-212.834);

\path [draw=lightgray!47.58169934640524!black, line width=4.0pt]
(axis cs:330.0462,-212.834)
--(axis cs:323.2118,-220.1137);

\path [draw=lightgray!95.68627450980392!black, line width=4.0pt]
(axis cs:323.2118,-220.1137)
--(axis cs:314.8874,-225.6253);

\path [draw=lightgray!36.60130718954249!black, line width=4.0pt]
(axis cs:314.8874,-225.6253)
--(axis cs:305.5398,-229.1319);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:305.5398,-229.1319)
--(axis cs:295.641,-230.4422);

\path [draw=lightgray!29.80392156862745!black, line width=4.0pt]
(axis cs:295.641,-230.4422)
--(axis cs:285.6767,-229.6874);

\path [draw=lightgray!46.01307189542484!black, line width=4.0pt]
(axis cs:285.6767,-229.6874)
--(axis cs:275.9511,-227.3606);

\path [draw=white!77.64705882352942!black, line width=4.0pt]
(axis cs:275.9511,-227.3606)
--(axis cs:266.57,-223.8839);

\path [draw=lightgray!63.79084967320261!black, line width=4.0pt]
(axis cs:266.57,-223.8839)
--(axis cs:257.5246,-219.6033);

\path [draw=lightgray!7.843137254901962!black, line width=4.0pt]
(axis cs:257.5246,-219.6033)
--(axis cs:248.7385,-214.8102);

\path [draw=lightgray!80.52287581699348!black, line width=4.0pt]
(axis cs:248.7385,-214.8102)
--(axis cs:240.1459,-209.6768);

\path [draw=lightgray!35.03267973856208!black, line width=4.0pt]
(axis cs:240.1459,-209.6768)
--(axis cs:231.6964,-204.3108);

\path [draw=lightgray!51.764705882352935!black, line width=4.0pt]
(axis cs:231.6964,-204.3108)
--(axis cs:223.3482,-198.7883);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:223.3482,-198.7883)
--(axis cs:215.0582,-193.1787);

\path [draw=lightgray!70.06535947712419!black, line width=4.0pt]
(axis cs:215.0582,-193.1787)
--(axis cs:206.7879,-187.54);

\path [draw=lightgray!66.40522875816993!black, line width=4.0pt]
(axis cs:206.7879,-187.54)
--(axis cs:198.5222,-181.8944);

\path [draw=lightgray!64.83660130718954!black, line width=4.0pt]
(axis cs:198.5222,-181.8944)
--(axis cs:190.2547,-176.2516);

\path [draw=lightgray!46.01307189542484!black, line width=4.0pt]
(axis cs:190.2547,-176.2516)
--(axis cs:181.9793,-170.6204);

\path [draw=lightgray!10.98039215686275!black, line width=4.0pt]
(axis cs:181.9793,-170.6204)
--(axis cs:173.6925,-165.0059);

\path [draw=lightgray!46.5359477124183!black, line width=4.0pt]
(axis cs:173.6925,-165.0059)
--(axis cs:165.3952,-159.4069);

\path [draw=lightgray!89.41176470588236!black, line width=4.0pt]
(axis cs:165.3952,-159.4069)
--(axis cs:157.0892,-153.8209);

\path [draw=lightgray!65.359477124183!black, line width=4.0pt]
(axis cs:157.0892,-153.8209)
--(axis cs:148.7761,-148.2455);

\path [draw=lightgray!40.7843137254902!black, line width=4.0pt]
(axis cs:148.7761,-148.2455)
--(axis cs:140.4573,-142.6785);

\path [draw=lightgray!75.81699346405229!black, line width=4.0pt]
(axis cs:140.4573,-142.6785)
--(axis cs:132.1346,-137.1175);

\path [draw=lightgray!52.28758169934641!black, line width=4.0pt]
(axis cs:132.1346,-137.1175)
--(axis cs:123.8091,-131.5605);

\path [draw=lightgray!91.50326797385621!black, line width=4.0pt]
(axis cs:123.8091,-131.5605)
--(axis cs:115.4816,-126.0066);

\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:115.4816,-126.0066)
--(axis cs:107.1524,-120.4553);

\path [draw=black, line width=4.0pt]
(axis cs:107.1524,-120.4553)
--(axis cs:98.8217,-114.9061);

\path [draw=lightgray!49.150326797385624!black, line width=4.0pt]
(axis cs:98.8217,-114.9061)
--(axis cs:90.4897,-109.359);

\path [draw=lightgray!21.960784313725487!black, line width=4.0pt]
(axis cs:90.4897,-109.359)
--(axis cs:82.1565,-103.8136);

\path [draw=lightgray!77.90849673202615!black, line width=4.0pt]
(axis cs:82.1565,-103.8136)
--(axis cs:73.8224,-98.2696);

\path [draw=lightgray!64.83660130718954!black, line width=4.0pt]
(axis cs:73.8224,-98.2696)
--(axis cs:65.4875,-92.7269);

\path [draw=lightgray!37.12418300653595!black, line width=4.0pt]
(axis cs:65.4875,-92.7269)
--(axis cs:57.152,-87.185);

\path [draw=lightgray!73.72549019607844!black, line width=4.0pt]
(axis cs:57.152,-87.185)
--(axis cs:48.816,-81.6438);

\path [draw=lightgray!70.58823529411765!black, line width=4.0pt]
(axis cs:48.816,-81.6438)
--(axis cs:40.4798,-76.103);

\path [draw=lightgray!20.3921568627451!black, line width=4.0pt]
(axis cs:40.4798,-76.103)
--(axis cs:32.1435,-70.5622);

\path [draw=lightgray!41.830065359477125!black, line width=4.0pt]
(axis cs:32.1435,-70.5622)
--(axis cs:23.8073,-65.0213);

\path [draw=lightgray!39.215686274509814!black, line width=4.0pt]
(axis cs:23.8073,-65.0213)
--(axis cs:15.4715,-59.48);

\path [draw=lightgray!66.92810457516339!black, line width=4.0pt]
(axis cs:15.4715,-59.48)
--(axis cs:7.136,-53.9381);

\path [draw=lightgray!58.56209150326798!black, line width=4.0pt]
(axis cs:7.136,-53.9381)
--(axis cs:-1.1994,-48.396);

==> ressources/variable_friction/friction_medium.tex <==
\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:-1.1994,-48.396)
--(axis cs:-9.5349,-42.8542);

\path [draw=lightgray!34.50980392156862!black, line width=4.0pt]
(axis cs:-9.5349,-42.8542)
--(axis cs:-17.8707,-37.3127);

\path [draw=lightgray!44.96732026143791!black, line width=4.0pt]
(axis cs:-17.8707,-37.3127)
--(axis cs:-26.2068,-31.7716);

\path [draw=lightgray!60.130718954248366!black, line width=4.0pt]
(axis cs:-26.2068,-31.7716)
--(axis cs:-34.5431,-26.231);

\path [draw=lightgray!64.31372549019608!black, line width=4.0pt]
(axis cs:-34.5431,-26.231)
--(axis cs:-42.8798,-20.6909);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:-42.8798,-20.6909)
--(axis cs:-51.2169,-15.1513);

\path [draw=lightgray!40.26143790849674!black, line width=4.0pt]
(axis cs:-51.2169,-15.1513)
--(axis cs:-59.5543,-9.6123);

\path [draw=lightgray!55.94771241830067!black, line width=4.0pt]
(axis cs:-59.5543,-9.6123)
--(axis cs:-67.8921,-4.0739);

\path [draw=lightgray!37.12418300653595!black, line width=4.0pt]
(axis cs:-67.8921,-4.0739)
--(axis cs:-76.2303,1.4639);

\path [draw=lightgray!44.44444444444445!black, line width=4.0pt]
(axis cs:-76.2303,1.4639)
--(axis cs:-84.569,7.001);

\path [draw=lightgray!54.37908496732026!black, line width=4.0pt]
(axis cs:-84.569,7.001)
--(axis cs:-92.9081,12.5375);

\path [draw=lightgray!53.8562091503268!black, line width=4.0pt]
(axis cs:-92.9081,12.5375)
--(axis cs:-101.2478,18.0731);

\path [draw=lightgray!17.77777777777777!black, line width=4.0pt]
(axis cs:-101.2478,18.0731)
--(axis cs:-109.5879,23.608);

\path [draw=lightgray!66.92810457516339!black, line width=4.0pt]
(axis cs:-109.5879,23.608)
--(axis cs:-117.9286,29.1421);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:-117.9286,29.1421)
--(axis cs:-126.2699,34.6753);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:-126.2699,34.6753)
--(axis cs:-134.6118,40.2076);

\path [draw=lightgray!72.15686274509805!black, line width=4.0pt]
(axis cs:-134.6118,40.2076)
--(axis cs:-142.9543,45.7389);

\path [draw=lightgray!61.69934640522876!black, line width=4.0pt]
(axis cs:-142.9543,45.7389)
--(axis cs:-151.2974,51.2693);

\path [draw=lightgray!42.87581699346405!black, line width=4.0pt]
(axis cs:-151.2974,51.2693)
--(axis cs:-159.6412,56.7987);

\path [draw=lightgray!46.5359477124183!black, line width=4.0pt]
(axis cs:-159.6412,56.7987)
--(axis cs:-167.9857,62.3271);

\path [draw=white!84.70588235294117!black, line width=4.0pt]
(axis cs:-167.9857,62.3271)
--(axis cs:-176.3309,67.8544);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-176.3309,67.8544)
--(axis cs:-184.6768,73.3805);

\path [draw=lightgray!79.47712418300654!black, line width=4.0pt]
(axis cs:-184.6768,73.3805)
--(axis cs:-193.0235,78.9055);

\path [draw=lightgray!44.44444444444445!black, line width=4.0pt]
(axis cs:-193.0235,78.9055)
--(axis cs:-201.371,84.4294);

\path [draw=lightgray!43.39869281045751!black, line width=4.0pt]
(axis cs:-201.371,84.4294)
--(axis cs:-209.7193,89.952);

\path [draw=lightgray!48.1045751633987!black, line width=4.0pt]
(axis cs:-209.7193,89.952)
--(axis cs:-218.0685,95.4733);

\path [draw=lightgray!24.05228758169935!black, line width=4.0pt]
(axis cs:-218.0685,95.4733)
--(axis cs:-226.4185,100.9933);

\path [draw=lightgray!42.87581699346405!black, line width=4.0pt]
(axis cs:-226.4185,100.9933)
--(axis cs:-234.7693,106.512);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-234.7693,106.512)
--(axis cs:-243.1211,112.0293);

\path [draw=lightgray!57.516339869281055!black, line width=4.0pt]
(axis cs:-243.1211,112.0293)
--(axis cs:-251.4738,117.5453);

\path [draw=lightgray!47.05882352941176!black, line width=4.0pt]
(axis cs:-251.4738,117.5453)
--(axis cs:-259.8272,123.0602);

\path [draw=lightgray!30.849673202614387!black, line width=4.0pt]
(axis cs:-259.8272,123.0602)
--(axis cs:-268.1812,128.5741);

\path [draw=lightgray!63.79084967320261!black, line width=4.0pt]
(axis cs:-268.1812,128.5741)
--(axis cs:-276.5358,134.0872);

\path [draw=lightgray!49.150326797385624!black, line width=4.0pt]
(axis cs:-276.5358,134.0872)
--(axis cs:-284.891,139.5994);

\path [draw=lightgray!67.97385620915031!black, line width=4.0pt]
(axis cs:-284.891,139.5994)
--(axis cs:-293.2466,145.111);

\path [draw=lightgray!62.22222222222222!black, line width=4.0pt]
(axis cs:-293.2466,145.111)
--(axis cs:-301.6025,150.622);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-301.6025,150.622)
--(axis cs:-309.9589,156.1324);

\path [draw=lightgray!68.49673202614377!black, line width=4.0pt]
(axis cs:-309.9589,156.1324)
--(axis cs:-318.3155,161.6424);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-318.3155,161.6424)
--(axis cs:-326.6724,167.152);

\path [draw=lightgray!42.87581699346405!black, line width=4.0pt]
(axis cs:-326.6724,167.152)
--(axis cs:-335.0295,172.6613);

\path [draw=lightgray!70.58823529411765!black, line width=4.0pt]
(axis cs:-335.0295,172.6613)
--(axis cs:-343.3866,178.1705);

\path [draw=lightgray!76.86274509803921!black, line width=4.0pt]
(axis cs:-343.3866,178.1705)
--(axis cs:-351.7439,183.6795);

\path [draw=lightgray!61.69934640522876!black, line width=4.0pt]
(axis cs:-351.7439,183.6795)
--(axis cs:-360.1012,189.1885);

\path [draw=lightgray!28.235294117647065!black, line width=4.0pt]
(axis cs:-360.1012,189.1885)
--(axis cs:-368.4584,194.6976);

\path [draw=lightgray!63.79084967320261!black, line width=4.0pt]
(axis cs:-368.4584,194.6976)
--(axis cs:-376.8155,200.2069);

\path [draw=lightgray!67.45098039215685!black, line width=4.0pt]
(axis cs:-376.8155,200.2069)
--(axis cs:-385.1724,205.7165);

\path [draw=lightgray!51.764705882352935!black, line width=4.0pt]
(axis cs:-385.1724,205.7165)
--(axis cs:-393.5287,211.2269);

\path [draw=lightgray!84.18300653594771!black, line width=4.0pt]
(axis cs:-393.5287,211.2269)
--(axis cs:-401.8843,216.7385);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:-401.8843,216.7385)
--(axis cs:-410.2388,222.2516);

\path [draw=white!78.43137254901961!black, line width=4.0pt]
(axis cs:-410.2388,222.2516)
--(axis cs:-418.592,227.7668);

\path [draw=lightgray!70.58823529411765!black, line width=4.0pt]
(axis cs:-418.592,227.7668)
--(axis cs:-426.9436,233.2844);

\path [draw=lightgray!35.555555555555564!black, line width=4.0pt]
(axis cs:-426.9436,233.2844)
--(axis cs:-435.2933,238.8049);

\path [draw=lightgray!75.29411764705883!black, line width=4.0pt]
(axis cs:-435.2933,238.8049)
--(axis cs:-443.6409,244.3285);

\path [draw=lightgray!58.56209150326798!black, line width=4.0pt]
(axis cs:-443.6409,244.3285)
--(axis cs:-451.9861,249.8559);

\path [draw=white!76.07843137254902!black, line width=4.0pt]
(axis cs:-451.9861,249.8559)
--(axis cs:-460.3286,255.3873);

\path [draw=lightgray!50.19607843137255!black, line width=4.0pt]
(axis cs:-460.3286,255.3873)
--(axis cs:-468.6681,260.9231);

\path [draw=lightgray!78.43137254901961!black, line width=4.0pt]
(axis cs:-468.6681,260.9231)
--(axis cs:-477.0043,266.4639);

\path [draw=lightgray!40.7843137254902!black, line width=4.0pt]
(axis cs:-477.0043,266.4639)
--(axis cs:-485.3371,272.0099);

\path [draw=lightgray!63.79084967320261!black, line width=4.0pt]
(axis cs:-485.3371,272.0099)
--(axis cs:-493.6661,277.5616);

\path [draw=lightgray!81.5686274509804!black, line width=4.0pt]
(axis cs:-493.6661,277.5616)
--(axis cs:-501.9815,283.1336);

\path [draw=lightgray!57.516339869281055!black, line width=4.0pt]
(axis cs:-501.9815,283.1336)
--(axis cs:-510.1823,288.8716);

\path [draw=lightgray!39.215686274509814!black, line width=4.0pt]
(axis cs:-510.1823,288.8716)
--(axis cs:-517.9559,295.1673);

\path [draw=lightgray!81.04575163398694!black, line width=4.0pt]
(axis cs:-517.9559,295.1673)
--(axis cs:-524.5873,302.6383);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:-524.5873,302.6383)
--(axis cs:-529.1885,311.4764);

\path [draw=lightgray!67.97385620915031!black, line width=4.0pt]
(axis cs:-529.1885,311.4764)
--(axis cs:-530.4952,321.3255);

\path [draw=lightgray!59.6078431372549!black, line width=4.0pt]
(axis cs:-530.4952,321.3255)
--(axis cs:-527.541,330.7944);

\path [draw=lightgray!51.764705882352935!black, line width=4.0pt]
(axis cs:-527.541,330.7944)
--(axis cs:-521.0243,338.2902);

\path [draw=lightgray!20.3921568627451!black, line width=4.0pt]
(axis cs:-521.0243,338.2902)
--(axis cs:-512.2902,343.0779);

\path [draw=lightgray!17.25490196078431!black, line width=4.0pt]
(axis cs:-512.2902,343.0779)
--(axis cs:-502.5372,345.1861);

\path [draw=lightgray!34.50980392156862!black, line width=4.0pt]
(axis cs:-502.5372,345.1861)
--(axis cs:-492.5422,345.2403);

\path [draw=lightgray!85.7516339869281!black, line width=4.0pt]
(axis cs:-492.5422,345.2403)
--(axis cs:-482.6228,343.9411);

\path [draw=white, line width=4.0pt]
(axis cs:-482.6228,343.9411)
--(axis cs:-472.8557,341.7641);

\path [draw=lightgray!46.01307189542484!black, line width=4.0pt]
(axis cs:-472.8557,341.7641)
--(axis cs:-463.2668,338.9004);

\path [draw=lightgray!76.86274509803921!black, line width=4.0pt]
(axis cs:-463.2668,338.9004)
--(axis cs:-453.8778,335.4356);

\path [draw=lightgray!70.06535947712419!black, line width=4.0pt]
(axis cs:-453.8778,335.4356)
--(axis cs:-444.7102,331.4211);

\path [draw=lightgray!86.27450980392157!black, line width=4.0pt]
(axis cs:-444.7102,331.4211)
--(axis cs:-435.7665,326.929);

\path [draw=lightgray!72.15686274509805!black, line width=4.0pt]
(axis cs:-435.7665,326.929)
--(axis cs:-427.0374,322.0323);

\path [draw=lightgray!50.71895424836601!black, line width=4.0pt]
(axis cs:-427.0374,322.0323)
--(axis cs:-418.5028,316.8032);

\path [draw=lightgray!94.11764705882352!black, line width=4.0pt]
(axis cs:-418.5028,316.8032)
--(axis cs:-410.1326,311.3146);

\path [draw=white!81.96078431372548!black, line width=4.0pt]
(axis cs:-410.1326,311.3146)
--(axis cs:-401.9019,305.6186);

\path [draw=lightgray!30.326797385620914!black, line width=4.0pt]
(axis cs:-401.9019,305.6186)
--(axis cs:-393.7647,299.7896);

\path [draw=lightgray!30.849673202614387!black, line width=4.0pt]
(axis cs:-393.7647,299.7896)
--(axis cs:-385.6672,293.9054);

\path [draw=lightgray!40.26143790849674!black, line width=4.0pt]
(axis cs:-385.6672,293.9054)
--(axis cs:-377.5663,288.0259);

\path [draw=lightgray!61.69934640522876!black, line width=4.0pt]
(axis cs:-377.5663,288.0259)
--(axis cs:-369.4533,282.163);

\path [draw=lightgray!17.77777777777777!black, line width=4.0pt]
(axis cs:-369.4533,282.163)
--(axis cs:-361.3271,276.3187);

\path [draw=lightgray!73.72549019607844!black, line width=4.0pt]
(axis cs:-361.3271,276.3187)
--(axis cs:-353.1078,270.6062);

\path [draw=lightgray!18.823529411764714!black, line width=4.0pt]
(axis cs:-353.1078,270.6062)
--(axis cs:-344.7821,265.0501);

\path [draw=lightgray!67.45098039215685!black, line width=4.0pt]
(axis cs:-344.7821,265.0501)
--(axis cs:-336.1884,259.9258);

\path [draw=lightgray!77.38562091503267!black, line width=4.0pt]
(axis cs:-336.1884,259.9258)
--(axis cs:-327.0159,255.9504);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:-327.0159,255.9504)
--(axis cs:-317.2399,253.9848);

\path [draw=lightgray!28.235294117647065!black, line width=4.0pt]
(axis cs:-317.2399,253.9848)
--(axis cs:-307.3934,255.3083);

\path [draw=lightgray!27.18954248366014!black, line width=4.0pt]
(axis cs:-307.3934,255.3083)
--(axis cs:-298.9726,260.5441);

\path [draw=white!76.47058823529412!black, line width=4.0pt]
(axis cs:-298.9726,260.5441)
--(axis cs:-293.4551,268.7963);

\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:-293.4551,268.7963)
--(axis cs:-290.9505,278.4527);

\path [draw=lightgray!17.77777777777777!black, line width=4.0pt]
(axis cs:-290.9505,278.4527)
--(axis cs:-290.1581,288.4283);

\path [draw=lightgray!64.83660130718954!black, line width=4.0pt]
(axis cs:-290.1581,288.4283)
--(axis cs:-289.0812,298.3724);

\path [draw=lightgray!38.69281045751634!black, line width=4.0pt]
(axis cs:-289.0812,298.3724)
--(axis cs:-286.2447,307.9439);

\path [draw=lightgray!49.150326797385624!black, line width=4.0pt]
(axis cs:-286.2447,307.9439)
--(axis cs:-281.045,316.4579);

\path [draw=lightgray!31.37254901960785!black, line width=4.0pt]
(axis cs:-281.045,316.4579)
--(axis cs:-273.8621,323.3829);

\path [draw=lightgray!52.81045751633987!black, line width=4.0pt]
(axis cs:-273.8621,323.3829)
--(axis cs:-265.2129,328.3673);

\path [draw=lightgray!37.12418300653595!black, line width=4.0pt]
(axis cs:-265.2129,328.3673)
--(axis cs:-255.6729,331.3363);

\path [draw=lightgray!79.47712418300654!black, line width=4.0pt]
(axis cs:-255.6729,331.3363)
--(axis cs:-245.7629,332.6653);

\path [draw=lightgray!34.50980392156862!black, line width=4.0pt]
(axis cs:-245.7629,332.6653)
--(axis cs:-235.7592,332.7092);

\path [draw=lightgray!64.83660130718954!black, line width=4.0pt]
(axis cs:-235.7592,332.7092)
--(axis cs:-225.7862,331.8767);

\path [draw=lightgray!58.56209150326798!black, line width=4.0pt]
(axis cs:-225.7862,331.8767)
--(axis cs:-215.8554,330.6253);

\path [draw=lightgray!21.960784313725487!black, line width=4.0pt]
(axis cs:-215.8554,330.6253)
--(axis cs:-205.9552,329.151);

\path [draw=lightgray!47.05882352941176!black, line width=4.0pt]
(axis cs:-205.9552,329.151)
--(axis cs:-196.0844,327.4902);

\path [draw=lightgray!68.49673202614377!black, line width=4.0pt]
(axis cs:-196.0844,327.4902)
--(axis cs:-186.2429,325.6638);

\path [draw=lightgray!48.1045751633987!black, line width=4.0pt]
(axis cs:-186.2429,325.6638)
--(axis cs:-176.4462,323.612);

\path [draw=lightgray!58.03921568627452!black, line width=4.0pt]
(axis cs:-176.4462,323.612)
--(axis cs:-166.7136,321.2753);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:-166.7136,321.2753)
--(axis cs:-157.0649,318.6138);

\path [draw=lightgray!48.62745098039216!black, line width=4.0pt]
(axis cs:-157.0649,318.6138)
--(axis cs:-147.5264,315.5818);

\path [draw=lightgray!28.758169934640527!black, line width=4.0pt]
(axis cs:-147.5264,315.5818)
--(axis cs:-138.1414,312.1048);

\path [draw=lightgray!71.63398692810458!black, line width=4.0pt]
(axis cs:-138.1414,312.1048)
--(axis cs:-128.9394,308.1688);

\path [draw=lightgray!60.130718954248366!black, line width=4.0pt]
(axis cs:-128.9394,308.1688)
--(axis cs:-119.9374,303.7943);

\path [draw=lightgray!71.63398692810458!black, line width=4.0pt]
(axis cs:-119.9374,303.7943)
--(axis cs:-111.1463,299.0101);

\path [draw=lightgray!3.137254901960788!black, line width=4.0pt]
(axis cs:-111.1463,299.0101)
--(axis cs:-102.5719,293.8472);

\path [draw=lightgray!31.89542483660131!black, line width=4.0pt]
(axis cs:-102.5719,293.8472)
--(axis cs:-94.2249,288.3242);

\path [draw=lightgray!96.73202614379085!black, line width=4.0pt]
(axis cs:-94.2249,288.3242)
--(axis cs:-86.1059,282.471);

\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:-86.1059,282.471)
--(axis cs:-78.1987,276.3343);

\path [draw=lightgray!72.67973856209152!black, line width=4.0pt]
(axis cs:-78.1987,276.3343)
--(axis cs:-70.4884,269.9518);

\path [draw=lightgray!53.333333333333336!black, line width=4.0pt]
(axis cs:-70.4884,269.9518)
--(axis cs:-62.9535,263.363);

\path [draw=lightgray!48.1045751633987!black, line width=4.0pt]
(axis cs:-62.9535,263.363)
--(axis cs:-55.572,256.6027);

\path [draw=lightgray!48.1045751633987!black, line width=4.0pt]
(axis cs:-55.572,256.6027)
--(axis cs:-48.3241,249.6993);

\path [draw=lightgray!52.28758169934641!black, line width=4.0pt]
(axis cs:-48.3241,249.6993)
--(axis cs:-41.1822,242.686);

\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:-41.1822,242.686)
--(axis cs:-34.1192,235.5933);

\path [draw=lightgray!58.03921568627452!black, line width=4.0pt]
(axis cs:-34.1192,235.5933)
--(axis cs:-27.1104,228.447);

\path [draw=lightgray!56.99346405228759!black, line width=4.0pt]
(axis cs:-27.1104,228.447)
--(axis cs:-20.1405,221.2628);

\path [draw=lightgray!92.02614379084967!black, line width=4.0pt]
(axis cs:-20.1405,221.2628)
--(axis cs:-13.1998,214.0503);

\path [draw=lightgray!65.88235294117646!black, line width=4.0pt]
(axis cs:-13.1998,214.0503)
--(axis cs:-6.2795,206.8183);

\path [draw=lightgray!94.640522875817!black, line width=4.0pt]
(axis cs:-6.2795,206.8183)
--(axis cs:0.6303,199.5761);

\path [draw=lightgray!67.45098039215685!black, line width=4.0pt]
(axis cs:0.6303,199.5761)
--(axis cs:7.5388,192.3329);

\path [draw=lightgray!51.24183006535947!black, line width=4.0pt]
(axis cs:7.5388,192.3329)
--(axis cs:14.4559,185.0977);

\path [draw=lightgray!70.58823529411765!black, line width=4.0pt]
(axis cs:14.4559,185.0977)
--(axis cs:21.3908,177.8796);

\path [draw=lightgray!53.8562091503268!black, line width=4.0pt]
(axis cs:21.3908,177.8796)
--(axis cs:28.3522,170.6872);

\path [draw=lightgray!47.58169934640524!black, line width=4.0pt]
(axis cs:28.3522,170.6872)
--(axis cs:35.347,163.5272);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:35.347,163.5272)
--(axis cs:42.3792,156.4039);

\path [draw=lightgray!96.20915032679738!black, line width=4.0pt]
(axis cs:42.3792,156.4039)
--(axis cs:49.4537,149.3226);

\path [draw=lightgray!16.732026143790847!black, line width=4.0pt]
(axis cs:49.4537,149.3226)
--(axis cs:56.5762,142.2897);

\path [draw=lightgray!41.830065359477125!black, line width=4.0pt]
(axis cs:56.5762,142.2897)
--(axis cs:63.7503,135.3093);

\path [draw=lightgray!40.7843137254902!black, line width=4.0pt]
(axis cs:63.7503,135.3093)
--(axis cs:70.9792,128.3858);

\path [draw=lightgray!58.56209150326798!black, line width=4.0pt]
(axis cs:70.9792,128.3858)
--(axis cs:78.2484,121.5045);

\path [draw=lightgray!60.653594771241835!black, line width=4.0pt]
(axis cs:78.2484,121.5045)
--(axis cs:85.5382,114.6451);

\path [draw=lightgray!59.08496732026144!black, line width=4.0pt]
(axis cs:85.5382,114.6451)
--(axis cs:92.851,107.8101);

\path [draw=lightgray!65.359477124183!black, line width=4.0pt]
(axis cs:92.851,107.8101)
--(axis cs:100.1909,101.0044);

\path [draw=lightgray!66.40522875816993!black, line width=4.0pt]
(axis cs:100.1909,101.0044)
--(axis cs:107.5806,94.2528);

\path [draw=lightgray!40.26143790849674!black, line width=4.0pt]
(axis cs:107.5806,94.2528)
--(axis cs:115.1067,87.6541);

\path [draw=lightgray!43.92156862745099!black, line width=4.0pt]
(axis cs:115.1067,87.6541)
--(axis cs:122.8881,81.3596);

\path [draw=lightgray!54.37908496732026!black, line width=4.0pt]
(axis cs:122.8881,81.3596)
--(axis cs:131.0096,75.5123);

\path [draw=lightgray!28.235294117647065!black, line width=4.0pt]
(axis cs:131.0096,75.5123)
--(axis cs:139.5498,70.2979);

\path [draw=lightgray!49.150326797385624!black, line width=4.0pt]
(axis cs:139.5498,70.2979)
--(axis cs:148.5069,65.8378);

\path [draw=lightgray!80.52287581699348!black, line width=4.0pt]
(axis cs:148.5069,65.8378)
--(axis cs:157.8094,62.1524);

\path [draw=lightgray!92.02614379084967!black, line width=4.0pt]
(axis cs:157.8094,62.1524)
--(axis cs:167.3963,59.2872);

\path [draw=lightgray!33.464052287581694!black, line width=4.0pt]
(axis cs:167.3963,59.2872)
--(axis cs:177.2027,57.2999);

\path [draw=lightgray!80.52287581699348!black, line width=4.0pt]
(axis cs:177.2027,57.2999)
--(axis cs:187.1481,56.2066);

\path [draw=lightgray!13.0718954248366!black, line width=4.0pt]
(axis cs:187.1481,56.2066)
--(axis cs:197.1521,56.0381);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:197.1521,56.0381)
--(axis cs:207.1271,56.8173);

\path [draw=lightgray!52.28758169934641!black, line width=4.0pt]
(axis cs:207.1271,56.8173)
--(axis cs:216.999,58.453);

\path [draw=lightgray!50.19607843137255!black, line width=4.0pt]
(axis cs:216.999,58.453)
--(axis cs:226.7268,60.8026);

\path [draw=lightgray!33.464052287581694!black, line width=4.0pt]
(axis cs:226.7268,60.8026)
--(axis cs:236.3057,63.7036);

\path [draw=white!81.17647058823529!black, line width=4.0pt]
(axis cs:236.3057,63.7036)
--(axis cs:245.7969,66.883);

\path [draw=lightgray!27.712418300653603!black, line width=4.0pt]
(axis cs:245.7969,66.883)
--(axis cs:255.3044,70.013);

\path [draw=lightgray!57.516339869281055!black, line width=4.0pt]
(axis cs:255.3044,70.013)
--(axis cs:264.9253,72.7698);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:264.9253,72.7698)
--(axis cs:274.7143,74.8418);

\path [draw=lightgray!89.41176470588236!black, line width=4.0pt]
(axis cs:274.7143,74.8418)
--(axis cs:284.6604,75.9157);

\path [draw=lightgray!83.66013071895425!black, line width=4.0pt]
(axis cs:284.6604,75.9157)
--(axis cs:294.6635,75.8808);

\path [draw=lightgray!44.96732026143791!black, line width=4.0pt]
(axis cs:294.6635,75.8808)
--(axis cs:304.5966,74.7025);

\path [draw=lightgray!83.66013071895425!black, line width=4.0pt]
(axis cs:304.5966,74.7025)
--(axis cs:314.3088,72.3128);

\path [draw=lightgray!25.620915032679736!black, line width=4.0pt]
(axis cs:314.3088,72.3128)
--(axis cs:323.6198,68.6648);

\path [draw=lightgray!1.0457516339869244!black, line width=4.0pt]
(axis cs:323.6198,68.6648)
--(axis cs:332.3287,63.7516);

\path [draw=lightgray!67.97385620915031!black, line width=4.0pt]
(axis cs:332.3287,63.7516)
--(axis cs:340.1802,57.5628);

\path [draw=lightgray!25.620915032679736!black, line width=4.0pt]
(axis cs:340.1802,57.5628)
--(axis cs:346.9426,50.2003);

\path [draw=lightgray!9.93464052287581!black, line width=4.0pt]
(axis cs:346.9426,50.2003)
--(axis cs:352.498,41.8871);

\path [draw=lightgray!55.94771241830067!black, line width=4.0pt]
(axis cs:352.498,41.8871)
--(axis cs:356.7546,32.8381);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:356.7546,32.8381)
--(axis cs:359.7572,23.2982);	

\path [draw=lightgray!54.90196078431372!black, line width=4.0pt]
(axis cs:359.7572,23.2982)
--(axis cs:361.6308,13.471);

\path [draw=lightgray!58.03921568627452!black, line width=4.0pt]
(axis cs:361.6308,13.471)
--(axis cs:362.5213,3.5047);

\path [draw=lightgray!39.215686274509814!black, line width=4.0pt]
(axis cs:362.5213,3.5047)
--(axis cs:362.6164,-6.5018);

\path [draw=lightgray!62.745098039215684!black, line width=4.0pt]
(axis cs:362.6164,-6.5018)
--(axis cs:362.0877,-16.4961);

\path [draw=lightgray!69.54248366013073!black, line width=4.0pt]
(axis cs:362.0877,-16.4961)
--(axis cs:361.1467,-26.4611);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:361.1467,-26.4611)
--(axis cs:359.98,-36.4023);

\path [draw=lightgray!76.33986928104575!black, line width=4.0pt]
(axis cs:359.98,-36.4023)
--(axis cs:358.7131,-46.3315);

\path [draw=lightgray!69.01960784313724!black, line width=4.0pt]
(axis cs:358.7131,-46.3315)
--(axis cs:357.424,-56.2578);

\path [draw=lightgray!65.88235294117646!black, line width=4.0pt]
(axis cs:357.424,-56.2578)
--(axis cs:356.1224,-66.1825);

\path [draw=white!78.03921568627452!black, line width=4.0pt]
(axis cs:356.1224,-66.1825)
--(axis cs:354.8297,-76.1083);

\path [draw=lightgray!88.8888888888889!black, line width=4.0pt]
(axis cs:354.8297,-76.1083)
--(axis cs:353.5684,-86.0382);

\path [draw=white!78.82352941176471!black, line width=4.0pt]
(axis cs:353.5684,-86.0382)
--(axis cs:352.3545,-95.9739);

\path [draw=lightgray!54.90196078431372!black, line width=4.0pt]
(axis cs:352.3545,-95.9739)
--(axis cs:351.1846,-105.915);

\path [draw=lightgray!29.80392156862745!black, line width=4.0pt]
(axis cs:351.1846,-105.915)
--(axis cs:350.051,-115.8602);

\path [draw=lightgray!43.39869281045751!black, line width=4.0pt]
(axis cs:350.051,-115.8602)
--(axis cs:348.9443,-125.8085);

\path [draw=lightgray!7.3202614379085!black, line width=4.0pt]
(axis cs:348.9443,-125.8085)
--(axis cs:347.8561,-135.7588);

\path [draw=lightgray!21.437908496732025!black, line width=4.0pt]
(axis cs:347.8561,-135.7588)
--(axis cs:346.778,-145.7103);

\path [draw=lightgray!50.71895424836601!black, line width=4.0pt]
(axis cs:346.778,-145.7103)
--(axis cs:345.7015,-155.6619);

\path [draw=lightgray!65.359477124183!black, line width=4.0pt]
(axis cs:345.7015,-155.6619)
--(axis cs:344.6084,-165.6116);

\path [draw=lightgray!20.915032679738562!black, line width=4.0pt]
(axis cs:344.6084,-165.6116)
--(axis cs:343.3479,-175.5411);

\path [draw=lightgray!15.163398692810462!black, line width=4.0pt]
(axis cs:343.3479,-175.5411)
--(axis cs:341.6186,-185.3981);

\path [draw=lightgray!78.95424836601308!black, line width=4.0pt]
(axis cs:341.6186,-185.3981)
--(axis cs:339.0784,-195.0746);

\path [draw=lightgray!69.54248366013073!black, line width=4.0pt]
(axis cs:339.0784,-195.0746)
--(axis cs:335.2924,-204.3284);

\path [draw=lightgray!19.869281045751638!black, line width=4.0pt]
(axis cs:335.2924,-204.3284)
--(axis cs:330.0462,-212.834);

\path [draw=lightgray!47.58169934640524!black, line width=4.0pt]
(axis cs:330.0462,-212.834)
--(axis cs:323.2118,-220.1137);

\path [draw=lightgray!95.68627450980392!black, line width=4.0pt]
(axis cs:323.2118,-220.1137)
--(axis cs:314.8874,-225.6253);

\path [draw=lightgray!36.60130718954249!black, line width=4.0pt]
(axis cs:314.8874,-225.6253)
--(axis cs:305.5398,-229.1319);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:305.5398,-229.1319)
--(axis cs:295.641,-230.4422);

\path [draw=lightgray!29.80392156862745!black, line width=4.0pt]
(axis cs:295.641,-230.4422)
--(axis cs:285.6767,-229.6874);

\path [draw=lightgray!46.01307189542484!black, line width=4.0pt]
(axis cs:285.6767,-229.6874)
--(axis cs:275.9511,-227.3606);

\path [draw=white!77.64705882352942!black, line width=4.0pt]
(axis cs:275.9511,-227.3606)
--(axis cs:266.57,-223.8839);

\path [draw=lightgray!63.79084967320261!black, line width=4.0pt]
(axis cs:266.57,-223.8839)
--(axis cs:257.5246,-219.6033);

\path [draw=lightgray!7.843137254901962!black, line width=4.0pt]
(axis cs:257.5246,-219.6033)
--(axis cs:248.7385,-214.8102);

\path [draw=lightgray!80.52287581699348!black, line width=4.0pt]
(axis cs:248.7385,-214.8102)
--(axis cs:240.1459,-209.6768);

\path [draw=lightgray!35.03267973856208!black, line width=4.0pt]
(axis cs:240.1459,-209.6768)
--(axis cs:231.6964,-204.3108);

\path [draw=lightgray!51.764705882352935!black, line width=4.0pt]
(axis cs:231.6964,-204.3108)
--(axis cs:223.3482,-198.7883);

\path [draw=lightgray!56.47058823529413!black, line width=4.0pt]
(axis cs:223.3482,-198.7883)
--(axis cs:215.0582,-193.1787);

\path [draw=lightgray!70.06535947712419!black, line width=4.0pt]
(axis cs:215.0582,-193.1787)
--(axis cs:206.7879,-187.54);

\path [draw=lightgray!66.40522875816993!black, line width=4.0pt]
(axis cs:206.7879,-187.54)
--(axis cs:198.5222,-181.8944);

\path [draw=lightgray!64.83660130718954!black, line width=4.0pt]
(axis cs:198.5222,-181.8944)
--(axis cs:190.2547,-176.2516);

\path [draw=lightgray!46.01307189542484!black, line width=4.0pt]
(axis cs:190.2547,-176.2516)
--(axis cs:181.9793,-170.6204);

\path [draw=lightgray!10.98039215686275!black, line width=4.0pt]
(axis cs:181.9793,-170.6204)
--(axis cs:173.6925,-165.0059);

\path [draw=lightgray!46.5359477124183!black, line width=4.0pt]
(axis cs:173.6925,-165.0059)
--(axis cs:165.3952,-159.4069);

\path [draw=lightgray!89.41176470588236!black, line width=4.0pt]
(axis cs:165.3952,-159.4069)
--(axis cs:157.0892,-153.8209);

\path [draw=lightgray!65.359477124183!black, line width=4.0pt]
(axis cs:157.0892,-153.8209)
--(axis cs:148.7761,-148.2455);

\path [draw=lightgray!40.7843137254902!black, line width=4.0pt]
(axis cs:148.7761,-148.2455)
--(axis cs:140.4573,-142.6785);

\path [draw=lightgray!75.81699346405229!black, line width=4.0pt]
(axis cs:140.4573,-142.6785)
--(axis cs:132.1346,-137.1175);

\path [draw=lightgray!52.28758169934641!black, line width=4.0pt]
(axis cs:132.1346,-137.1175)
--(axis cs:123.8091,-131.5605);

\path [draw=lightgray!91.50326797385621!black, line width=4.0pt]
(axis cs:123.8091,-131.5605)
--(axis cs:115.4816,-126.0066);

\path [draw=lightgray!39.738562091503276!black, line width=4.0pt]
(axis cs:115.4816,-126.0066)
--(axis cs:107.1524,-120.4553);

\path [draw=black, line width=4.0pt]
(axis cs:107.1524,-120.4553)
--(axis cs:98.8217,-114.9061);

\path [draw=lightgray!49.150326797385624!black, line width=4.0pt]
(axis cs:98.8217,-114.9061)
--(axis cs:90.4897,-109.359);

\path [draw=lightgray!21.960784313725487!black, line width=4.0pt]
(axis cs:90.4897,-109.359)
--(axis cs:82.1565,-103.8136);

\path [draw=lightgray!77.90849673202615!black, line width=4.0pt]
(axis cs:82.1565,-103.8136)
--(axis cs:73.8224,-98.2696);

\path [draw=lightgray!64.83660130718954!black, line width=4.0pt]
(axis cs:73.8224,-98.2696)
--(axis cs:65.4875,-92.7269);

\path [draw=lightgray!37.12418300653595!black, line width=4.0pt]
(axis cs:65.4875,-92.7269)
--(axis cs:57.152,-87.185);

\path [draw=lightgray!73.72549019607844!black, line width=4.0pt]
(axis cs:57.152,-87.185)
--(axis cs:48.816,-81.6438);

\path [draw=lightgray!70.58823529411765!black, line width=4.0pt]
(axis cs:48.816,-81.6438)
--(axis cs:40.4798,-76.103);

\path [draw=lightgray!20.3921568627451!black, line width=4.0pt]
(axis cs:40.4798,-76.103)
--(axis cs:32.1435,-70.5622);

\path [draw=lightgray!41.830065359477125!black, line width=4.0pt]
(axis cs:32.1435,-70.5622)
--(axis cs:23.8073,-65.0213);

\path [draw=lightgray!39.215686274509814!black, line width=4.0pt]
(axis cs:23.8073,-65.0213)
--(axis cs:15.4715,-59.48);

\path [draw=lightgray!66.92810457516339!black, line width=4.0pt]
(axis cs:15.4715,-59.48)
--(axis cs:7.136,-53.9381);

\path [draw=lightgray!58.56209150326798!black, line width=4.0pt]
(axis cs:7.136,-53.9381)
--(axis cs:-1.1994,-48.396);

==> ressources/variable_friction/local_map.tex <==
% This file was created by tikzplotlib v0.9.1.
%
\definecolor{TUMred}{RGB}{227,114,34}%
\definecolor{TUMgray}{rgb}{0.5977,0.5977,0.5977}
\definecolor{TUMgrayLight}{rgb}{0.8516,0.8398,0.7929}
\definecolor{TUMblue}{RGB}{0,101,189}%
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\def\xmin_varFric{100.0}
\def\xmax_varFric{370.0}
\def\ymin_varFric{-50.0}
\def\ymax_varFric{150.0}
%
%
%
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 2, vertical sep=40pt,
	horizontal sep=10pt},
width=5.25cm,
%height=2cm,
%xmajorgrids,
xmin=\xmin_varFric,
xmax=\xmax_varFric,
ymin=\ymin_varFric,
ymax=\ymax_varFric,
tick align=outside,
xtick style={color=black},
x grid style={white!69.0!black},
y grid style={white!69.0!black},
axis equal,
xtick pos=left,
ytick pos=left
]
\nextgroupplot[%
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.97)}, anchor=north west, draw=white!80!black},
%tick pos=both,
ylabel={north in m},
xticklabels={,,},
title=lap 1
]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Scenario high mu
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Bounds
\input{ressources/variable_friction/bounds.tex}
\addlegendentry{Bounds}
% Nodes
%\input{ressources/variable_friction/nodes.tex}
%\addlegendentry{Nodes}
%\draw[draw=color7,fill=color7] (axis cs:161.017068167805,-156.460218242343) circle (2);
% Ego-Vehicle
\addplot [semithick, black, mark=*, mark size=3, mark options={solid}, only marks, forget plot]
table {%
	188.367574290479 -174.868489956856
};
% Friction Plot
\input{ressources/variable_friction/friction_high.tex}
%\subcaption{\label{fig:b}}
%
% Raceline
\input{ressources/variable_friction/raceline.tex}
\addlegendentry{To be chosen Path!}
%
% Chosen Path
\input{ressources/variable_friction/chosen_path.tex}
%
%
% Colorbar
\nextgroupplot[
hide axis,
colormap/blackwhite,
colorbar horizontal,
colorbar style={at={(1,1)},anchor=north east,
	axis line style={draw=none},
	point meta max=16.7482092230782,
	point meta min=11.1784381596894,
	xlabel=$\bar{a}_\mathrm{y}$ in \SI{}{\meter\per\second\squared}},
legend cell align={left},
%legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80.0!black},
]
\end{groupplot}
\end{tikzpicture}


==> ressources/variable_friction/nodes.tex <==
\addplot [semithick, TUMblue, mark=x, mark size=0.2, mark options={solid}, only marks]
table {%
	-1.75329377814429 -49.228601104573
	-1.47634682814429 -48.812307454573
	-1.19939987814429 -48.396013804573
	-0.92245292814429 -47.979720154573
	-0.64550597814429 -47.563426504573
	-0.36855902814429 -47.147132854573
	-0.09161207814429 -46.730839204573
	0.18533487185571 -46.314545554573
	0.46228182185571 -45.898251904573
	0.73922877185571 -45.481958254573
	1.01617572185571 -45.065664604573
	1.29312267185571 -44.649370954573
	1.57006962185571 -44.233077304573
	1.84701657185571 -43.816783654573
	2.12396352185571 -43.400490004573
	2.40091047185571 -42.984196354573
	2.67785742185571 -42.567902704573
	2.95480437185571 -42.151609054573
	3.23175132185571 -41.735315404573
	3.50869827185571 -41.319021754573
	3.78564522185571 -40.902728104573
	4.06259217185571 -40.486434454573
	4.33953912185571 -40.070140804573
	-26.7258494442021 -32.6273644165333
	-26.4486917442021 -32.2112110665333
	-26.1715340442021 -31.7950577165333
	-25.8943763442021 -31.3789043665333
	-25.6172186442021 -30.9627510165333
	-25.3400609442021 -30.5465976665333
	-25.0629032442021 -30.1304443165333
	-24.7857455442021 -29.7142909665333
	-24.5085878442021 -29.2981376165333
	-24.2314301442021 -28.8819842665333
	-23.9542724442021 -28.4658309165333
	-23.6771147442021 -28.0496775665333
	-23.3999570442021 -27.6335242165333
	-23.1227993442021 -27.2173708665333
	-22.8456416442021 -26.8012175165333
	-22.5684839442021 -26.3850641665333
	-22.2913262442021 -25.9689108165333
	-22.0141685442021 -25.5527574665333
	-21.7370108442021 -25.1366041165333
	-21.4598531442021 -24.7204507665333
	-21.1826954442021 -24.3042974165333
	-20.9055377442021 -23.8881440665333
	-20.6283800442021 -23.4719907165333
	-51.701341994585 -16.0300217450733
	-51.424054394585 -15.6139549450733
	-51.146766794585 -15.1978881450733
	-50.869479194585 -14.7818213450733
	-50.592191594585 -14.3657545450733
	-50.314903994585 -13.9496877450733
	-50.037616394585 -13.5336209450733
	-49.760328794585 -13.1175541450733
	-49.483041194585 -12.7014873450733
	-49.205753594585 -12.2854205450733
	-48.928465994585 -11.8693537450733
	-48.651178394585 -11.4532869450733
	-48.373890794585 -11.0372201450733
	-48.096603194585 -10.6211533450733
	-47.819315594585 -10.2050865450733
	-47.542027994585 -9.78901974507328
	-47.264740394585 -9.37295294507328
	-46.987452794585 -8.95688614507328
	-46.710165194585 -8.54081934507328
	-46.432877594585 -8.12475254507328
	-46.155589994585 -7.70868574507328
	-45.878302394585 -7.29261894507328
	-45.601014794585 -6.87655214507328
	-76.680309189896 0.56235655954599
	-76.402972589896 0.97839070954599
	-76.125635989896 1.39442485954599
	-75.848299389896 1.81045900954599
	-75.570962789896 2.22649315954599
	-75.293626189896 2.64252730954599
	-75.016289589896 3.05856145954599
	-74.738952989896 3.47459560954599
	-74.461616389896 3.89062975954599
	-74.184279789896 4.30666390954599
	-73.906943189896 4.72269805954599
	-73.629606589896 5.13873220954599
	-73.352269989896 5.55476635954599
	-73.074933389896 5.97080050954599
	-72.797596789896 6.38683465954599
	-72.520260189896 6.80286880954599
	-72.242923589896 7.21890295954599
	-71.965586989896 7.63493710954599
	-71.688250389896 8.05097125954599
	-71.410913789896 8.46700540954599
	-71.133577189896 8.88303955954599
	-70.856240589896 9.29907370954599
	-70.578903989896 9.71510785954599
	-101.663273987831 17.1486899736175
	-101.385969237831 17.5647453736175
	-101.108664487831 17.9808007736175
	-100.831359737831 18.3968561736175
	-100.554054987831 18.8129115736175
	-100.276750237831 19.2289669736175
	-99.9994454878307 19.6450223736175
	-99.7221407378307 20.0610777736175
	-99.4448359878307 20.4771331736175
	-99.1675312378307 20.8931885736175
	-98.8902264878307 21.3092439736175
	-98.6129217378307 21.7252993736175
	-98.3356169878307 22.1413547736175
	-98.0583122378307 22.5574101736175
	-97.7810074878307 22.9734655736175
	-97.5037027378307 23.3895209736175
	-97.2263979878307 23.8055763736175
	-96.9490932378307 24.2216317736175
	-96.6717884878307 24.6376871736175
	-96.3944837378307 25.0537425736175
	-96.1171789878307 25.4697979736175
	-95.8398742378307 25.8858533736175
	-95.5625694878307 26.3019087736175
	-126.650751380691 33.7278921282357
	-126.373559330691 34.1440225782357
	-126.096367280691 34.5601530282357
	-125.819175230691 34.9762834782357
	-125.541983180691 35.3924139282357
	-125.264791130691 35.8085443782357
	-124.987599080691 36.2246748282357
	-124.710407030691 36.6408052782357
	-124.433214980691 37.0569357282357
	-124.156022930691 37.4730661782357
	-123.878830880691 37.8891966282357
	-123.601638830691 38.3053270782357
	-123.324446780691 38.7214575282357
	-123.047254730691 39.1375879782357
	-122.770062680691 39.5537184282357
	-122.492870630691 39.9698488782357
	-122.215678580691 40.3859793282357
	-121.938486530691 40.8021097782357
	-121.661294480691 41.2182402282357
	-121.384102430691 41.6343706782357
	-121.106910380691 42.0505011282357
	-120.829718330691 42.4666315782357
	-120.552526280691 42.8827620282357
	-151.643255697699 50.2988766434079
	-151.366257197699 50.7151359934079
	-151.089258697699 51.1313953434079
	-150.812260197699 51.5476546934079
	-150.535261697699 51.9639140434079
	-150.258263197699 52.3801733934079
	-149.981264697699 52.7964327434079
	-149.704266197699 53.2126920934079
	-149.427267697699 53.6289514434079
	-149.150269197699 54.0452107934079
	-148.873270697699 54.4614701434079
	-148.596272197699 54.8777294934079
	-148.319273697699 55.2939888434079
	-148.042275197699 55.7102481934079
	-147.765276697699 56.1265075434079
	-147.488278197699 56.5427668934079
	-147.211279697699 56.9590262434079
	-146.934281197699 57.3752855934079
	-146.657282697699 57.7915449434079
	-146.380284197699 58.2078042934079
	-146.103285697699 58.6240636434079
	-145.826287197699 59.0403229934079
	-145.549288697699 59.4565823434079
	-176.641307621955 66.8605631054873
	-176.364583671955 67.2770050054873
	-176.087859721955 67.6934469054873
	-175.811135771955 68.1098888054873
	-175.534411821955 68.5263307054873
	-175.257687871955 68.9427726054873
	-174.980963921955 69.3592145054873
	-174.704239971955 69.7756564054873
	-174.427516021955 70.1920983054873
	-174.150792071955 70.6085402054873
	-173.874068121955 71.0249821054873
	-173.597344171955 71.4414240054873
	-173.320620221955 71.8578659054873
	-173.043896271955 72.2743078054873
	-172.767172321955 72.6907497054873
	-172.490448371955 73.1071916054873
	-172.213724421955 73.5236335054873
	-171.937000471955 73.9400754054873
	-171.660276521955 74.3565173054873
	-171.383552571955 74.7729592054873
	-171.106828621955 75.1894011054873
	-170.830104671955 75.6058430054873
	-170.553380721955 76.0222849054873
	-201.645441748717 83.4118816206171
	-201.369073398717 83.8285595706171
	-201.092705048717 84.2452375206171
	-200.816336698717 84.6619154706171
	-200.539968348717 85.0785934206171
	-200.263599998717 85.4952713706171
	-199.987231648717 85.9119493206171
	-199.710863298717 86.3286272706171
	-199.434494948717 86.7453052206171
	-199.158126598717 87.1619831706171
	-198.881758248717 87.5786611206171
	-198.605389898717 87.9953390706171
	-198.329021548717 88.4120170206171
	-198.052653198717 88.8286949706171
	-197.776284848717 89.2453729206171
	-197.499916498717 89.6620508706171
	-197.223548148717 90.0787288206171
	-196.947179798717 90.4954067706171
	-196.670811448717 90.9120847206171
	-196.394443098717 91.3287626706171
	-196.118074748717 91.7454406206171
	-195.841706398717 92.1621185706171
	-195.565338048717 92.5787965206171
	-226.656213599453 99.9517783895372
	-226.380282099453 100.368745789537
	-226.104350599453 100.785713189537
	-225.828419099453 101.202680589537
	-225.552487599453 101.619647989537
	-225.276556099453 102.036615389537
	-225.000624599453 102.453582789537
	-224.724693099453 102.870550189537
	-224.448761599453 103.287517589537
	-224.172830099453 103.704484989537
	-223.896898599453 104.121452389537
	-223.620967099453 104.538419789537
	-223.345035599453 104.955387189537
	-223.069104099453 105.372354589537
	-222.793172599453 105.789321989537
	-222.517241099453 106.206289389537
	-222.241309599453 106.623256789537
	-221.965378099453 107.040224189537
	-221.689446599453 107.457191589537
	-221.413515099453 107.874158989537
	-221.137583599453 108.291126389537
	-220.861652099453 108.708093789537
	-220.585720599453 109.125061189537
	-251.674172161192 116.479278211943
	-251.398758211192 116.896587661943
	-251.123344261192 117.313897111943
	-250.847930311192 117.731206561943
	-250.572516361192 118.148516011943
	-250.297102411192 118.565825461943
	-250.021688461192 118.983134911943
	-249.746274511192 119.400444361943
	-249.470860561192 119.817753811943
	-249.195446611192 120.235063261943
	-248.920032661192 120.652372711943
	-248.644618711192 121.069682161943
	-248.369204761192 121.486991611943
	-248.093790811192 121.904301061943
	-247.818376861192 122.321610511943
	-247.542962911192 122.738919961943
	-247.267548961192 123.156229411943
	-246.992135011192 123.573538861943
	-246.716721061192 123.990848311943
	-246.441307111192 124.408157761943
	-246.165893161192 124.825467211943
	-245.890479211192 125.242776661943
	-245.615065261192 125.660086111943
	-276.148649158058 133.831706351418
	-275.873676758058 134.249306851418
	-275.598704358058 134.666907351418
	-275.323731958058 135.084507851418
	-275.048759558058 135.502108351418
	-274.773787158058 135.919708851418
	-274.498814758058 136.337309351418
	-274.223842358058 136.754909851418
	-273.948869958058 137.172510351418
	-273.673897558058 137.590110851418
	-273.398925158058 138.007711351418
	-273.123952758058 138.425311851418
	-272.848980358058 138.842912351418
	-272.574007958058 139.260512851418
	-272.299035558058 139.678113351418
	-272.024063158058 140.095713851418
	-271.749090758058 140.513314351418
	-271.474118358058 140.930914851418
	-271.199145958058 141.348515351418
	-270.924173558058 141.766115851418
	-270.649201158058 142.183716351418
	-270.374228758058 142.601316851418
	-301.453551376352 149.924773450582
	-301.178822226352 150.342534000582
	-300.904093076352 150.760294550582
	-300.629363926352 151.178055100582
	-300.354634776352 151.595815650582
	-300.079905626352 152.013576200582
	-299.805176476352 152.431336750582
	-299.530447326352 152.849097300582
	-299.255718176352 153.266857850582
	-298.980989026352 153.684618400582
	-298.706259876352 154.102378950582
	-298.431530726352 154.520139500582
	-298.156801576352 154.937900050582
	-297.882072426352 155.355660600582
	-297.607343276352 155.773421150582
	-297.332614126352 156.191181700582
	-297.057884976352 156.608942250582
	-296.783155826352 157.026702800582
	-296.508426676352 157.444463350582
	-296.233697526352 157.862223900582
	-295.958968376352 158.279984450582
	-295.684239226352 158.697745000582
	-326.487566151275 166.431234234324
	-326.212881751275 166.849024234324
	-325.938197351275 167.266814234324
	-325.663512951275 167.684604234324
	-325.388828551275 168.102394234324
	-325.114144151275 168.520184234324
	-324.839459751275 168.937974234324
	-324.564775351275 169.355764234324
	-324.290090951275 169.773554234324
	-324.015406551275 170.191344234324
	-323.740722151275 170.609134234324
	-323.466037751275 171.026924234324
	-323.191353351275 171.444714234324
	-322.916668951275 171.862504234324
	-322.641984551275 172.280294234324
	-322.367300151275 172.698084234324
	-322.092615751275 173.115874234324
	-321.817931351275 173.533664234324
	-321.543246951275 173.951454234324
	-321.268562551275 174.369244234324
	-320.993878151275 174.787034234324
	-320.719193751275 175.204824234324
	-320.444509351275 175.622614234324
	-351.52465919704 182.936117923386
	-351.24982109704 183.353806823386
	-350.97498299704 183.771495723386
	-350.70014489704 184.189184623386
	-350.42530679704 184.606873523386
	-350.15046869704 185.024562423386
	-349.87563059704 185.442251323386
	-349.60079249704 185.859940223386
	-349.32595439704 186.277629123386
	-349.05111629704 186.695318023386
	-348.77627819704 187.113006923386
	-348.50144009704 187.530695823386
	-348.22660199704 187.948384723386
	-347.95176389704 188.366073623386
	-347.67692579704 188.783762523386
	-347.40208769704 189.201451423386
	-347.12724959704 189.619140323386
	-346.85241149704 190.036829223386
	-346.57757339704 190.454518123386
	-346.30273529704 190.872207023386
	-346.02789719704 191.289895923386
	-345.75305909704 191.707584823386
	-345.47822099704 192.125273723386
	-376.563838348732 199.442075947812
	-376.288648948732 199.859533447812
	-376.013459548732 200.276990947811
	-375.738270148732 200.694448447812
	-375.463080748732 201.111905947812
	-375.187891348732 201.529363447812
	-374.912701948732 201.946820947812
	-374.637512548732 202.364278447812
	-374.362323148732 202.781735947812
	-374.087133748732 203.199193447811
	-373.811944348732 203.616650947812
	-373.536754948732 204.034108447812
	-373.261565548732 204.451565947812
	-372.986376148732 204.869023447812
	-372.711186748732 205.286480947811
	-372.435997348732 205.703938447812
	-372.160807948732 206.121395947812
	-371.885618548732 206.538853447812
	-371.610429148732 206.956310947812
	-371.335239748732 207.373768447811
	-371.060050348732 207.791225947812
	-370.784860948732 208.208683447811
	-370.509671548732 208.626140947812
	-401.601938551231 215.953135769848
	-401.326287201231 216.370288419848
	-401.050635851231 216.787441069848
	-400.774984501231 217.204593719848
	-400.499333151231 217.621746369848
	-400.223681801231 218.038899019848
	-399.948030451231 218.456051669848
	-399.672379101231 218.873204319848
	-399.396727751231 219.290356969848
	-399.121076401231 219.707509619848
	-398.845425051231 220.124662269848
	-398.569773701231 220.541814919848
	-398.294122351231 220.958967569848
	-398.018471001231 221.376120219848
	-397.742819651231 221.793272869848
	-397.467168301231 222.210425519848
	-397.191516951231 222.627578169848
	-396.915865601231 223.044730819848
	-396.640214251231 223.461883469848
	-396.364562901231 223.879036119848
	-396.088911551231 224.296188769848
	-395.813260201231 224.713341419848
	-395.537608851231 225.130494069848
	-426.353362317105 232.894303170476
	-426.077197917105 233.311116370476
	-425.801033517105 233.727929570476
	-425.524869117105 234.144742770476
	-425.248704717105 234.561555970476
	-424.972540317105 234.978369170476
	-424.696375917105 235.395182370476
	-424.420211517105 235.811995570476
	-424.144047117105 236.228808770476
	-423.867882717105 236.645621970476
	-423.591718317105 237.062435170476
	-423.315553917105 237.479248370476
	-423.039389517105 237.896061570476
	-422.763225117105 238.312874770476
	-422.487060717105 238.729687970476
	-422.210896317105 239.146501170476
	-421.934731917105 239.563314370476
	-421.658567517105 239.980127570476
	-421.382403117105 240.396940770476
	-421.106238717105 240.813753970476
	-420.830074317105 241.230567170476
	-420.553909917105 241.647380370476
	-451.359340468007 249.440522135324
	-451.082611918007 249.856960985324
	-450.805883368007 250.273399835324
	-450.529154818007 250.689838685324
	-450.252426268007 251.106277535324
	-449.975697718007 251.522716385324
	-449.698969168007 251.939155235324
	-449.422240618007 252.355594085324
	-449.145512068007 252.772032935324
	-448.868783518007 253.188471785324
	-448.592054968007 253.604910635324
	-448.315326418007 254.021349485324
	-448.038597868007 254.437788335324
	-447.761869318007 254.854227185324
	-447.485140768007 255.270666035324
	-447.208412218007 255.687104885324
	-446.931683668007 256.103543735324
	-446.654955118007 256.519982585324
	-446.378226568007 256.936421435324
	-446.101498018007 257.352860285324
	-445.824769468007 257.769299135324
	-445.548040918007 258.185737985324
	-476.333697423046 266.01779843358
	-476.056353423046 266.433827633581
	-475.779009423046 266.849856833581
	-475.501665423046 267.265886033581
	-475.224321423046 267.681915233581
	-474.946977423046 268.09794443358
	-474.669633423046 268.513973633581
	-474.392289423046 268.93000283358
	-474.114945423046 269.346032033581
	-473.837601423046 269.76206123358
	-473.560257423046 270.178090433581
	-473.282913423046 270.594119633581
	-473.005569423046 271.010148833581
	-472.728225423046 271.426178033581
	-472.450881423046 271.84220723358
	-472.173537423046 272.258236433581
	-471.896193423046 272.67426563358
	-471.618849423046 273.090294833581
	-471.341505423046 273.50632403358
	-471.064161423046 273.922353233581
	-470.786817423046 274.33838243358
	-470.509473423046 274.754411633581
	-501.260677496731 282.644457982621
	-500.981400246731 283.059191882621
	-500.702122996731 283.473925782621
	-500.422845746731 283.888659682621
	-500.143568496731 284.303393582621
	-499.864291246731 284.718127482621
	-499.585013996731 285.132861382621
	-499.305736746731 285.547595282621
	-499.026459496731 285.962329182621
	-498.747182246731 286.377063082621
	-498.467904996731 286.791796982621
	-498.188627746731 287.206530882621
	-497.909350496731 287.621264782621
	-497.630073246731 288.035998682621
	-497.350795996731 288.450732582621
	-497.071518746731 288.865466482621
	-496.792241496731 289.280200382621
	-496.512964246731 289.694934282621
	-496.233686996731 290.109668182621
	-495.954409746731 290.524402082621
	-495.675132496731 290.939135982621
	-495.395855246731 291.353869882621
	-513.808438287183 290.977594395685
	-513.501989287183 291.372675395685
	-513.195540287183 291.767756395685
	-512.889091287183 292.162837395685
	-512.582642287183 292.557918395685
	-512.276193287183 292.952999395685
	-511.969744287183 293.348080395685
	-511.663295287183 293.743161395685
	-511.356846287183 294.138242395685
	-511.050397287183 294.533323395685
	-510.743948287183 294.928404395685
	-510.437499287183 295.323485395685
	-510.131050287183 295.718566395685
	-509.824601287183 296.113647395685
	-509.518152287183 296.508728395685
	-509.211703287183 296.903809395685
	-508.905254287183 297.298890395685
	-508.598805287183 297.693971395685
	-508.292356287183 298.089052395685
	-507.985907287183 298.484133395685
	-507.679458287183 298.879214395685
	-507.373009287183 299.274295395685
	-521.657933982711 295.992842815265
	-521.307939532711 296.349919665265
	-520.957945082711 296.706996515265
	-520.607950632711 297.064073365265
	-520.257956182711 297.421150215265
	-519.907961732711 297.778227065265
	-519.557967282711 298.135303915265
	-519.207972832711 298.492380765265
	-518.857978382711 298.849457615265
	-518.507983932711 299.206534465265
	-518.157989482711 299.563611315265
	-517.807995032711 299.920688165265
	-517.458000582711 300.277765015265
	-517.108006132711 300.634841865265
	-516.758011682711 300.991918715265
	-516.408017232711 301.348995565265
	-516.058022782711 301.706072415265
	-515.708028332711 302.063149265265
	-515.358033882711 302.420226115265
	-515.008039432711 302.777302965265
	-514.658044982711 303.134379815265
	-514.308050532711 303.491456665265
	-530.01851428 301.71173256
	-529.59828498 301.98267046
	-529.17805568 302.25360836
	-528.75782638 302.52454626
	-528.33759708 302.79548416
	-527.91736778 303.06642206
	-527.49713848 303.33735996
	-527.07690918 303.60829786
	-526.65667988 303.87923576
	-526.23645058 304.15017366
	-525.81622128 304.42111156
	-525.39599198 304.69204946
	-524.97576268 304.96298736
	-524.55553338 305.23392526
	-524.13530408 305.50486316
	-523.71507478 305.77580106
	-523.29484548 306.04673896
	-522.87461618 306.31767686
	-522.45438688 306.58861476
	-522.03415758 306.85955266
	-521.61392828 307.13049056
	-521.19369898 307.40142846
	-520.77346968 307.67236636
	-538.692989317081 309.931243343113
	-538.212261117081 310.068722043113
	-537.731532917081 310.206200743113
	-537.250804717081 310.343679443113
	-536.770076517081 310.481158143113
	-536.289348317081 310.618636843113
	-535.808620117081 310.756115543113
	-535.327891917081 310.893594243113
	-534.847163717081 311.031072943113
	-534.366435517081 311.168551643113
	-533.885707317081 311.306030343113
	-533.404979117081 311.443509043113
	-532.924250917081 311.580987743113
	-532.443522717081 311.718466443113
	-531.962794517081 311.855945143113
	-531.482066317081 311.993423843113
	-531.001338117081 312.130902543113
	-530.520609917081 312.268381243113
	-530.039881717081 312.405859943113
	-529.559153517081 312.543338643113
	-529.078425317081 312.680817343113
	-528.597697117081 312.818296043113
	-528.116968917081 312.955774743113
	-527.636240717081 313.093253443113
	-527.155512517081 313.230732143113
	-541.96620718 322.15571497
	-541.46756038 322.11895402
	-540.96891358 322.08219307
	-540.47026678 322.04543212
	-539.97161998 322.00867117
	-539.47297318 321.97191022
	-538.97432638 321.93514927
	-538.47567958 321.89838832
	-537.97703278 321.86162737
	-537.47838598 321.82486642
	-536.97973918 321.78810547
	-536.48109238 321.75134452
	-535.98244558 321.71458357
	-535.48379878 321.67782262
	-534.98515198 321.64106167
	-534.48650518 321.60430072
	-533.98785838 321.56753977
	-533.48921158 321.53077882
	-532.99056478 321.49401787
	-532.49191798 321.45725692
	-531.99327118 321.42049597
	-531.49462438 321.38373502
	-530.99597758 321.34697407
	-530.49733078 321.31021312
	-538.426609180911 334.909991547851
	-537.980094380911 334.684992547851
	-537.533579580911 334.459993547851
	-537.087064780911 334.234994547851
	-536.640549980911 334.009995547851
	-536.194035180911 333.784996547851
	-535.747520380911 333.559997547851
	-535.301005580911 333.334998547851
	-534.854490780911 333.109999547851
	-534.407975980911 332.885000547851
	-533.961461180911 332.660001547851
	-533.514946380911 332.435002547851
	-533.068431580911 332.210003547851
	-532.621916780911 331.985004547851
	-532.175401980911 331.760005547851
	-531.728887180911 331.535006547851
	-531.282372380911 331.310007547851
	-530.835857580911 331.085008547851
	-530.389342780911 330.860009547851
	-529.942827980911 330.635010547851
	-529.496313180911 330.410011547851
	-529.049798380911 330.185012547851
	-528.603283580911 329.960013547851
	-528.156768780911 329.735014547851
	-527.710253980911 329.510015547851
	-528.61645312 343.01207597
	-528.27475992 342.64704752
	-527.93306672 342.28201907
	-527.59137352 341.91699062
	-527.24968032 341.55196217
	-526.90798712 341.18693372
	-526.56629392 340.82190527
	-526.22460072 340.45687682
	-525.88290752 340.09184837
	-525.54121432 339.72681992
	-525.19952112 339.36179147
	-524.85782792 338.99676302
	-524.51613472 338.63173457
	-524.17444152 338.26670612
	-523.83274832 337.90167767
	-523.49105512 337.53664922
	-523.14936192 337.17162077
	-522.80766872 336.80659232
	-522.46597552 336.44156387
	-522.12428232 336.07653542
	-521.78258912 335.71150697
	-521.44089592 335.34647852
	-521.09920272 334.98145007
	-517.310878953819 345.866398663633
	-517.104737353819 345.410870813633
	-516.898595753819 344.955342963633
	-516.692454153819 344.499815113633
	-516.486312553819 344.044287263633
	-516.280170953819 343.588759413633
	-516.074029353819 343.133231563633
	-515.867887753819 342.677703713633
	-515.661746153819 342.222175863633
	-515.455604553819 341.766648013633
	-515.249462953819 341.311120163633
	-515.043321353819 340.855592313633
	-514.837179753819 340.400064463633
	-514.631038153819 339.944536613633
	-514.424896553819 339.489008763633
	-514.218754953819 339.033480913633
	-514.012613353819 338.577953063633
	-513.806471753819 338.122425213633
	-513.600330153819 337.666897363633
	-513.394188553819 337.211369513633
	-513.188046953819 336.755841663633
	-512.981905353819 336.300313813633
	-512.775763753819 335.844785963633
	-507.135419840701 346.063360918649
	-507.044966190701 345.571610818649
	-506.954512540701 345.079860718649
	-506.864058890701 344.588110618649
	-506.773605240701 344.096360518649
	-506.683151590701 343.604610418649
	-506.592697940701 343.112860318649
	-506.502244290701 342.621110218649
	-506.411790640701 342.129360118649
	-506.321336990701 341.637610018649
	-506.230883340701 341.145859918649
	-506.140429690701 340.654109818649
	-506.049976040701 340.162359718649
	-505.959522390701 339.670609618649
	-505.869068740701 339.178859518649
	-505.778615090701 338.687109418649
	-505.688161440701 338.195359318649
	-505.597707790701 337.703609218649
	-505.507254140701 337.211859118649
	-505.416800490701 336.720109018649
	-505.326346840701 336.228358918649
	-505.235893190701 335.736608818649
	-497.847317199148 345.43830545114
	-497.846610499148 344.93830595114
	-497.845903799148 344.43830645114
	-497.845197099148 343.93830695114
	-497.844490399148 343.43830745114
	-497.843783699148 342.93830795114
	-497.843076999148 342.43830845114
	-497.842370299148 341.93830895114
	-497.841663599148 341.43830945114
	-497.840956899148 340.93830995114
	-497.840250199148 340.43831045114
	-497.839543499148 339.93831095114
	-497.838836799148 339.43831145114
	-497.838130099148 338.93831195114
	-497.837423399148 338.43831245114
	-497.836716699148 337.93831295114
	-497.836009999148 337.43831345114
	-497.835303299148 336.93831395114
	-497.834596599148 336.43831445114
	-497.833889899148 335.93831495114
	-497.833183199148 335.43831545114
	-488.789701639795 345.387888171598
	-488.850950039795 344.891653721598
	-488.912198439795 344.395419271598
	-488.973446839795 343.899184821598
	-489.034695239795 343.402950371598
	-489.095943639795 342.906715921598
	-489.157192039795 342.410481471598
	-489.218440439795 341.914247021598
	-489.279688839795 341.418012571598
	-489.340937239795 340.921778121598
	-489.402185639795 340.425543671598
	-489.463434039795 339.929309221598
	-489.524682439795 339.433074771598
	-489.585930839795 338.936840321598
	-489.647179239795 338.440605871598
	-489.708427639795 337.944371421598
	-489.769676039795 337.448136971598
	-489.830924439795 336.951902521598
	-489.892172839795 336.455668071598
	-489.953421239795 335.959433621598
	-490.014669639795 335.463199171598
	-479.668224873176 344.901742521253
	-479.767978473176 344.411794321253
	-479.867732073176 343.921846121253
	-479.967485673176 343.431897921253
	-480.067239273176 342.941949721253
	-480.166992873176 342.452001521253
	-480.266746473176 341.962053321253
	-480.366500073176 341.472105121253
	-480.466253673176 340.982156921253
	-480.566007273176 340.492208721253
	-480.665760873176 340.002260521253
	-480.765514473176 339.512312321253
	-480.865268073176 339.022364121253
	-480.965021673176 338.532415921253
	-481.064775273176 338.042467721253
	-481.164528873176 337.552519521253
	-481.264282473176 337.062571321253
	-481.364036073176 336.572623121253
	-481.463789673176 336.082674921253
	-481.563543273176 335.592726721253
	-481.663296873176 335.102778521253
	-447.939771003183 342.724166999321
	-448.132247803183 342.262699049321
	-448.324724603183 341.801231099321
	-448.517201403183 341.339763149321
	-448.709678203183 340.878295199321
	-448.902155003183 340.416827249321
	-449.094631803183 339.955359299321
	-449.287108603183 339.493891349321
	-449.479585403183 339.032423399321
	-449.672062203183 338.570955449321
	-449.864539003183 338.109487499321
	-450.057015803183 337.648019549321
	-450.249492603183 337.186551599321
	-450.441969403183 336.725083649321
	-450.634446203183 336.263615699321
	-450.826923003183 335.802147749321
	-451.019399803183 335.340679799321
	-451.211876603183 334.879211849321
	-451.404353403183 334.417743899321
	-451.596830203183 333.956275949321
	-451.789307003183 333.494807999321
	-420.955129282292 327.142491436508
	-421.208553932292 326.711474086508
	-421.461978582292 326.280456736508
	-421.715403232292 325.849439386508
	-421.968827882292 325.418422036508
	-422.222252532292 324.987404686508
	-422.475677182292 324.556387336508
	-422.729101832292 324.125369986508
	-422.982526482292 323.694352636508
	-423.235951132292 323.263335286508
	-423.489375782292 322.832317936508
	-423.742800432292 322.401300586508
	-423.996225082292 321.970283236508
	-424.249649732292 321.539265886508
	-424.503074382292 321.108248536508
	-424.756499032292 320.677231186508
	-425.009923682292 320.246213836508
	-425.263348332292 319.815196486508
	-425.516772982292 319.384179136508
	-425.770197632292 318.953161786508
	-395.392247174727 310.196494961
	-395.685584674727 309.791583761
	-395.978922174727 309.386672561
	-396.272259674727 308.981761361
	-396.565597174727 308.576850161
	-396.858934674727 308.171938961
	-397.152272174727 307.767027761
	-397.445609674727 307.362116561
	-397.738947174727 306.957205361
	-398.032284674727 306.552294161
	-398.325622174727 306.147382961
	-398.618959674727 305.742471761
	-398.912297174727 305.337560561
	-399.205634674727 304.932649361
	-399.498972174727 304.527738161
	-399.792309674727 304.122826961
	-400.085647174727 303.717915761
	-400.378984674727 303.313004561
	-400.672322174727 302.908093361
	-400.965659674727 302.503182161
	-370.21131762 293.8136828
	-370.50544782 293.40934705
	-370.79957802 293.0050113
	-371.09370822 292.60067555
	-371.38783842 292.1963398
	-371.68196862 291.79200405
	-371.97609882 291.3876683
	-372.27022902 290.98333255
	-372.56435922 290.5789968
	-372.85848942 290.17466105
	-373.15261962 289.7703253
	-373.44674982 289.36598955
	-373.74088002 288.9616538
	-374.03501022 288.55731805
	-374.32914042 288.1529823
	-374.62327062 287.74864655
	-374.91740082 287.3443108
	-375.21153102 286.93997505
	-375.50566122 286.5356393
	-375.79979142 286.13130355
	-376.09392162 285.7269678
	-345.45268854 277.49728232
	-345.73271314 277.08305262
	-346.01273774 276.66882292
	-346.29276234 276.25459322
	-346.57278694 275.84036352
	-346.85281154 275.42613382
	-347.13283614 275.01190412
	-347.41286074 274.59767442
	-347.69288534 274.18344472
	-347.97290994 273.76921502
	-348.25293454 273.35498532
	-348.53295914 272.94075562
	-348.81298374 272.52652592
	-349.09300834 272.11229622
	-349.37303294 271.69806652
	-349.65305754 271.28383682
	-349.93308214 270.86960712
	-350.21310674 270.45537742
	-350.49313134 270.04114772
	-350.77315594 269.62691802
	-351.05318054 269.21268832
	-336.001018270444 270.733668467147
	-336.265155220444 270.309131467147
	-336.529292170444 269.884594467147
	-336.793429120444 269.460057467147
	-337.057566070444 269.035520467147
	-337.321703020444 268.610983467147
	-337.585839970444 268.186446467147
	-337.849976920444 267.761909467147
	-338.114113870444 267.337372467147
	-338.378250820444 266.912835467147
	-338.642387770444 266.488298467147
	-338.906524720444 266.063761467147
	-339.170661670444 265.639224467147
	-339.434798620444 265.214687467147
	-339.698935570444 264.790150467147
	-339.963072520444 264.365613467147
	-340.227209470444 263.941076467147
	-340.491346420444 263.516539467147
	-340.755483370444 263.092002467147
	-341.019620320444 262.667465467147
	-329.273864734266 265.974284291099
	-329.496918534266 265.526794641099
	-329.719972334266 265.079304991099
	-329.943026134266 264.631815341099
	-330.166079934266 264.1843256911
	-330.389133734266 263.736836041099
	-330.612187534266 263.289346391099
	-330.835241334266 262.841856741099
	-331.058295134266 262.394367091099
	-331.281348934266 261.9468774411
	-331.504402734266 261.499387791099
	-331.727456534266 261.051898141099
	-331.950510334266 260.604408491099
	-332.173564134266 260.156918841099
	-332.396617934266 259.7094291911
	-332.619671734266 259.261939541099
	-332.842725534266 258.814449891099
	-333.065779334266 258.366960241099
	-333.288833134266 257.919470591099
	-333.511886934266 257.4719809411
	-322.909829395966 261.473775018368
	-323.042079545966 260.991582218368
	-323.174329695966 260.509389418368
	-323.306579845966 260.027196618368
	-323.438829995966 259.545003818368
	-323.571080145966 259.062811018368
	-323.703330295966 258.580618218368
	-323.835580445966 258.098425418368
	-323.967830595966 257.616232618368
	-324.100080745966 257.134039818368
	-324.232330895966 256.651847018368
	-324.364581045966 256.169654218368
	-324.496831195966 255.687461418368
	-324.629081345966 255.205268618368
	-324.761331495966 254.723075818368
	-324.893581645966 254.240883018368
	-325.025831795966 253.758690218368
	-325.158081945966 253.276497418368
	-325.290332095966 252.794304618368
	-325.422582245966 252.312111818368
	-315.661558214901 257.406329529307
	-315.662463864901 256.906330329307
	-315.663369514901 256.406331129307
	-315.664275164901 255.906331929307
	-315.665180814901 255.406332729307
	-315.666086464901 254.906333529307
	-315.666992114901 254.406334329307
	-315.667897764901 253.906335129307
	-315.668803414901 253.406335929307
	-315.669709064901 252.906336729307
	-315.670614714901 252.406337529307
	-315.671520364901 251.906338329307
	-315.672426014901 251.406339129307
	-315.673331664901 250.906339929307
	-315.674237314901 250.406340729307
	-315.675142964901 249.906341529307
	-315.676048614901 249.406342329307
	-315.676954264901 248.906343129307
	-315.677859914901 248.406343929307
	-315.678765564901 247.906344729307
	-315.679671214901 247.406345529307
	-307.32450448 256.37224002
	-307.15322128 255.90249322
	-306.98193808 255.43274642
	-306.81065488 254.96299962
	-306.63937168 254.49325282
	-306.46808848 254.02350602
	-306.29680528 253.55375922
	-306.12552208 253.08401242
	-305.95423888 252.61426562
	-305.78295568 252.14451882
	-305.61167248 251.67477202
	-305.44038928 251.20502522
	-305.26910608 250.73527842
	-305.09782288 250.26553162
	-304.92653968 249.79578482
	-304.75525648 249.32603802
	-304.58397328 248.85629122
	-304.41269008 248.38654442
	-304.24140688 247.91679762
	-304.07012368 247.44705082
	-303.89884048 246.97730402
	-299.541650593178 259.957250896896
	-299.203918243178 259.588554696896
	-298.866185893178 259.219858496896
	-298.528453543178 258.851162296896
	-298.190721193178 258.482466096896
	-297.852988843178 258.113769896896
	-297.515256493178 257.745073696896
	-297.177524143178 257.376377496896
	-296.839791793178 257.007681296896
	-296.502059443178 256.638985096896
	-296.164327093178 256.270288896896
	-295.826594743178 255.901592696896
	-295.488862393178 255.532896496896
	-295.151130043178 255.164200296896
	-294.813397693178 254.795504096896
	-294.475665343178 254.426807896896
	-294.137932993178 254.058111696896
	-293.800200643178 253.689415496896
	-293.462468293178 253.320719296896
	-293.124735943178 252.952023096896
	-294.69388277 267.20559837
	-294.24848772 266.97839082
	-293.80309267 266.75118327
	-293.35769762 266.52397572
	-292.91230257 266.29676817
	-292.46690752 266.06956062
	-292.02151247 265.84235307
	-291.57611742 265.61514552
	-291.13072237 265.38793797
	-290.68532732 265.16073042
	-290.23993227 264.93352287
	-289.79453722 264.70631532
	-289.34914217 264.47910777
	-288.90374712 264.25190022
	-288.45835207 264.02469267
	-288.01295702 263.79748512
	-287.56756197 263.57027757
	-287.12216692 263.34307002
	-286.67677187 263.11586247
	-286.23137682 262.88865492
	-285.78598177 262.66144737
	-293.435881624009 275.679821645176
	-292.942690424009 275.597587595176
	-292.449499224009 275.515353545176
	-291.956308024009 275.433119495176
	-291.463116824009 275.350885445176
	-290.969925624009 275.268651395176
	-290.476734424009 275.186417345176
	-289.983543224009 275.104183295176
	-289.490352024009 275.021949245176
	-288.997160824009 274.939715195176
	-288.503969624009 274.857481145176
	-288.010778424009 274.775247095176
	-287.517587224009 274.693013045176
	-287.024396024009 274.610778995176
	-286.531204824009 274.528544945176
	-286.038013624009 274.446310895176
	-285.544822424009 274.364076845176
	-285.051631224009 274.281842795176
	-284.558440024009 274.199608745176
	-284.065248824009 274.117374695176
	-283.572057624009 274.035140645176
	-292.395191519092 284.523025000787
	-291.895862019092 284.497140100787
	-291.396532519092 284.471255200787
	-290.897203019092 284.445370300787
	-290.397873519092 284.419485400787
	-289.898544019092 284.393600500787
	-289.399214519092 284.367715600787
	-288.899885019092 284.341830700787
	-288.400555519092 284.315945800787
	-287.901226019092 284.290060900787
	-287.401896519092 284.264176000787
	-286.902567019092 284.238291100787
	-286.403237519092 284.212406200787
	-285.903908019092 284.186521300787
	-285.404578519092 284.160636400787
	-284.905249019092 284.134751500787
	-284.405919519092 284.108866600787
	-283.906590019092 284.082981700787
	-283.407260519092 284.057096800787
	-282.907931019092 284.031211900787
	-291.262700648538 293.653555794974
	-290.765328148538 293.602363844974
	-290.267955648538 293.551171894974
	-289.770583148538 293.499979944974
	-289.273210648538 293.448787994974
	-288.775838148538 293.397596044974
	-288.278465648538 293.346404094974
	-287.781093148538 293.295212144974
	-287.283720648538 293.244020194974
	-286.786348148538 293.192828244974
	-286.288975648538 293.141636294974
	-285.791603148538 293.090444344974
	-285.294230648538 293.039252394974
	-284.796858148538 292.988060444974
	-284.299485648538 292.936868494974
	-283.802113148538 292.885676544974
	-283.304740648538 292.834484594974
	-282.807368148538 292.783292644974
	-282.309995648538 292.732100694974
	-281.812623148538 292.680908744974
	-290.17816098 302.74833012
	-289.69497893 302.61974117
	-289.21179688 302.49115222
	-288.72861483 302.36256327
	-288.24543278 302.23397432
	-287.76225073 302.10538537
	-287.27906868 301.97679642
	-286.79588663 301.84820747
	-286.31270458 301.71961852
	-285.82952253 301.59102957
	-285.34634048 301.46244062
	-284.86315843 301.33385167
	-284.37997638 301.20526272
	-283.89679433 301.07667377
	-283.41361228 300.94808482
	-282.93043023 300.81949587
	-282.44724818 300.69090692
	-281.96406613 300.56231797
	-281.48088408 300.43372902
	-280.99770203 300.30514007
	-288.55195865689 312.363020297248
	-288.11103110689 312.127260097248
	-287.67010355689 311.891499897248
	-287.22917600689 311.655739697248
	-286.78824845689 311.419979497248
	-286.34732090689 311.184219297248
	-285.90639335689 310.948459097248
	-285.46546580689 310.712698897248
	-285.02453825689 310.476938697248
	-284.58361070689 310.241178497248
	-284.14268315689 310.005418297248
	-283.70175560689 309.769658097248
	-283.26082805689 309.533897897248
	-282.81990050689 309.298137697248
	-282.37897295689 309.062377497248
	-281.93804540689 308.826617297248
	-281.49711785689 308.590857097248
	-281.05619030689 308.355096897248
	-280.61526275689 308.119336697248
	-280.17433520689 307.883576497248
	-285.550018223383 322.791126305838
	-285.173988873383 322.461578255838
	-284.797959523383 322.132030205838
	-284.421930173383 321.802482155838
	-284.045900823383 321.472934105838
	-283.669871473383 321.143386055838
	-283.293842123383 320.813838005838
	-282.917812773383 320.484289955838
	-282.541783423383 320.154741905838
	-282.165754073383 319.825193855838
	-281.789724723383 319.495645805838
	-281.413695373383 319.166097755838
	-281.037666023383 318.836549705838
	-280.661636673383 318.507001655838
	-280.285607323383 318.177453605838
	-279.909577973383 317.847905555838
	-279.533548623383 317.518357505838
	-279.157519273383 317.188809455838
	-278.781489923383 316.859261405838
	-278.405460573383 316.529713355838
	-278.752234293172 331.60230552638
	-278.461854793172 331.19526777638
	-278.171475293172 330.78823002638
	-277.881095793172 330.38119227638
	-277.590716293172 329.97415452638
	-277.300336793172 329.56711677638
	-277.009957293172 329.16007902638
	-276.719577793172 328.75304127638
	-276.429198293172 328.34600352638
	-276.138818793172 327.93896577638
	-275.848439293172 327.53192802638
	-275.558059793172 327.12489027638
	-275.267680293172 326.71785252638
	-274.977300793172 326.31081477638
	-274.686921293172 325.90377702638
	-274.396541793172 325.49673927638
	-274.106162293172 325.08970152638
	-273.815782793172 324.68266377638
	-273.525403293172 324.27562602638
	-273.235023793172 323.86858827638
	-269.026745191005 336.530697014884
	-268.826222241005 336.072668014884
	-268.625699291005 335.614639014884
	-268.425176341005 335.156610014884
	-268.224653391005 334.698581014884
	-268.024130441005 334.240552014884
	-267.823607491005 333.782523014884
	-267.623084541005 333.324494014884
	-267.422561591005 332.866465014884
	-267.222038641005 332.408436014884
	-267.021515691005 331.950407014884
	-266.820992741005 331.492378014884
	-266.620469791005 331.034349014884
	-266.419946841005 330.576320014884
	-266.219423891005 330.118291014884
	-266.018900941005 329.660262014884
	-265.818377991005 329.202233014884
	-265.617855041005 328.744204014884
	-265.417332091005 328.286175014884
	-265.216809141005 327.828146014884
	-265.016286191005 327.370117014884
	-258.31700722631 336.910956087495
	-258.20523747631 336.423608637495
	-258.09346772631 335.936261187495
	-257.98169797631 335.448913737495
	-257.86992822631 334.961566287495
	-257.75815847631 334.474218837495
	-257.64638872631 333.986871387495
	-257.53461897631 333.499523937495
	-257.42284922631 333.012176487495
	-257.31107947631 332.524829037495
	-257.19930972631 332.037481587495
	-257.08753997631 331.550134137495
	-256.97577022631 331.062786687495
	-256.86400047631 330.575439237495
	-256.75223072631 330.088091787495
	-256.64046097631 329.600744337495
	-256.52869122631 329.113396887495
	-256.41692147631 328.626049437495
	-256.30515172631 328.138701987495
	-256.19338197631 327.651354537495
	-248.487509471732 335.970856944646
	-248.449441471732 335.472308244646
	-248.411373471732 334.973759544646
	-248.373305471732 334.475210844646
	-248.335237471732 333.976662144646
	-248.297169471732 333.478113444646
	-248.259101471732 332.979564744646
	-248.221033471732 332.481016044646
	-248.182965471732 331.982467344646
	-248.144897471732 331.483918644646
	-248.106829471732 330.985369944646
	-248.068761471732 330.486821244646
	-248.030693471732 329.988272544646
	-247.992625471732 329.489723844646
	-247.954557471732 328.991175144646
	-247.916489471732 328.492626444646
	-247.878421471732 327.994077744646
	-247.840353471732 327.495529044646
	-247.802285471732 326.996980344646
	-247.764217471732 326.498431644646
	-239.197356146667 334.321421217921
	-239.212071096667 333.821637817921
	-239.226786046667 333.321854417921
	-239.241500996667 332.822071017921
	-239.256215946667 332.322287617921
	-239.270930896667 331.822504217921
	-239.285645846667 331.322720817921
	-239.300360796667 330.822937417921
	-239.315075746667 330.323154017921
	-239.329790696667 329.823370617921
	-239.344505646667 329.323587217921
	-239.359220596667 328.823803817921
	-239.373935546667 328.324020417921
	-239.388650496667 327.824237017921
	-239.403365446667 327.324453617921
	-239.418080396667 326.824670217921
	-239.432795346667 326.324886817921
	-239.447510296667 325.825103417921
	-239.462225246667 325.325320017921
	-239.476940196667 324.825536617921
	-230.07839239072 333.321245965909
	-230.12530889072 332.823451965909
	-230.17222539072 332.325657965909
	-230.21914189072 331.827863965909
	-230.26605839072 331.330069965909
	-230.31297489072 330.832275965909
	-230.35989139072 330.334481965909
	-230.40680789072 329.836687965909
	-230.45372439072 329.338893965909
	-230.50064089072 328.841099965909
	-230.54755739072 328.343305965909
	-230.59447389072 327.845511965909
	-230.64139039072 327.347717965909
	-230.68830689072 326.849923965909
	-230.73522339072 326.352129965909
	-230.78213989072 325.854335965909
	-230.82905639072 325.356541965909
	-230.87597289072 324.858747965909
	-230.92288939072 324.360953965909
	-230.96980589072 323.863159965909
	-231.01672239072 323.365365965909
	-200.431984645119 328.244718019374
	-200.515947795119 327.751818269374
	-200.599910945119 327.258918519375
	-200.683874095119 326.766018769375
	-200.767837245119 326.273119019375
	-200.851800395119 325.780219269375
	-200.935763545119 325.287319519374
	-201.019726695119 324.794419769374
	-201.103689845119 324.301520019374
	-201.187652995119 323.808620269375
	-201.271616145119 323.315720519375
	-201.355579295119 322.822820769375
	-201.439542445119 322.329921019375
	-201.523505595119 321.837021269374
	-201.607468745119 321.344121519374
	-201.691431895119 320.851221769374
	-201.775395045119 320.358322019374
	-201.859358195119 319.865422269375
	-201.943321345119 319.372522519375
	-202.027284495119 318.879622769375
	-170.836779028555 323.336738526597
	-170.947334678555 322.849114226597
	-171.057890328555 322.361489926597
	-171.168445978555 321.873865626597
	-171.279001628555 321.386241326597
	-171.389557278555 320.898617026597
	-171.500112928555 320.410992726597
	-171.610668578555 319.923368426597
	-171.721224228555 319.435744126597
	-171.831779878555 318.948119826597
	-171.942335528555 318.460495526597
	-172.052891178555 317.972871226597
	-172.163446828555 317.485246926597
	-172.274002478555 316.997622626597
	-172.384558128555 316.509998326597
	-172.495113778555 316.022374026597
	-172.605669428555 315.534749726597
	-172.716225078555 315.047125426597
	-172.826780728555 314.559501126597
	-140.58761773771 318.414923101222
	-140.76253253771 317.946516401222
	-140.93744733771 317.478109701222
	-141.11236213771 317.009703001222
	-141.28727693771 316.541296301223
	-141.46219173771 316.072889601223
	-141.63710653771 315.604482901223
	-141.81202133771 315.136076201223
	-141.98693613771 314.667669501223
	-142.16185093771 314.199262801223
	-142.33676573771 313.730856101223
	-142.51168053771 313.262449401223
	-142.68659533771 312.794042701223
	-142.86151013771 312.325636001223
	-143.03642493771 311.857229301223
	-143.21133973771 311.388822601223
	-143.38625453771 310.920415901222
	-143.56116933771 310.452009201222
	-143.73608413771 309.983602501222
	-111.305616031182 308.272941445288
	-111.545403731182 307.834191095288
	-111.785191431182 307.395440745288
	-112.024979131182 306.956690395288
	-112.264766831182 306.517940045288
	-112.504554531182 306.079189695288
	-112.744342231182 305.640439345288
	-112.984129931182 305.201688995288
	-113.223917631182 304.762938645288
	-113.463705331182 304.324188295288
	-113.703493031182 303.885437945288
	-113.943280731182 303.446687595288
	-114.183068431182 303.007937245288
	-114.422856131182 302.569186895288
	-114.662643831182 302.130436545288
	-114.902431531182 301.691686195288
	-115.142219231182 301.252935845288
	-115.382006931182 300.814185495288
	-115.621794631182 300.375435145288
	-115.861582331182 299.936684795288
	-88.38049847 287.2560421
	-88.67355452 286.8509271
	-88.96661057 286.4458121
	-89.25966662 286.0406971
	-89.55272267 285.6355821
	-89.84577872 285.2304671
	-90.13883477 284.8253521
	-90.43189082 284.4202371
	-90.72494687 284.0151221
	-91.01800292 283.6100071
	-91.31105897 283.2048921
	-91.60411502 282.7997771
	-91.89717107 282.3946621
	-92.19022712 281.9895471
	-92.48328317 281.5844321
	-92.77633922 281.1793171
	-93.06939527 280.7742021
	-93.36245132 280.3690871
	-93.65550737 279.9639721
	-93.94856342 279.5588571
	-66.171091941681 266.885604712332
	-66.503272741681 266.511899062332
	-66.835453541681 266.138193412332
	-67.167634341681 265.764487762332
	-67.499815141681 265.390782112332
	-67.831995941681 265.017076462332
	-68.164176741681 264.643370812332
	-68.496357541681 264.269665162332
	-68.828538341681 263.895959512332
	-69.160719141681 263.522253862332
	-69.492899941681 263.148548212332
	-69.825080741681 262.774842562332
	-70.157261541681 262.401136912332
	-70.489442341681 262.027431262332
	-70.821623141681 261.653725612332
	-71.153803941681 261.280019962332
	-71.485984741681 260.906314312332
	-71.818165541681 260.532608662332
	-72.150346341681 260.158903012332
	-72.482527141681 259.785197362332
	-44.2190941209642 246.393958938745
	-44.5715747709642 246.039336038745
	-44.9240554209642 245.684713138745
	-45.2765360709642 245.330090238745
	-45.6290167209642 244.975467338745
	-45.9814973709642 244.620844438745
	-46.3339780209642 244.266221538745
	-46.6864586709642 243.911598638745
	-47.0389393209642 243.556975738745
	-47.3914199709642 243.202352838745
	-47.7439006209642 242.847729938745
	-48.0963812709642 242.493107038745
	-48.4488619209642 242.138484138745
	-48.8013425709642 241.783861238745
	-49.1538232209642 241.429238338745
	-49.5063038709642 241.074615438745
	-49.8587845209642 240.719992538745
	-50.2112651709642 240.365369638745
	-50.5637458209642 240.010746738745
	-50.9162264709642 239.656123838745
	-22.0276812163313 226.08944608524
	-22.3851555163313 225.73985758524
	-22.7426298163313 225.39026908524
	-23.1001041163313 225.04068058524
	-23.4575784163313 224.69109208524
	-23.8150527163313 224.34150358524
	-24.1725270163313 223.99191508524
	-24.5300013163313 223.64232658524
	-24.8874756163313 223.29273808524
	-25.2449499163313 222.94314958524
	-25.6024242163313 222.59356108524
	-25.9598985163313 222.24397258524
	-26.3173728163313 221.89438408524
	-26.6748471163313 221.54479558524
	-27.0323214163313 221.19520708524
	-27.3897957163313 220.84561858524
	-27.7472700163313 220.49603008524
	-28.1047443163313 220.14644158524
	-28.4622186163313 219.79685308524
	-28.8196929163313 219.44726458524
	0.17003962354202 205.854384046441
	-0.18897142645798 205.506373896441
	-0.54798247645798 205.158363746441
	-0.90699352645798 204.810353596441
	-1.26600457645798 204.462343446441
	-1.62501562645798 204.114333296441
	-1.98402667645798 203.766323146441
	-2.34303772645798 203.418312996441
	-2.70204877645798 203.070302846441
	-3.06105982645798 202.722292696441
	-3.42007087645798 202.374282546441
	-3.77908192645798 202.026272396441
	-4.13809297645798 201.678262246441
	-4.49710402645798 201.330252096441
	-4.85611507645798 200.982241946441
	-5.21512612645798 200.634231796441
	-5.57413717645798 200.286221646441
	-5.93314822645798 199.938211496441
	-6.29215927645798 199.590201346441
	-6.65117032645798 199.242191196441
	22.3185236069918 185.568149428077
	21.9583905569918 185.221300478077
	21.5982575069918 184.874451528077
	21.2381244569918 184.527602578077
	20.8779914069918 184.180753628077
	20.5178583569918 183.833904678077
	20.1577253069918 183.487055728077
	19.7975922569918 183.140206778077
	19.4374592069918 182.793357828077
	19.0773261569918 182.446508878077
	18.7171931069918 182.099659928077
	18.3570600569918 181.752810978077
	17.9969270069918 181.405962028077
	17.6367939569918 181.059113078077
	17.2766609069918 180.712264128077
	16.9165278569918 180.365415178077
	16.5563948069918 180.018566228077
	16.1962617569918 179.671717278077
	15.8361287069918 179.324868328077
	15.4759956569918 178.978019378077
	44.2947553724756 165.127872232704
	43.9361562224756 164.779437682704
	43.5775570724756 164.431003132704
	43.2189579224756 164.082568582704
	42.8603587724756 163.734134032704
	42.5017596224756 163.385699482704
	42.1431604724756 163.037264932704
	41.7845613224756 162.688830382704
	41.4259621724756 162.340395832704
	41.0673630224756 161.991961282704
	40.7087638724756 161.643526732704
	40.3501647224756 161.295092182704
	39.9915655724756 160.946657632704
	39.6329664224756 160.598223082704
	39.2743672724756 160.249788532704
	38.9157681224756 159.901353982704
	38.5571689724756 159.552919432704
	38.1985698224756 159.204484882704
	37.8399706724756 158.856050332704
	37.4813715224756 158.507615782704
	66.1555732055899 144.813892209106
	65.8049554555899 144.457427359106
	65.4543377055899 144.100962509106
	65.10371995559 143.744497659106
	64.75310220559 143.388032809106
	64.4024844555899 143.031567959106
	64.0518667055899 142.675103109106
	63.7012489555899 142.318638259106
	63.3506312055899 141.962173409106
	63.00001345559 141.605708559106
	62.6493957055899 141.249243709106
	62.2987779555899 140.892778859106
	61.94816020559 140.536314009106
	61.5975424555899 140.179849159106
	61.2469247055899 139.823384309106
	60.8963069555899 139.466919459106
	60.5456892055899 139.110454609106
	60.1950714555899 138.753989759106
	59.8444537055899 138.397524909106
	59.4938359555899 138.041060059106
	87.9539327344448 124.722880743987
	87.6163107844448 124.354083443987
	87.2786888344448 123.985286143987
	86.9410668844448 123.616488843987
	86.6034449344448 123.247691543987
	86.2658229844448 122.878894243987
	85.9282010344448 122.510096943987
	85.5905790844448 122.141299643987
	85.2529571344448 121.772502343987
	84.9153351844448 121.403705043987
	84.5777132344448 121.034907743987
	84.2400912844448 120.666110443987
	83.9024693344448 120.297313143987
	83.5648473844448 119.928515843987
	83.2272254344448 119.559718543987
	82.8896034844448 119.190921243987
	82.5519815344448 118.822123943987
	82.2143595844448 118.453326643987
	81.8767376344448 118.084529343987
	81.5391156844448 117.715732043987
	110.298710618359 104.615280607871
	109.958758068359 104.248630557871
	109.618805518359 103.881980507871
	109.278852968359 103.515330457871
	108.938900418359 103.148680407871
	108.598947868359 102.782030357871
	108.258995318359 102.415380307871
	107.919042768359 102.048730257871
	107.579090218359 101.682080207871
	107.239137668359 101.315430157871
	106.899185118359 100.948780107871
	106.559232568359 100.582130057871
	106.219280018359 100.215480007871
	105.879327468359 99.8488299578706
	105.539374918359 99.4821799078706
	105.199422368359 99.1155298578706
	104.859469818359 98.7488798078706
	104.519517268359 98.3822297578706
	104.179564718359 98.0155797078706
	103.839612168359 97.6489296578706
	131.552258974802 84.8701590097299
	131.257043574802 84.4666148597299
	130.961828174802 84.0630707097299
	130.666612774802 83.6595265597299
	130.371397374802 83.2559824097299
	130.076181974802 82.8524382597299
	129.780966574802 82.4488941097299
	129.485751174802 82.0453499597299
	129.190535774802 81.6418058097299
	128.895320374802 81.2382616597299
	128.600104974802 80.8347175097299
	128.304889574802 80.4311733597299
	128.009674174802 80.0276292097299
	127.714458774802 79.6240850597299
	127.419243374802 79.2205409097299
	127.124027974802 78.8169967597299
	126.828812574802 78.4134526097299
	126.533597174802 78.0099084597299
	126.238381774802 77.6063643097299
	125.943166374802 77.2028201597299
	137.6822505985 78.9303189598792
	137.4184183985 78.5055925098792
	137.1545861985 78.0808660598792
	136.8907539985 77.6561396098792
	136.6269217985 77.2314131598792
	136.3630895985 76.8066867098792
	136.0992573985 76.3819602598792
	135.8354251985 75.9572338098792
	135.5715929985 75.5325073598792
	135.3077607985 75.1077809098792
	135.0439285985 74.6830544598792
	134.7800963985 74.2583280098792
	134.5162641985 73.8336015598792
	134.2524319985 73.4088751098792
	133.9885997985 72.9841486598792
	133.7247675985 72.5594222098792
	133.4609353985 72.1346957598792
	133.1971031985 71.7099693098792
	132.9332709985 71.2852428598792
	132.6694387985 70.8605164098792
	144.109905682285 72.952565981099
	143.879338632285 72.5089007310989
	143.648771582285 72.065235481099
	143.418204532285 71.621570231099
	143.187637482285 71.1779049810989
	142.957070432285 70.734239731099
	142.726503382285 70.290574481099
	142.495936332285 69.8469092310989
	142.265369282285 69.403243981099
	142.034802232285 68.9595787310989
	141.804235182285 68.5159134810989
	141.573668132285 68.072248231099
	141.343101082285 67.6285829810989
	141.112534032285 67.1849177310989
	140.881966982285 66.741252481099
	140.651399932285 66.2975872310989
	140.420832882285 65.8539219810989
	140.190265832285 65.410256731099
	139.959698782285 64.9665914810989
	139.729131732285 64.5229262310989
	150.929101035321 66.9510322093478
	150.733189085321 66.4910120593478
	150.537277135321 66.0309919093478
	150.341365185321 65.5709717593478
	150.145453235321 65.1109516093478
	149.949541285321 64.6509314593478
	149.753629335321 64.1909113093478
	149.557717385321 63.7308911593478
	149.361805435321 63.2708710093478
	149.165893485321 62.8108508593478
	148.969981535321 62.3508307093478
	148.774069585321 61.8908105593478
	148.578157635321 61.4307904093478
	148.382245685321 60.9707702593478
	148.186333735321 60.5107501093478
	147.990421785321 60.0507299593478
	147.794509835321 59.5907098093478
	147.598597885321 59.1306896593478
	147.402685935321 58.6706695093478
	147.206773985321 58.2106493593478
	158.540835322447 61.8936258274158
	158.380977422447 61.4198690774158
	158.221119522447 60.9461123274158
	158.061261622447 60.4723555774158
	157.901403722447 59.9985988274158
	157.741545822447 59.5248420774158
	157.581687922447 59.0510853274158
	157.421830022447 58.5773285774158
	157.261972122447 58.1035718274158
	157.102114222447 57.6298150774158
	156.942256322447 57.1560583274158
	156.782398422447 56.6823015774158
	156.622540522447 56.2085448274158
	156.462682622447 55.7347880774158
	156.302824722447 55.2610313274158
	156.142966822447 54.7872745774158
	155.983108922447 54.3135178274158
	155.823251022447 53.8397610774158
	155.663393122447 53.3660043274158
	155.503535222447 52.8922475774158
	167.420941088867 60.3093747901648
	167.298524738867 59.8245920901648
	167.176108388867 59.3398093901648
	167.053692038867 58.8550266901648
	166.931275688867 58.3702439901648
	166.808859338867 57.8854612901648
	166.686442988867 57.4006785901648
	166.564026638867 56.9158958901648
	166.441610288867 56.4311131901648
	166.319193938867 55.9463304901648
	166.196777588867 55.4615477901648
	166.074361238867 54.9767650901648
	165.951944888867 54.4919823901648
	165.829528538867 54.0071996901648
	165.707112188867 53.5224169901648
	165.584695838867 53.0376342901648
	165.462279488867 52.5528515901648
	165.339863138867 52.0680688901648
	165.217446788867 51.5832861901648
	165.095030438867 51.0985034901648
	164.972614088867 50.6137207901648
	176.664187601337 61.4293897571094
	176.580539201337 60.9364364571094
	176.496890801337 60.4434831571094
	176.413242401337 59.9505298571094
	176.329594001337 59.4575765571094
	176.245945601337 58.9646232571094
	176.162297201337 58.4716699571094
	176.078648801337 57.9787166571094
	175.995000401337 57.4857633571094
	175.911352001337 56.9928100571094
	175.827703601337 56.4998567571094
	175.744055201337 56.0069034571094
	175.660406801337 55.5139501571094
	175.576758401337 55.0209968571094
	175.493110001337 54.5280435571094
	175.409461601337 54.0350902571094
	175.325813201337 53.5421369571094
	175.242164801337 53.0491836571094
	175.158516401337 52.5562303571094
	175.074868001337 52.0632770571094
	185.48957805396 62.8375493918338
	185.44622545396 62.3394323918338
	185.40287285396 61.8413153918338
	185.35952025396 61.3431983918338
	185.31616765396 60.8450813918338
	185.27281505396 60.3469643918338
	185.22946245396 59.8488473918338
	185.18610985396 59.3507303918338
	185.14275725396 58.8526133918338
	185.09940465396 58.3544963918338
	185.05605205396 57.8563793918338
	185.01269945396 57.3582623918338
	184.96934685396 56.8601453918338
	184.92599425396 56.3620283918338
	184.88264165396 55.8639113918338
	184.83928905396 55.3657943918338
	184.79593645396 54.8676773918338
	184.75258385396 54.3695603918338
	184.70923125396 53.8714433918338
	184.66587865396 53.3733263918338
	184.62252605396 52.8752093918338
	193.917352701934 63.9851403357542
	193.916025401934 63.4851420857542
	193.914698101934 62.9851438357542
	193.913370801934 62.4851455857542
	193.912043501934 61.9851473357542
	193.910716201934 61.4851490857542
	193.909388901934 60.9851508357542
	193.908061601934 60.4851525857542
	193.906734301934 59.9851543357542
	193.905407001934 59.4851560857542
	193.904079701934 58.9851578357543
	193.902752401934 58.4851595857542
	193.901425101934 57.9851613357542
	193.900097801934 57.4851630857542
	193.898770501934 56.9851648357542
	193.897443201934 56.4851665857542
	193.896115901934 55.9851683357542
	193.894788601934 55.4851700857542
	193.893461301934 54.9851718357542
	193.892134001934 54.4851735857542
	202.0800591 65.32850746
	202.1221476 64.83028206
	202.1642361 64.33205666
	202.2063246 63.83383126
	202.2484131 63.33560586
	202.2905016 62.83738046
	202.3325901 62.33915506
	202.3746786 61.84092966
	202.4167671 61.34270426
	202.4588556 60.84447886
	202.5009441 60.34625346
	202.5430326 59.84802806
	202.5851211 59.34980266
	202.6272096 58.85157726
	202.6692981 58.35335186
	202.7113866 57.85512646
	202.7534751 57.35690106
	202.7955636 56.85867566
	202.8376521 56.36045026
	202.8797406 55.86222486
	210.253295715122 66.3490984097875
	210.334229415122 65.8556921597875
	210.415163115122 65.3622859097875
	210.496096815122 64.8688796597875
	210.577030515122 64.3754734097875
	210.657964215122 63.8820671597875
	210.738897915122 63.3886609097875
	210.819831615122 62.8952546597875
	210.900765315122 62.4018484097875
	210.981699015122 61.9084421597875
	211.062632715122 61.4150359097875
	211.143566415122 60.9216296597875
	211.224500115122 60.4282234097875
	211.305433815122 59.9348171597875
	211.386367515122 59.4414109097875
	211.467301215122 58.9480046597875
	211.548234915122 58.4545984097875
	211.629168615122 57.9611921597875
	211.710102315122 57.4677859097875
	211.791036015122 56.9743796597875
	238.85492942924 70.3400372414483
	239.01796402924 69.8673642914483
	239.18099862924 69.3946913414483
	239.34403322924 68.9220183914483
	239.50706782924 68.4493454414483
	239.67010242924 67.9766724914483
	239.83313702924 67.5039995414483
	239.99617162924 67.0313265914483
	240.15920622924 66.5586536414483
	240.32224082924 66.0859806914483
	240.48527542924 65.6133077414483
	240.64831002924 65.1406347914483
	240.81134462924 64.6679618414483
	240.97437922924 64.1952888914483
	241.13741382924 63.7226159414483
	241.30044842924 63.2499429914483
	241.46348302924 62.7772700414483
	241.62651762924 62.3045970914483
	241.78955222924 61.8319241414483
	241.95258682924 61.3592511914483
	269.062130859088 74.7852112969529
	269.170862609088 74.2971770469529
	269.279594359088 73.8091427969529
	269.388326109088 73.3211085469529
	269.497057859088 72.8330742969528
	269.605789609088 72.3450400469528
	269.714521359088 71.8570057969528
	269.823253109088 71.3689715469528
	269.931984859088 70.8809372969529
	270.040716609088 70.3929030469529
	270.149448359088 69.9048687969529
	270.258180109088 69.4168345469529
	270.366911859088 68.9288002969529
	270.475643609088 68.4407660469528
	270.584375359088 67.9527317969528
	270.693107109088 67.4646975469528
	270.801838859088 66.9766632969529
	270.910570609088 66.4886290469529
	271.019302359088 66.0005947969529
	271.128034109088 65.5125605469529
	277.980771401385 76.3289255904152
	278.042604101385 75.8327635904152
	278.104436801385 75.3366015904152
	278.166269501385 74.8404395904152
	278.228102201385 74.3442775904152
	278.289934901385 73.8481155904152
	278.351767601385 73.3519535904152
	278.413600301385 72.8557915904152
	278.475433001385 72.3596295904152
	278.537265701385 71.8634675904152
	278.599098401385 71.3673055904152
	278.660931101385 70.8711435904152
	278.722763801385 70.3749815904152
	278.784596501385 69.8788195904152
	278.846429201385 69.3826575904152
	278.908261901385 68.8864955904152
	278.970094601385 68.3903335904152
	279.031927301385 67.8941715904152
	279.093760001385 67.3980095904152
	279.155592701385 66.9018475904152
	287.024526117414 77.51899875804
	287.037272667414 77.01916125804
	287.050019217414 76.51932375804
	287.062765767414 76.01948625804
	287.075512317414 75.51964875804
	287.088258867414 75.01981125804
	287.101005417414 74.51997375804
	287.113751967414 74.02013625804
	287.126498517414 73.52029875804
	287.139245067414 73.02046125804
	287.151991617414 72.52062375804
	287.164738167414 72.02078625804
	287.177484717414 71.52094875804
	287.190231267414 71.02111125804
	287.202977817414 70.52127375804
	287.215724367414 70.02143625804
	287.228470917414 69.52159875804
	287.241217467414 69.02176125804
	287.253964017414 68.52192375804
	287.266710567414 68.02208625804
	296.285397062368 78.790073133122
	296.246951712368 78.291553383122
	296.208506362368 77.793033633122
	296.170061012368 77.294513883122
	296.131615662368 76.795994133122
	296.093170312368 76.297474383122
	296.054724962368 75.798954633122
	296.016279612368 75.300434883122
	295.977834262368 74.801915133122
	295.939388912368 74.303395383122
	295.900943562368 73.804875633122
	295.862498212368 73.306355883122
	295.824052862368 72.807836133122
	295.785607512368 72.309316383122
	295.747162162368 71.810796633122
	295.708716812368 71.312276883122
	295.670271462368 70.813757133122
	295.631826112368 70.315237383122
	295.593380762368 69.816717633122
	295.554935412368 69.318197883122
	305.895364518415 79.5541243408225
	305.803523868415 79.0626313908225
	305.711683218415 78.5711384408225
	305.619842568415 78.0796454908225
	305.528001918415 77.5881525408225
	305.436161268415 77.0966595908225
	305.344320618415 76.6051666408225
	305.252479968415 76.1136736908225
	305.160639318415 75.6221807408225
	305.068798668415 75.1306877908225
	304.976958018415 74.6391948408225
	304.885117368415 74.1477018908225
	304.793276718415 73.6562089408225
	304.701436068415 73.1647159908225
	304.609595418415 72.6732230408225
	304.517754768415 72.1817300908225
	304.425914118415 71.6902371408225
	304.334073468415 71.1987441908225
	304.242232818415 70.7072512408225
	304.150392168415 70.2157582908225
	315.637030530082 78.7166837875511
	315.490033230082 78.2387802375511
	315.343035930082 77.7608766875511
	315.196038630082 77.2829731375511
	315.049041330082 76.8050695875511
	314.902044030082 76.3271660375511
	314.755046730082 75.8492624875511
	314.608049430082 75.3713589375511
	314.461052130082 74.8934553875511
	314.314054830082 74.4155518375511
	314.167057530082 73.9376482875511
	314.020060230082 73.4597447375511
	313.873062930082 72.9818411875511
	313.726065630082 72.5039376375511
	313.579068330082 72.0260340875511
	313.432071030082 71.5481305375511
	313.285073730082 71.0702269875511
	313.138076430082 70.5923234375511
	312.991079130082 70.1144198875511
	312.844081830082 69.6365163375511
	325.402682291208 76.6663495670234
	325.199763791208 76.2093768170234
	324.996845291208 75.7524040670234
	324.793926791208 75.2954313170234
	324.591008291208 74.8384585670234
	324.388089791208 74.3814858170234
	324.185171291208 73.9245130670234
	323.982252791208 73.4675403170234
	323.779334291208 73.0105675670234
	323.576415791208 72.5535948170234
	323.373497291208 72.0966220670234
	323.170578791208 71.6396493170234
	322.967660291208 71.1826765670234
	322.764741791208 70.7257038170234
	322.561823291208 70.2687310670234
	322.358904791208 69.8117583170234
	322.155986291208 69.3547855670234
	321.953067791208 68.8978128170234
	321.750149291208 68.4408400670234
	321.547230791208 67.9838673170234
	334.501957202755 72.45497493461
	334.242381202755 72.0276339846099
	333.982805202755 71.6002930346099
	333.723229202755 71.1729520846099
	333.463653202755 70.7456111346099
	333.204077202755 70.3182701846099
	332.944501202755 69.8909292346099
	332.684925202755 69.4635882846099
	332.425349202755 69.03624733461
	332.165773202755 68.60890638461
	331.906197202755 68.18156543461
	331.646621202755 67.7542244846099
	331.387045202755 67.3268835346099
	331.127469202755 66.8995425846099
	330.867893202755 66.4722016346099
	330.608317202755 66.0448606846099
	330.348741202755 65.6175197346099
	330.089165202755 65.1901787846099
	329.829589202755 64.76283783461
	329.570013202755 64.33549688461
	343.054336778755 67.0070948469335
	342.738137228756 66.6197734969335
	342.421937678756 66.2324521469335
	342.105738128756 65.8451307969335
	341.789538578756 65.4578094469335
	341.473339028756 65.0704880969335
	341.157139478756 64.6831667469335
	340.840939928756 64.2958453969335
	340.524740378756 63.9085240469335
	340.208540828756 63.5212026969335
	339.892341278756 63.1338813469335
	339.576141728756 62.7465599969335
	339.259942178756 62.3592386469335
	338.943742628756 61.9719172969335
	338.627543078756 61.5845959469335
	338.311343528756 61.1972745969335
	337.995143978756 60.8099532469335
	337.678944428756 60.4226318969335
	337.362744878756 60.0353105469335
	337.046545328756 59.6479891969335
	350.485687594669 59.9645137371982
	350.115712294669 59.6281831371982
	349.745736994669 59.2918525371982
	349.375761694669 58.9555219371982
	349.005786394669 58.6191913371982
	348.635811094669 58.2828607371982
	348.265835794669 57.9465301371982
	347.895860494669 57.6101995371982
	347.525885194669 57.2738689371982
	347.155909894669 56.9375383371982
	346.785934594669 56.6012077371982
	346.415959294669 56.2648771371982
	346.045983994669 55.9285465371982
	345.676008694669 55.5922159371982
	345.306033394669 55.2558853371982
	344.936058094669 54.9195547371982
	344.566082794669 54.5832241371982
	344.196107494669 54.2468935371982
	343.826132194669 53.9105629371982
	356.820329149639 51.9654872241304
	356.407166199639 51.6838911241304
	355.994003249639 51.4022950241304
	355.580840299639 51.1206989241304
	355.167677349639 50.8391028241304
	354.754514399639 50.5575067241304
	354.341351449639 50.2759106241304
	353.928188499639 49.9943145241304
	353.515025549639 49.7127184241304
	353.101862599639 49.4311223241304
	352.688699649639 49.1495262241304
	352.275536699639 48.8679301241304
	351.862373749639 48.5863340241304
	351.449210799639 48.3047379241304
	351.036047849639 48.0231418241304
	350.622884899639 47.7415457241304
	350.209721949639 47.4599496241304
	349.796558999639 47.1783535241304
	349.383396049639 46.8967574241304
	348.970233099639 46.6151613241304
	361.543750565182 42.9898954907515
	361.097680365182 42.7640163407515
	360.651610165182 42.5381371907515
	360.205539965182 42.3122580407515
	359.759469765182 42.0863788907515
	359.313399565182 41.8604997407515
	358.867329365182 41.6346205907515
	358.421259165182 41.4087414407515
	357.975188965182 41.1828622907515
	357.529118765182 40.9569831407515
	357.083048565182 40.7311039907515
	356.636978365182 40.5052248407515
	356.190908165182 40.2793456907515
	355.744837965182 40.0534665407515
	355.298767765182 39.8275873907515
	354.852697565182 39.6017082407515
	354.406627365182 39.3758290907515
	353.960557165182 39.1499499407515
	353.514486965182 38.9240707907515
	353.068416765182 38.6981916407515
	365.030019330575 33.57354636904
	364.559605330575 33.40410416904
	364.089191330575 33.23466196904
	363.618777330575 33.06521976904
	363.148363330575 32.89577756904
	362.677949330575 32.72633536904
	362.207535330575 32.55689316904
	361.737121330575 32.38745096904
	361.266707330575 32.21800876904
	360.796293330575 32.04856656904
	360.325879330575 31.87912436904
	359.855465330575 31.70968216904
	359.385051330575 31.54023996904
	358.914637330575 31.37079776904
	358.444223330575 31.20135556904
	357.973809330575 31.03191336904
	357.503395330575 30.86247116904
	357.032981330575 30.69302896904
	356.562567330575 30.52358676904
	356.092153330575 30.35414456904
	366.356577683826 23.7063531447758
	365.869331533826 23.5941427947758
	365.382085383826 23.4819324447759
	364.894839233826 23.3697220947758
	364.407593083826 23.2575117447759
	363.920346933826 23.1453013947758
	363.433100783826 23.0330910447759
	362.945854633826 22.9208806947758
	362.458608483826 22.8086703447759
	361.971362333826 22.6964599947759
	361.484116183826 22.5842496447758
	360.996870033826 22.4720392947759
	360.509623883826 22.3598289447758
	360.022377733826 22.2476185947759
	359.535131583826 22.1354082447758
	359.047885433826 22.0231978947759
	358.560639283826 21.9109875447758
	358.073393133826 21.7987771947759
	357.586146983826 21.6865668447759
	357.098900833826 21.5743564947758
	366.100330927486 13.9994246306477
	365.604082827486 13.9382867806477
	365.107834727486 13.8771489306477
	364.611586627486 13.8160110806477
	364.115338527486 13.7548732306477
	363.619090427486 13.6937353806477
	363.122842327486 13.6325975306477
	362.626594227486 13.5714596806477
	362.130346127486 13.5103218306477
	361.634098027486 13.4491839806477
	361.137849927486 13.3880461306477
	360.641601827486 13.3269082806477
	360.145353727486 13.2657704306477
	359.649105627486 13.2046325806477
	359.152857527486 13.1434947306477
	358.656609427486 13.0823568806477
	358.160361327486 13.0212190306477
	357.664113227486 12.9600811806477
	357.167865127486 12.8989433306477
	356.671617027486 12.8378054806477
	364.976005671279 4.6115907675806
	364.476395771279 4.5918437675806
	363.976785871279 4.5720967675806
	363.477175971279 4.5523497675806
	362.977566071279 4.5326027675806
	362.477956171279 4.5128557675806
	361.978346271279 4.4931087675806
	361.478736371279 4.4733617675806
	360.979126471279 4.4536147675806
	360.479516571279 4.4338677675806
	359.979906671279 4.4141207675806
	359.480296771279 4.3943737675806
	358.980686871279 4.3746267675806
	358.481076971279 4.3548797675806
	357.981467071279 4.3351327675806
	357.481857171279 4.3153857675806
	356.982247271279 4.2956387675806
	356.482637371279 4.2758917675806
	355.983027471279 4.2561447675806
	355.483417571279 4.2363977675806
	364.160143606405 -4.53740955731017
	363.660278356405 -4.52580270731017
	363.160413106405 -4.51419585731017
	362.660547856405 -4.50258900731017
	362.160682606405 -4.49098215731017
	361.660817356405 -4.47937530731017
	361.160952106405 -4.46776845731017
	360.661086856405 -4.45616160731017
	360.161221606405 -4.44455475731017
	359.661356356405 -4.43294790731017
	359.161491106405 -4.42134105731017
	358.661625856405 -4.40973420731017
	358.161760606405 -4.39812735731017
	357.661895356405 -4.38652050731017
	357.162030106405 -4.37491365731017
	356.662164856405 -4.36330680731017
	356.162299606405 -4.35169995731017
	355.662434356405 -4.34009310731017
	355.162569106405 -4.32848625731017
	354.662703856405 -4.31687940731017
	360.228269226936 -34.4022135428782
	359.731979426936 -34.3414154428782
	359.235689626936 -34.2806173428782
	358.739399826936 -34.2198192428782
	358.243110026936 -34.1590211428782
	357.746820226936 -34.0982230428782
	357.250530426936 -34.0374249428782
	356.754240626936 -33.9766268428782
	356.257950826936 -33.9158287428782
	355.761661026936 -33.8550306428782
	355.265371226936 -33.7942325428782
	354.769081426936 -33.7334344428782
	354.272791626936 -33.6726363428782
	353.776501826936 -33.6118382428782
	353.280212026936 -33.5510401428782
	352.783922226936 -33.4902420428782
	352.287632426936 -33.4294439428782
	351.791342626936 -33.3686458428782
	351.295052826936 -33.3078477428782
	356.887395661852 -64.1941705865344
	356.390938261852 -64.1347561865344
	355.894480861852 -64.0753417865344
	355.398023461852 -64.0159273865344
	354.901566061852 -63.9565129865344
	354.405108661852 -63.8970985865344
	353.908651261852 -63.8376841865344
	353.412193861852 -63.7782697865344
	352.915736461852 -63.7188553865344
	352.419279061852 -63.6594409865344
	351.922821661852 -63.6000265865344
	351.426364261852 -63.5406121865344
	350.929906861852 -63.4811977865344
	350.433449461852 -63.4217833865344
	349.936992061852 -63.3623689865344
	349.440534661852 -63.3029545865344
	348.944077261852 -63.2435401865344
	348.447619861852 -63.1841257865344
	347.951162461852 -63.1247113865344
	347.454705061852 -63.0652969865344
	353.099793436261 -93.9598623674527
	352.603319086261 -93.9005901174527
	352.106844736261 -93.8413178674527
	351.610370386261 -93.7820456174527
	351.113896036261 -93.7227733674527
	350.617421686261 -93.6635011174527
	350.120947336261 -93.6042288674527
	349.624472986261 -93.5449566174527
	349.127998636261 -93.4856843674527
	348.631524286261 -93.4264121174527
	348.135049936261 -93.3671398674527
	347.638575586261 -93.3078676174527
	347.142101236261 -93.2485953674527
	346.645626886261 -93.1893231174527
	346.149152536261 -93.1300508674527
	345.652678186261 -93.0707786174527
	345.156203836261 -93.0115063674527
	344.659729486261 -92.9522341174527
	344.163255136261 -92.8929618674527
	343.666780786261 -92.8336896174527
	349.677185328163 -123.724041282439
	349.180709028163 -123.664785082439
	348.684232728163 -123.605528882439
	348.187756428163 -123.546272682439
	347.691280128163 -123.487016482439
	347.194803828163 -123.427760282439
	346.698327528163 -123.368504082439
	346.201851228163 -123.309247882439
	345.705374928163 -123.249991682439
	345.208898628163 -123.190735482439
	344.712422328163 -123.131479282439
	344.215946028163 -123.072223082439
	343.719469728163 -123.012966882439
	343.222993428163 -122.953710682439
	342.726517128163 -122.894454482439
	342.230040828163 -122.835198282439
	341.733564528163 -122.775942082439
	341.237088228163 -122.716685882439
	345.937579448675 -153.482527603975
	345.440687598675 -153.426863503975
	344.943795748675 -153.371199403975
	344.446903898675 -153.315535303975
	343.950012048675 -153.259871203975
	343.453120198675 -153.204207103975
	342.956228348675 -153.148543003975
	342.459336498675 -153.092878903975
	341.962444648675 -153.037214803975
	341.465552798675 -152.981550703975
	340.968660948675 -152.925886603975
	340.471769098675 -152.870222503975
	339.974877248675 -152.814558403975
	342.5490179 -183.35696065
	342.0581559 -183.2618054
	341.5672939 -183.16665015
	341.0764319 -183.0714949
	340.5855699 -182.97633965
	340.0947079 -182.8811844
	339.6038459 -182.78602915
	339.1129839 -182.6908739
	338.6221219 -182.59571865
	338.1312599 -182.5005634
	337.6403979 -182.40540815
	337.1495359 -182.3102529
	336.6586739 -182.21509765
	336.1678119 -182.1199424
	335.6769499 -182.02478715
	335.1860879 -181.9296319
	341.459312899886 -192.398307377297
	340.977484849886 -192.264734477297
	340.495656799886 -192.131161577297
	340.013828749886 -191.997588677297
	339.532000699886 -191.864015777297
	339.050172649886 -191.730442877297
	338.568344599886 -191.596869977297
	338.086516549886 -191.463297077297
	337.604688499886 -191.329724177297
	337.122860449886 -191.196151277297
	336.641032399886 -191.062578377297
	336.159204349886 -190.929005477297
	335.677376299886 -190.795432577297
	335.195548249886 -190.661859677297
	334.713720199886 -190.528286777297
	334.231892149886 -190.394713877297
	333.750064099886 -190.261140977297
	339.864444389768 -201.599747992258
	339.399535939768 -201.415736792258
	338.934627489768 -201.231725592258
	338.469719039768 -201.047714392258
	338.004810589768 -200.863703192258
	337.539902139768 -200.679691992258
	337.074993689768 -200.495680792258
	336.610085239768 -200.311669592258
	336.145176789768 -200.127658392258
	335.680268339768 -199.943647192258
	335.215359889768 -199.759635992258
	334.750451439768 -199.575624792258
	334.285542989768 -199.391613592258
	333.820634539768 -199.207602392258
	333.355726089768 -199.023591192258
	332.890817639768 -198.839579992258
	332.425909189768 -198.655568792258
	331.961000739768 -198.471557592258
	338.620464912885 -211.768586326081
	338.188344512885 -211.517047126081
	337.756224112885 -211.265507926081
	337.324103712885 -211.013968726081
	336.891983312885 -210.762429526081
	336.459862912885 -210.510890326081
	336.027742512885 -210.259351126081
	335.595622112885 -210.007811926081
	335.163501712885 -209.756272726081
	334.731381312885 -209.504733526081
	334.299260912885 -209.253194326081
	333.867140512885 -209.001655126081
	333.435020112885 -208.750115926081
	333.002899712885 -208.498576726081
	332.570779312885 -208.247037526081
	332.138658912885 -207.995498326081
	331.706538512885 -207.743959126081
	331.274418112885 -207.492419926081
	330.842297712885 -207.240880726081
	330.410177312885 -206.989341526081
	329.978056912885 -206.737802326081
	329.545936512885 -206.486263126081
	334.09162688 -221.34126301
	333.71742908 -221.00963666
	333.34323128 -220.67801031
	332.96903348 -220.34638396
	332.59483568 -220.01475761
	332.22063788 -219.68313126
	331.84644008 -219.35150491
	331.47224228 -219.01987856
	331.09804448 -218.68825221
	330.72384668 -218.35662586
	330.34964888 -218.02499951
	329.97545108 -217.69337316
	329.60125328 -217.36174681
	329.22705548 -217.03012046
	328.85285768 -216.69849411
	328.47865988 -216.36686776
	328.10446208 -216.03524141
	327.73026428 -215.70361506
	327.35606648 -215.37198871
	326.98186868 -215.04036236
	326.60767088 -214.70873601
	326.23347308 -214.37710966
	326.81812678371 -229.387946670167
	326.51904638371 -228.987258620167
	326.21996598371 -228.586570570167
	325.92088558371 -228.185882520167
	325.62180518371 -227.785194470167
	325.32272478371 -227.384506420167
	325.02364438371 -226.983818370167
	324.72456398371 -226.583130320167
	324.42548358371 -226.182442270167
	324.12640318371 -225.781754220167
	323.82732278371 -225.381066170167
	323.52824238371 -224.980378120167
	323.22916198371 -224.579690070167
	322.93008158371 -224.179002020167
	322.63100118371 -223.778313970167
	322.33192078371 -223.377625920167
	322.03284038371 -222.976937870167
	321.73375998371 -222.576249820167
	321.43467958371 -222.175561770167
	321.13559918371 -221.774873720167
	320.83651878371 -221.374185670167
	317.847487 -235.88858774
	317.637206 -235.43495584
	317.426925 -234.98132394
	317.216644 -234.52769204
	317.006363 -234.07406014
	316.796082 -233.62042824
	316.585801 -233.16679634
	316.37552 -232.71316444
	316.165239 -232.25953254
	315.954958 -231.80590064
	315.744677 -231.35226874
	315.534396 -230.89863684
	315.324115 -230.44500494
	315.113834 -229.99137304
	314.903553 -229.53774114
	314.693272 -229.08410924
	314.482991 -228.63047734
	314.27271 -228.17684544
	314.062429 -227.72321354
	313.852148 -227.26958164
	313.641867 -226.81594974
	313.431586 -226.36231784
	307.380601154546 -239.50587506884
	307.266045054546 -239.01917506884
	307.151488954546 -238.53247506884
	307.036932854546 -238.04577506884
	306.922376754546 -237.55907506884
	306.807820654546 -237.07237506884
	306.693264554546 -236.58567506884
	306.578708454546 -236.09897506884
	306.464152354546 -235.61227506884
	306.349596254546 -235.12557506884
	306.235040154546 -234.63887506884
	306.120484054546 -234.15217506884
	306.005927954546 -233.66547506884
	305.891371854546 -233.17877506884
	305.776815754546 -232.69207506884
	305.662259654546 -232.20537506884
	305.547703554546 -231.71867506884
	305.433147454546 -231.23197506884
	305.318591354546 -230.74527506884
	305.204035254546 -230.25857506884
	305.089479154546 -229.77187506884
	304.974923054546 -229.28517506884
	296.43059338 -240.43728412
	296.41546933 -239.93751292
	296.40034528 -239.43774172
	296.38522123 -238.93797052
	296.37009718 -238.43819932
	296.35497313 -237.93842812
	296.33984908 -237.43865692
	296.32472503 -236.93888572
	296.30960098 -236.43911452
	296.29447693 -235.93934332
	296.27935288 -235.43957212
	296.26422883 -234.93980092
	296.24910478 -234.44002972
	296.23398073 -233.94025852
	296.21885668 -233.44048732
	296.20373263 -232.94071612
	296.18860858 -232.44094492
	296.17348453 -231.94117372
	296.15836048 -231.44140252
	296.14323643 -230.94163132
	296.12811238 -230.44186012
	296.11298833 -229.94208892
	296.09786428 -229.44231772
	285.978674662639 -238.348869014865
	286.051139962639 -237.854148114865
	286.123605262638 -237.359427214865
	286.196070562639 -236.864706314865
	286.268535862638 -236.369985414865
	286.341001162639 -235.875264514865
	286.413466462638 -235.380543614865
	286.485931762639 -234.885822714865
	286.558397062639 -234.391101814865
	286.630862362638 -233.896380914865
	286.703327662639 -233.401660014865
	286.775792962638 -232.906939114865
	286.848258262639 -232.412218214865
	286.920723562638 -231.917497314865
	286.993188862638 -231.422776414865
	287.065654162639 -230.928055514865
	287.138119462638 -230.433334614865
	287.210584762639 -229.938613714865
	287.283050062638 -229.443892814865
	287.355515362639 -228.949171914865
	287.427980662639 -228.454451014865
	287.500445962638 -227.959730114865
	287.572911262639 -227.465009214865
	276.732983116108 -233.850123195605
	276.873991366108 -233.370418395605
	277.014999616108 -232.890713595605
	277.156007866108 -232.411008795605
	277.297016116108 -231.931303995605
	277.438024366108 -231.451599195605
	277.579032616108 -230.971894395605
	277.720040866108 -230.492189595605
	277.861049116108 -230.012484795605
	278.002057366108 -229.532779995605
	278.143065616108 -229.053075195605
	278.284073866108 -228.573370395605
	278.425082116108 -228.093665595605
	278.566090366108 -227.613960795605
	278.707098616108 -227.134255995605
	278.848106866108 -226.654551195605
	278.989115116108 -226.174846395605
	279.130123366108 -225.695141595605
	279.271131616108 -225.215436795605
	279.412139866108 -224.735731995605
	279.553148116108 -224.256027195605
	279.694156366108 -223.776322395605
	268.378743623341 -228.948501717087
	268.567712173341 -228.485586067087
	268.756680723341 -228.022670417087
	268.945649273341 -227.559754767087
	269.134617823341 -227.096839117087
	269.323586373341 -226.633923467087
	269.512554923341 -226.171007817087
	269.701523473341 -225.708092167087
	269.890492023341 -225.245176517087
	270.079460573341 -224.782260867087
	270.268429123341 -224.319345217087
	270.457397673341 -223.856429567087
	270.646366223341 -223.393513917087
	270.835334773341 -222.930598267087
	271.024303323341 -222.467682617087
	271.213271873341 -222.004766967087
	271.402240423341 -221.541851317087
	271.591208973341 -221.078935667087
	271.780177523341 -220.616020017087
	271.969146073341 -220.153104367087
	272.158114623341 -219.690188717087
	272.347083173341 -219.227273067087
	272.536051723341 -218.764357417087
	260.5362362 -223.89788425
	260.7526992 -223.4471695
	260.9691622 -222.99645475
	261.1856252 -222.54574
	261.4020882 -222.09502525
	261.6185512 -221.6443105
	261.8350142 -221.19359575
	262.0514772 -220.742881
	262.2679402 -220.29216625
	262.4844032 -219.8414515
	262.7008662 -219.39073675
	262.9173292 -218.940022
	263.1337922 -218.48930725
	263.3502552 -218.0385925
	263.5667182 -217.58787775
	263.7831812 -217.137163
	263.9996442 -216.68644825
	264.2161072 -216.2357335
	264.4325702 -215.78501875
	264.6490332 -215.334304
	264.8654962 -214.88358925
	265.0819592 -214.4328745
	265.2984222 -213.98215975
	235.57422251168 -206.809604498743
	235.84427721168 -206.388807098743
	236.11433191168 -205.968009698743
	236.38438661168 -205.547212298743
	236.65444131168 -205.126414898743
	236.92449601168 -204.705617498743
	237.19455071168 -204.284820098743
	237.46460541168 -203.864022698743
	237.73466011168 -203.443225298743
	238.00471481168 -203.022427898743
	238.27476951168 -202.601630498743
	238.54482421168 -202.180833098743
	238.81487891168 -201.760035698743
	239.08493361168 -201.339238298743
	239.35498831168 -200.918440898743
	239.62504301168 -200.497643498743
	239.89509771168 -200.076846098743
	240.16515241168 -199.656048698743
	240.43520711168 -199.235251298743
	240.70526181168 -198.814453898743
	240.97531651168 -198.393656498743
	241.24537121168 -197.972859098743
	241.51542591168 -197.552061698743
	210.624480422329 -190.158143478173
	210.90503327233 -189.744271378173
	211.18558612233 -189.330399278173
	211.46613897233 -188.916527178173
	211.74669182233 -188.502655078173
	212.02724467233 -188.088782978173
	212.30779752233 -187.674910878173
	212.58835037233 -187.261038778173
	212.86890322233 -186.847166678173
	213.14945607233 -186.433294578173
	213.43000892233 -186.019422478173
	213.710561772329 -185.605550378173
	213.99111462233 -185.191678278173
	214.27166747233 -184.777806178173
	214.55222032233 -184.363934078173
	214.832773172329 -183.950061978173
	215.11332602233 -183.536189878173
	215.39387887233 -183.122317778173
	215.67443172233 -182.708445678173
	215.95498457233 -182.294573578173
	216.23553742233 -181.880701478173
	216.51609027233 -181.466829378173
	216.796643122329 -181.052957278173
	185.578785901757 -173.671318669997
	185.856748151757 -173.255702269997
	186.134710401757 -172.840085869997
	186.412672651757 -172.424469469997
	186.690634901757 -172.008853069997
	186.968597151757 -171.593236669997
	187.246559401757 -171.177620269997
	187.524521651757 -170.762003869997
	187.802483901757 -170.346387469997
	188.080446151757 -169.930771069997
	188.358408401757 -169.515154669997
	188.636370651757 -169.099538269997
	188.914332901757 -168.683921869997
	189.192295151757 -168.268305469997
	189.470257401757 -167.852689069997
	189.748219651757 -167.437072669997
	190.026181901757 -167.021456269997
	190.304144151757 -166.605839869997
	190.582106401757 -166.190223469997
	190.860068651757 -165.774607069997
	191.138030901757 -165.358990669997
	191.415993151757 -164.943374269997
	191.693955401757 -164.527757869997
	160.461066867805 -157.291399742343
	160.739067517805 -156.875808992343
	161.017068167805 -156.460218242343
	161.295068817805 -156.044627492343
	161.573069467805 -155.629036742343
	161.851070117805 -155.213445992343
	162.129070767805 -154.797855242343
	162.407071417805 -154.382264492343
	162.685072067805 -153.966673742343
	162.963072717805 -153.551082992343
	163.241073367805 -153.135492242343
	163.519074017805 -152.719901492343
	163.797074667805 -152.304310742343
	164.075075317805 -151.888719992343
	164.353075967805 -151.473129242343
	164.631076617805 -151.057538492343
	164.909077267805 -150.641947742343
	165.187077917805 -150.226356992343
	165.465078567805 -149.810766242343
	165.743079217805 -149.395175492343
	166.021079867805 -148.979584742343
	166.299080517805 -148.563993992343
	166.577081167805 -148.148403242343
	135.54823248 -140.60014206
	135.82601493 -140.18440546
	136.10379738 -139.76866886
	136.38157983 -139.35293226
	136.65936228 -138.93719566
	136.93714473 -138.52145906
	137.21492718 -138.10572246
	137.49270963 -137.68998586
	137.77049208 -137.27424926
	138.04827453 -136.85851266
	138.32605698 -136.44277606
	138.60383943 -136.02703946
	138.88162188 -135.61130286
	139.15940433 -135.19556626
	139.43718678 -134.77982966
	139.71496923 -134.36409306
	139.99275168 -133.94835646
	140.27053413 -133.53261986
	140.54831658 -133.11688326
	140.82609903 -132.70114666
	141.10388148 -132.28541006
	141.38166393 -131.86967346
	141.65944638 -131.45393686
	110.603542236609 -123.956707039106
	110.880883186609 -123.540675789106
	111.158224136609 -123.124644539106
	111.435565086609 -122.708613289106
	111.712906036609 -122.292582039106
	111.990246986609 -121.876550789106
	112.267587936609 -121.460519539106
	112.544928886609 -121.044488289106
	112.822269836609 -120.628457039106
	113.099610786609 -120.212425789106
	113.376951736609 -119.796394539106
	113.654292686609 -119.380363289106
	113.931633636609 -118.964332039106
	114.208974586609 -118.548300789106
	114.486315536609 -118.132269539106
	114.763656486609 -117.716238289106
	115.040997436609 -117.300207039106
	115.318338386609 -116.884175789106
	115.595679336609 -116.468144539106
	115.873020286609 -116.052113289106
	116.150361236609 -115.636082039106
	116.427702186609 -115.220050789106
	116.705043136609 -114.804019539106
	85.6448477903712 -107.335812634054
	85.9218377403712 -106.919547634054
	86.1988276903712 -106.503282634054
	86.4758176403712 -106.087017634054
	86.7528075903712 -105.670752634054
	87.0297975403712 -105.254487634054
	87.3067874903712 -104.838222634054
	87.5837774403712 -104.421957634054
	87.8607673903712 -104.005692634054
	88.1377573403712 -103.589427634054
	88.4147472903712 -103.173162634054
	88.6917372403712 -102.756897634054
	88.9687271903712 -102.340632634054
	89.2457171403712 -101.924367634054
	89.5227070903712 -101.508102634054
	89.7996970403712 -101.091837634054
	90.0766869903712 -100.675572634054
	90.3536769403712 -100.259307634054
	90.6306668903712 -99.843042634054
	90.9076568403712 -99.426777634054
	91.1846467903712 -99.010512634054
	91.4616367403712 -98.594247634054
	91.7386266903712 -98.177982634054
	60.6770553502117 -90.7293567744541
	60.9538447502117 -90.3129583744541
	61.2306341502117 -89.8965599744541
	61.5074235502117 -89.4801615744541
	61.7842129502117 -89.0637631744541
	62.0610023502117 -88.6473647744541
	62.3377917502117 -88.2309663744541
	62.6145811502117 -87.8145679744541
	62.8913705502117 -87.3981695744541
	63.1681599502117 -86.9817711744541
	63.4449493502117 -86.5653727744541
	63.7217387502117 -86.1489743744541
	63.9985281502117 -85.7325759744541
	64.2753175502117 -85.3161775744541
	64.5521069502117 -84.8997791744541
	64.8288963502117 -84.4833807744541
	65.1056857502117 -84.0669823744541
	65.3824751502117 -83.6505839744541
	65.6592645502117 -83.2341855744541
	65.9360539502117 -82.8177871744541
	66.2128433502117 -82.4013887744541
	66.4896327502117 -81.9849903744541
	66.7664221502117 -81.5685919744541
	35.7046765844827 -74.1299019835669
	35.9814160344827 -73.7134703835669
	36.2581554844827 -73.2970387835669
	36.5348949344827 -72.8806071835669
	36.8116343844827 -72.4641755835669
	37.0883738344827 -72.0477439835669
	37.3651132844827 -71.6313123835669
	37.6418527344827 -71.2148807835669
	37.9185921844827 -70.7984491835669
	38.1953316344827 -70.3820175835669
	38.4720710844827 -69.9655859835669
	38.7488105344827 -69.5491543835669
	39.0255499844827 -69.1327227835669
	39.3022894344827 -68.7162911835669
	39.5790288844827 -68.2998595835669
	39.8557683344827 -67.8834279835669
	40.1325077844827 -67.4669963835669
	40.4092472344827 -67.0505647835669
	40.6859866844827 -66.6341331835669
	40.9627261344827 -66.2177015835669
	41.2394655844827 -65.8012699835669
	41.5162050344827 -65.3848383835669
	41.7929444844827 -64.9684067835669
	10.7322114652489 -57.5300351430109
	11.0090516152489 -57.1136704930109
	11.2858917652489 -56.6973058430109
	11.5627319152489 -56.2809411930109
	11.8395720652489 -55.8645765430109
	12.1164122152489 -55.4482118930109
	12.3932523652489 -55.0318472430109
	12.6700925152489 -54.6154825930109
	12.9469326652489 -54.1991179430109
	13.2237728152489 -53.7827532930109
	13.5006129652489 -53.3663886430109
	13.7774531152489 -52.9500239930109
	14.0542932652489 -52.5336593430109
	14.3311334152489 -52.1172946930109
	14.6079735652489 -51.7009300430109
	14.8848137152489 -51.2845653930109
	15.1616538652489 -50.8682007430109
	15.4384940152489 -50.4518360930109
	15.7153341652489 -50.0354714430109
	15.9921743152489 -49.6191067930109
	16.2690144652489 -49.2027421430109
	16.5458546152489 -48.7863774930109
	16.8226947652489 -48.3700128430109
};

==> ressources/variable_friction/raceline.tex <==
\addplot [line width=1pt, TUMred]
table {%
	-1.19939987814429 -48.396013804573
	-26.1715340442021 -31.7950577165333
	-51.146766794585 -15.1978881450733
	-76.125635989896 1.39442485954599
	-101.108664487831 17.9808007736175
	-126.096367280691 34.5601530282357
	-151.089258697699 51.1313953434079
	-176.087859721955 67.6934469054873
	-201.092705048717 84.2452375206171
	-226.104350599453 100.785713189537
	-251.123344261192 117.313897111943
	-276.148649158058 133.831706351418
	-301.178822226352 150.342534000582
	-326.212881751275 166.849024234324
	-351.24982109704 183.353806823386
	-376.288648948732 199.859533447812
	-401.326287201231 216.370288419848
	-426.353362317105 232.894303170476
	-451.359340468007 249.440522135324
	-476.333697423046 266.01779843358
	-501.260677496731 282.644457982621
	-513.501989287183 291.372675395685
	-520.257956182711 297.421150215265
	-525.81622128 304.42111156
	-529.559153517081 312.543338643113
	-530.49733078 321.31021312
	-528.156768780911 329.735014547851
	-522.80766872 336.80659232
	-515.455604553819 341.766648013633
	-506.864058890701 344.588110618649
	-497.847317199148 345.43830545114
	-488.850950039795 344.891653721598
	-479.967485673176 343.431897921253
	-451.404353403183 334.417743899321
	-424.756499032292 320.677231186508
	-399.792309674727 304.122826961
	-375.50566122 286.5356393
	-351.05318054 269.21268832
	-341.019620320444 262.667465467147
	-333.065779334266 258.366960241099
	-324.629081345966 255.205268618368
	-315.667897764901 253.906335129307
	-306.98193808 255.43274642
	-299.541650593178 259.957250896896
	-294.24848772 266.97839082
	-291.463116824009 275.350885445176
	-290.397873519092 284.419485400787
	-289.770583148538 293.499979944974
	-288.24543278 302.23397432
	-285.02453825689 310.476938697248
	-279.909577973383 317.847905555838
	-273.235023793172 323.86858827638
	-265.417332091005 328.286175014884
	-256.97577022631 331.062786687495
	-248.221033471732 332.481016044646
	-239.241500996667 332.822071017921
	-230.17222539072 332.325657965909
	-200.431984645119 328.244718019374
	-171.057890328555 322.361489926597
	-142.33676573771 313.730856101223
	-115.142219231182 301.252935845288
	-89.84577872 285.2304671
	-66.503272741681 266.511899062332
	-44.5715747709642 246.039336038745
	-23.4575784163313 224.69109208524
	-2.70204877645798 203.070302846441
	17.9969270069918 181.405962028077
	38.9157681224756 159.901353982704
	60.1950714555899 138.753989759106
	81.8767376344448 118.084529343987
	103.839612168359 97.6489296578706
	126.828812574802 78.4134526097299
	134.2524319985 73.4088751098792
	142.034802232285 68.9595787310989
	150.145453235321 65.1109516093478
	158.540835322447 61.8936258274158
	167.176108388867 59.3398093901648
	175.995000401337 57.4857633571094
	184.92599425396 56.3620283918338
	193.896115901934 55.9851683357542
	202.8376521 56.36045026
	211.710102315122 57.4677859097875
	240.64831002924 65.1406347914483
	269.279594359088 73.8091427969529
	278.104436801385 75.3366015904152
	287.062765767414 76.01948625804
	296.054724962368 75.798954633122
	304.976958018415 74.6391948408225
	313.726065630082 72.5039376375511
	322.155986291208 69.3547855670234
	330.089165202755 65.1901787846099
	337.362744878756 60.0353105469335
	343.826132194669 53.9105629371982
	349.383396049639 46.8967574241304
	353.960557165182 39.1499499407515
	357.503395330575 30.86247116904
	360.022377733826 22.2476185947759
	361.634098027486 13.4491839806477
	362.477956171279 4.5128557675806
	362.660547856405 -4.50258900731017
	360.228269226936 -34.4022135428782
	356.390938261852 -64.1347561865344
	352.603319086261 -93.9005901174527
	349.180709028163 -123.664785082439
	345.937579448675 -153.482527603975
	342.0581559 -183.2618054
	340.013828749886 -191.997588677297
	337.074993689768 -200.495680792258
	333.002899712885 -208.498576726081
	327.73026428 -215.70361506
	321.13559918371 -221.774873720167
	313.431586 -226.36231784
	304.974923054546 -229.28517506884
	296.12811238 -230.44186012
	287.210584762639 -229.938613714865
	278.425082116108 -228.093665595605
	269.890492023341 -225.245176517087
	261.6185512 -221.6443105
	235.57422251168 -206.809604498743
	210.624480422329 -190.158143478173
	185.856748151757 -173.255702269997
	161.017068167805 -156.460218242343
	136.10379738 -139.76866886
	111.158224136609 -123.124644539106
	86.1988276903712 -106.503282634054
	61.2306341502117 -89.8965599744541
	36.2581554844827 -73.2970387835669
	11.2858917652489 -56.6973058430109
};
